Forecasting Retail Sales at Every Grain: Trees, Foundation Models, Transformers and World Models Compared on Four Public Data Sets

A retailer makes decisions from the same demand at different grains: store orders by item and day, promotions by item and week, category reviews and supplier terms. This paper asks whether one forecast, built at the finest grain and summed to every coarser grain, can serve them all, and which model does that best. It compares LightGBM, pretrained foundation models (TimesFM, Chronos-Bolt, Timestral), the Temporal Fusion Transformer and a world model that carries each item's state forward under the price and promotion plan, on M5, six Dominick's categories, Breakfast at the Frat and Corporacion Favorita, with the world model and LightGBM tuned by a common search. When to use the average: the average of the tuned world model and LightGBM, summed to every grain, has the lowest error in 22 of 27 grain and data set cases and is never the least accurate on the final held-out periods. When to use the world model: on existing items kept out of training it loses at most 0.040 in scaled error, against up to 0.311 for LightGBM, and on lines with short history it is clearly more accurate on six of nine data sets. When to use LightGBM: on heavily promoted lines, fast sellers and lines with long history (six of nine data sets each) and in price-cut weeks. Inconclusive: lines never promoted and slow lines are close to even, and 52 weeks ahead the average is the most accurate on five of seven data sets, with the world model ahead of LightGBM on two of seven. The findings hold for these data sets and the price and promotion levers; anyone adopting them should rerun every comparison on their own data.

==> generated/rev_values.tex <==
% Generated by figs/make_revision.py from results/paper1_revision/tables. Do not edit.
\makeatletter
\newcommand{\revget}[1]{\ifcsname rev@#1\endcsname\csname rev@#1\endcsname\else\errmessage{Revision value #1 is not in the result tables}\fi}
\expandafter\def\csname rev@rab@ana@fittedalllevels@ixs@hi\endcsname{0.014}
\expandafter\def\csname rev@rab@ana@fittedalllevels@ixs@lo\endcsname{0.002}
\expandafter\def\csname rev@rab@ana@fittedalllevels@ixs@meandiff\endcsname{0.008}
\expandafter\def\csname rev@rab@ana@fittedalllevels@total@hi\endcsname{0.057}
\expandafter\def\csname rev@rab@ana@fittedalllevels@total@lo\endcsname{\textminus 0.025}
\expandafter\def\csname rev@rab@ana@fittedalllevels@total@meandiff\endcsname{0.012}
\expandafter\def\csname rev@rab@ana@fittedbottom@ixs@hi\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rab@ana@fittedbottom@ixs@lo\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rab@ana@fittedbottom@ixs@meandiff\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rab@ana@fittedbottom@total@hi\endcsname{0.069}
\expandafter\def\csname rev@rab@ana@fittedbottom@total@lo\endcsname{\textminus 0.016}
\expandafter\def\csname rev@rab@ana@fittedbottom@total@meandiff\endcsname{0.031}
\expandafter\def\csname rev@rab@ana@fittedtotal@ixs@hi\endcsname{0.016}
\expandafter\def\csname rev@rab@ana@fittedtotal@ixs@lo\endcsname{0.009}
\expandafter\def\csname rev@rab@ana@fittedtotal@ixs@meandiff\endcsname{0.012}
\expandafter\def\csname rev@rab@ana@fittedtotal@total@hi\endcsname{0.065}
\expandafter\def\csname rev@rab@ana@fittedtotal@total@lo\endcsname{\textminus 0.030}
\expandafter\def\csname rev@rab@ana@fittedtotal@total@meandiff\endcsname{0.014}
\expandafter\def\csname rev@rab@ana@liftforworldmodel@ixs@hi\endcsname{0.005}
\expandafter\def\csname rev@rab@ana@liftforworldmodel@ixs@lo\endcsname{0.000}
\expandafter\def\csname rev@rab@ana@liftforworldmodel@ixs@meandiff\endcsname{0.003}
\expandafter\def\csname rev@rab@ana@liftforworldmodel@total@hi\endcsname{0.042}
\expandafter\def\csname rev@rab@ana@liftforworldmodel@total@lo\endcsname{0.009}
\expandafter\def\csname rev@rab@ana@liftforworldmodel@total@meandiff\endcsname{0.025}
\expandafter\def\csname rev@rab@ana@withoutlightgbm@ixs@hi\endcsname{0.017}
\expandafter\def\csname rev@rab@ana@withoutlightgbm@ixs@lo\endcsname{0.010}
\expandafter\def\csname rev@rab@ana@withoutlightgbm@ixs@meandiff\endcsname{0.014}
\expandafter\def\csname rev@rab@ana@withoutlightgbm@total@hi\endcsname{0.026}
\expandafter\def\csname rev@rab@ana@withoutlightgbm@total@lo\endcsname{\textminus 0.034}
\expandafter\def\csname rev@rab@ana@withoutlightgbm@total@meandiff\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rab@ana@withouttimesfm@ixs@hi\endcsname{0.005}
\expandafter\def\csname rev@rab@ana@withouttimesfm@ixs@lo\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rab@ana@withouttimesfm@ixs@meandiff\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@ana@withouttimesfm@total@hi\endcsname{0.082}
\expandafter\def\csname rev@rab@ana@withouttimesfm@total@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rab@ana@withouttimesfm@total@meandiff\endcsname{0.038}
\expandafter\def\csname rev@rab@ana@withoutworldmodel@ixs@hi\endcsname{0.002}
\expandafter\def\csname rev@rab@ana@withoutworldmodel@ixs@lo\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rab@ana@withoutworldmodel@ixs@meandiff\endcsname{0.000}
\expandafter\def\csname rev@rab@ana@withoutworldmodel@total@hi\endcsname{0.059}
\expandafter\def\csname rev@rab@ana@withoutworldmodel@total@lo\endcsname{\textminus 0.020}
\expandafter\def\csname rev@rab@ana@withoutworldmodel@total@meandiff\endcsname{0.019}
\expandafter\def\csname rev@rab@bjc@fittedalllevels@ixs@hi\endcsname{0.006}
\expandafter\def\csname rev@rab@bjc@fittedalllevels@ixs@lo\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rab@bjc@fittedalllevels@ixs@meandiff\endcsname{0.000}
\expandafter\def\csname rev@rab@bjc@fittedalllevels@total@hi\endcsname{0.015}
\expandafter\def\csname rev@rab@bjc@fittedalllevels@total@lo\endcsname{\textminus 0.062}
\expandafter\def\csname rev@rab@bjc@fittedalllevels@total@meandiff\endcsname{\textminus 0.015}
\expandafter\def\csname rev@rab@bjc@fittedbottom@ixs@hi\endcsname{0.006}
\expandafter\def\csname rev@rab@bjc@fittedbottom@ixs@lo\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rab@bjc@fittedbottom@ixs@meandiff\endcsname{0.002}
\expandafter\def\csname rev@rab@bjc@fittedbottom@total@hi\endcsname{0.065}
\expandafter\def\csname rev@rab@bjc@fittedbottom@total@lo\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rab@bjc@fittedbottom@total@meandiff\endcsname{0.025}
\expandafter\def\csname rev@rab@bjc@fittedtotal@ixs@hi\endcsname{0.008}
\expandafter\def\csname rev@rab@bjc@fittedtotal@ixs@lo\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rab@bjc@fittedtotal@ixs@meandiff\endcsname{0.002}
\expandafter\def\csname rev@rab@bjc@fittedtotal@total@hi\endcsname{0.027}
\expandafter\def\csname rev@rab@bjc@fittedtotal@total@lo\endcsname{\textminus 0.112}
\expandafter\def\csname rev@rab@bjc@fittedtotal@total@meandiff\endcsname{\textminus 0.028}
\expandafter\def\csname rev@rab@bjc@liftforworldmodel@ixs@hi\endcsname{0.007}
\expandafter\def\csname rev@rab@bjc@liftforworldmodel@ixs@lo\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rab@bjc@liftforworldmodel@ixs@meandiff\endcsname{0.002}
\expandafter\def\csname rev@rab@bjc@liftforworldmodel@total@hi\endcsname{0.110}
\expandafter\def\csname rev@rab@bjc@liftforworldmodel@total@lo\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rab@bjc@liftforworldmodel@total@meandiff\endcsname{0.051}
\expandafter\def\csname rev@rab@bjc@withoutlightgbm@ixs@hi\endcsname{0.024}
\expandafter\def\csname rev@rab@bjc@withoutlightgbm@ixs@lo\endcsname{0.008}
\expandafter\def\csname rev@rab@bjc@withoutlightgbm@ixs@meandiff\endcsname{0.016}
\expandafter\def\csname rev@rab@bjc@withoutlightgbm@total@hi\endcsname{0.071}
\expandafter\def\csname rev@rab@bjc@withoutlightgbm@total@lo\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rab@bjc@withoutlightgbm@total@meandiff\endcsname{0.031}
\expandafter\def\csname rev@rab@bjc@withouttimesfm@ixs@hi\endcsname{0.033}
\expandafter\def\csname rev@rab@bjc@withouttimesfm@ixs@lo\endcsname{0.001}
\expandafter\def\csname rev@rab@bjc@withouttimesfm@ixs@meandiff\endcsname{0.015}
\expandafter\def\csname rev@rab@bjc@withouttimesfm@total@hi\endcsname{0.028}
\expandafter\def\csname rev@rab@bjc@withouttimesfm@total@lo\endcsname{\textminus 0.140}
\expandafter\def\csname rev@rab@bjc@withouttimesfm@total@meandiff\endcsname{\textminus 0.042}
\expandafter\def\csname rev@rab@bjc@withoutworldmodel@ixs@hi\endcsname{0.021}
\expandafter\def\csname rev@rab@bjc@withoutworldmodel@ixs@lo\endcsname{0.004}
\expandafter\def\csname rev@rab@bjc@withoutworldmodel@ixs@meandiff\endcsname{0.012}
\expandafter\def\csname rev@rab@bjc@withoutworldmodel@total@hi\endcsname{0.199}
\expandafter\def\csname rev@rab@bjc@withoutworldmodel@total@lo\endcsname{0.013}
\expandafter\def\csname rev@rab@bjc@withoutworldmodel@total@meandiff\endcsname{0.103}
\expandafter\def\csname rev@rab@che@fittedalllevels@ixs@hi\endcsname{0.035}
\expandafter\def\csname rev@rab@che@fittedalllevels@ixs@lo\endcsname{0.001}
\expandafter\def\csname rev@rab@che@fittedalllevels@ixs@meandiff\endcsname{0.015}
\expandafter\def\csname rev@rab@che@fittedalllevels@total@hi\endcsname{0.178}
\expandafter\def\csname rev@rab@che@fittedalllevels@total@lo\endcsname{\textminus 0.025}
\expandafter\def\csname rev@rab@che@fittedalllevels@total@meandiff\endcsname{0.056}
\expandafter\def\csname rev@rab@che@fittedbottom@ixs@hi\endcsname{0.025}
\expandafter\def\csname rev@rab@che@fittedbottom@ixs@lo\endcsname{0.002}
\expandafter\def\csname rev@rab@che@fittedbottom@ixs@meandiff\endcsname{0.012}
\expandafter\def\csname rev@rab@che@fittedbottom@total@hi\endcsname{0.137}
\expandafter\def\csname rev@rab@che@fittedbottom@total@lo\endcsname{\textminus 0.045}
\expandafter\def\csname rev@rab@che@fittedbottom@total@meandiff\endcsname{0.034}
\expandafter\def\csname rev@rab@che@fittedtotal@ixs@hi\endcsname{0.007}
\expandafter\def\csname rev@rab@che@fittedtotal@ixs@lo\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@che@fittedtotal@ixs@meandiff\endcsname{0.002}
\expandafter\def\csname rev@rab@che@fittedtotal@total@hi\endcsname{0.059}
\expandafter\def\csname rev@rab@che@fittedtotal@total@lo\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rab@che@fittedtotal@total@meandiff\endcsname{0.022}
\expandafter\def\csname rev@rab@che@liftforworldmodel@ixs@hi\endcsname{0.006}
\expandafter\def\csname rev@rab@che@liftforworldmodel@ixs@lo\endcsname{\textminus 0.594}
\expandafter\def\csname rev@rab@che@liftforworldmodel@ixs@meandiff\endcsname{\textminus 0.196}
\expandafter\def\csname rev@rab@che@liftforworldmodel@total@hi\endcsname{0.088}
\expandafter\def\csname rev@rab@che@liftforworldmodel@total@lo\endcsname{\textminus 0.039}
\expandafter\def\csname rev@rab@che@liftforworldmodel@total@meandiff\endcsname{0.021}
\expandafter\def\csname rev@rab@che@withoutlightgbm@ixs@hi\endcsname{0.561}
\expandafter\def\csname rev@rab@che@withoutlightgbm@ixs@lo\endcsname{0.013}
\expandafter\def\csname rev@rab@che@withoutlightgbm@ixs@meandiff\endcsname{0.199}
\expandafter\def\csname rev@rab@che@withoutlightgbm@total@hi\endcsname{0.114}
\expandafter\def\csname rev@rab@che@withoutlightgbm@total@lo\endcsname{0.001}
\expandafter\def\csname rev@rab@che@withoutlightgbm@total@meandiff\endcsname{0.056}
\expandafter\def\csname rev@rab@che@withouttimesfm@ixs@hi\endcsname{0.546}
\expandafter\def\csname rev@rab@che@withouttimesfm@ixs@lo\endcsname{0.009}
\expandafter\def\csname rev@rab@che@withouttimesfm@ixs@meandiff\endcsname{0.190}
\expandafter\def\csname rev@rab@che@withouttimesfm@total@hi\endcsname{0.124}
\expandafter\def\csname rev@rab@che@withouttimesfm@total@lo\endcsname{\textminus 0.059}
\expandafter\def\csname rev@rab@che@withouttimesfm@total@meandiff\endcsname{0.029}
\expandafter\def\csname rev@rab@che@withoutworldmodel@ixs@hi\endcsname{0.021}
\expandafter\def\csname rev@rab@che@withoutworldmodel@ixs@lo\endcsname{\textminus 1.013}
\expandafter\def\csname rev@rab@che@withoutworldmodel@ixs@meandiff\endcsname{\textminus 0.328}
\expandafter\def\csname rev@rab@che@withoutworldmodel@total@hi\endcsname{0.164}
\expandafter\def\csname rev@rab@che@withoutworldmodel@total@lo\endcsname{\textminus 0.016}
\expandafter\def\csname rev@rab@che@withoutworldmodel@total@meandiff\endcsname{0.072}
\expandafter\def\csname rev@rab@fav@fittedalllevels@ixs@hi\endcsname{0.012}
\expandafter\def\csname rev@rab@fav@fittedalllevels@ixs@lo\endcsname{0.003}
\expandafter\def\csname rev@rab@fav@fittedalllevels@ixs@meandiff\endcsname{0.007}
\expandafter\def\csname rev@rab@fav@fittedalllevels@total@hi\endcsname{0.036}
\expandafter\def\csname rev@rab@fav@fittedalllevels@total@lo\endcsname{\textminus 0.014}
\expandafter\def\csname rev@rab@fav@fittedalllevels@total@meandiff\endcsname{0.004}
\expandafter\def\csname rev@rab@fav@fittedbottom@ixs@hi\endcsname{0.003}
\expandafter\def\csname rev@rab@fav@fittedbottom@ixs@lo\endcsname{\textminus 0.000}
\expandafter\def\csname rev@rab@fav@fittedbottom@ixs@meandiff\endcsname{0.001}
\expandafter\def\csname rev@rab@fav@fittedbottom@total@hi\endcsname{0.016}
\expandafter\def\csname rev@rab@fav@fittedbottom@total@lo\endcsname{0.008}
\expandafter\def\csname rev@rab@fav@fittedbottom@total@meandiff\endcsname{0.012}
\expandafter\def\csname rev@rab@fav@fittedtotal@ixs@hi\endcsname{0.020}
\expandafter\def\csname rev@rab@fav@fittedtotal@ixs@lo\endcsname{0.005}
\expandafter\def\csname rev@rab@fav@fittedtotal@ixs@meandiff\endcsname{0.011}
\expandafter\def\csname rev@rab@fav@fittedtotal@total@hi\endcsname{0.056}
\expandafter\def\csname rev@rab@fav@fittedtotal@total@lo\endcsname{\textminus 0.018}
\expandafter\def\csname rev@rab@fav@fittedtotal@total@meandiff\endcsname{0.008}
\expandafter\def\csname rev@rab@fav@liftforworldmodel@ixs@hi\endcsname{0.016}
\expandafter\def\csname rev@rab@fav@liftforworldmodel@ixs@lo\endcsname{0.006}
\expandafter\def\csname rev@rab@fav@liftforworldmodel@ixs@meandiff\endcsname{0.010}
\expandafter\def\csname rev@rab@fav@liftforworldmodel@total@hi\endcsname{0.096}
\expandafter\def\csname rev@rab@fav@liftforworldmodel@total@lo\endcsname{0.032}
\expandafter\def\csname rev@rab@fav@liftforworldmodel@total@meandiff\endcsname{0.067}
\expandafter\def\csname rev@rab@fav@withoutlightgbm@ixs@hi\endcsname{0.010}
\expandafter\def\csname rev@rab@fav@withoutlightgbm@ixs@lo\endcsname{0.001}
\expandafter\def\csname rev@rab@fav@withoutlightgbm@ixs@meandiff\endcsname{0.006}
\expandafter\def\csname rev@rab@fav@withoutlightgbm@total@hi\endcsname{0.031}
\expandafter\def\csname rev@rab@fav@withoutlightgbm@total@lo\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rab@fav@withoutlightgbm@total@meandiff\endcsname{0.013}
\expandafter\def\csname rev@rab@fav@withouttimesfm@ixs@hi\endcsname{0.010}
\expandafter\def\csname rev@rab@fav@withouttimesfm@ixs@lo\endcsname{0.005}
\expandafter\def\csname rev@rab@fav@withouttimesfm@ixs@meandiff\endcsname{0.007}
\expandafter\def\csname rev@rab@fav@withouttimesfm@total@hi\endcsname{\textminus 0.000}
\expandafter\def\csname rev@rab@fav@withouttimesfm@total@lo\endcsname{\textminus 0.029}
\expandafter\def\csname rev@rab@fav@withouttimesfm@total@meandiff\endcsname{\textminus 0.015}
\expandafter\def\csname rev@rab@fav@withoutworldmodel@ixs@hi\endcsname{0.014}
\expandafter\def\csname rev@rab@fav@withoutworldmodel@ixs@lo\endcsname{0.002}
\expandafter\def\csname rev@rab@fav@withoutworldmodel@ixs@meandiff\endcsname{0.007}
\expandafter\def\csname rev@rab@fav@withoutworldmodel@total@hi\endcsname{0.086}
\expandafter\def\csname rev@rab@fav@withoutworldmodel@total@lo\endcsname{\textminus 0.000}
\expandafter\def\csname rev@rab@fav@withoutworldmodel@total@meandiff\endcsname{0.037}
\expandafter\def\csname rev@rab@frat@fittedalllevels@ixs@hi\endcsname{0.010}
\expandafter\def\csname rev@rab@frat@fittedalllevels@ixs@lo\endcsname{0.004}
\expandafter\def\csname rev@rab@frat@fittedalllevels@ixs@meandiff\endcsname{0.007}
\expandafter\def\csname rev@rab@frat@fittedalllevels@total@hi\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rab@frat@fittedalllevels@total@lo\endcsname{\textminus 0.032}
\expandafter\def\csname rev@rab@frat@fittedalllevels@total@meandiff\endcsname{\textminus 0.022}
\expandafter\def\csname rev@rab@frat@fittedbottom@ixs@hi\endcsname{0.003}
\expandafter\def\csname rev@rab@frat@fittedbottom@ixs@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rab@frat@fittedbottom@ixs@meandiff\endcsname{0.001}
\expandafter\def\csname rev@rab@frat@fittedbottom@total@hi\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rab@frat@fittedbottom@total@lo\endcsname{\textminus 0.052}
\expandafter\def\csname rev@rab@frat@fittedbottom@total@meandiff\endcsname{\textminus 0.025}
\expandafter\def\csname rev@rab@frat@fittedtotal@ixs@hi\endcsname{0.012}
\expandafter\def\csname rev@rab@frat@fittedtotal@ixs@lo\endcsname{0.004}
\expandafter\def\csname rev@rab@frat@fittedtotal@ixs@meandiff\endcsname{0.008}
\expandafter\def\csname rev@rab@frat@fittedtotal@total@hi\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rab@frat@fittedtotal@total@lo\endcsname{\textminus 0.032}
\expandafter\def\csname rev@rab@frat@fittedtotal@total@meandiff\endcsname{\textminus 0.023}
\expandafter\def\csname rev@rab@frat@liftforworldmodel@ixs@hi\endcsname{0.007}
\expandafter\def\csname rev@rab@frat@liftforworldmodel@ixs@lo\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rab@frat@liftforworldmodel@ixs@meandiff\endcsname{0.001}
\expandafter\def\csname rev@rab@frat@liftforworldmodel@total@hi\endcsname{0.013}
\expandafter\def\csname rev@rab@frat@liftforworldmodel@total@lo\endcsname{\textminus 0.047}
\expandafter\def\csname rev@rab@frat@liftforworldmodel@total@meandiff\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rab@frat@liftmatchedforworldmodel@ixs@hi\endcsname{0.008}
\expandafter\def\csname rev@rab@frat@liftmatchedforworldmodel@ixs@lo\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@frat@liftmatchedforworldmodel@ixs@meandiff\endcsname{0.003}
\expandafter\def\csname rev@rab@frat@liftmatchedforworldmodel@total@hi\endcsname{0.038}
\expandafter\def\csname rev@rab@frat@liftmatchedforworldmodel@total@lo\endcsname{\textminus 0.020}
\expandafter\def\csname rev@rab@frat@liftmatchedforworldmodel@total@meandiff\endcsname{0.007}
\expandafter\def\csname rev@rab@frat@withoutlightgbm@ixs@hi\endcsname{0.013}
\expandafter\def\csname rev@rab@frat@withoutlightgbm@ixs@lo\endcsname{0.007}
\expandafter\def\csname rev@rab@frat@withoutlightgbm@ixs@meandiff\endcsname{0.010}
\expandafter\def\csname rev@rab@frat@withoutlightgbm@total@hi\endcsname{0.039}
\expandafter\def\csname rev@rab@frat@withoutlightgbm@total@lo\endcsname{0.005}
\expandafter\def\csname rev@rab@frat@withoutlightgbm@total@meandiff\endcsname{0.021}
\expandafter\def\csname rev@rab@frat@withouttimesfm@ixs@hi\endcsname{0.019}
\expandafter\def\csname rev@rab@frat@withouttimesfm@ixs@lo\endcsname{0.005}
\expandafter\def\csname rev@rab@frat@withouttimesfm@ixs@meandiff\endcsname{0.012}
\expandafter\def\csname rev@rab@frat@withouttimesfm@total@hi\endcsname{0.082}
\expandafter\def\csname rev@rab@frat@withouttimesfm@total@lo\endcsname{0.020}
\expandafter\def\csname rev@rab@frat@withouttimesfm@total@meandiff\endcsname{0.051}
\expandafter\def\csname rev@rab@frat@withoutworldmodel@ixs@hi\endcsname{0.007}
\expandafter\def\csname rev@rab@frat@withoutworldmodel@ixs@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rab@frat@withoutworldmodel@ixs@meandiff\endcsname{0.002}
\expandafter\def\csname rev@rab@frat@withoutworldmodel@total@hi\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rab@frat@withoutworldmodel@total@lo\endcsname{\textminus 0.064}
\expandafter\def\csname rev@rab@frat@withoutworldmodel@total@meandiff\endcsname{\textminus 0.040}
\expandafter\def\csname rev@rab@fre@fittedalllevels@ixs@hi\endcsname{0.010}
\expandafter\def\csname rev@rab@fre@fittedalllevels@ixs@lo\endcsname{\textminus 0.012}
\expandafter\def\csname rev@rab@fre@fittedalllevels@ixs@meandiff\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@fre@fittedalllevels@total@hi\endcsname{0.013}
\expandafter\def\csname rev@rab@fre@fittedalllevels@total@lo\endcsname{\textminus 0.044}
\expandafter\def\csname rev@rab@fre@fittedalllevels@total@meandiff\endcsname{\textminus 0.015}
\expandafter\def\csname rev@rab@fre@fittedbottom@ixs@hi\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@fre@fittedbottom@ixs@lo\endcsname{\textminus 0.013}
\expandafter\def\csname rev@rab@fre@fittedbottom@ixs@meandiff\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rab@fre@fittedbottom@total@hi\endcsname{0.009}
\expandafter\def\csname rev@rab@fre@fittedbottom@total@lo\endcsname{\textminus 0.047}
\expandafter\def\csname rev@rab@fre@fittedbottom@total@meandiff\endcsname{\textminus 0.018}
\expandafter\def\csname rev@rab@fre@fittedtotal@ixs@hi\endcsname{0.039}
\expandafter\def\csname rev@rab@fre@fittedtotal@ixs@lo\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rab@fre@fittedtotal@ixs@meandiff\endcsname{0.011}
\expandafter\def\csname rev@rab@fre@fittedtotal@total@hi\endcsname{0.028}
\expandafter\def\csname rev@rab@fre@fittedtotal@total@lo\endcsname{\textminus 0.031}
\expandafter\def\csname rev@rab@fre@fittedtotal@total@meandiff\endcsname{0.002}
\expandafter\def\csname rev@rab@fre@liftforworldmodel@ixs@hi\endcsname{0.016}
\expandafter\def\csname rev@rab@fre@liftforworldmodel@ixs@lo\endcsname{\textminus 0.010}
\expandafter\def\csname rev@rab@fre@liftforworldmodel@ixs@meandiff\endcsname{0.005}
\expandafter\def\csname rev@rab@fre@liftforworldmodel@total@hi\endcsname{0.047}
\expandafter\def\csname rev@rab@fre@liftforworldmodel@total@lo\endcsname{\textminus 0.020}
\expandafter\def\csname rev@rab@fre@liftforworldmodel@total@meandiff\endcsname{0.013}
\expandafter\def\csname rev@rab@fre@withoutlightgbm@ixs@hi\endcsname{0.026}
\expandafter\def\csname rev@rab@fre@withoutlightgbm@ixs@lo\endcsname{0.013}
\expandafter\def\csname rev@rab@fre@withoutlightgbm@ixs@meandiff\endcsname{0.019}
\expandafter\def\csname rev@rab@fre@withoutlightgbm@total@hi\endcsname{0.069}
\expandafter\def\csname rev@rab@fre@withoutlightgbm@total@lo\endcsname{0.002}
\expandafter\def\csname rev@rab@fre@withoutlightgbm@total@meandiff\endcsname{0.034}
\expandafter\def\csname rev@rab@fre@withouttimesfm@ixs@hi\endcsname{0.006}
\expandafter\def\csname rev@rab@fre@withouttimesfm@ixs@lo\endcsname{\textminus 0.010}
\expandafter\def\csname rev@rab@fre@withouttimesfm@ixs@meandiff\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rab@fre@withouttimesfm@total@hi\endcsname{0.003}
\expandafter\def\csname rev@rab@fre@withouttimesfm@total@lo\endcsname{\textminus 0.053}
\expandafter\def\csname rev@rab@fre@withouttimesfm@total@meandiff\endcsname{\textminus 0.026}
\expandafter\def\csname rev@rab@fre@withoutworldmodel@ixs@hi\endcsname{0.019}
\expandafter\def\csname rev@rab@fre@withoutworldmodel@ixs@lo\endcsname{0.006}
\expandafter\def\csname rev@rab@fre@withoutworldmodel@ixs@meandiff\endcsname{0.012}
\expandafter\def\csname rev@rab@fre@withoutworldmodel@total@hi\endcsname{0.041}
\expandafter\def\csname rev@rab@fre@withoutworldmodel@total@lo\endcsname{0.009}
\expandafter\def\csname rev@rab@fre@withoutworldmodel@total@meandiff\endcsname{0.025}
\expandafter\def\csname rev@rab@mfive@fittedalllevels@ixs@hi\endcsname{0.021}
\expandafter\def\csname rev@rab@mfive@fittedalllevels@ixs@lo\endcsname{0.009}
\expandafter\def\csname rev@rab@mfive@fittedalllevels@ixs@meandiff\endcsname{0.013}
\expandafter\def\csname rev@rab@mfive@fittedalllevels@total@hi\endcsname{0.047}
\expandafter\def\csname rev@rab@mfive@fittedalllevels@total@lo\endcsname{\textminus 0.144}
\expandafter\def\csname rev@rab@mfive@fittedalllevels@total@meandiff\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rab@mfive@fittedbottom@ixs@hi\endcsname{0.004}
\expandafter\def\csname rev@rab@mfive@fittedbottom@ixs@lo\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@mfive@fittedbottom@ixs@meandiff\endcsname{0.001}
\expandafter\def\csname rev@rab@mfive@fittedbottom@total@hi\endcsname{0.105}
\expandafter\def\csname rev@rab@mfive@fittedbottom@total@lo\endcsname{0.021}
\expandafter\def\csname rev@rab@mfive@fittedbottom@total@meandiff\endcsname{0.049}
\expandafter\def\csname rev@rab@mfive@fittedtotal@ixs@hi\endcsname{0.021}
\expandafter\def\csname rev@rab@mfive@fittedtotal@ixs@lo\endcsname{0.009}
\expandafter\def\csname rev@rab@mfive@fittedtotal@ixs@meandiff\endcsname{0.016}
\expandafter\def\csname rev@rab@mfive@fittedtotal@total@hi\endcsname{0.142}
\expandafter\def\csname rev@rab@mfive@fittedtotal@total@lo\endcsname{\textminus 0.153}
\expandafter\def\csname rev@rab@mfive@fittedtotal@total@meandiff\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rab@mfive@liftforworldmodel@ixs@hi\endcsname{0.001}
\expandafter\def\csname rev@rab@mfive@liftforworldmodel@ixs@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rab@mfive@liftforworldmodel@ixs@meandiff\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@mfive@liftforworldmodel@total@hi\endcsname{0.061}
\expandafter\def\csname rev@rab@mfive@liftforworldmodel@total@lo\endcsname{\textminus 0.100}
\expandafter\def\csname rev@rab@mfive@liftforworldmodel@total@meandiff\endcsname{0.000}
\expandafter\def\csname rev@rab@mfive@withoutlightgbm@ixs@hi\endcsname{0.008}
\expandafter\def\csname rev@rab@mfive@withoutlightgbm@ixs@lo\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@mfive@withoutlightgbm@ixs@meandiff\endcsname{0.003}
\expandafter\def\csname rev@rab@mfive@withoutlightgbm@total@hi\endcsname{0.155}
\expandafter\def\csname rev@rab@mfive@withoutlightgbm@total@lo\endcsname{\textminus 0.022}
\expandafter\def\csname rev@rab@mfive@withoutlightgbm@total@meandiff\endcsname{0.050}
\expandafter\def\csname rev@rab@mfive@withouttimesfm@ixs@hi\endcsname{0.009}
\expandafter\def\csname rev@rab@mfive@withouttimesfm@ixs@lo\endcsname{0.002}
\expandafter\def\csname rev@rab@mfive@withouttimesfm@ixs@meandiff\endcsname{0.006}
\expandafter\def\csname rev@rab@mfive@withouttimesfm@total@hi\endcsname{\textminus 0.052}
\expandafter\def\csname rev@rab@mfive@withouttimesfm@total@lo\endcsname{\textminus 0.144}
\expandafter\def\csname rev@rab@mfive@withouttimesfm@total@meandiff\endcsname{\textminus 0.112}
\expandafter\def\csname rev@rab@mfive@withoutworldmodel@ixs@hi\endcsname{0.007}
\expandafter\def\csname rev@rab@mfive@withoutworldmodel@ixs@lo\endcsname{0.003}
\expandafter\def\csname rev@rab@mfive@withoutworldmodel@ixs@meandiff\endcsname{0.005}
\expandafter\def\csname rev@rab@mfive@withoutworldmodel@total@hi\endcsname{0.190}
\expandafter\def\csname rev@rab@mfive@withoutworldmodel@total@lo\endcsname{0.018}
\expandafter\def\csname rev@rab@mfive@withoutworldmodel@total@meandiff\endcsname{0.113}
\expandafter\def\csname rev@rab@sdr@fittedalllevels@ixs@hi\endcsname{0.006}
\expandafter\def\csname rev@rab@sdr@fittedalllevels@ixs@lo\endcsname{\textminus 0.016}
\expandafter\def\csname rev@rab@sdr@fittedalllevels@ixs@meandiff\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rab@sdr@fittedalllevels@total@hi\endcsname{0.018}
\expandafter\def\csname rev@rab@sdr@fittedalllevels@total@lo\endcsname{\textminus 0.038}
\expandafter\def\csname rev@rab@sdr@fittedalllevels@total@meandiff\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rab@sdr@fittedbottom@ixs@hi\endcsname{0.009}
\expandafter\def\csname rev@rab@sdr@fittedbottom@ixs@lo\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rab@sdr@fittedbottom@ixs@meandiff\endcsname{0.001}
\expandafter\def\csname rev@rab@sdr@fittedbottom@total@hi\endcsname{0.034}
\expandafter\def\csname rev@rab@sdr@fittedbottom@total@lo\endcsname{\textminus 0.030}
\expandafter\def\csname rev@rab@sdr@fittedbottom@total@meandiff\endcsname{0.003}
\expandafter\def\csname rev@rab@sdr@fittedtotal@ixs@hi\endcsname{0.013}
\expandafter\def\csname rev@rab@sdr@fittedtotal@ixs@lo\endcsname{\textminus 0.018}
\expandafter\def\csname rev@rab@sdr@fittedtotal@ixs@meandiff\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rab@sdr@fittedtotal@total@hi\endcsname{0.036}
\expandafter\def\csname rev@rab@sdr@fittedtotal@total@lo\endcsname{\textminus 0.039}
\expandafter\def\csname rev@rab@sdr@fittedtotal@total@meandiff\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rab@sdr@liftforworldmodel@ixs@hi\endcsname{0.023}
\expandafter\def\csname rev@rab@sdr@liftforworldmodel@ixs@lo\endcsname{0.009}
\expandafter\def\csname rev@rab@sdr@liftforworldmodel@ixs@meandiff\endcsname{0.015}
\expandafter\def\csname rev@rab@sdr@liftforworldmodel@total@hi\endcsname{0.032}
\expandafter\def\csname rev@rab@sdr@liftforworldmodel@total@lo\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rab@sdr@liftforworldmodel@total@meandiff\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rab@sdr@withoutlightgbm@ixs@hi\endcsname{0.035}
\expandafter\def\csname rev@rab@sdr@withoutlightgbm@ixs@lo\endcsname{0.010}
\expandafter\def\csname rev@rab@sdr@withoutlightgbm@ixs@meandiff\endcsname{0.023}
\expandafter\def\csname rev@rab@sdr@withoutlightgbm@total@hi\endcsname{0.088}
\expandafter\def\csname rev@rab@sdr@withoutlightgbm@total@lo\endcsname{0.008}
\expandafter\def\csname rev@rab@sdr@withoutlightgbm@total@meandiff\endcsname{0.045}
\expandafter\def\csname rev@rab@sdr@withouttimesfm@ixs@hi\endcsname{0.025}
\expandafter\def\csname rev@rab@sdr@withouttimesfm@ixs@lo\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rab@sdr@withouttimesfm@ixs@meandiff\endcsname{0.009}
\expandafter\def\csname rev@rab@sdr@withouttimesfm@total@hi\endcsname{0.016}
\expandafter\def\csname rev@rab@sdr@withouttimesfm@total@lo\endcsname{\textminus 0.054}
\expandafter\def\csname rev@rab@sdr@withouttimesfm@total@meandiff\endcsname{\textminus 0.022}
\expandafter\def\csname rev@rab@sdr@withoutworldmodel@ixs@hi\endcsname{0.022}
\expandafter\def\csname rev@rab@sdr@withoutworldmodel@ixs@lo\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rab@sdr@withoutworldmodel@ixs@meandiff\endcsname{0.008}
\expandafter\def\csname rev@rab@sdr@withoutworldmodel@total@hi\endcsname{0.065}
\expandafter\def\csname rev@rab@sdr@withoutworldmodel@total@lo\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rab@sdr@withoutworldmodel@total@meandiff\endcsname{0.025}
\expandafter\def\csname rev@rab@sna@fittedalllevels@ixs@hi\endcsname{0.009}
\expandafter\def\csname rev@rab@sna@fittedalllevels@ixs@lo\endcsname{\textminus 0.000}
\expandafter\def\csname rev@rab@sna@fittedalllevels@ixs@meandiff\endcsname{0.004}
\expandafter\def\csname rev@rab@sna@fittedalllevels@total@hi\endcsname{0.042}
\expandafter\def\csname rev@rab@sna@fittedalllevels@total@lo\endcsname{\textminus 0.255}
\expandafter\def\csname rev@rab@sna@fittedalllevels@total@meandiff\endcsname{\textminus 0.073}
\expandafter\def\csname rev@rab@sna@fittedbottom@ixs@hi\endcsname{0.002}
\expandafter\def\csname rev@rab@sna@fittedbottom@ixs@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rab@sna@fittedbottom@ixs@meandiff\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@sna@fittedbottom@total@hi\endcsname{0.014}
\expandafter\def\csname rev@rab@sna@fittedbottom@total@lo\endcsname{\textminus 0.243}
\expandafter\def\csname rev@rab@sna@fittedbottom@total@meandiff\endcsname{\textminus 0.085}
\expandafter\def\csname rev@rab@sna@fittedtotal@ixs@hi\endcsname{0.018}
\expandafter\def\csname rev@rab@sna@fittedtotal@ixs@lo\endcsname{0.004}
\expandafter\def\csname rev@rab@sna@fittedtotal@ixs@meandiff\endcsname{0.011}
\expandafter\def\csname rev@rab@sna@fittedtotal@total@hi\endcsname{0.062}
\expandafter\def\csname rev@rab@sna@fittedtotal@total@lo\endcsname{\textminus 0.274}
\expandafter\def\csname rev@rab@sna@fittedtotal@total@meandiff\endcsname{\textminus 0.060}
\expandafter\def\csname rev@rab@sna@liftforworldmodel@ixs@hi\endcsname{0.006}
\expandafter\def\csname rev@rab@sna@liftforworldmodel@ixs@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rab@sna@liftforworldmodel@ixs@meandiff\endcsname{0.002}
\expandafter\def\csname rev@rab@sna@liftforworldmodel@total@hi\endcsname{0.012}
\expandafter\def\csname rev@rab@sna@liftforworldmodel@total@lo\endcsname{\textminus 0.318}
\expandafter\def\csname rev@rab@sna@liftforworldmodel@total@meandiff\endcsname{\textminus 0.145}
\expandafter\def\csname rev@rab@sna@withoutlightgbm@ixs@hi\endcsname{0.022}
\expandafter\def\csname rev@rab@sna@withoutlightgbm@ixs@lo\endcsname{0.014}
\expandafter\def\csname rev@rab@sna@withoutlightgbm@ixs@meandiff\endcsname{0.018}
\expandafter\def\csname rev@rab@sna@withoutlightgbm@total@hi\endcsname{0.324}
\expandafter\def\csname rev@rab@sna@withoutlightgbm@total@lo\endcsname{\textminus 0.013}
\expandafter\def\csname rev@rab@sna@withoutlightgbm@total@meandiff\endcsname{0.118}
\expandafter\def\csname rev@rab@sna@withouttimesfm@ixs@hi\endcsname{0.009}
\expandafter\def\csname rev@rab@sna@withouttimesfm@ixs@lo\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@sna@withouttimesfm@ixs@meandiff\endcsname{0.004}
\expandafter\def\csname rev@rab@sna@withouttimesfm@total@hi\endcsname{0.050}
\expandafter\def\csname rev@rab@sna@withouttimesfm@total@lo\endcsname{\textminus 0.026}
\expandafter\def\csname rev@rab@sna@withouttimesfm@total@meandiff\endcsname{0.013}
\expandafter\def\csname rev@rab@sna@withoutworldmodel@ixs@hi\endcsname{0.005}
\expandafter\def\csname rev@rab@sna@withoutworldmodel@ixs@lo\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rab@sna@withoutworldmodel@ixs@meandiff\endcsname{0.002}
\expandafter\def\csname rev@rab@sna@withoutworldmodel@total@hi\endcsname{0.019}
\expandafter\def\csname rev@rab@sna@withoutworldmodel@total@lo\endcsname{\textminus 0.290}
\expandafter\def\csname rev@rab@sna@withoutworldmodel@total@meandiff\endcsname{\textminus 0.095}
\expandafter\def\csname rev@raft@ana@afterpromow2@afterpromoerr\endcsname{0.561}
\expandafter\def\csname rev@raft@ana@afterpromow2@afterpromofa\endcsname{1.01}
\expandafter\def\csname rev@raft@ana@afterpromow2@overall\endcsname{0.699}
\expandafter\def\csname rev@raft@ana@afterpromow5@afterpromoerr\endcsname{0.550}
\expandafter\def\csname rev@raft@ana@afterpromow5@afterpromofa\endcsname{1.03}
\expandafter\def\csname rev@raft@ana@afterpromow5@overall\endcsname{0.691}
\expandafter\def\csname rev@raft@ana@worldmodel@afterpromoerr\endcsname{0.571}
\expandafter\def\csname rev@raft@ana@worldmodel@afterpromofa\endcsname{0.99}
\expandafter\def\csname rev@raft@ana@worldmodel@overall\endcsname{0.653}
\expandafter\def\csname rev@raft@bjc@afterpromow2@afterpromoerr\endcsname{0.495}
\expandafter\def\csname rev@raft@bjc@afterpromow2@afterpromofa\endcsname{1.00}
\expandafter\def\csname rev@raft@bjc@afterpromow2@overall\endcsname{1.084}
\expandafter\def\csname rev@raft@bjc@afterpromow5@afterpromoerr\endcsname{0.482}
\expandafter\def\csname rev@raft@bjc@afterpromow5@afterpromofa\endcsname{0.97}
\expandafter\def\csname rev@raft@bjc@afterpromow5@overall\endcsname{1.030}
\expandafter\def\csname rev@raft@bjc@worldmodel@afterpromoerr\endcsname{0.526}
\expandafter\def\csname rev@raft@bjc@worldmodel@afterpromofa\endcsname{1.02}
\expandafter\def\csname rev@raft@bjc@worldmodel@overall\endcsname{1.092}
\expandafter\def\csname rev@raft@che@afterpromow2@afterpromoerr\endcsname{0.393}
\expandafter\def\csname rev@raft@che@afterpromow2@afterpromofa\endcsname{0.99}
\expandafter\def\csname rev@raft@che@afterpromow2@overall\endcsname{1.094}
\expandafter\def\csname rev@raft@che@afterpromow5@afterpromoerr\endcsname{0.388}
\expandafter\def\csname rev@raft@che@afterpromow5@afterpromofa\endcsname{1.00}
\expandafter\def\csname rev@raft@che@afterpromow5@overall\endcsname{1.043}
\expandafter\def\csname rev@raft@che@worldmodel@afterpromoerr\endcsname{0.402}
\expandafter\def\csname rev@raft@che@worldmodel@afterpromofa\endcsname{1.04}
\expandafter\def\csname rev@raft@che@worldmodel@overall\endcsname{1.281}
\expandafter\def\csname rev@raft@fre@afterpromow2@afterpromoerr\endcsname{0.382}
\expandafter\def\csname rev@raft@fre@afterpromow2@afterpromofa\endcsname{0.66}
\expandafter\def\csname rev@raft@fre@afterpromow2@overall\endcsname{0.411}
\expandafter\def\csname rev@raft@fre@afterpromow5@afterpromoerr\endcsname{0.383}
\expandafter\def\csname rev@raft@fre@afterpromow5@afterpromofa\endcsname{0.64}
\expandafter\def\csname rev@raft@fre@afterpromow5@overall\endcsname{0.408}
\expandafter\def\csname rev@raft@fre@worldmodel@afterpromoerr\endcsname{0.391}
\expandafter\def\csname rev@raft@fre@worldmodel@afterpromofa\endcsname{0.66}
\expandafter\def\csname rev@raft@fre@worldmodel@overall\endcsname{0.387}
\expandafter\def\csname rev@raft@sdr@afterpromow2@afterpromoerr\endcsname{0.150}
\expandafter\def\csname rev@raft@sdr@afterpromow2@afterpromofa\endcsname{0.98}
\expandafter\def\csname rev@raft@sdr@afterpromow2@overall\endcsname{0.861}
\expandafter\def\csname rev@raft@sdr@afterpromow5@afterpromoerr\endcsname{0.174}
\expandafter\def\csname rev@raft@sdr@afterpromow5@afterpromofa\endcsname{1.03}
\expandafter\def\csname rev@raft@sdr@afterpromow5@overall\endcsname{0.833}
\expandafter\def\csname rev@raft@sdr@worldmodel@afterpromoerr\endcsname{0.174}
\expandafter\def\csname rev@raft@sdr@worldmodel@afterpromofa\endcsname{0.97}
\expandafter\def\csname rev@raft@sdr@worldmodel@overall\endcsname{0.829}
\expandafter\def\csname rev@raft@sna@afterpromow2@afterpromoerr\endcsname{0.413}
\expandafter\def\csname rev@raft@sna@afterpromow2@afterpromofa\endcsname{0.93}
\expandafter\def\csname rev@raft@sna@afterpromow2@overall\endcsname{0.857}
\expandafter\def\csname rev@raft@sna@afterpromow5@afterpromoerr\endcsname{0.422}
\expandafter\def\csname rev@raft@sna@afterpromow5@afterpromofa\endcsname{1.11}
\expandafter\def\csname rev@raft@sna@afterpromow5@overall\endcsname{0.854}
\expandafter\def\csname rev@raft@sna@worldmodel@afterpromoerr\endcsname{0.477}
\expandafter\def\csname rev@raft@sna@worldmodel@afterpromofa\endcsname{1.02}
\expandafter\def\csname rev@raft@sna@worldmodel@overall\endcsname{0.749}
\expandafter\def\csname rev@rcc@ana@asfirstrun@ens@cost\endcsname{2073500000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@ens@hi\endcsname{336030000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@ens@lo\endcsname{\textminus 52393000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@ens@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@ana@asfirstrun@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@asfirstrun@ens@worldminus\endcsname{90909000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lgb@cost\endcsname{1916400000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lgb@hi\endcsname{810390000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lgb@lo\endcsname{\textminus 60939000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lgb@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lgb@worldminus\endcsname{247970000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lift@cost\endcsname{1990700000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lift@hi\endcsname{538610000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lift@lo\endcsname{\textminus 0.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@asfirstrun@lift@worldminus\endcsname{173670000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@naive@cost\endcsname{5061600000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@naive@hi\endcsname{\textminus 151530000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@naive@lo\endcsname{\textminus 8650100000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@ana@asfirstrun@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@asfirstrun@naive@worldminus\endcsname{\textminus 2897200000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@tfmplan@cost\endcsname{2139600000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@tfmplan@hi\endcsname{215570000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@tfmplan@lo\endcsname{\textminus 116140000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@tfmplan@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@ana@asfirstrun@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@asfirstrun@tfmplan@worldminus\endcsname{24755000.000}
\expandafter\def\csname rev@rcc@ana@asfirstrun@world@cost\endcsname{2164400000.000}
\expandafter\def\csname rev@rcc@ana@dollars@ens@cost\endcsname{0.103}
\expandafter\def\csname rev@rcc@ana@dollars@ens@hi\endcsname{0.007}
\expandafter\def\csname rev@rcc@ana@dollars@ens@lo\endcsname{0.003}
\expandafter\def\csname rev@rcc@ana@dollars@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@ana@dollars@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@dollars@ens@worldminus\endcsname{0.005}
\expandafter\def\csname rev@rcc@ana@dollars@lgb@cost\endcsname{0.107}
\expandafter\def\csname rev@rcc@ana@dollars@lgb@hi\endcsname{0.005}
\expandafter\def\csname rev@rcc@ana@dollars@lgb@lo\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@ana@dollars@lgb@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@ana@dollars@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@dollars@lgb@worldminus\endcsname{0.001}
\expandafter\def\csname rev@rcc@ana@dollars@lift@cost\endcsname{0.109}
\expandafter\def\csname rev@rcc@ana@dollars@lift@hi\endcsname{0.002}
\expandafter\def\csname rev@rcc@ana@dollars@lift@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rcc@ana@dollars@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@ana@dollars@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@dollars@lift@worldminus\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rcc@ana@dollars@naive@cost\endcsname{0.224}
\expandafter\def\csname rev@rcc@ana@dollars@naive@hi\endcsname{\textminus 0.101}
\expandafter\def\csname rev@rcc@ana@dollars@naive@lo\endcsname{\textminus 0.132}
\expandafter\def\csname rev@rcc@ana@dollars@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@ana@dollars@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@dollars@naive@worldminus\endcsname{\textminus 0.116}
\expandafter\def\csname rev@rcc@ana@dollars@tfmplan@cost\endcsname{0.114}
\expandafter\def\csname rev@rcc@ana@dollars@tfmplan@hi\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@ana@dollars@tfmplan@lo\endcsname{\textminus 0.009}
\expandafter\def\csname rev@rcc@ana@dollars@tfmplan@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@ana@dollars@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@dollars@tfmplan@worldminus\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rcc@ana@dollars@world@cost\endcsname{0.109}
\expandafter\def\csname rev@rcc@ana@firsthalf@ens@cost\endcsname{0.104}
\expandafter\def\csname rev@rcc@ana@firsthalf@ens@hi\endcsname{0.005}
\expandafter\def\csname rev@rcc@ana@firsthalf@ens@lo\endcsname{0.001}
\expandafter\def\csname rev@rcc@ana@firsthalf@ens@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@ana@firsthalf@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@firsthalf@ens@worldminus\endcsname{0.003}
\expandafter\def\csname rev@rcc@ana@firsthalf@lgb@cost\endcsname{0.106}
\expandafter\def\csname rev@rcc@ana@firsthalf@lgb@hi\endcsname{0.006}
\expandafter\def\csname rev@rcc@ana@firsthalf@lgb@lo\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@ana@firsthalf@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@ana@firsthalf@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@firsthalf@lgb@worldminus\endcsname{0.002}
\expandafter\def\csname rev@rcc@ana@firsthalf@lift@cost\endcsname{0.112}
\expandafter\def\csname rev@rcc@ana@firsthalf@lift@hi\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@ana@firsthalf@lift@lo\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rcc@ana@firsthalf@lift@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@ana@firsthalf@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@firsthalf@lift@worldminus\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rcc@ana@firsthalf@naive@cost\endcsname{0.255}
\expandafter\def\csname rev@rcc@ana@firsthalf@naive@hi\endcsname{\textminus 0.132}
\expandafter\def\csname rev@rcc@ana@firsthalf@naive@lo\endcsname{\textminus 0.163}
\expandafter\def\csname rev@rcc@ana@firsthalf@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@ana@firsthalf@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@firsthalf@naive@worldminus\endcsname{\textminus 0.147}
\expandafter\def\csname rev@rcc@ana@firsthalf@tfmplan@cost\endcsname{0.116}
\expandafter\def\csname rev@rcc@ana@firsthalf@tfmplan@hi\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rcc@ana@firsthalf@tfmplan@lo\endcsname{\textminus 0.013}
\expandafter\def\csname rev@rcc@ana@firsthalf@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@ana@firsthalf@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@firsthalf@tfmplan@worldminus\endcsname{\textminus 0.009}
\expandafter\def\csname rev@rcc@ana@firsthalf@world@cost\endcsname{0.108}
\expandafter\def\csname rev@rcc@ana@nodemean@ens@cost\endcsname{0.145}
\expandafter\def\csname rev@rcc@ana@nodemean@ens@hi\endcsname{0.009}
\expandafter\def\csname rev@rcc@ana@nodemean@ens@lo\endcsname{0.005}
\expandafter\def\csname rev@rcc@ana@nodemean@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@ana@nodemean@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@nodemean@ens@worldminus\endcsname{0.007}
\expandafter\def\csname rev@rcc@ana@nodemean@lgb@cost\endcsname{0.146}
\expandafter\def\csname rev@rcc@ana@nodemean@lgb@hi\endcsname{0.011}
\expandafter\def\csname rev@rcc@ana@nodemean@lgb@lo\endcsname{0.002}
\expandafter\def\csname rev@rcc@ana@nodemean@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@ana@nodemean@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@nodemean@lgb@worldminus\endcsname{0.006}
\expandafter\def\csname rev@rcc@ana@nodemean@lift@cost\endcsname{0.152}
\expandafter\def\csname rev@rcc@ana@nodemean@lift@hi\endcsname{0.003}
\expandafter\def\csname rev@rcc@ana@nodemean@lift@lo\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@ana@nodemean@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@ana@nodemean@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@nodemean@lift@worldminus\endcsname{0.000}
\expandafter\def\csname rev@rcc@ana@nodemean@naive@cost\endcsname{0.262}
\expandafter\def\csname rev@rcc@ana@nodemean@naive@hi\endcsname{\textminus 0.095}
\expandafter\def\csname rev@rcc@ana@nodemean@naive@lo\endcsname{\textminus 0.128}
\expandafter\def\csname rev@rcc@ana@nodemean@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@ana@nodemean@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@nodemean@naive@worldminus\endcsname{\textminus 0.110}
\expandafter\def\csname rev@rcc@ana@nodemean@tfmplan@cost\endcsname{0.157}
\expandafter\def\csname rev@rcc@ana@nodemean@tfmplan@hi\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rcc@ana@nodemean@tfmplan@lo\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rcc@ana@nodemean@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@ana@nodemean@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@nodemean@tfmplan@worldminus\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rcc@ana@nodemean@world@cost\endcsname{0.152}
\expandafter\def\csname rev@rcc@ana@units@ens@cost\endcsname{0.114}
\expandafter\def\csname rev@rcc@ana@units@ens@hi\endcsname{0.008}
\expandafter\def\csname rev@rcc@ana@units@ens@lo\endcsname{0.004}
\expandafter\def\csname rev@rcc@ana@units@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@ana@units@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@units@ens@worldminus\endcsname{0.006}
\expandafter\def\csname rev@rcc@ana@units@lgb@cost\endcsname{0.118}
\expandafter\def\csname rev@rcc@ana@units@lgb@hi\endcsname{0.006}
\expandafter\def\csname rev@rcc@ana@units@lgb@lo\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rcc@ana@units@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@ana@units@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@units@lgb@worldminus\endcsname{0.002}
\expandafter\def\csname rev@rcc@ana@units@lift@cost\endcsname{0.120}
\expandafter\def\csname rev@rcc@ana@units@lift@hi\endcsname{0.002}
\expandafter\def\csname rev@rcc@ana@units@lift@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rcc@ana@units@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@ana@units@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@units@lift@worldminus\endcsname{\textminus 0.000}
\expandafter\def\csname rev@rcc@ana@units@naive@cost\endcsname{0.239}
\expandafter\def\csname rev@rcc@ana@units@naive@hi\endcsname{\textminus 0.104}
\expandafter\def\csname rev@rcc@ana@units@naive@lo\endcsname{\textminus 0.136}
\expandafter\def\csname rev@rcc@ana@units@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@ana@units@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@units@naive@worldminus\endcsname{\textminus 0.119}
\expandafter\def\csname rev@rcc@ana@units@tfmplan@cost\endcsname{0.125}
\expandafter\def\csname rev@rcc@ana@units@tfmplan@hi\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rcc@ana@units@tfmplan@lo\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rcc@ana@units@tfmplan@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@ana@units@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@units@tfmplan@worldminus\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rcc@ana@units@world@cost\endcsname{0.120}
\expandafter\def\csname rev@rcc@ana@weekly@ens@cost\endcsname{0.103}
\expandafter\def\csname rev@rcc@ana@weekly@ens@hi\endcsname{0.007}
\expandafter\def\csname rev@rcc@ana@weekly@ens@lo\endcsname{0.003}
\expandafter\def\csname rev@rcc@ana@weekly@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@ana@weekly@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@weekly@ens@worldminus\endcsname{0.005}
\expandafter\def\csname rev@rcc@ana@weekly@lgb@cost\endcsname{0.107}
\expandafter\def\csname rev@rcc@ana@weekly@lgb@hi\endcsname{0.005}
\expandafter\def\csname rev@rcc@ana@weekly@lgb@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rcc@ana@weekly@lgb@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@ana@weekly@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@weekly@lgb@worldminus\endcsname{0.001}
\expandafter\def\csname rev@rcc@ana@weekly@lift@cost\endcsname{0.109}
\expandafter\def\csname rev@rcc@ana@weekly@lift@hi\endcsname{0.002}
\expandafter\def\csname rev@rcc@ana@weekly@lift@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rcc@ana@weekly@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@ana@weekly@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@weekly@lift@worldminus\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rcc@ana@weekly@naive@cost\endcsname{0.224}
\expandafter\def\csname rev@rcc@ana@weekly@naive@hi\endcsname{\textminus 0.101}
\expandafter\def\csname rev@rcc@ana@weekly@naive@lo\endcsname{\textminus 0.132}
\expandafter\def\csname rev@rcc@ana@weekly@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@ana@weekly@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@weekly@naive@worldminus\endcsname{\textminus 0.116}
\expandafter\def\csname rev@rcc@ana@weekly@tfmplan@cost\endcsname{0.114}
\expandafter\def\csname rev@rcc@ana@weekly@tfmplan@hi\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@ana@weekly@tfmplan@lo\endcsname{\textminus 0.009}
\expandafter\def\csname rev@rcc@ana@weekly@tfmplan@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@ana@weekly@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@weekly@tfmplan@worldminus\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rcc@ana@weekly@world@cost\endcsname{0.109}
\expandafter\def\csname rev@rcc@ana@windowtotal@ens@cost\endcsname{0.059}
\expandafter\def\csname rev@rcc@ana@windowtotal@ens@hi\endcsname{0.013}
\expandafter\def\csname rev@rcc@ana@windowtotal@ens@lo\endcsname{0.007}
\expandafter\def\csname rev@rcc@ana@windowtotal@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@ana@windowtotal@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@windowtotal@ens@worldminus\endcsname{0.010}
\expandafter\def\csname rev@rcc@ana@windowtotal@lgb@cost\endcsname{0.059}
\expandafter\def\csname rev@rcc@ana@windowtotal@lgb@hi\endcsname{0.014}
\expandafter\def\csname rev@rcc@ana@windowtotal@lgb@lo\endcsname{0.005}
\expandafter\def\csname rev@rcc@ana@windowtotal@lgb@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@ana@windowtotal@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@windowtotal@lgb@worldminus\endcsname{0.010}
\expandafter\def\csname rev@rcc@ana@windowtotal@lift@cost\endcsname{0.068}
\expandafter\def\csname rev@rcc@ana@windowtotal@lift@hi\endcsname{0.005}
\expandafter\def\csname rev@rcc@ana@windowtotal@lift@lo\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@ana@windowtotal@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@ana@windowtotal@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@windowtotal@lift@worldminus\endcsname{0.001}
\expandafter\def\csname rev@rcc@ana@windowtotal@naive@cost\endcsname{0.163}
\expandafter\def\csname rev@rcc@ana@windowtotal@naive@hi\endcsname{\textminus 0.077}
\expandafter\def\csname rev@rcc@ana@windowtotal@naive@lo\endcsname{\textminus 0.112}
\expandafter\def\csname rev@rcc@ana@windowtotal@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@ana@windowtotal@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@windowtotal@naive@worldminus\endcsname{\textminus 0.094}
\expandafter\def\csname rev@rcc@ana@windowtotal@tfmplan@cost\endcsname{0.075}
\expandafter\def\csname rev@rcc@ana@windowtotal@tfmplan@hi\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rcc@ana@windowtotal@tfmplan@lo\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rcc@ana@windowtotal@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@ana@windowtotal@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@ana@windowtotal@tfmplan@worldminus\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rcc@ana@windowtotal@world@cost\endcsname{0.069}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@ens@cost\endcsname{8161500000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@ens@hi\endcsname{\textminus 209450000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@ens@lo\endcsname{\textminus 9702000000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@ens@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@ens@worldminus\endcsname{\textminus 3954800000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lgb@cost\endcsname{10057000000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lgb@hi\endcsname{\textminus 205740000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lgb@lo\endcsname{\textminus 14697000000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lgb@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lgb@worldminus\endcsname{\textminus 5849800000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lift@cost\endcsname{6480900000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lift@hi\endcsname{\textminus 85448000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lift@lo\endcsname{\textminus 5672400000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lift@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@lift@worldminus\endcsname{\textminus 2274200000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@naive@cost\endcsname{35392000000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@naive@hi\endcsname{\textminus 3040100000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@naive@lo\endcsname{\textminus 76130000000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@naive@worldminus\endcsname{\textminus 31186000000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@tfmplan@cost\endcsname{10221000000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@tfmplan@hi\endcsname{\textminus 405430000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@tfmplan@lo\endcsname{\textminus 14200000000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@tfmplan@worldminus\endcsname{\textminus 6014500000.000}
\expandafter\def\csname rev@rcc@bjc@asfirstrun@world@cost\endcsname{4206700000.000}
\expandafter\def\csname rev@rcc@bjc@dollars@ens@cost\endcsname{0.122}
\expandafter\def\csname rev@rcc@bjc@dollars@ens@hi\endcsname{0.037}
\expandafter\def\csname rev@rcc@bjc@dollars@ens@lo\endcsname{0.029}
\expandafter\def\csname rev@rcc@bjc@dollars@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@bjc@dollars@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@dollars@ens@worldminus\endcsname{0.033}
\expandafter\def\csname rev@rcc@bjc@dollars@lgb@cost\endcsname{0.130}
\expandafter\def\csname rev@rcc@bjc@dollars@lgb@hi\endcsname{0.031}
\expandafter\def\csname rev@rcc@bjc@dollars@lgb@lo\endcsname{0.019}
\expandafter\def\csname rev@rcc@bjc@dollars@lgb@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@bjc@dollars@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@dollars@lgb@worldminus\endcsname{0.025}
\expandafter\def\csname rev@rcc@bjc@dollars@lift@cost\endcsname{0.150}
\expandafter\def\csname rev@rcc@bjc@dollars@lift@hi\endcsname{0.027}
\expandafter\def\csname rev@rcc@bjc@dollars@lift@lo\endcsname{\textminus 0.036}
\expandafter\def\csname rev@rcc@bjc@dollars@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@bjc@dollars@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@dollars@lift@worldminus\endcsname{0.004}
\expandafter\def\csname rev@rcc@bjc@dollars@naive@cost\endcsname{0.324}
\expandafter\def\csname rev@rcc@bjc@dollars@naive@hi\endcsname{\textminus 0.157}
\expandafter\def\csname rev@rcc@bjc@dollars@naive@lo\endcsname{\textminus 0.184}
\expandafter\def\csname rev@rcc@bjc@dollars@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@dollars@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@dollars@naive@worldminus\endcsname{\textminus 0.170}
\expandafter\def\csname rev@rcc@bjc@dollars@tfmplan@cost\endcsname{0.147}
\expandafter\def\csname rev@rcc@bjc@dollars@tfmplan@hi\endcsname{0.015}
\expandafter\def\csname rev@rcc@bjc@dollars@tfmplan@lo\endcsname{0.001}
\expandafter\def\csname rev@rcc@bjc@dollars@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@bjc@dollars@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@dollars@tfmplan@worldminus\endcsname{0.008}
\expandafter\def\csname rev@rcc@bjc@dollars@world@cost\endcsname{0.155}
\expandafter\def\csname rev@rcc@bjc@firsthalf@ens@cost\endcsname{0.105}
\expandafter\def\csname rev@rcc@bjc@firsthalf@ens@hi\endcsname{0.031}
\expandafter\def\csname rev@rcc@bjc@firsthalf@ens@lo\endcsname{0.020}
\expandafter\def\csname rev@rcc@bjc@firsthalf@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@bjc@firsthalf@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@firsthalf@ens@worldminus\endcsname{0.026}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lgb@cost\endcsname{0.122}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lgb@hi\endcsname{0.016}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lgb@lo\endcsname{0.001}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lgb@worldminus\endcsname{0.009}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lift@cost\endcsname{0.111}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lift@hi\endcsname{0.025}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lift@lo\endcsname{0.014}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@firsthalf@lift@worldminus\endcsname{0.019}
\expandafter\def\csname rev@rcc@bjc@firsthalf@naive@cost\endcsname{0.352}
\expandafter\def\csname rev@rcc@bjc@firsthalf@naive@hi\endcsname{\textminus 0.206}
\expandafter\def\csname rev@rcc@bjc@firsthalf@naive@lo\endcsname{\textminus 0.239}
\expandafter\def\csname rev@rcc@bjc@firsthalf@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@firsthalf@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@firsthalf@naive@worldminus\endcsname{\textminus 0.222}
\expandafter\def\csname rev@rcc@bjc@firsthalf@tfmplan@cost\endcsname{0.132}
\expandafter\def\csname rev@rcc@bjc@firsthalf@tfmplan@hi\endcsname{0.006}
\expandafter\def\csname rev@rcc@bjc@firsthalf@tfmplan@lo\endcsname{\textminus 0.009}
\expandafter\def\csname rev@rcc@bjc@firsthalf@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@bjc@firsthalf@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@firsthalf@tfmplan@worldminus\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@bjc@firsthalf@world@cost\endcsname{0.130}
\expandafter\def\csname rev@rcc@bjc@nodemean@ens@cost\endcsname{0.166}
\expandafter\def\csname rev@rcc@bjc@nodemean@ens@hi\endcsname{0.035}
\expandafter\def\csname rev@rcc@bjc@nodemean@ens@lo\endcsname{0.027}
\expandafter\def\csname rev@rcc@bjc@nodemean@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@bjc@nodemean@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@nodemean@ens@worldminus\endcsname{0.031}
\expandafter\def\csname rev@rcc@bjc@nodemean@lgb@cost\endcsname{0.176}
\expandafter\def\csname rev@rcc@bjc@nodemean@lgb@hi\endcsname{0.027}
\expandafter\def\csname rev@rcc@bjc@nodemean@lgb@lo\endcsname{0.015}
\expandafter\def\csname rev@rcc@bjc@nodemean@lgb@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@bjc@nodemean@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@nodemean@lgb@worldminus\endcsname{0.021}
\expandafter\def\csname rev@rcc@bjc@nodemean@lift@cost\endcsname{0.194}
\expandafter\def\csname rev@rcc@bjc@nodemean@lift@hi\endcsname{0.023}
\expandafter\def\csname rev@rcc@bjc@nodemean@lift@lo\endcsname{\textminus 0.032}
\expandafter\def\csname rev@rcc@bjc@nodemean@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@bjc@nodemean@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@nodemean@lift@worldminus\endcsname{0.003}
\expandafter\def\csname rev@rcc@bjc@nodemean@naive@cost\endcsname{0.385}
\expandafter\def\csname rev@rcc@bjc@nodemean@naive@hi\endcsname{\textminus 0.160}
\expandafter\def\csname rev@rcc@bjc@nodemean@naive@lo\endcsname{\textminus 0.230}
\expandafter\def\csname rev@rcc@bjc@nodemean@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@nodemean@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@nodemean@naive@worldminus\endcsname{\textminus 0.188}
\expandafter\def\csname rev@rcc@bjc@nodemean@tfmplan@cost\endcsname{0.191}
\expandafter\def\csname rev@rcc@bjc@nodemean@tfmplan@hi\endcsname{0.013}
\expandafter\def\csname rev@rcc@bjc@nodemean@tfmplan@lo\endcsname{0.000}
\expandafter\def\csname rev@rcc@bjc@nodemean@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@bjc@nodemean@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@nodemean@tfmplan@worldminus\endcsname{0.007}
\expandafter\def\csname rev@rcc@bjc@nodemean@world@cost\endcsname{0.197}
\expandafter\def\csname rev@rcc@bjc@units@ens@cost\endcsname{0.131}
\expandafter\def\csname rev@rcc@bjc@units@ens@hi\endcsname{0.036}
\expandafter\def\csname rev@rcc@bjc@units@ens@lo\endcsname{0.028}
\expandafter\def\csname rev@rcc@bjc@units@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@bjc@units@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@units@ens@worldminus\endcsname{0.032}
\expandafter\def\csname rev@rcc@bjc@units@lgb@cost\endcsname{0.140}
\expandafter\def\csname rev@rcc@bjc@units@lgb@hi\endcsname{0.029}
\expandafter\def\csname rev@rcc@bjc@units@lgb@lo\endcsname{0.018}
\expandafter\def\csname rev@rcc@bjc@units@lgb@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@bjc@units@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@units@lgb@worldminus\endcsname{0.024}
\expandafter\def\csname rev@rcc@bjc@units@lift@cost\endcsname{0.158}
\expandafter\def\csname rev@rcc@bjc@units@lift@hi\endcsname{0.026}
\expandafter\def\csname rev@rcc@bjc@units@lift@lo\endcsname{\textminus 0.036}
\expandafter\def\csname rev@rcc@bjc@units@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@bjc@units@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@units@lift@worldminus\endcsname{0.005}
\expandafter\def\csname rev@rcc@bjc@units@naive@cost\endcsname{0.342}
\expandafter\def\csname rev@rcc@bjc@units@naive@hi\endcsname{\textminus 0.164}
\expandafter\def\csname rev@rcc@bjc@units@naive@lo\endcsname{\textminus 0.196}
\expandafter\def\csname rev@rcc@bjc@units@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@units@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@units@naive@worldminus\endcsname{\textminus 0.178}
\expandafter\def\csname rev@rcc@bjc@units@tfmplan@cost\endcsname{0.157}
\expandafter\def\csname rev@rcc@bjc@units@tfmplan@hi\endcsname{0.013}
\expandafter\def\csname rev@rcc@bjc@units@tfmplan@lo\endcsname{0.000}
\expandafter\def\csname rev@rcc@bjc@units@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@bjc@units@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@units@tfmplan@worldminus\endcsname{0.007}
\expandafter\def\csname rev@rcc@bjc@units@world@cost\endcsname{0.163}
\expandafter\def\csname rev@rcc@bjc@weekly@ens@cost\endcsname{0.122}
\expandafter\def\csname rev@rcc@bjc@weekly@ens@hi\endcsname{0.037}
\expandafter\def\csname rev@rcc@bjc@weekly@ens@lo\endcsname{0.029}
\expandafter\def\csname rev@rcc@bjc@weekly@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@bjc@weekly@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@weekly@ens@worldminus\endcsname{0.033}
\expandafter\def\csname rev@rcc@bjc@weekly@lgb@cost\endcsname{0.130}
\expandafter\def\csname rev@rcc@bjc@weekly@lgb@hi\endcsname{0.030}
\expandafter\def\csname rev@rcc@bjc@weekly@lgb@lo\endcsname{0.019}
\expandafter\def\csname rev@rcc@bjc@weekly@lgb@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@bjc@weekly@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@weekly@lgb@worldminus\endcsname{0.025}
\expandafter\def\csname rev@rcc@bjc@weekly@lift@cost\endcsname{0.150}
\expandafter\def\csname rev@rcc@bjc@weekly@lift@hi\endcsname{0.027}
\expandafter\def\csname rev@rcc@bjc@weekly@lift@lo\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rcc@bjc@weekly@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@bjc@weekly@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@weekly@lift@worldminus\endcsname{0.004}
\expandafter\def\csname rev@rcc@bjc@weekly@naive@cost\endcsname{0.324}
\expandafter\def\csname rev@rcc@bjc@weekly@naive@hi\endcsname{\textminus 0.157}
\expandafter\def\csname rev@rcc@bjc@weekly@naive@lo\endcsname{\textminus 0.185}
\expandafter\def\csname rev@rcc@bjc@weekly@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@weekly@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@weekly@naive@worldminus\endcsname{\textminus 0.170}
\expandafter\def\csname rev@rcc@bjc@weekly@tfmplan@cost\endcsname{0.147}
\expandafter\def\csname rev@rcc@bjc@weekly@tfmplan@hi\endcsname{0.015}
\expandafter\def\csname rev@rcc@bjc@weekly@tfmplan@lo\endcsname{0.002}
\expandafter\def\csname rev@rcc@bjc@weekly@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@bjc@weekly@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@weekly@tfmplan@worldminus\endcsname{0.008}
\expandafter\def\csname rev@rcc@bjc@weekly@world@cost\endcsname{0.155}
\expandafter\def\csname rev@rcc@bjc@windowtotal@ens@cost\endcsname{0.074}
\expandafter\def\csname rev@rcc@bjc@windowtotal@ens@hi\endcsname{0.039}
\expandafter\def\csname rev@rcc@bjc@windowtotal@ens@lo\endcsname{0.027}
\expandafter\def\csname rev@rcc@bjc@windowtotal@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@bjc@windowtotal@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@windowtotal@ens@worldminus\endcsname{0.033}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lgb@cost\endcsname{0.072}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lgb@hi\endcsname{0.043}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lgb@lo\endcsname{0.027}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lgb@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lgb@worldminus\endcsname{0.035}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lift@cost\endcsname{0.100}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lift@hi\endcsname{0.030}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lift@lo\endcsname{\textminus 0.038}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@windowtotal@lift@worldminus\endcsname{0.007}
\expandafter\def\csname rev@rcc@bjc@windowtotal@naive@cost\endcsname{0.170}
\expandafter\def\csname rev@rcc@bjc@windowtotal@naive@hi\endcsname{\textminus 0.047}
\expandafter\def\csname rev@rcc@bjc@windowtotal@naive@lo\endcsname{\textminus 0.080}
\expandafter\def\csname rev@rcc@bjc@windowtotal@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@bjc@windowtotal@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@windowtotal@naive@worldminus\endcsname{\textminus 0.063}
\expandafter\def\csname rev@rcc@bjc@windowtotal@tfmplan@cost\endcsname{0.106}
\expandafter\def\csname rev@rcc@bjc@windowtotal@tfmplan@hi\endcsname{0.009}
\expandafter\def\csname rev@rcc@bjc@windowtotal@tfmplan@lo\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rcc@bjc@windowtotal@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@bjc@windowtotal@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@bjc@windowtotal@tfmplan@worldminus\endcsname{0.001}
\expandafter\def\csname rev@rcc@bjc@windowtotal@world@cost\endcsname{0.107}
\expandafter\def\csname rev@rcc@che@asfirstrun@ens@cost\endcsname{24602000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@ens@hi\endcsname{\textminus 599130000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@ens@lo\endcsname{\textminus 34600000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@ens@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@che@asfirstrun@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@asfirstrun@ens@worldminus\endcsname{\textminus 13369000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@lgb@cost\endcsname{28549000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@lgb@hi\endcsname{\textminus 391270000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@lgb@lo\endcsname{\textminus 46869000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@lgb@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@che@asfirstrun@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@asfirstrun@lgb@worldminus\endcsname{\textminus 17317000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@lift@cost\endcsname{14824000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@lift@hi\endcsname{1725200000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@lift@lo\endcsname{\textminus 11391000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@lift@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@che@asfirstrun@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@asfirstrun@lift@worldminus\endcsname{\textminus 3591300000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@naive@cost\endcsname{94310000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@naive@hi\endcsname{\textminus 8860100000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@naive@lo\endcsname{\textminus 198210000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@che@asfirstrun@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@asfirstrun@naive@worldminus\endcsname{\textminus 83078000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@tfmplan@cost\endcsname{34023000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@tfmplan@hi\endcsname{\textminus 1234700000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@tfmplan@lo\endcsname{\textminus 57194000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@che@asfirstrun@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@asfirstrun@tfmplan@worldminus\endcsname{\textminus 22791000000.000}
\expandafter\def\csname rev@rcc@che@asfirstrun@world@cost\endcsname{11232000000.000}
\expandafter\def\csname rev@rcc@che@dollars@ens@cost\endcsname{0.142}
\expandafter\def\csname rev@rcc@che@dollars@ens@hi\endcsname{0.164}
\expandafter\def\csname rev@rcc@che@dollars@ens@lo\endcsname{0.050}
\expandafter\def\csname rev@rcc@che@dollars@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@che@dollars@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@dollars@ens@worldminus\endcsname{0.107}
\expandafter\def\csname rev@rcc@che@dollars@lgb@cost\endcsname{0.121}
\expandafter\def\csname rev@rcc@che@dollars@lgb@hi\endcsname{0.212}
\expandafter\def\csname rev@rcc@che@dollars@lgb@lo\endcsname{0.046}
\expandafter\def\csname rev@rcc@che@dollars@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@che@dollars@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@dollars@lgb@worldminus\endcsname{0.129}
\expandafter\def\csname rev@rcc@che@dollars@lift@cost\endcsname{0.185}
\expandafter\def\csname rev@rcc@che@dollars@lift@hi\endcsname{0.125}
\expandafter\def\csname rev@rcc@che@dollars@lift@lo\endcsname{0.016}
\expandafter\def\csname rev@rcc@che@dollars@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@che@dollars@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@dollars@lift@worldminus\endcsname{0.064}
\expandafter\def\csname rev@rcc@che@dollars@naive@cost\endcsname{0.267}
\expandafter\def\csname rev@rcc@che@dollars@naive@hi\endcsname{0.068}
\expandafter\def\csname rev@rcc@che@dollars@naive@lo\endcsname{\textminus 0.101}
\expandafter\def\csname rev@rcc@che@dollars@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@che@dollars@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@dollars@naive@worldminus\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rcc@che@dollars@tfmplan@cost\endcsname{0.132}
\expandafter\def\csname rev@rcc@che@dollars@tfmplan@hi\endcsname{0.200}
\expandafter\def\csname rev@rcc@che@dollars@tfmplan@lo\endcsname{0.035}
\expandafter\def\csname rev@rcc@che@dollars@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@che@dollars@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@dollars@tfmplan@worldminus\endcsname{0.117}
\expandafter\def\csname rev@rcc@che@dollars@world@cost\endcsname{0.249}
\expandafter\def\csname rev@rcc@che@firsthalf@ens@cost\endcsname{0.159}
\expandafter\def\csname rev@rcc@che@firsthalf@ens@hi\endcsname{0.230}
\expandafter\def\csname rev@rcc@che@firsthalf@ens@lo\endcsname{0.056}
\expandafter\def\csname rev@rcc@che@firsthalf@ens@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@che@firsthalf@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@firsthalf@ens@worldminus\endcsname{0.140}
\expandafter\def\csname rev@rcc@che@firsthalf@lgb@cost\endcsname{0.116}
\expandafter\def\csname rev@rcc@che@firsthalf@lgb@hi\endcsname{0.311}
\expandafter\def\csname rev@rcc@che@firsthalf@lgb@lo\endcsname{0.062}
\expandafter\def\csname rev@rcc@che@firsthalf@lgb@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@che@firsthalf@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@firsthalf@lgb@worldminus\endcsname{0.183}
\expandafter\def\csname rev@rcc@che@firsthalf@lift@cost\endcsname{0.174}
\expandafter\def\csname rev@rcc@che@firsthalf@lift@hi\endcsname{0.221}
\expandafter\def\csname rev@rcc@che@firsthalf@lift@lo\endcsname{0.042}
\expandafter\def\csname rev@rcc@che@firsthalf@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@che@firsthalf@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@firsthalf@lift@worldminus\endcsname{0.125}
\expandafter\def\csname rev@rcc@che@firsthalf@naive@cost\endcsname{0.287}
\expandafter\def\csname rev@rcc@che@firsthalf@naive@hi\endcsname{0.140}
\expandafter\def\csname rev@rcc@che@firsthalf@naive@lo\endcsname{\textminus 0.111}
\expandafter\def\csname rev@rcc@che@firsthalf@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@che@firsthalf@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@firsthalf@naive@worldminus\endcsname{0.011}
\expandafter\def\csname rev@rcc@che@firsthalf@tfmplan@cost\endcsname{0.113}
\expandafter\def\csname rev@rcc@che@firsthalf@tfmplan@hi\endcsname{0.315}
\expandafter\def\csname rev@rcc@che@firsthalf@tfmplan@lo\endcsname{0.066}
\expandafter\def\csname rev@rcc@che@firsthalf@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@che@firsthalf@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@firsthalf@tfmplan@worldminus\endcsname{0.186}
\expandafter\def\csname rev@rcc@che@firsthalf@world@cost\endcsname{0.299}
\expandafter\def\csname rev@rcc@che@nodemean@ens@cost\endcsname{0.158}
\expandafter\def\csname rev@rcc@che@nodemean@ens@hi\endcsname{0.086}
\expandafter\def\csname rev@rcc@che@nodemean@ens@lo\endcsname{0.037}
\expandafter\def\csname rev@rcc@che@nodemean@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@che@nodemean@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@nodemean@ens@worldminus\endcsname{0.059}
\expandafter\def\csname rev@rcc@che@nodemean@lgb@cost\endcsname{0.158}
\expandafter\def\csname rev@rcc@che@nodemean@lgb@hi\endcsname{0.098}
\expandafter\def\csname rev@rcc@che@nodemean@lgb@lo\endcsname{0.027}
\expandafter\def\csname rev@rcc@che@nodemean@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@che@nodemean@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@nodemean@lgb@worldminus\endcsname{0.059}
\expandafter\def\csname rev@rcc@che@nodemean@lift@cost\endcsname{0.192}
\expandafter\def\csname rev@rcc@che@nodemean@lift@hi\endcsname{0.048}
\expandafter\def\csname rev@rcc@che@nodemean@lift@lo\endcsname{0.005}
\expandafter\def\csname rev@rcc@che@nodemean@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@che@nodemean@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@nodemean@lift@worldminus\endcsname{0.024}
\expandafter\def\csname rev@rcc@che@nodemean@naive@cost\endcsname{0.302}
\expandafter\def\csname rev@rcc@che@nodemean@naive@hi\endcsname{\textminus 0.043}
\expandafter\def\csname rev@rcc@che@nodemean@naive@lo\endcsname{\textminus 0.123}
\expandafter\def\csname rev@rcc@che@nodemean@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@che@nodemean@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@nodemean@naive@worldminus\endcsname{\textminus 0.086}
\expandafter\def\csname rev@rcc@che@nodemean@tfmplan@cost\endcsname{0.170}
\expandafter\def\csname rev@rcc@che@nodemean@tfmplan@hi\endcsname{0.087}
\expandafter\def\csname rev@rcc@che@nodemean@tfmplan@lo\endcsname{0.015}
\expandafter\def\csname rev@rcc@che@nodemean@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@che@nodemean@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@nodemean@tfmplan@worldminus\endcsname{0.047}
\expandafter\def\csname rev@rcc@che@nodemean@world@cost\endcsname{0.217}
\expandafter\def\csname rev@rcc@che@units@ens@cost\endcsname{0.135}
\expandafter\def\csname rev@rcc@che@units@ens@hi\endcsname{0.097}
\expandafter\def\csname rev@rcc@che@units@ens@lo\endcsname{0.039}
\expandafter\def\csname rev@rcc@che@units@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@che@units@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@units@ens@worldminus\endcsname{0.066}
\expandafter\def\csname rev@rcc@che@units@lgb@cost\endcsname{0.131}
\expandafter\def\csname rev@rcc@che@units@lgb@hi\endcsname{0.115}
\expandafter\def\csname rev@rcc@che@units@lgb@lo\endcsname{0.030}
\expandafter\def\csname rev@rcc@che@units@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@che@units@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@units@lgb@worldminus\endcsname{0.069}
\expandafter\def\csname rev@rcc@che@units@lift@cost\endcsname{0.167}
\expandafter\def\csname rev@rcc@che@units@lift@hi\endcsname{0.065}
\expandafter\def\csname rev@rcc@che@units@lift@lo\endcsname{0.009}
\expandafter\def\csname rev@rcc@che@units@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@che@units@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@units@lift@worldminus\endcsname{0.034}
\expandafter\def\csname rev@rcc@che@units@naive@cost\endcsname{0.286}
\expandafter\def\csname rev@rcc@che@units@naive@hi\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rcc@che@units@naive@lo\endcsname{\textminus 0.129}
\expandafter\def\csname rev@rcc@che@units@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@che@units@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@units@naive@worldminus\endcsname{\textminus 0.085}
\expandafter\def\csname rev@rcc@che@units@tfmplan@cost\endcsname{0.143}
\expandafter\def\csname rev@rcc@che@units@tfmplan@hi\endcsname{0.103}
\expandafter\def\csname rev@rcc@che@units@tfmplan@lo\endcsname{0.018}
\expandafter\def\csname rev@rcc@che@units@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@che@units@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@units@tfmplan@worldminus\endcsname{0.057}
\expandafter\def\csname rev@rcc@che@units@world@cost\endcsname{0.201}
\expandafter\def\csname rev@rcc@che@weekly@ens@cost\endcsname{0.142}
\expandafter\def\csname rev@rcc@che@weekly@ens@hi\endcsname{0.165}
\expandafter\def\csname rev@rcc@che@weekly@ens@lo\endcsname{0.050}
\expandafter\def\csname rev@rcc@che@weekly@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@che@weekly@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@weekly@ens@worldminus\endcsname{0.107}
\expandafter\def\csname rev@rcc@che@weekly@lgb@cost\endcsname{0.121}
\expandafter\def\csname rev@rcc@che@weekly@lgb@hi\endcsname{0.213}
\expandafter\def\csname rev@rcc@che@weekly@lgb@lo\endcsname{0.046}
\expandafter\def\csname rev@rcc@che@weekly@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@che@weekly@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@weekly@lgb@worldminus\endcsname{0.129}
\expandafter\def\csname rev@rcc@che@weekly@lift@cost\endcsname{0.185}
\expandafter\def\csname rev@rcc@che@weekly@lift@hi\endcsname{0.128}
\expandafter\def\csname rev@rcc@che@weekly@lift@lo\endcsname{0.015}
\expandafter\def\csname rev@rcc@che@weekly@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@che@weekly@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@weekly@lift@worldminus\endcsname{0.064}
\expandafter\def\csname rev@rcc@che@weekly@naive@cost\endcsname{0.267}
\expandafter\def\csname rev@rcc@che@weekly@naive@hi\endcsname{0.067}
\expandafter\def\csname rev@rcc@che@weekly@naive@lo\endcsname{\textminus 0.101}
\expandafter\def\csname rev@rcc@che@weekly@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@che@weekly@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@weekly@naive@worldminus\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rcc@che@weekly@tfmplan@cost\endcsname{0.132}
\expandafter\def\csname rev@rcc@che@weekly@tfmplan@hi\endcsname{0.200}
\expandafter\def\csname rev@rcc@che@weekly@tfmplan@lo\endcsname{0.034}
\expandafter\def\csname rev@rcc@che@weekly@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@che@weekly@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@weekly@tfmplan@worldminus\endcsname{0.117}
\expandafter\def\csname rev@rcc@che@weekly@world@cost\endcsname{0.249}
\expandafter\def\csname rev@rcc@che@windowtotal@ens@cost\endcsname{0.114}
\expandafter\def\csname rev@rcc@che@windowtotal@ens@hi\endcsname{0.158}
\expandafter\def\csname rev@rcc@che@windowtotal@ens@lo\endcsname{0.048}
\expandafter\def\csname rev@rcc@che@windowtotal@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@che@windowtotal@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@windowtotal@ens@worldminus\endcsname{0.102}
\expandafter\def\csname rev@rcc@che@windowtotal@lgb@cost\endcsname{0.070}
\expandafter\def\csname rev@rcc@che@windowtotal@lgb@hi\endcsname{0.228}
\expandafter\def\csname rev@rcc@che@windowtotal@lgb@lo\endcsname{0.067}
\expandafter\def\csname rev@rcc@che@windowtotal@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@che@windowtotal@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@windowtotal@lgb@worldminus\endcsname{0.146}
\expandafter\def\csname rev@rcc@che@windowtotal@lift@cost\endcsname{0.152}
\expandafter\def\csname rev@rcc@che@windowtotal@lift@hi\endcsname{0.125}
\expandafter\def\csname rev@rcc@che@windowtotal@lift@lo\endcsname{0.016}
\expandafter\def\csname rev@rcc@che@windowtotal@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@che@windowtotal@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@windowtotal@lift@worldminus\endcsname{0.063}
\expandafter\def\csname rev@rcc@che@windowtotal@naive@cost\endcsname{0.176}
\expandafter\def\csname rev@rcc@che@windowtotal@naive@hi\endcsname{0.119}
\expandafter\def\csname rev@rcc@che@windowtotal@naive@lo\endcsname{\textminus 0.040}
\expandafter\def\csname rev@rcc@che@windowtotal@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@che@windowtotal@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@windowtotal@naive@worldminus\endcsname{0.040}
\expandafter\def\csname rev@rcc@che@windowtotal@tfmplan@cost\endcsname{0.112}
\expandafter\def\csname rev@rcc@che@windowtotal@tfmplan@hi\endcsname{0.185}
\expandafter\def\csname rev@rcc@che@windowtotal@tfmplan@lo\endcsname{0.025}
\expandafter\def\csname rev@rcc@che@windowtotal@tfmplan@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@che@windowtotal@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@che@windowtotal@tfmplan@worldminus\endcsname{0.104}
\expandafter\def\csname rev@rcc@che@windowtotal@world@cost\endcsname{0.216}
\expandafter\def\csname rev@rcc@frat@asfirstrun@ens@cost\endcsname{0.146}
\expandafter\def\csname rev@rcc@frat@asfirstrun@ens@hi\endcsname{0.023}
\expandafter\def\csname rev@rcc@frat@asfirstrun@ens@lo\endcsname{0.019}
\expandafter\def\csname rev@rcc@frat@asfirstrun@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@asfirstrun@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@asfirstrun@ens@worldminus\endcsname{0.021}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lgb@cost\endcsname{0.149}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lgb@hi\endcsname{0.021}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lgb@lo\endcsname{0.015}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lgb@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lgb@worldminus\endcsname{0.018}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lift@cost\endcsname{0.163}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lift@hi\endcsname{0.006}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lift@lo\endcsname{0.002}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lift@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@asfirstrun@lift@worldminus\endcsname{0.004}
\expandafter\def\csname rev@rcc@frat@asfirstrun@naive@cost\endcsname{0.294}
\expandafter\def\csname rev@rcc@frat@asfirstrun@naive@hi\endcsname{\textminus 0.118}
\expandafter\def\csname rev@rcc@frat@asfirstrun@naive@lo\endcsname{\textminus 0.135}
\expandafter\def\csname rev@rcc@frat@asfirstrun@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@frat@asfirstrun@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@asfirstrun@naive@worldminus\endcsname{\textminus 0.126}
\expandafter\def\csname rev@rcc@frat@asfirstrun@tfmplan@cost\endcsname{0.153}
\expandafter\def\csname rev@rcc@frat@asfirstrun@tfmplan@hi\endcsname{0.018}
\expandafter\def\csname rev@rcc@frat@asfirstrun@tfmplan@lo\endcsname{0.012}
\expandafter\def\csname rev@rcc@frat@asfirstrun@tfmplan@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@asfirstrun@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@asfirstrun@tfmplan@worldminus\endcsname{0.015}
\expandafter\def\csname rev@rcc@frat@asfirstrun@world@cost\endcsname{0.167}
\expandafter\def\csname rev@rcc@frat@dollars@ens@cost\endcsname{0.145}
\expandafter\def\csname rev@rcc@frat@dollars@ens@hi\endcsname{0.023}
\expandafter\def\csname rev@rcc@frat@dollars@ens@lo\endcsname{0.019}
\expandafter\def\csname rev@rcc@frat@dollars@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@dollars@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@dollars@ens@worldminus\endcsname{0.021}
\expandafter\def\csname rev@rcc@frat@dollars@lgb@cost\endcsname{0.148}
\expandafter\def\csname rev@rcc@frat@dollars@lgb@hi\endcsname{0.022}
\expandafter\def\csname rev@rcc@frat@dollars@lgb@lo\endcsname{0.015}
\expandafter\def\csname rev@rcc@frat@dollars@lgb@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@dollars@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@dollars@lgb@worldminus\endcsname{0.019}
\expandafter\def\csname rev@rcc@frat@dollars@lift@cost\endcsname{0.162}
\expandafter\def\csname rev@rcc@frat@dollars@lift@hi\endcsname{0.006}
\expandafter\def\csname rev@rcc@frat@dollars@lift@lo\endcsname{0.002}
\expandafter\def\csname rev@rcc@frat@dollars@lift@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@frat@dollars@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@dollars@lift@worldminus\endcsname{0.004}
\expandafter\def\csname rev@rcc@frat@dollars@naive@cost\endcsname{0.291}
\expandafter\def\csname rev@rcc@frat@dollars@naive@hi\endcsname{\textminus 0.117}
\expandafter\def\csname rev@rcc@frat@dollars@naive@lo\endcsname{\textminus 0.133}
\expandafter\def\csname rev@rcc@frat@dollars@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@frat@dollars@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@dollars@naive@worldminus\endcsname{\textminus 0.125}
\expandafter\def\csname rev@rcc@frat@dollars@tfmplan@cost\endcsname{0.151}
\expandafter\def\csname rev@rcc@frat@dollars@tfmplan@hi\endcsname{0.018}
\expandafter\def\csname rev@rcc@frat@dollars@tfmplan@lo\endcsname{0.012}
\expandafter\def\csname rev@rcc@frat@dollars@tfmplan@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@dollars@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@dollars@tfmplan@worldminus\endcsname{0.015}
\expandafter\def\csname rev@rcc@frat@dollars@world@cost\endcsname{0.166}
\expandafter\def\csname rev@rcc@frat@firsthalf@ens@cost\endcsname{0.147}
\expandafter\def\csname rev@rcc@frat@firsthalf@ens@hi\endcsname{0.027}
\expandafter\def\csname rev@rcc@frat@firsthalf@ens@lo\endcsname{0.022}
\expandafter\def\csname rev@rcc@frat@firsthalf@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@firsthalf@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@firsthalf@ens@worldminus\endcsname{0.024}
\expandafter\def\csname rev@rcc@frat@firsthalf@lgb@cost\endcsname{0.149}
\expandafter\def\csname rev@rcc@frat@firsthalf@lgb@hi\endcsname{0.027}
\expandafter\def\csname rev@rcc@frat@firsthalf@lgb@lo\endcsname{0.019}
\expandafter\def\csname rev@rcc@frat@firsthalf@lgb@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@frat@firsthalf@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@firsthalf@lgb@worldminus\endcsname{0.023}
\expandafter\def\csname rev@rcc@frat@firsthalf@lift@cost\endcsname{0.164}
\expandafter\def\csname rev@rcc@frat@firsthalf@lift@hi\endcsname{0.011}
\expandafter\def\csname rev@rcc@frat@firsthalf@lift@lo\endcsname{0.005}
\expandafter\def\csname rev@rcc@frat@firsthalf@lift@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@frat@firsthalf@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@firsthalf@lift@worldminus\endcsname{0.008}
\expandafter\def\csname rev@rcc@frat@firsthalf@naive@cost\endcsname{0.287}
\expandafter\def\csname rev@rcc@frat@firsthalf@naive@hi\endcsname{\textminus 0.106}
\expandafter\def\csname rev@rcc@frat@firsthalf@naive@lo\endcsname{\textminus 0.125}
\expandafter\def\csname rev@rcc@frat@firsthalf@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@frat@firsthalf@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@firsthalf@naive@worldminus\endcsname{\textminus 0.115}
\expandafter\def\csname rev@rcc@frat@firsthalf@tfmplan@cost\endcsname{0.154}
\expandafter\def\csname rev@rcc@frat@firsthalf@tfmplan@hi\endcsname{0.023}
\expandafter\def\csname rev@rcc@frat@firsthalf@tfmplan@lo\endcsname{0.013}
\expandafter\def\csname rev@rcc@frat@firsthalf@tfmplan@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@frat@firsthalf@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@firsthalf@tfmplan@worldminus\endcsname{0.018}
\expandafter\def\csname rev@rcc@frat@firsthalf@world@cost\endcsname{0.172}
\expandafter\def\csname rev@rcc@frat@nodemean@ens@cost\endcsname{0.167}
\expandafter\def\csname rev@rcc@frat@nodemean@ens@hi\endcsname{0.020}
\expandafter\def\csname rev@rcc@frat@nodemean@ens@lo\endcsname{0.016}
\expandafter\def\csname rev@rcc@frat@nodemean@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@nodemean@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@nodemean@ens@worldminus\endcsname{0.018}
\expandafter\def\csname rev@rcc@frat@nodemean@lgb@cost\endcsname{0.171}
\expandafter\def\csname rev@rcc@frat@nodemean@lgb@hi\endcsname{0.016}
\expandafter\def\csname rev@rcc@frat@nodemean@lgb@lo\endcsname{0.010}
\expandafter\def\csname rev@rcc@frat@nodemean@lgb@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@nodemean@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@nodemean@lgb@worldminus\endcsname{0.013}
\expandafter\def\csname rev@rcc@frat@nodemean@lift@cost\endcsname{0.187}
\expandafter\def\csname rev@rcc@frat@nodemean@lift@hi\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rcc@frat@nodemean@lift@lo\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rcc@frat@nodemean@lift@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@frat@nodemean@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@nodemean@lift@worldminus\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@frat@nodemean@naive@cost\endcsname{0.312}
\expandafter\def\csname rev@rcc@frat@nodemean@naive@hi\endcsname{\textminus 0.120}
\expandafter\def\csname rev@rcc@frat@nodemean@naive@lo\endcsname{\textminus 0.136}
\expandafter\def\csname rev@rcc@frat@nodemean@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@frat@nodemean@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@nodemean@naive@worldminus\endcsname{\textminus 0.128}
\expandafter\def\csname rev@rcc@frat@nodemean@tfmplan@cost\endcsname{0.177}
\expandafter\def\csname rev@rcc@frat@nodemean@tfmplan@hi\endcsname{0.011}
\expandafter\def\csname rev@rcc@frat@nodemean@tfmplan@lo\endcsname{0.004}
\expandafter\def\csname rev@rcc@frat@nodemean@tfmplan@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@frat@nodemean@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@nodemean@tfmplan@worldminus\endcsname{0.008}
\expandafter\def\csname rev@rcc@frat@nodemean@world@cost\endcsname{0.184}
\expandafter\def\csname rev@rcc@frat@units@ens@cost\endcsname{0.138}
\expandafter\def\csname rev@rcc@frat@units@ens@hi\endcsname{0.023}
\expandafter\def\csname rev@rcc@frat@units@ens@lo\endcsname{0.019}
\expandafter\def\csname rev@rcc@frat@units@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@units@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@units@ens@worldminus\endcsname{0.021}
\expandafter\def\csname rev@rcc@frat@units@lgb@cost\endcsname{0.140}
\expandafter\def\csname rev@rcc@frat@units@lgb@hi\endcsname{0.023}
\expandafter\def\csname rev@rcc@frat@units@lgb@lo\endcsname{0.016}
\expandafter\def\csname rev@rcc@frat@units@lgb@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@units@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@units@lgb@worldminus\endcsname{0.019}
\expandafter\def\csname rev@rcc@frat@units@lift@cost\endcsname{0.154}
\expandafter\def\csname rev@rcc@frat@units@lift@hi\endcsname{0.007}
\expandafter\def\csname rev@rcc@frat@units@lift@lo\endcsname{0.003}
\expandafter\def\csname rev@rcc@frat@units@lift@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@frat@units@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@units@lift@worldminus\endcsname{0.005}
\expandafter\def\csname rev@rcc@frat@units@naive@cost\endcsname{0.267}
\expandafter\def\csname rev@rcc@frat@units@naive@hi\endcsname{\textminus 0.101}
\expandafter\def\csname rev@rcc@frat@units@naive@lo\endcsname{\textminus 0.115}
\expandafter\def\csname rev@rcc@frat@units@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@frat@units@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@units@naive@worldminus\endcsname{\textminus 0.108}
\expandafter\def\csname rev@rcc@frat@units@tfmplan@cost\endcsname{0.143}
\expandafter\def\csname rev@rcc@frat@units@tfmplan@hi\endcsname{0.019}
\expandafter\def\csname rev@rcc@frat@units@tfmplan@lo\endcsname{0.013}
\expandafter\def\csname rev@rcc@frat@units@tfmplan@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@units@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@units@tfmplan@worldminus\endcsname{0.016}
\expandafter\def\csname rev@rcc@frat@units@world@cost\endcsname{0.159}
\expandafter\def\csname rev@rcc@frat@weekly@ens@cost\endcsname{0.145}
\expandafter\def\csname rev@rcc@frat@weekly@ens@hi\endcsname{0.023}
\expandafter\def\csname rev@rcc@frat@weekly@ens@lo\endcsname{0.019}
\expandafter\def\csname rev@rcc@frat@weekly@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@weekly@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@weekly@ens@worldminus\endcsname{0.021}
\expandafter\def\csname rev@rcc@frat@weekly@lgb@cost\endcsname{0.148}
\expandafter\def\csname rev@rcc@frat@weekly@lgb@hi\endcsname{0.022}
\expandafter\def\csname rev@rcc@frat@weekly@lgb@lo\endcsname{0.015}
\expandafter\def\csname rev@rcc@frat@weekly@lgb@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@weekly@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@weekly@lgb@worldminus\endcsname{0.019}
\expandafter\def\csname rev@rcc@frat@weekly@lift@cost\endcsname{0.162}
\expandafter\def\csname rev@rcc@frat@weekly@lift@hi\endcsname{0.006}
\expandafter\def\csname rev@rcc@frat@weekly@lift@lo\endcsname{0.002}
\expandafter\def\csname rev@rcc@frat@weekly@lift@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@frat@weekly@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@weekly@lift@worldminus\endcsname{0.004}
\expandafter\def\csname rev@rcc@frat@weekly@naive@cost\endcsname{0.291}
\expandafter\def\csname rev@rcc@frat@weekly@naive@hi\endcsname{\textminus 0.118}
\expandafter\def\csname rev@rcc@frat@weekly@naive@lo\endcsname{\textminus 0.133}
\expandafter\def\csname rev@rcc@frat@weekly@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@frat@weekly@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@weekly@naive@worldminus\endcsname{\textminus 0.125}
\expandafter\def\csname rev@rcc@frat@weekly@tfmplan@cost\endcsname{0.151}
\expandafter\def\csname rev@rcc@frat@weekly@tfmplan@hi\endcsname{0.018}
\expandafter\def\csname rev@rcc@frat@weekly@tfmplan@lo\endcsname{0.012}
\expandafter\def\csname rev@rcc@frat@weekly@tfmplan@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@weekly@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@weekly@tfmplan@worldminus\endcsname{0.015}
\expandafter\def\csname rev@rcc@frat@weekly@world@cost\endcsname{0.166}
\expandafter\def\csname rev@rcc@frat@windowtotal@ens@cost\endcsname{0.073}
\expandafter\def\csname rev@rcc@frat@windowtotal@ens@hi\endcsname{0.014}
\expandafter\def\csname rev@rcc@frat@windowtotal@ens@lo\endcsname{0.008}
\expandafter\def\csname rev@rcc@frat@windowtotal@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@windowtotal@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@windowtotal@ens@worldminus\endcsname{0.011}
\expandafter\def\csname rev@rcc@frat@windowtotal@lgb@cost\endcsname{0.081}
\expandafter\def\csname rev@rcc@frat@windowtotal@lgb@hi\endcsname{0.007}
\expandafter\def\csname rev@rcc@frat@windowtotal@lgb@lo\endcsname{\textminus 0.000}
\expandafter\def\csname rev@rcc@frat@windowtotal@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@frat@windowtotal@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@windowtotal@lgb@worldminus\endcsname{0.003}
\expandafter\def\csname rev@rcc@frat@windowtotal@lift@cost\endcsname{0.085}
\expandafter\def\csname rev@rcc@frat@windowtotal@lift@hi\endcsname{0.002}
\expandafter\def\csname rev@rcc@frat@windowtotal@lift@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rcc@frat@windowtotal@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@frat@windowtotal@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@windowtotal@lift@worldminus\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rcc@frat@windowtotal@naive@cost\endcsname{0.160}
\expandafter\def\csname rev@rcc@frat@windowtotal@naive@hi\endcsname{\textminus 0.067}
\expandafter\def\csname rev@rcc@frat@windowtotal@naive@lo\endcsname{\textminus 0.084}
\expandafter\def\csname rev@rcc@frat@windowtotal@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@frat@windowtotal@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@windowtotal@naive@worldminus\endcsname{\textminus 0.075}
\expandafter\def\csname rev@rcc@frat@windowtotal@tfmplan@cost\endcsname{0.077}
\expandafter\def\csname rev@rcc@frat@windowtotal@tfmplan@hi\endcsname{0.012}
\expandafter\def\csname rev@rcc@frat@windowtotal@tfmplan@lo\endcsname{0.003}
\expandafter\def\csname rev@rcc@frat@windowtotal@tfmplan@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@frat@windowtotal@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@frat@windowtotal@tfmplan@worldminus\endcsname{0.007}
\expandafter\def\csname rev@rcc@frat@windowtotal@world@cost\endcsname{0.084}
\expandafter\def\csname rev@rcc@fre@asfirstrun@ens@cost\endcsname{6311900000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@ens@hi\endcsname{\textminus 304500000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@ens@lo\endcsname{\textminus 8855100000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@ens@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@fre@asfirstrun@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@asfirstrun@ens@worldminus\endcsname{\textminus 3658800000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lgb@cost\endcsname{6410800000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lgb@hi\endcsname{\textminus 316440000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lgb@lo\endcsname{\textminus 9218400000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lgb@worldminus\endcsname{\textminus 3757700000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lift@cost\endcsname{6981300000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lift@hi\endcsname{\textminus 346670000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lift@lo\endcsname{\textminus 10449000000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lift@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@asfirstrun@lift@worldminus\endcsname{\textminus 4328200000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@naive@cost\endcsname{36995000000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@naive@hi\endcsname{\textminus 3066400000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@naive@lo\endcsname{\textminus 85404000000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@asfirstrun@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@asfirstrun@naive@worldminus\endcsname{\textminus 34342000000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@tfmplan@cost\endcsname{9871800000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@tfmplan@hi\endcsname{\textminus 597050000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@tfmplan@lo\endcsname{\textminus 17340000000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@tfmplan@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@asfirstrun@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@asfirstrun@tfmplan@worldminus\endcsname{\textminus 7218700000.000}
\expandafter\def\csname rev@rcc@fre@asfirstrun@world@cost\endcsname{2653100000.000}
\expandafter\def\csname rev@rcc@fre@dollars@ens@cost\endcsname{0.231}
\expandafter\def\csname rev@rcc@fre@dollars@ens@hi\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rcc@fre@dollars@ens@lo\endcsname{\textminus 0.012}
\expandafter\def\csname rev@rcc@fre@dollars@ens@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@fre@dollars@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@dollars@ens@worldminus\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rcc@fre@dollars@lgb@cost\endcsname{0.199}
\expandafter\def\csname rev@rcc@fre@dollars@lgb@hi\endcsname{0.028}
\expandafter\def\csname rev@rcc@fre@dollars@lgb@lo\endcsname{0.020}
\expandafter\def\csname rev@rcc@fre@dollars@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@fre@dollars@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@dollars@lgb@worldminus\endcsname{0.024}
\expandafter\def\csname rev@rcc@fre@dollars@lift@cost\endcsname{0.267}
\expandafter\def\csname rev@rcc@fre@dollars@lift@hi\endcsname{\textminus 0.038}
\expandafter\def\csname rev@rcc@fre@dollars@lift@lo\endcsname{\textminus 0.050}
\expandafter\def\csname rev@rcc@fre@dollars@lift@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@fre@dollars@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@dollars@lift@worldminus\endcsname{\textminus 0.044}
\expandafter\def\csname rev@rcc@fre@dollars@naive@cost\endcsname{0.399}
\expandafter\def\csname rev@rcc@fre@dollars@naive@hi\endcsname{\textminus 0.164}
\expandafter\def\csname rev@rcc@fre@dollars@naive@lo\endcsname{\textminus 0.190}
\expandafter\def\csname rev@rcc@fre@dollars@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@dollars@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@dollars@naive@worldminus\endcsname{\textminus 0.176}
\expandafter\def\csname rev@rcc@fre@dollars@tfmplan@cost\endcsname{0.332}
\expandafter\def\csname rev@rcc@fre@dollars@tfmplan@hi\endcsname{\textminus 0.101}
\expandafter\def\csname rev@rcc@fre@dollars@tfmplan@lo\endcsname{\textminus 0.117}
\expandafter\def\csname rev@rcc@fre@dollars@tfmplan@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@dollars@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@dollars@tfmplan@worldminus\endcsname{\textminus 0.109}
\expandafter\def\csname rev@rcc@fre@dollars@world@cost\endcsname{0.223}
\expandafter\def\csname rev@rcc@fre@firsthalf@ens@cost\endcsname{0.230}
\expandafter\def\csname rev@rcc@fre@firsthalf@ens@hi\endcsname{\textminus 0.014}
\expandafter\def\csname rev@rcc@fre@firsthalf@ens@lo\endcsname{\textminus 0.022}
\expandafter\def\csname rev@rcc@fre@firsthalf@ens@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@fre@firsthalf@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@firsthalf@ens@worldminus\endcsname{\textminus 0.018}
\expandafter\def\csname rev@rcc@fre@firsthalf@lgb@cost\endcsname{0.191}
\expandafter\def\csname rev@rcc@fre@firsthalf@lgb@hi\endcsname{0.027}
\expandafter\def\csname rev@rcc@fre@firsthalf@lgb@lo\endcsname{0.015}
\expandafter\def\csname rev@rcc@fre@firsthalf@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@fre@firsthalf@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@firsthalf@lgb@worldminus\endcsname{0.021}
\expandafter\def\csname rev@rcc@fre@firsthalf@lift@cost\endcsname{0.284}
\expandafter\def\csname rev@rcc@fre@firsthalf@lift@hi\endcsname{\textminus 0.065}
\expandafter\def\csname rev@rcc@fre@firsthalf@lift@lo\endcsname{\textminus 0.079}
\expandafter\def\csname rev@rcc@fre@firsthalf@lift@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@fre@firsthalf@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@firsthalf@lift@worldminus\endcsname{\textminus 0.072}
\expandafter\def\csname rev@rcc@fre@firsthalf@naive@cost\endcsname{0.376}
\expandafter\def\csname rev@rcc@fre@firsthalf@naive@hi\endcsname{\textminus 0.151}
\expandafter\def\csname rev@rcc@fre@firsthalf@naive@lo\endcsname{\textminus 0.178}
\expandafter\def\csname rev@rcc@fre@firsthalf@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@fre@firsthalf@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@firsthalf@naive@worldminus\endcsname{\textminus 0.164}
\expandafter\def\csname rev@rcc@fre@firsthalf@tfmplan@cost\endcsname{0.344}
\expandafter\def\csname rev@rcc@fre@firsthalf@tfmplan@hi\endcsname{\textminus 0.123}
\expandafter\def\csname rev@rcc@fre@firsthalf@tfmplan@lo\endcsname{\textminus 0.141}
\expandafter\def\csname rev@rcc@fre@firsthalf@tfmplan@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@firsthalf@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@firsthalf@tfmplan@worldminus\endcsname{\textminus 0.132}
\expandafter\def\csname rev@rcc@fre@firsthalf@world@cost\endcsname{0.212}
\expandafter\def\csname rev@rcc@fre@nodemean@ens@cost\endcsname{0.257}
\expandafter\def\csname rev@rcc@fre@nodemean@ens@hi\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rcc@fre@nodemean@ens@lo\endcsname{\textminus 0.016}
\expandafter\def\csname rev@rcc@fre@nodemean@ens@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@fre@nodemean@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@nodemean@ens@worldminus\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rcc@fre@nodemean@lgb@cost\endcsname{0.224}
\expandafter\def\csname rev@rcc@fre@nodemean@lgb@hi\endcsname{0.028}
\expandafter\def\csname rev@rcc@fre@nodemean@lgb@lo\endcsname{0.016}
\expandafter\def\csname rev@rcc@fre@nodemean@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@fre@nodemean@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@nodemean@lgb@worldminus\endcsname{0.022}
\expandafter\def\csname rev@rcc@fre@nodemean@lift@cost\endcsname{0.294}
\expandafter\def\csname rev@rcc@fre@nodemean@lift@hi\endcsname{\textminus 0.041}
\expandafter\def\csname rev@rcc@fre@nodemean@lift@lo\endcsname{\textminus 0.056}
\expandafter\def\csname rev@rcc@fre@nodemean@lift@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@fre@nodemean@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@nodemean@lift@worldminus\endcsname{\textminus 0.048}
\expandafter\def\csname rev@rcc@fre@nodemean@naive@cost\endcsname{0.424}
\expandafter\def\csname rev@rcc@fre@nodemean@naive@hi\endcsname{\textminus 0.162}
\expandafter\def\csname rev@rcc@fre@nodemean@naive@lo\endcsname{\textminus 0.197}
\expandafter\def\csname rev@rcc@fre@nodemean@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@nodemean@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@nodemean@naive@worldminus\endcsname{\textminus 0.178}
\expandafter\def\csname rev@rcc@fre@nodemean@tfmplan@cost\endcsname{0.361}
\expandafter\def\csname rev@rcc@fre@nodemean@tfmplan@hi\endcsname{\textminus 0.107}
\expandafter\def\csname rev@rcc@fre@nodemean@tfmplan@lo\endcsname{\textminus 0.125}
\expandafter\def\csname rev@rcc@fre@nodemean@tfmplan@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@nodemean@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@nodemean@tfmplan@worldminus\endcsname{\textminus 0.115}
\expandafter\def\csname rev@rcc@fre@nodemean@world@cost\endcsname{0.246}
\expandafter\def\csname rev@rcc@fre@units@ens@cost\endcsname{0.239}
\expandafter\def\csname rev@rcc@fre@units@ens@hi\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rcc@fre@units@ens@lo\endcsname{\textminus 0.012}
\expandafter\def\csname rev@rcc@fre@units@ens@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@fre@units@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@units@ens@worldminus\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rcc@fre@units@lgb@cost\endcsname{0.207}
\expandafter\def\csname rev@rcc@fre@units@lgb@hi\endcsname{0.028}
\expandafter\def\csname rev@rcc@fre@units@lgb@lo\endcsname{0.019}
\expandafter\def\csname rev@rcc@fre@units@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@fre@units@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@units@lgb@worldminus\endcsname{0.024}
\expandafter\def\csname rev@rcc@fre@units@lift@cost\endcsname{0.274}
\expandafter\def\csname rev@rcc@fre@units@lift@hi\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rcc@fre@units@lift@lo\endcsname{\textminus 0.049}
\expandafter\def\csname rev@rcc@fre@units@lift@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@fre@units@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@units@lift@worldminus\endcsname{\textminus 0.043}
\expandafter\def\csname rev@rcc@fre@units@naive@cost\endcsname{0.409}
\expandafter\def\csname rev@rcc@fre@units@naive@hi\endcsname{\textminus 0.165}
\expandafter\def\csname rev@rcc@fre@units@naive@lo\endcsname{\textminus 0.193}
\expandafter\def\csname rev@rcc@fre@units@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@units@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@units@naive@worldminus\endcsname{\textminus 0.178}
\expandafter\def\csname rev@rcc@fre@units@tfmplan@cost\endcsname{0.339}
\expandafter\def\csname rev@rcc@fre@units@tfmplan@hi\endcsname{\textminus 0.101}
\expandafter\def\csname rev@rcc@fre@units@tfmplan@lo\endcsname{\textminus 0.117}
\expandafter\def\csname rev@rcc@fre@units@tfmplan@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@units@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@units@tfmplan@worldminus\endcsname{\textminus 0.109}
\expandafter\def\csname rev@rcc@fre@units@world@cost\endcsname{0.231}
\expandafter\def\csname rev@rcc@fre@weekly@ens@cost\endcsname{0.231}
\expandafter\def\csname rev@rcc@fre@weekly@ens@hi\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rcc@fre@weekly@ens@lo\endcsname{\textminus 0.012}
\expandafter\def\csname rev@rcc@fre@weekly@ens@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@fre@weekly@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@weekly@ens@worldminus\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rcc@fre@weekly@lgb@cost\endcsname{0.199}
\expandafter\def\csname rev@rcc@fre@weekly@lgb@hi\endcsname{0.028}
\expandafter\def\csname rev@rcc@fre@weekly@lgb@lo\endcsname{0.019}
\expandafter\def\csname rev@rcc@fre@weekly@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@fre@weekly@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@weekly@lgb@worldminus\endcsname{0.024}
\expandafter\def\csname rev@rcc@fre@weekly@lift@cost\endcsname{0.267}
\expandafter\def\csname rev@rcc@fre@weekly@lift@hi\endcsname{\textminus 0.038}
\expandafter\def\csname rev@rcc@fre@weekly@lift@lo\endcsname{\textminus 0.049}
\expandafter\def\csname rev@rcc@fre@weekly@lift@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@fre@weekly@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@weekly@lift@worldminus\endcsname{\textminus 0.044}
\expandafter\def\csname rev@rcc@fre@weekly@naive@cost\endcsname{0.399}
\expandafter\def\csname rev@rcc@fre@weekly@naive@hi\endcsname{\textminus 0.163}
\expandafter\def\csname rev@rcc@fre@weekly@naive@lo\endcsname{\textminus 0.190}
\expandafter\def\csname rev@rcc@fre@weekly@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@weekly@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@weekly@naive@worldminus\endcsname{\textminus 0.176}
\expandafter\def\csname rev@rcc@fre@weekly@tfmplan@cost\endcsname{0.332}
\expandafter\def\csname rev@rcc@fre@weekly@tfmplan@hi\endcsname{\textminus 0.101}
\expandafter\def\csname rev@rcc@fre@weekly@tfmplan@lo\endcsname{\textminus 0.117}
\expandafter\def\csname rev@rcc@fre@weekly@tfmplan@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@fre@weekly@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@weekly@tfmplan@worldminus\endcsname{\textminus 0.109}
\expandafter\def\csname rev@rcc@fre@weekly@world@cost\endcsname{0.223}
\expandafter\def\csname rev@rcc@fre@windowtotal@ens@cost\endcsname{0.138}
\expandafter\def\csname rev@rcc@fre@windowtotal@ens@hi\endcsname{0.006}
\expandafter\def\csname rev@rcc@fre@windowtotal@ens@lo\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rcc@fre@windowtotal@ens@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@fre@windowtotal@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@windowtotal@ens@worldminus\endcsname{0.000}
\expandafter\def\csname rev@rcc@fre@windowtotal@lgb@cost\endcsname{0.112}
\expandafter\def\csname rev@rcc@fre@windowtotal@lgb@hi\endcsname{0.033}
\expandafter\def\csname rev@rcc@fre@windowtotal@lgb@lo\endcsname{0.021}
\expandafter\def\csname rev@rcc@fre@windowtotal@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@fre@windowtotal@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@windowtotal@lgb@worldminus\endcsname{0.027}
\expandafter\def\csname rev@rcc@fre@windowtotal@lift@cost\endcsname{0.185}
\expandafter\def\csname rev@rcc@fre@windowtotal@lift@hi\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rcc@fre@windowtotal@lift@lo\endcsname{\textminus 0.056}
\expandafter\def\csname rev@rcc@fre@windowtotal@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@fre@windowtotal@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@windowtotal@lift@worldminus\endcsname{\textminus 0.047}
\expandafter\def\csname rev@rcc@fre@windowtotal@naive@cost\endcsname{0.142}
\expandafter\def\csname rev@rcc@fre@windowtotal@naive@hi\endcsname{0.012}
\expandafter\def\csname rev@rcc@fre@windowtotal@naive@lo\endcsname{\textminus 0.020}
\expandafter\def\csname rev@rcc@fre@windowtotal@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@fre@windowtotal@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@windowtotal@naive@worldminus\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rcc@fre@windowtotal@tfmplan@cost\endcsname{0.228}
\expandafter\def\csname rev@rcc@fre@windowtotal@tfmplan@hi\endcsname{\textminus 0.079}
\expandafter\def\csname rev@rcc@fre@windowtotal@tfmplan@lo\endcsname{\textminus 0.100}
\expandafter\def\csname rev@rcc@fre@windowtotal@tfmplan@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@fre@windowtotal@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@fre@windowtotal@tfmplan@worldminus\endcsname{\textminus 0.090}
\expandafter\def\csname rev@rcc@fre@windowtotal@world@cost\endcsname{0.138}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@ens@cost\endcsname{0.109}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@ens@hi\endcsname{0.003}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@ens@lo\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@ens@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@ens@worldminus\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lgb@cost\endcsname{0.110}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lgb@hi\endcsname{0.004}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lgb@lo\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lgb@worldminus\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lift@cost\endcsname{0.224}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lift@hi\endcsname{0.005}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lift@lo\endcsname{\textminus 0.385}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@lift@worldminus\endcsname{\textminus 0.117}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@naive@cost\endcsname{0.169}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@naive@hi\endcsname{\textminus 0.051}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@naive@lo\endcsname{\textminus 0.073}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@naive@worldminus\endcsname{\textminus 0.062}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@tfmplan@cost\endcsname{0.142}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@tfmplan@hi\endcsname{\textminus 0.030}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@tfmplan@lo\endcsname{\textminus 0.040}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@tfmplan@worldminus\endcsname{\textminus 0.035}
\expandafter\def\csname rev@rcc@mfive@asfirstrun@world@cost\endcsname{0.107}
\expandafter\def\csname rev@rcc@mfive@dollars@ens@cost\endcsname{0.109}
\expandafter\def\csname rev@rcc@mfive@dollars@ens@hi\endcsname{0.003}
\expandafter\def\csname rev@rcc@mfive@dollars@ens@lo\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rcc@mfive@dollars@ens@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@dollars@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@dollars@ens@worldminus\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@mfive@dollars@lgb@cost\endcsname{0.111}
\expandafter\def\csname rev@rcc@mfive@dollars@lgb@hi\endcsname{0.004}
\expandafter\def\csname rev@rcc@mfive@dollars@lgb@lo\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rcc@mfive@dollars@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@dollars@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@dollars@lgb@worldminus\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rcc@mfive@dollars@lift@cost\endcsname{0.220}
\expandafter\def\csname rev@rcc@mfive@dollars@lift@hi\endcsname{0.005}
\expandafter\def\csname rev@rcc@mfive@dollars@lift@lo\endcsname{\textminus 0.373}
\expandafter\def\csname rev@rcc@mfive@dollars@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@dollars@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@dollars@lift@worldminus\endcsname{\textminus 0.112}
\expandafter\def\csname rev@rcc@mfive@dollars@naive@cost\endcsname{0.170}
\expandafter\def\csname rev@rcc@mfive@dollars@naive@hi\endcsname{\textminus 0.051}
\expandafter\def\csname rev@rcc@mfive@dollars@naive@lo\endcsname{\textminus 0.074}
\expandafter\def\csname rev@rcc@mfive@dollars@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@dollars@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@dollars@naive@worldminus\endcsname{\textminus 0.062}
\expandafter\def\csname rev@rcc@mfive@dollars@tfmplan@cost\endcsname{0.143}
\expandafter\def\csname rev@rcc@mfive@dollars@tfmplan@hi\endcsname{\textminus 0.030}
\expandafter\def\csname rev@rcc@mfive@dollars@tfmplan@lo\endcsname{\textminus 0.041}
\expandafter\def\csname rev@rcc@mfive@dollars@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@dollars@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@dollars@tfmplan@worldminus\endcsname{\textminus 0.036}
\expandafter\def\csname rev@rcc@mfive@dollars@world@cost\endcsname{0.107}
\expandafter\def\csname rev@rcc@mfive@firsthalf@ens@cost\endcsname{0.094}
\expandafter\def\csname rev@rcc@mfive@firsthalf@ens@hi\endcsname{0.003}
\expandafter\def\csname rev@rcc@mfive@firsthalf@ens@lo\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rcc@mfive@firsthalf@ens@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@mfive@firsthalf@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@firsthalf@ens@worldminus\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lgb@cost\endcsname{0.098}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lgb@hi\endcsname{0.001}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lgb@lo\endcsname{\textminus 0.014}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lgb@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lgb@worldminus\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lift@cost\endcsname{0.122}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lift@hi\endcsname{0.001}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lift@lo\endcsname{\textminus 0.095}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@firsthalf@lift@worldminus\endcsname{\textminus 0.030}
\expandafter\def\csname rev@rcc@mfive@firsthalf@naive@cost\endcsname{0.156}
\expandafter\def\csname rev@rcc@mfive@firsthalf@naive@hi\endcsname{\textminus 0.049}
\expandafter\def\csname rev@rcc@mfive@firsthalf@naive@lo\endcsname{\textminus 0.077}
\expandafter\def\csname rev@rcc@mfive@firsthalf@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@firsthalf@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@firsthalf@naive@worldminus\endcsname{\textminus 0.063}
\expandafter\def\csname rev@rcc@mfive@firsthalf@tfmplan@cost\endcsname{0.126}
\expandafter\def\csname rev@rcc@mfive@firsthalf@tfmplan@hi\endcsname{\textminus 0.026}
\expandafter\def\csname rev@rcc@mfive@firsthalf@tfmplan@lo\endcsname{\textminus 0.040}
\expandafter\def\csname rev@rcc@mfive@firsthalf@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@firsthalf@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@firsthalf@tfmplan@worldminus\endcsname{\textminus 0.033}
\expandafter\def\csname rev@rcc@mfive@firsthalf@world@cost\endcsname{0.092}
\expandafter\def\csname rev@rcc@mfive@nodemean@ens@cost\endcsname{0.115}
\expandafter\def\csname rev@rcc@mfive@nodemean@ens@hi\endcsname{0.005}
\expandafter\def\csname rev@rcc@mfive@nodemean@ens@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rcc@mfive@nodemean@ens@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@nodemean@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@nodemean@ens@worldminus\endcsname{0.001}
\expandafter\def\csname rev@rcc@mfive@nodemean@lgb@cost\endcsname{0.113}
\expandafter\def\csname rev@rcc@mfive@nodemean@lgb@hi\endcsname{0.008}
\expandafter\def\csname rev@rcc@mfive@nodemean@lgb@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rcc@mfive@nodemean@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@nodemean@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@nodemean@lgb@worldminus\endcsname{0.002}
\expandafter\def\csname rev@rcc@mfive@nodemean@lift@cost\endcsname{0.215}
\expandafter\def\csname rev@rcc@mfive@nodemean@lift@hi\endcsname{0.005}
\expandafter\def\csname rev@rcc@mfive@nodemean@lift@lo\endcsname{\textminus 0.303}
\expandafter\def\csname rev@rcc@mfive@nodemean@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@nodemean@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@nodemean@lift@worldminus\endcsname{\textminus 0.100}
\expandafter\def\csname rev@rcc@mfive@nodemean@naive@cost\endcsname{0.175}
\expandafter\def\csname rev@rcc@mfive@nodemean@naive@hi\endcsname{\textminus 0.051}
\expandafter\def\csname rev@rcc@mfive@nodemean@naive@lo\endcsname{\textminus 0.067}
\expandafter\def\csname rev@rcc@mfive@nodemean@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@nodemean@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@nodemean@naive@worldminus\endcsname{\textminus 0.059}
\expandafter\def\csname rev@rcc@mfive@nodemean@tfmplan@cost\endcsname{0.150}
\expandafter\def\csname rev@rcc@mfive@nodemean@tfmplan@hi\endcsname{\textminus 0.029}
\expandafter\def\csname rev@rcc@mfive@nodemean@tfmplan@lo\endcsname{\textminus 0.039}
\expandafter\def\csname rev@rcc@mfive@nodemean@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@nodemean@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@nodemean@tfmplan@worldminus\endcsname{\textminus 0.034}
\expandafter\def\csname rev@rcc@mfive@nodemean@world@cost\endcsname{0.116}
\expandafter\def\csname rev@rcc@mfive@units@ens@cost\endcsname{0.110}
\expandafter\def\csname rev@rcc@mfive@units@ens@hi\endcsname{0.002}
\expandafter\def\csname rev@rcc@mfive@units@ens@lo\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rcc@mfive@units@ens@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@units@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@units@ens@worldminus\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rcc@mfive@units@lgb@cost\endcsname{0.112}
\expandafter\def\csname rev@rcc@mfive@units@lgb@hi\endcsname{0.003}
\expandafter\def\csname rev@rcc@mfive@units@lgb@lo\endcsname{\textminus 0.014}
\expandafter\def\csname rev@rcc@mfive@units@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@units@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@units@lgb@worldminus\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rcc@mfive@units@lift@cost\endcsname{0.188}
\expandafter\def\csname rev@rcc@mfive@units@lift@hi\endcsname{0.004}
\expandafter\def\csname rev@rcc@mfive@units@lift@lo\endcsname{\textminus 0.283}
\expandafter\def\csname rev@rcc@mfive@units@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@mfive@units@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@units@lift@worldminus\endcsname{\textminus 0.081}
\expandafter\def\csname rev@rcc@mfive@units@naive@cost\endcsname{0.171}
\expandafter\def\csname rev@rcc@mfive@units@naive@hi\endcsname{\textminus 0.052}
\expandafter\def\csname rev@rcc@mfive@units@naive@lo\endcsname{\textminus 0.077}
\expandafter\def\csname rev@rcc@mfive@units@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@units@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@units@naive@worldminus\endcsname{\textminus 0.064}
\expandafter\def\csname rev@rcc@mfive@units@tfmplan@cost\endcsname{0.143}
\expandafter\def\csname rev@rcc@mfive@units@tfmplan@hi\endcsname{\textminus 0.031}
\expandafter\def\csname rev@rcc@mfive@units@tfmplan@lo\endcsname{\textminus 0.043}
\expandafter\def\csname rev@rcc@mfive@units@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@units@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@units@tfmplan@worldminus\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rcc@mfive@units@world@cost\endcsname{0.106}
\expandafter\def\csname rev@rcc@mfive@weekly@ens@cost\endcsname{0.068}
\expandafter\def\csname rev@rcc@mfive@weekly@ens@hi\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rcc@mfive@weekly@ens@lo\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rcc@mfive@weekly@ens@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@weekly@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@weekly@ens@worldminus\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rcc@mfive@weekly@lgb@cost\endcsname{0.078}
\expandafter\def\csname rev@rcc@mfive@weekly@lgb@hi\endcsname{\textminus 0.013}
\expandafter\def\csname rev@rcc@mfive@weekly@lgb@lo\endcsname{\textminus 0.031}
\expandafter\def\csname rev@rcc@mfive@weekly@lgb@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@weekly@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@weekly@lgb@worldminus\endcsname{\textminus 0.022}
\expandafter\def\csname rev@rcc@mfive@weekly@lift@cost\endcsname{0.172}
\expandafter\def\csname rev@rcc@mfive@weekly@lift@hi\endcsname{0.003}
\expandafter\def\csname rev@rcc@mfive@weekly@lift@lo\endcsname{\textminus 0.372}
\expandafter\def\csname rev@rcc@mfive@weekly@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@mfive@weekly@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@weekly@lift@worldminus\endcsname{\textminus 0.115}
\expandafter\def\csname rev@rcc@mfive@weekly@naive@cost\endcsname{0.097}
\expandafter\def\csname rev@rcc@mfive@weekly@naive@hi\endcsname{\textminus 0.029}
\expandafter\def\csname rev@rcc@mfive@weekly@naive@lo\endcsname{\textminus 0.051}
\expandafter\def\csname rev@rcc@mfive@weekly@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@weekly@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@weekly@naive@worldminus\endcsname{\textminus 0.040}
\expandafter\def\csname rev@rcc@mfive@weekly@tfmplan@cost\endcsname{0.096}
\expandafter\def\csname rev@rcc@mfive@weekly@tfmplan@hi\endcsname{\textminus 0.031}
\expandafter\def\csname rev@rcc@mfive@weekly@tfmplan@lo\endcsname{\textminus 0.047}
\expandafter\def\csname rev@rcc@mfive@weekly@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@weekly@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@weekly@tfmplan@worldminus\endcsname{\textminus 0.039}
\expandafter\def\csname rev@rcc@mfive@weekly@world@cost\endcsname{0.057}
\expandafter\def\csname rev@rcc@mfive@windowtotal@ens@cost\endcsname{0.058}
\expandafter\def\csname rev@rcc@mfive@windowtotal@ens@hi\endcsname{\textminus 0.014}
\expandafter\def\csname rev@rcc@mfive@windowtotal@ens@lo\endcsname{\textminus 0.027}
\expandafter\def\csname rev@rcc@mfive@windowtotal@ens@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@windowtotal@ens@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@windowtotal@ens@worldminus\endcsname{\textminus 0.021}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lgb@cost\endcsname{0.074}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lgb@hi\endcsname{\textminus 0.026}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lgb@lo\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lgb@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lgb@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lgb@worldminus\endcsname{\textminus 0.036}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lift@cost\endcsname{0.156}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lift@hi\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lift@lo\endcsname{\textminus 0.376}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lift@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@windowtotal@lift@worldminus\endcsname{\textminus 0.118}
\expandafter\def\csname rev@rcc@mfive@windowtotal@naive@cost\endcsname{0.086}
\expandafter\def\csname rev@rcc@mfive@windowtotal@naive@hi\endcsname{\textminus 0.036}
\expandafter\def\csname rev@rcc@mfive@windowtotal@naive@lo\endcsname{\textminus 0.061}
\expandafter\def\csname rev@rcc@mfive@windowtotal@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@windowtotal@naive@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@windowtotal@naive@worldminus\endcsname{\textminus 0.049}
\expandafter\def\csname rev@rcc@mfive@windowtotal@tfmplan@cost\endcsname{0.085}
\expandafter\def\csname rev@rcc@mfive@windowtotal@tfmplan@hi\endcsname{\textminus 0.040}
\expandafter\def\csname rev@rcc@mfive@windowtotal@tfmplan@lo\endcsname{\textminus 0.055}
\expandafter\def\csname rev@rcc@mfive@windowtotal@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@windowtotal@tfmplan@windows\endcsname{4}
\expandafter\def\csname rev@rcc@mfive@windowtotal@tfmplan@worldminus\endcsname{\textminus 0.048}
\expandafter\def\csname rev@rcc@mfive@windowtotal@world@cost\endcsname{0.038}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@ens@cost\endcsname{26277000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@ens@hi\endcsname{\textminus 661890000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@ens@lo\endcsname{\textminus 38911000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@ens@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@ens@worldminus\endcsname{\textminus 15419000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lgb@cost\endcsname{23015000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lgb@hi\endcsname{\textminus 504850000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lgb@lo\endcsname{\textminus 33636000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lgb@worldminus\endcsname{\textminus 12157000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lift@cost\endcsname{19453000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lift@hi\endcsname{\textminus 145030000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lift@lo\endcsname{\textminus 26953000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lift@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@lift@worldminus\endcsname{\textminus 8594800000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@naive@cost\endcsname{136310000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@naive@hi\endcsname{\textminus 8365000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@naive@lo\endcsname{\textminus 297700000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@naive@worldminus\endcsname{\textminus 125450000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@tfmplan@cost\endcsname{44958000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@tfmplan@hi\endcsname{\textminus 1480800000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@tfmplan@lo\endcsname{\textminus 83188000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@tfmplan@worldminus\endcsname{\textminus 34100000000.000}
\expandafter\def\csname rev@rcc@sdr@asfirstrun@world@cost\endcsname{10858000000.000}
\expandafter\def\csname rev@rcc@sdr@dollars@ens@cost\endcsname{0.196}
\expandafter\def\csname rev@rcc@sdr@dollars@ens@hi\endcsname{0.019}
\expandafter\def\csname rev@rcc@sdr@dollars@ens@lo\endcsname{0.014}
\expandafter\def\csname rev@rcc@sdr@dollars@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sdr@dollars@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@dollars@ens@worldminus\endcsname{0.017}
\expandafter\def\csname rev@rcc@sdr@dollars@lgb@cost\endcsname{0.201}
\expandafter\def\csname rev@rcc@sdr@dollars@lgb@hi\endcsname{0.015}
\expandafter\def\csname rev@rcc@sdr@dollars@lgb@lo\endcsname{0.007}
\expandafter\def\csname rev@rcc@sdr@dollars@lgb@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sdr@dollars@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@dollars@lgb@worldminus\endcsname{0.012}
\expandafter\def\csname rev@rcc@sdr@dollars@lift@cost\endcsname{0.253}
\expandafter\def\csname rev@rcc@sdr@dollars@lift@hi\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rcc@sdr@dollars@lift@lo\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rcc@sdr@dollars@lift@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@dollars@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@dollars@lift@worldminus\endcsname{\textminus 0.041}
\expandafter\def\csname rev@rcc@sdr@dollars@naive@cost\endcsname{0.271}
\expandafter\def\csname rev@rcc@sdr@dollars@naive@hi\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rcc@sdr@dollars@naive@lo\endcsname{\textminus 0.074}
\expandafter\def\csname rev@rcc@sdr@dollars@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@sdr@dollars@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@dollars@naive@worldminus\endcsname{\textminus 0.059}
\expandafter\def\csname rev@rcc@sdr@dollars@tfmplan@cost\endcsname{0.236}
\expandafter\def\csname rev@rcc@sdr@dollars@tfmplan@hi\endcsname{\textminus 0.019}
\expandafter\def\csname rev@rcc@sdr@dollars@tfmplan@lo\endcsname{\textminus 0.029}
\expandafter\def\csname rev@rcc@sdr@dollars@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sdr@dollars@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@dollars@tfmplan@worldminus\endcsname{\textminus 0.024}
\expandafter\def\csname rev@rcc@sdr@dollars@world@cost\endcsname{0.212}
\expandafter\def\csname rev@rcc@sdr@firsthalf@ens@cost\endcsname{0.216}
\expandafter\def\csname rev@rcc@sdr@firsthalf@ens@hi\endcsname{0.007}
\expandafter\def\csname rev@rcc@sdr@firsthalf@ens@lo\endcsname{0.001}
\expandafter\def\csname rev@rcc@sdr@firsthalf@ens@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@sdr@firsthalf@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@firsthalf@ens@worldminus\endcsname{0.004}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lgb@cost\endcsname{0.222}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lgb@hi\endcsname{0.003}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lgb@lo\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lgb@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lgb@worldminus\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lift@cost\endcsname{0.234}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lift@hi\endcsname{\textminus 0.010}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lift@lo\endcsname{\textminus 0.019}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lift@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@firsthalf@lift@worldminus\endcsname{\textminus 0.015}
\expandafter\def\csname rev@rcc@sdr@firsthalf@naive@cost\endcsname{0.289}
\expandafter\def\csname rev@rcc@sdr@firsthalf@naive@hi\endcsname{\textminus 0.055}
\expandafter\def\csname rev@rcc@sdr@firsthalf@naive@lo\endcsname{\textminus 0.084}
\expandafter\def\csname rev@rcc@sdr@firsthalf@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@sdr@firsthalf@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@firsthalf@naive@worldminus\endcsname{\textminus 0.069}
\expandafter\def\csname rev@rcc@sdr@firsthalf@tfmplan@cost\endcsname{0.265}
\expandafter\def\csname rev@rcc@sdr@firsthalf@tfmplan@hi\endcsname{\textminus 0.040}
\expandafter\def\csname rev@rcc@sdr@firsthalf@tfmplan@lo\endcsname{\textminus 0.052}
\expandafter\def\csname rev@rcc@sdr@firsthalf@tfmplan@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@sdr@firsthalf@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@firsthalf@tfmplan@worldminus\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rcc@sdr@firsthalf@world@cost\endcsname{0.220}
\expandafter\def\csname rev@rcc@sdr@nodemean@ens@cost\endcsname{0.216}
\expandafter\def\csname rev@rcc@sdr@nodemean@ens@hi\endcsname{0.019}
\expandafter\def\csname rev@rcc@sdr@nodemean@ens@lo\endcsname{0.013}
\expandafter\def\csname rev@rcc@sdr@nodemean@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sdr@nodemean@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@nodemean@ens@worldminus\endcsname{0.016}
\expandafter\def\csname rev@rcc@sdr@nodemean@lgb@cost\endcsname{0.221}
\expandafter\def\csname rev@rcc@sdr@nodemean@lgb@hi\endcsname{0.016}
\expandafter\def\csname rev@rcc@sdr@nodemean@lgb@lo\endcsname{0.007}
\expandafter\def\csname rev@rcc@sdr@nodemean@lgb@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sdr@nodemean@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@nodemean@lgb@worldminus\endcsname{0.011}
\expandafter\def\csname rev@rcc@sdr@nodemean@lift@cost\endcsname{0.276}
\expandafter\def\csname rev@rcc@sdr@nodemean@lift@hi\endcsname{\textminus 0.039}
\expandafter\def\csname rev@rcc@sdr@nodemean@lift@lo\endcsname{\textminus 0.050}
\expandafter\def\csname rev@rcc@sdr@nodemean@lift@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@nodemean@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@nodemean@lift@worldminus\endcsname{\textminus 0.044}
\expandafter\def\csname rev@rcc@sdr@nodemean@naive@cost\endcsname{0.294}
\expandafter\def\csname rev@rcc@sdr@nodemean@naive@hi\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rcc@sdr@nodemean@naive@lo\endcsname{\textminus 0.081}
\expandafter\def\csname rev@rcc@sdr@nodemean@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@sdr@nodemean@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@nodemean@naive@worldminus\endcsname{\textminus 0.062}
\expandafter\def\csname rev@rcc@sdr@nodemean@tfmplan@cost\endcsname{0.256}
\expandafter\def\csname rev@rcc@sdr@nodemean@tfmplan@hi\endcsname{\textminus 0.019}
\expandafter\def\csname rev@rcc@sdr@nodemean@tfmplan@lo\endcsname{\textminus 0.029}
\expandafter\def\csname rev@rcc@sdr@nodemean@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sdr@nodemean@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@nodemean@tfmplan@worldminus\endcsname{\textminus 0.024}
\expandafter\def\csname rev@rcc@sdr@nodemean@world@cost\endcsname{0.232}
\expandafter\def\csname rev@rcc@sdr@units@ens@cost\endcsname{0.202}
\expandafter\def\csname rev@rcc@sdr@units@ens@hi\endcsname{0.019}
\expandafter\def\csname rev@rcc@sdr@units@ens@lo\endcsname{0.014}
\expandafter\def\csname rev@rcc@sdr@units@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sdr@units@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@units@ens@worldminus\endcsname{0.016}
\expandafter\def\csname rev@rcc@sdr@units@lgb@cost\endcsname{0.207}
\expandafter\def\csname rev@rcc@sdr@units@lgb@hi\endcsname{0.015}
\expandafter\def\csname rev@rcc@sdr@units@lgb@lo\endcsname{0.008}
\expandafter\def\csname rev@rcc@sdr@units@lgb@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sdr@units@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@units@lgb@worldminus\endcsname{0.012}
\expandafter\def\csname rev@rcc@sdr@units@lift@cost\endcsname{0.259}
\expandafter\def\csname rev@rcc@sdr@units@lift@hi\endcsname{\textminus 0.036}
\expandafter\def\csname rev@rcc@sdr@units@lift@lo\endcsname{\textminus 0.045}
\expandafter\def\csname rev@rcc@sdr@units@lift@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@units@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@units@lift@worldminus\endcsname{\textminus 0.041}
\expandafter\def\csname rev@rcc@sdr@units@naive@cost\endcsname{0.275}
\expandafter\def\csname rev@rcc@sdr@units@naive@hi\endcsname{\textminus 0.045}
\expandafter\def\csname rev@rcc@sdr@units@naive@lo\endcsname{\textminus 0.070}
\expandafter\def\csname rev@rcc@sdr@units@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@sdr@units@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@units@naive@worldminus\endcsname{\textminus 0.057}
\expandafter\def\csname rev@rcc@sdr@units@tfmplan@cost\endcsname{0.242}
\expandafter\def\csname rev@rcc@sdr@units@tfmplan@hi\endcsname{\textminus 0.019}
\expandafter\def\csname rev@rcc@sdr@units@tfmplan@lo\endcsname{\textminus 0.029}
\expandafter\def\csname rev@rcc@sdr@units@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sdr@units@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@units@tfmplan@worldminus\endcsname{\textminus 0.024}
\expandafter\def\csname rev@rcc@sdr@units@world@cost\endcsname{0.218}
\expandafter\def\csname rev@rcc@sdr@weekly@ens@cost\endcsname{0.196}
\expandafter\def\csname rev@rcc@sdr@weekly@ens@hi\endcsname{0.019}
\expandafter\def\csname rev@rcc@sdr@weekly@ens@lo\endcsname{0.014}
\expandafter\def\csname rev@rcc@sdr@weekly@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sdr@weekly@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@weekly@ens@worldminus\endcsname{0.017}
\expandafter\def\csname rev@rcc@sdr@weekly@lgb@cost\endcsname{0.201}
\expandafter\def\csname rev@rcc@sdr@weekly@lgb@hi\endcsname{0.015}
\expandafter\def\csname rev@rcc@sdr@weekly@lgb@lo\endcsname{0.008}
\expandafter\def\csname rev@rcc@sdr@weekly@lgb@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sdr@weekly@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@weekly@lgb@worldminus\endcsname{0.012}
\expandafter\def\csname rev@rcc@sdr@weekly@lift@cost\endcsname{0.253}
\expandafter\def\csname rev@rcc@sdr@weekly@lift@hi\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rcc@sdr@weekly@lift@lo\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rcc@sdr@weekly@lift@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@weekly@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@weekly@lift@worldminus\endcsname{\textminus 0.041}
\expandafter\def\csname rev@rcc@sdr@weekly@naive@cost\endcsname{0.271}
\expandafter\def\csname rev@rcc@sdr@weekly@naive@hi\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rcc@sdr@weekly@naive@lo\endcsname{\textminus 0.074}
\expandafter\def\csname rev@rcc@sdr@weekly@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@sdr@weekly@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@weekly@naive@worldminus\endcsname{\textminus 0.059}
\expandafter\def\csname rev@rcc@sdr@weekly@tfmplan@cost\endcsname{0.236}
\expandafter\def\csname rev@rcc@sdr@weekly@tfmplan@hi\endcsname{\textminus 0.019}
\expandafter\def\csname rev@rcc@sdr@weekly@tfmplan@lo\endcsname{\textminus 0.029}
\expandafter\def\csname rev@rcc@sdr@weekly@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sdr@weekly@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@weekly@tfmplan@worldminus\endcsname{\textminus 0.024}
\expandafter\def\csname rev@rcc@sdr@weekly@world@cost\endcsname{0.212}
\expandafter\def\csname rev@rcc@sdr@windowtotal@ens@cost\endcsname{0.077}
\expandafter\def\csname rev@rcc@sdr@windowtotal@ens@hi\endcsname{0.016}
\expandafter\def\csname rev@rcc@sdr@windowtotal@ens@lo\endcsname{0.006}
\expandafter\def\csname rev@rcc@sdr@windowtotal@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sdr@windowtotal@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@windowtotal@ens@worldminus\endcsname{0.011}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lgb@cost\endcsname{0.091}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lgb@hi\endcsname{0.005}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lgb@lo\endcsname{\textminus 0.009}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lgb@worldminus\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lift@cost\endcsname{0.107}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lift@hi\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lift@lo\endcsname{\textminus 0.027}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lift@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@windowtotal@lift@worldminus\endcsname{\textminus 0.019}
\expandafter\def\csname rev@rcc@sdr@windowtotal@naive@cost\endcsname{0.128}
\expandafter\def\csname rev@rcc@sdr@windowtotal@naive@hi\endcsname{\textminus 0.024}
\expandafter\def\csname rev@rcc@sdr@windowtotal@naive@lo\endcsname{\textminus 0.056}
\expandafter\def\csname rev@rcc@sdr@windowtotal@naive@lowerwin\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@windowtotal@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@windowtotal@naive@worldminus\endcsname{\textminus 0.040}
\expandafter\def\csname rev@rcc@sdr@windowtotal@tfmplan@cost\endcsname{0.109}
\expandafter\def\csname rev@rcc@sdr@windowtotal@tfmplan@hi\endcsname{\textminus 0.013}
\expandafter\def\csname rev@rcc@sdr@windowtotal@tfmplan@lo\endcsname{\textminus 0.029}
\expandafter\def\csname rev@rcc@sdr@windowtotal@tfmplan@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sdr@windowtotal@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sdr@windowtotal@tfmplan@worldminus\endcsname{\textminus 0.021}
\expandafter\def\csname rev@rcc@sdr@windowtotal@world@cost\endcsname{0.088}
\expandafter\def\csname rev@rcc@sna@asfirstrun@ens@cost\endcsname{9935300000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@ens@hi\endcsname{981520000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@ens@lo\endcsname{\textminus 2641000000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@ens@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sna@asfirstrun@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@asfirstrun@ens@worldminus\endcsname{\textminus 512840000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lgb@cost\endcsname{9941700000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lgb@hi\endcsname{1700200000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lgb@lo\endcsname{\textminus 3411700000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lgb@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lgb@worldminus\endcsname{\textminus 519240000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lift@cost\endcsname{10793000000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lift@hi\endcsname{457620000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lift@lo\endcsname{\textminus 4269200000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lift@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@asfirstrun@lift@worldminus\endcsname{\textminus 1370800000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@naive@cost\endcsname{21730000000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@naive@hi\endcsname{\textminus 704760000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@naive@lo\endcsname{\textminus 31520000000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@naive@lowerwin\endcsname{5}
\expandafter\def\csname rev@rcc@sna@asfirstrun@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@asfirstrun@naive@worldminus\endcsname{\textminus 12307000000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@tfmplan@cost\endcsname{10442000000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@tfmplan@hi\endcsname{1318400000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@tfmplan@lo\endcsname{\textminus 4521800000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@tfmplan@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sna@asfirstrun@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@asfirstrun@tfmplan@worldminus\endcsname{\textminus 1019300000.000}
\expandafter\def\csname rev@rcc@sna@asfirstrun@world@cost\endcsname{9422400000.000}
\expandafter\def\csname rev@rcc@sna@dollars@ens@cost\endcsname{0.229}
\expandafter\def\csname rev@rcc@sna@dollars@ens@hi\endcsname{0.082}
\expandafter\def\csname rev@rcc@sna@dollars@ens@lo\endcsname{0.057}
\expandafter\def\csname rev@rcc@sna@dollars@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sna@dollars@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@dollars@ens@worldminus\endcsname{0.069}
\expandafter\def\csname rev@rcc@sna@dollars@lgb@cost\endcsname{0.198}
\expandafter\def\csname rev@rcc@sna@dollars@lgb@hi\endcsname{0.122}
\expandafter\def\csname rev@rcc@sna@dollars@lgb@lo\endcsname{0.081}
\expandafter\def\csname rev@rcc@sna@dollars@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sna@dollars@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@dollars@lgb@worldminus\endcsname{0.100}
\expandafter\def\csname rev@rcc@sna@dollars@lift@cost\endcsname{0.290}
\expandafter\def\csname rev@rcc@sna@dollars@lift@hi\endcsname{0.050}
\expandafter\def\csname rev@rcc@sna@dollars@lift@lo\endcsname{\textminus 0.059}
\expandafter\def\csname rev@rcc@sna@dollars@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@sna@dollars@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@dollars@lift@worldminus\endcsname{0.008}
\expandafter\def\csname rev@rcc@sna@dollars@naive@cost\endcsname{0.382}
\expandafter\def\csname rev@rcc@sna@dollars@naive@hi\endcsname{\textminus 0.060}
\expandafter\def\csname rev@rcc@sna@dollars@naive@lo\endcsname{\textminus 0.108}
\expandafter\def\csname rev@rcc@sna@dollars@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sna@dollars@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@dollars@naive@worldminus\endcsname{\textminus 0.084}
\expandafter\def\csname rev@rcc@sna@dollars@tfmplan@cost\endcsname{0.237}
\expandafter\def\csname rev@rcc@sna@dollars@tfmplan@hi\endcsname{0.079}
\expandafter\def\csname rev@rcc@sna@dollars@tfmplan@lo\endcsname{0.044}
\expandafter\def\csname rev@rcc@sna@dollars@tfmplan@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sna@dollars@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@dollars@tfmplan@worldminus\endcsname{0.061}
\expandafter\def\csname rev@rcc@sna@dollars@world@cost\endcsname{0.298}
\expandafter\def\csname rev@rcc@sna@firsthalf@ens@cost\endcsname{0.155}
\expandafter\def\csname rev@rcc@sna@firsthalf@ens@hi\endcsname{0.068}
\expandafter\def\csname rev@rcc@sna@firsthalf@ens@lo\endcsname{0.043}
\expandafter\def\csname rev@rcc@sna@firsthalf@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sna@firsthalf@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@firsthalf@ens@worldminus\endcsname{0.055}
\expandafter\def\csname rev@rcc@sna@firsthalf@lgb@cost\endcsname{0.143}
\expandafter\def\csname rev@rcc@sna@firsthalf@lgb@hi\endcsname{0.090}
\expandafter\def\csname rev@rcc@sna@firsthalf@lgb@lo\endcsname{0.047}
\expandafter\def\csname rev@rcc@sna@firsthalf@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sna@firsthalf@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@firsthalf@lgb@worldminus\endcsname{0.068}
\expandafter\def\csname rev@rcc@sna@firsthalf@lift@cost\endcsname{0.189}
\expandafter\def\csname rev@rcc@sna@firsthalf@lift@hi\endcsname{0.043}
\expandafter\def\csname rev@rcc@sna@firsthalf@lift@lo\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rcc@sna@firsthalf@lift@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sna@firsthalf@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@firsthalf@lift@worldminus\endcsname{0.021}
\expandafter\def\csname rev@rcc@sna@firsthalf@naive@cost\endcsname{0.371}
\expandafter\def\csname rev@rcc@sna@firsthalf@naive@hi\endcsname{\textminus 0.134}
\expandafter\def\csname rev@rcc@sna@firsthalf@naive@lo\endcsname{\textminus 0.183}
\expandafter\def\csname rev@rcc@sna@firsthalf@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sna@firsthalf@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@firsthalf@naive@worldminus\endcsname{\textminus 0.160}
\expandafter\def\csname rev@rcc@sna@firsthalf@tfmplan@cost\endcsname{0.164}
\expandafter\def\csname rev@rcc@sna@firsthalf@tfmplan@hi\endcsname{0.063}
\expandafter\def\csname rev@rcc@sna@firsthalf@tfmplan@lo\endcsname{0.031}
\expandafter\def\csname rev@rcc@sna@firsthalf@tfmplan@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sna@firsthalf@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@firsthalf@tfmplan@worldminus\endcsname{0.046}
\expandafter\def\csname rev@rcc@sna@firsthalf@world@cost\endcsname{0.211}
\expandafter\def\csname rev@rcc@sna@nodemean@ens@cost\endcsname{0.256}
\expandafter\def\csname rev@rcc@sna@nodemean@ens@hi\endcsname{0.096}
\expandafter\def\csname rev@rcc@sna@nodemean@ens@lo\endcsname{0.070}
\expandafter\def\csname rev@rcc@sna@nodemean@ens@lowerwin\endcsname{0}
\expandafter\def\csname rev@rcc@sna@nodemean@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@nodemean@ens@worldminus\endcsname{0.083}
\expandafter\def\csname rev@rcc@sna@nodemean@lgb@cost\endcsname{0.213}
\expandafter\def\csname rev@rcc@sna@nodemean@lgb@hi\endcsname{0.150}
\expandafter\def\csname rev@rcc@sna@nodemean@lgb@lo\endcsname{0.104}
\expandafter\def\csname rev@rcc@sna@nodemean@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sna@nodemean@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@nodemean@lgb@worldminus\endcsname{0.126}
\expandafter\def\csname rev@rcc@sna@nodemean@lift@cost\endcsname{0.314}
\expandafter\def\csname rev@rcc@sna@nodemean@lift@hi\endcsname{0.059}
\expandafter\def\csname rev@rcc@sna@nodemean@lift@lo\endcsname{\textminus 0.025}
\expandafter\def\csname rev@rcc@sna@nodemean@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@sna@nodemean@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@nodemean@lift@worldminus\endcsname{0.025}
\expandafter\def\csname rev@rcc@sna@nodemean@naive@cost\endcsname{0.402}
\expandafter\def\csname rev@rcc@sna@nodemean@naive@hi\endcsname{\textminus 0.039}
\expandafter\def\csname rev@rcc@sna@nodemean@naive@lo\endcsname{\textminus 0.086}
\expandafter\def\csname rev@rcc@sna@nodemean@naive@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@sna@nodemean@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@nodemean@naive@worldminus\endcsname{\textminus 0.063}
\expandafter\def\csname rev@rcc@sna@nodemean@tfmplan@cost\endcsname{0.264}
\expandafter\def\csname rev@rcc@sna@nodemean@tfmplan@hi\endcsname{0.092}
\expandafter\def\csname rev@rcc@sna@nodemean@tfmplan@lo\endcsname{0.059}
\expandafter\def\csname rev@rcc@sna@nodemean@tfmplan@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sna@nodemean@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@nodemean@tfmplan@worldminus\endcsname{0.075}
\expandafter\def\csname rev@rcc@sna@nodemean@world@cost\endcsname{0.339}
\expandafter\def\csname rev@rcc@sna@units@ens@cost\endcsname{0.238}
\expandafter\def\csname rev@rcc@sna@units@ens@hi\endcsname{0.083}
\expandafter\def\csname rev@rcc@sna@units@ens@lo\endcsname{0.060}
\expandafter\def\csname rev@rcc@sna@units@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sna@units@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@units@ens@worldminus\endcsname{0.071}
\expandafter\def\csname rev@rcc@sna@units@lgb@cost\endcsname{0.204}
\expandafter\def\csname rev@rcc@sna@units@lgb@hi\endcsname{0.125}
\expandafter\def\csname rev@rcc@sna@units@lgb@lo\endcsname{0.087}
\expandafter\def\csname rev@rcc@sna@units@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sna@units@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@units@lgb@worldminus\endcsname{0.105}
\expandafter\def\csname rev@rcc@sna@units@lift@cost\endcsname{0.297}
\expandafter\def\csname rev@rcc@sna@units@lift@hi\endcsname{0.053}
\expandafter\def\csname rev@rcc@sna@units@lift@lo\endcsname{\textminus 0.052}
\expandafter\def\csname rev@rcc@sna@units@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@sna@units@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@units@lift@worldminus\endcsname{0.012}
\expandafter\def\csname rev@rcc@sna@units@naive@cost\endcsname{0.390}
\expandafter\def\csname rev@rcc@sna@units@naive@hi\endcsname{\textminus 0.058}
\expandafter\def\csname rev@rcc@sna@units@naive@lo\endcsname{\textminus 0.105}
\expandafter\def\csname rev@rcc@sna@units@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sna@units@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@units@naive@worldminus\endcsname{\textminus 0.081}
\expandafter\def\csname rev@rcc@sna@units@tfmplan@cost\endcsname{0.245}
\expandafter\def\csname rev@rcc@sna@units@tfmplan@hi\endcsname{0.080}
\expandafter\def\csname rev@rcc@sna@units@tfmplan@lo\endcsname{0.048}
\expandafter\def\csname rev@rcc@sna@units@tfmplan@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sna@units@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@units@tfmplan@worldminus\endcsname{0.064}
\expandafter\def\csname rev@rcc@sna@units@world@cost\endcsname{0.309}
\expandafter\def\csname rev@rcc@sna@weekly@ens@cost\endcsname{0.229}
\expandafter\def\csname rev@rcc@sna@weekly@ens@hi\endcsname{0.081}
\expandafter\def\csname rev@rcc@sna@weekly@ens@lo\endcsname{0.057}
\expandafter\def\csname rev@rcc@sna@weekly@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sna@weekly@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@weekly@ens@worldminus\endcsname{0.069}
\expandafter\def\csname rev@rcc@sna@weekly@lgb@cost\endcsname{0.198}
\expandafter\def\csname rev@rcc@sna@weekly@lgb@hi\endcsname{0.122}
\expandafter\def\csname rev@rcc@sna@weekly@lgb@lo\endcsname{0.081}
\expandafter\def\csname rev@rcc@sna@weekly@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sna@weekly@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@weekly@lgb@worldminus\endcsname{0.100}
\expandafter\def\csname rev@rcc@sna@weekly@lift@cost\endcsname{0.290}
\expandafter\def\csname rev@rcc@sna@weekly@lift@hi\endcsname{0.050}
\expandafter\def\csname rev@rcc@sna@weekly@lift@lo\endcsname{\textminus 0.058}
\expandafter\def\csname rev@rcc@sna@weekly@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@sna@weekly@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@weekly@lift@worldminus\endcsname{0.008}
\expandafter\def\csname rev@rcc@sna@weekly@naive@cost\endcsname{0.382}
\expandafter\def\csname rev@rcc@sna@weekly@naive@hi\endcsname{\textminus 0.059}
\expandafter\def\csname rev@rcc@sna@weekly@naive@lo\endcsname{\textminus 0.107}
\expandafter\def\csname rev@rcc@sna@weekly@naive@lowerwin\endcsname{4}
\expandafter\def\csname rev@rcc@sna@weekly@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@weekly@naive@worldminus\endcsname{\textminus 0.084}
\expandafter\def\csname rev@rcc@sna@weekly@tfmplan@cost\endcsname{0.237}
\expandafter\def\csname rev@rcc@sna@weekly@tfmplan@hi\endcsname{0.079}
\expandafter\def\csname rev@rcc@sna@weekly@tfmplan@lo\endcsname{0.045}
\expandafter\def\csname rev@rcc@sna@weekly@tfmplan@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sna@weekly@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@weekly@tfmplan@worldminus\endcsname{0.061}
\expandafter\def\csname rev@rcc@sna@weekly@world@cost\endcsname{0.298}
\expandafter\def\csname rev@rcc@sna@windowtotal@ens@cost\endcsname{0.181}
\expandafter\def\csname rev@rcc@sna@windowtotal@ens@hi\endcsname{0.090}
\expandafter\def\csname rev@rcc@sna@windowtotal@ens@lo\endcsname{0.065}
\expandafter\def\csname rev@rcc@sna@windowtotal@ens@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sna@windowtotal@ens@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@windowtotal@ens@worldminus\endcsname{0.077}
\expandafter\def\csname rev@rcc@sna@windowtotal@lgb@cost\endcsname{0.149}
\expandafter\def\csname rev@rcc@sna@windowtotal@lgb@hi\endcsname{0.131}
\expandafter\def\csname rev@rcc@sna@windowtotal@lgb@lo\endcsname{0.088}
\expandafter\def\csname rev@rcc@sna@windowtotal@lgb@lowerwin\endcsname{2}
\expandafter\def\csname rev@rcc@sna@windowtotal@lgb@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@windowtotal@lgb@worldminus\endcsname{0.109}
\expandafter\def\csname rev@rcc@sna@windowtotal@lift@cost\endcsname{0.244}
\expandafter\def\csname rev@rcc@sna@windowtotal@lift@hi\endcsname{0.055}
\expandafter\def\csname rev@rcc@sna@windowtotal@lift@lo\endcsname{\textminus 0.057}
\expandafter\def\csname rev@rcc@sna@windowtotal@lift@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@sna@windowtotal@lift@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@windowtotal@lift@worldminus\endcsname{0.013}
\expandafter\def\csname rev@rcc@sna@windowtotal@naive@cost\endcsname{0.280}
\expandafter\def\csname rev@rcc@sna@windowtotal@naive@hi\endcsname{0.004}
\expandafter\def\csname rev@rcc@sna@windowtotal@naive@lo\endcsname{\textminus 0.048}
\expandafter\def\csname rev@rcc@sna@windowtotal@naive@lowerwin\endcsname{3}
\expandafter\def\csname rev@rcc@sna@windowtotal@naive@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@windowtotal@naive@worldminus\endcsname{\textminus 0.023}
\expandafter\def\csname rev@rcc@sna@windowtotal@tfmplan@cost\endcsname{0.178}
\expandafter\def\csname rev@rcc@sna@windowtotal@tfmplan@hi\endcsname{0.098}
\expandafter\def\csname rev@rcc@sna@windowtotal@tfmplan@lo\endcsname{0.062}
\expandafter\def\csname rev@rcc@sna@windowtotal@tfmplan@lowerwin\endcsname{1}
\expandafter\def\csname rev@rcc@sna@windowtotal@tfmplan@windows\endcsname{6}
\expandafter\def\csname rev@rcc@sna@windowtotal@tfmplan@worldminus\endcsname{0.079}
\expandafter\def\csname rev@rcc@sna@windowtotal@world@cost\endcsname{0.258}
\expandafter\def\csname rev@rcore@ens@ixs@better\endcsname{35}
\expandafter\def\csname rev@rcore@ens@ixs@max\endcsname{3.7}
\expandafter\def\csname rev@rcore@ens@ixs@median\endcsname{0.97}
\expandafter\def\csname rev@rcore@ens@ixs@n\endcsname{48}
\expandafter\def\csname rev@rcore@ens@total@better\endcsname{28}
\expandafter\def\csname rev@rcore@ens@total@max\endcsname{2.0}
\expandafter\def\csname rev@rcore@ens@total@median\endcsname{0.95}
\expandafter\def\csname rev@rcore@ens@total@n\endcsname{48}
\expandafter\def\csname rev@rcore@tfmplan@ixs@better\endcsname{12}
\expandafter\def\csname rev@rcore@tfmplan@ixs@max\endcsname{1.4}
\expandafter\def\csname rev@rcore@tfmplan@ixs@median\endcsname{1.03}
\expandafter\def\csname rev@rcore@tfmplan@ixs@n\endcsname{48}
\expandafter\def\csname rev@rcore@tfmplan@total@better\endcsname{14}
\expandafter\def\csname rev@rcore@tfmplan@total@max\endcsname{2.9}
\expandafter\def\csname rev@rcore@tfmplan@total@median\endcsname{1.15}
\expandafter\def\csname rev@rcore@tfmplan@total@n\endcsname{48}
\expandafter\def\csname rev@rcore@world@ixs@better\endcsname{7}
\expandafter\def\csname rev@rcore@world@ixs@max\endcsname{9.6}
\expandafter\def\csname rev@rcore@world@ixs@median\endcsname{1.04}
\expandafter\def\csname rev@rcore@world@ixs@n\endcsname{48}
\expandafter\def\csname rev@rcore@world@total@better\endcsname{22}
\expandafter\def\csname rev@rcore@world@total@max\endcsname{4.7}
\expandafter\def\csname rev@rcore@world@total@median\endcsname{1.10}
\expandafter\def\csname rev@rcore@world@total@n\endcsname{48}
\expandafter\def\csname rev@rcount@addsnotliftixslist\endcsname{bottled juice, frozen entrees and M5}
\expandafter\def\csname rev@rcount@addsnotlifttotallist\endcsname{bottled juice, frozen entrees and M5}
\expandafter\def\csname rev@rcount@bothaddixs\endcsname{one}
\expandafter\def\csname rev@rcount@bothaddixslist\endcsname{Favorita}
\expandafter\def\csname rev@rcount@bothaddtotal\endcsname{none}
\expandafter\def\csname rev@rcount@bothaddtotallist\endcsname{none}
\expandafter\def\csname rev@rcount@ccclearother\endcsname{seven}
\expandafter\def\csname rev@rcount@ccclearotherlist\endcsname{cheese, snack crackers, soft drinks, bottled juice, analgesics, frozen entrees and Frat}
\expandafter\def\csname rev@rcount@ccclearworld\endcsname{none}
\expandafter\def\csname rev@rcount@ccdollarsens\endcsname{four}
\expandafter\def\csname rev@rcount@ccdollarsenslist\endcsname{analgesics, bottled juice, soft drinks and Frat}
\expandafter\def\csname rev@rcount@ccdollarslgb\endcsname{three}
\expandafter\def\csname rev@rcount@ccdollarslgblist\endcsname{cheese, frozen entrees and snack crackers}
\expandafter\def\csname rev@rcount@ccdollarsworld\endcsname{one}
\expandafter\def\csname rev@rcount@ccdollarsworldlist\endcsname{M5}
\expandafter\def\csname rev@rcount@ccfirsthalfens\endcsname{four}
\expandafter\def\csname rev@rcount@ccfirsthalfenslist\endcsname{analgesics, bottled juice, soft drinks and Frat}
\expandafter\def\csname rev@rcount@ccfirsthalflgb\endcsname{two}
\expandafter\def\csname rev@rcount@ccfirsthalflgblist\endcsname{frozen entrees and snack crackers}
\expandafter\def\csname rev@rcount@ccfirsthalfworld\endcsname{one}
\expandafter\def\csname rev@rcount@ccfirsthalfworldlist\endcsname{M5}
\expandafter\def\csname rev@rcount@ccnodemeanens\endcsname{five}
\expandafter\def\csname rev@rcount@ccnodemeanenslist\endcsname{analgesics, bottled juice, cheese, soft drinks and Frat}
\expandafter\def\csname rev@rcount@ccnodemeanlgb\endcsname{three}
\expandafter\def\csname rev@rcount@ccnodemeanlgblist\endcsname{frozen entrees, snack crackers and M5}
\expandafter\def\csname rev@rcount@ccnodemeanworld\endcsname{none}
\expandafter\def\csname rev@rcount@ccnodemeanworldlist\endcsname{none}
\expandafter\def\csname rev@rcount@ccunitsens\endcsname{four}
\expandafter\def\csname rev@rcount@ccunitsenslist\endcsname{analgesics, bottled juice, soft drinks and Frat}
\expandafter\def\csname rev@rcount@ccunitslgb\endcsname{three}
\expandafter\def\csname rev@rcount@ccunitslgblist\endcsname{cheese, frozen entrees and snack crackers}
\expandafter\def\csname rev@rcount@ccunitsworld\endcsname{one}
\expandafter\def\csname rev@rcount@ccunitsworldlist\endcsname{M5}
\expandafter\def\csname rev@rcount@ccwindowtotalens\endcsname{two}
\expandafter\def\csname rev@rcount@ccwindowtotalenslist\endcsname{soft drinks and Frat}
\expandafter\def\csname rev@rcount@ccwindowtotallgb\endcsname{five}
\expandafter\def\csname rev@rcount@ccwindowtotallgblist\endcsname{analgesics, bottled juice, cheese, frozen entrees and snack crackers}
\expandafter\def\csname rev@rcount@ccwindowtotalworld\endcsname{one}
\expandafter\def\csname rev@rcount@ccwindowtotalworldlist\endcsname{M5}
\expandafter\def\csname rev@rcount@cczerohi\endcsname{5}
\expandafter\def\csname rev@rcount@cczerolo\endcsname{4}
\expandafter\def\csname rev@rcount@cczeron\endcsname{558}
\expandafter\def\csname rev@rcount@changen\endcsname{23}
\expandafter\def\csname rev@rcount@changepairs\endcsname{157}
\expandafter\def\csname rev@rcount@decenscat\endcsname{four}
\expandafter\def\csname rev@rcount@decenscatlist\endcsname{analgesics, bottled juice, soft drinks and Frat}
\expandafter\def\csname rev@rcount@decensorder\endcsname{three}
\expandafter\def\csname rev@rcount@decensorderlist\endcsname{bottled juice, Frat and M5}
\expandafter\def\csname rev@rcount@declgbcat\endcsname{three}
\expandafter\def\csname rev@rcount@declgbcatlist\endcsname{cheese, frozen entrees and snack crackers}
\expandafter\def\csname rev@rcount@declgborder\endcsname{five}
\expandafter\def\csname rev@rcount@declgborderlist\endcsname{analgesics, cheese, frozen entrees, soft drinks and snack crackers}
\expandafter\def\csname rev@rcount@decliftcat\endcsname{none}
\expandafter\def\csname rev@rcount@decliftcatlist\endcsname{none}
\expandafter\def\csname rev@rcount@decliftorder\endcsname{none}
\expandafter\def\csname rev@rcount@decliftorderlist\endcsname{none}
\expandafter\def\csname rev@rcount@decworldcat\endcsname{one}
\expandafter\def\csname rev@rcount@decworldcatlist\endcsname{M5}
\expandafter\def\csname rev@rcount@decworldorder\endcsname{none}
\expandafter\def\csname rev@rcount@decworldorderlist\endcsname{none}
\expandafter\def\csname rev@rcount@ensaloneixs\endcsname{five}
\expandafter\def\csname rev@rcount@ensaloneixslist\endcsname{snack crackers, bottled juice, Frat, M5 and Favorita}
\expandafter\def\csname rev@rcount@ensbeatslgbixs\endcsname{four}
\expandafter\def\csname rev@rcount@ensbeatslgbixslist\endcsname{bottled juice, snack crackers, Frat and M5}
\expandafter\def\csname rev@rcount@ensbeatslgbtotal\endcsname{one}
\expandafter\def\csname rev@rcount@ensbeatslgbtotallist\endcsname{analgesics}
\expandafter\def\csname rev@rcount@ensbeatsnaiveixs\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatsnaiveixslist\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatsnaivetotal\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatsnaivetotallist\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatstfmixs\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatstfmixslist\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatstfmtotal\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatstfmtotallist\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatstftixs\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatstftixslist\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatstfttotal\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatstfttotallist\endcsname{none}
\expandafter\def\csname rev@rcount@ensbeatsworldixs\endcsname{eight}
\expandafter\def\csname rev@rcount@ensbeatsworldixslist\endcsname{analgesics, bottled juice, cheese, frozen entrees, soft drinks, snack crackers, Frat and M5}
\expandafter\def\csname rev@rcount@ensbeatsworldtotal\endcsname{two}
\expandafter\def\csname rev@rcount@ensbeatsworldtotallist\endcsname{cheese and Frat}
\expandafter\def\csname rev@rcount@ensinsetixs\endcsname{eight}
\expandafter\def\csname rev@rcount@ensinsettotal\endcsname{nine}
\expandafter\def\csname rev@rcount@enslosestolgbixs\endcsname{none}
\expandafter\def\csname rev@rcount@enslosestolgbtotal\endcsname{none}
\expandafter\def\csname rev@rcount@enslosestonaiveixs\endcsname{none}
\expandafter\def\csname rev@rcount@enslosestonaivetotal\endcsname{none}
\expandafter\def\csname rev@rcount@enslosestotfmixs\endcsname{none}
\expandafter\def\csname rev@rcount@enslosestotfmtotal\endcsname{none}
\expandafter\def\csname rev@rcount@enslosestotftixs\endcsname{none}
\expandafter\def\csname rev@rcount@enslosestotfttotal\endcsname{none}
\expandafter\def\csname rev@rcount@enslosestoworldixs\endcsname{none}
\expandafter\def\csname rev@rcount@enslosestoworldtotal\endcsname{none}
\expandafter\def\csname rev@rcount@enslowestixs\endcsname{seven}
\expandafter\def\csname rev@rcount@enslowestixsnot\endcsname{analgesics (LightGBM), cheese (LightGBM)}
\expandafter\def\csname rev@rcount@enslowesttotal\endcsname{four}
\expandafter\def\csname rev@rcount@ensnlgbixs\endcsname{eight}
\expandafter\def\csname rev@rcount@ensnlgbtotal\endcsname{eight}
\expandafter\def\csname rev@rcount@ensnnaiveixs\endcsname{none}
\expandafter\def\csname rev@rcount@ensnnaivetotal\endcsname{none}
\expandafter\def\csname rev@rcount@ensnotinsetixs\endcsname{cheese}
\expandafter\def\csname rev@rcount@ensntfmixs\endcsname{none}
\expandafter\def\csname rev@rcount@ensntfmtotal\endcsname{none}
\expandafter\def\csname rev@rcount@ensntftixs\endcsname{none}
\expandafter\def\csname rev@rcount@ensntfttotal\endcsname{none}
\expandafter\def\csname rev@rcount@ensnworldixs\endcsname{eight}
\expandafter\def\csname rev@rcount@ensnworldtotal\endcsname{eight}
\expandafter\def\csname rev@rcount@finalsgap\endcsname{0.02}
\expandafter\def\csname rev@rcount@fittedalllevelsixsens\endcsname{five}
\expandafter\def\csname rev@rcount@fittedalllevelsixsenslist\endcsname{analgesics, cheese, Frat, M5 and Favorita}
\expandafter\def\csname rev@rcount@fittedalllevelsixsvar\endcsname{none}
\expandafter\def\csname rev@rcount@fittedalllevelsixsvarlist\endcsname{none}
\expandafter\def\csname rev@rcount@fittedalllevelstotalens\endcsname{none}
\expandafter\def\csname rev@rcount@fittedalllevelstotalenslist\endcsname{none}
\expandafter\def\csname rev@rcount@fittedalllevelstotalvar\endcsname{one}
\expandafter\def\csname rev@rcount@fittedalllevelstotalvarlist\endcsname{Frat}
\expandafter\def\csname rev@rcount@fittedbottomixsens\endcsname{one}
\expandafter\def\csname rev@rcount@fittedbottomixsenslist\endcsname{cheese}
\expandafter\def\csname rev@rcount@fittedbottomixsvar\endcsname{two}
\expandafter\def\csname rev@rcount@fittedbottomixsvarlist\endcsname{analgesics and frozen entrees}
\expandafter\def\csname rev@rcount@fittedbottomtotalens\endcsname{two}
\expandafter\def\csname rev@rcount@fittedbottomtotalenslist\endcsname{M5 and Favorita}
\expandafter\def\csname rev@rcount@fittedbottomtotalvar\endcsname{one}
\expandafter\def\csname rev@rcount@fittedbottomtotalvarlist\endcsname{Frat}
\expandafter\def\csname rev@rcount@fittedlosses\endcsname{13}
\expandafter\def\csname rev@rcount@fittedn\endcsname{54}
\expandafter\def\csname rev@rcount@fittedtotalixsens\endcsname{five}
\expandafter\def\csname rev@rcount@fittedtotalixsenslist\endcsname{analgesics, snack crackers, Frat, M5 and Favorita}
\expandafter\def\csname rev@rcount@fittedtotalixsvar\endcsname{none}
\expandafter\def\csname rev@rcount@fittedtotalixsvarlist\endcsname{none}
\expandafter\def\csname rev@rcount@fittedtotaltotalens\endcsname{none}
\expandafter\def\csname rev@rcount@fittedtotaltotalenslist\endcsname{none}
\expandafter\def\csname rev@rcount@fittedtotaltotalvar\endcsname{one}
\expandafter\def\csname rev@rcount@fittedtotaltotalvarlist\endcsname{Frat}
\expandafter\def\csname rev@rcount@fittedwins\endcsname{five}
\expandafter\def\csname rev@rcount@lgbbeatstfmplanixs\endcsname{six}
\expandafter\def\csname rev@rcount@lgbbeatstfmplanixslist\endcsname{analgesics, bottled juice, cheese, frozen entrees, soft drinks and snack crackers}
\expandafter\def\csname rev@rcount@lgbbeatstfmplantotal\endcsname{four}
\expandafter\def\csname rev@rcount@lgbbeatstfmplantotallist\endcsname{bottled juice, frozen entrees, soft drinks and M5}
\expandafter\def\csname rev@rcount@lgbbeatstftixs\endcsname{seven}
\expandafter\def\csname rev@rcount@lgbbeatstftixslist\endcsname{analgesics, bottled juice, cheese, frozen entrees, soft drinks, snack crackers and Frat}
\expandafter\def\csname rev@rcount@lgbbeatstfttotal\endcsname{three}
\expandafter\def\csname rev@rcount@lgbbeatstfttotallist\endcsname{bottled juice, frozen entrees and soft drinks}
\expandafter\def\csname rev@rcount@lgbbeatsworldixs\endcsname{six}
\expandafter\def\csname rev@rcount@lgbbeatsworldixslist\endcsname{analgesics, bottled juice, cheese, soft drinks, snack crackers and Frat}
\expandafter\def\csname rev@rcount@lgbbeatsworldtotal\endcsname{one}
\expandafter\def\csname rev@rcount@lgbbeatsworldtotallist\endcsname{Frat}
\expandafter\def\csname rev@rcount@lgbtfmplanixsn\endcsname{eight}
\expandafter\def\csname rev@rcount@lgbtfmplantotaln\endcsname{eight}
\expandafter\def\csname rev@rcount@lgbtftixsn\endcsname{seven}
\expandafter\def\csname rev@rcount@lgbtfttotaln\endcsname{seven}
\expandafter\def\csname rev@rcount@lgbworldixsn\endcsname{eight}
\expandafter\def\csname rev@rcount@lgbworldtotaln\endcsname{eight}
\expandafter\def\csname rev@rcount@liftbeatsworldixs\endcsname{two}
\expandafter\def\csname rev@rcount@liftbeatsworldixslist\endcsname{bottled juice and M5}
\expandafter\def\csname rev@rcount@liftbeatsworldtotal\endcsname{none}
\expandafter\def\csname rev@rcount@liftbeatsworldtotallist\endcsname{none}
\expandafter\def\csname rev@rcount@liftforworldmodelixsens\endcsname{three}
\expandafter\def\csname rev@rcount@liftforworldmodelixsenslist\endcsname{analgesics, soft drinks and Favorita}
\expandafter\def\csname rev@rcount@liftforworldmodelixsvar\endcsname{none}
\expandafter\def\csname rev@rcount@liftforworldmodelixsvarlist\endcsname{none}
\expandafter\def\csname rev@rcount@liftforworldmodeltotalens\endcsname{two}
\expandafter\def\csname rev@rcount@liftforworldmodeltotalenslist\endcsname{analgesics and Favorita}
\expandafter\def\csname rev@rcount@liftforworldmodeltotalvar\endcsname{none}
\expandafter\def\csname rev@rcount@liftforworldmodeltotalvarlist\endcsname{none}
\expandafter\def\csname rev@rcount@liftonlyixslist\endcsname{soft drinks and analgesics}
\expandafter\def\csname rev@rcount@liftonlytotallist\endcsname{analgesics and Favorita}
\expandafter\def\csname rev@rcount@liftworldixsn\endcsname{eight}
\expandafter\def\csname rev@rcount@liftworldtotaln\endcsname{eight}
\expandafter\def\csname rev@rcount@lossbetter\endcsname{10}
\expandafter\def\csname rev@rcount@losschanges\endcsname{16}
\expandafter\def\csname rev@rcount@lossn\endcsname{44}
\expandafter\def\csname rev@rcount@lowesttotallist\endcsname{LightGBM in frozen entrees; LightGBM in soft drinks; the lift model in snack crackers; TimesFM with the plan on Frat; the world model on M5}
\expandafter\def\csname rev@rcount@reclgbworsedom\endcsname{six}
\expandafter\def\csname rev@rcount@tfmbeatstsmean\endcsname{10}
\expandafter\def\csname rev@rcount@tfmbeatstsplan\endcsname{16}
\expandafter\def\csname rev@rcount@tfmplanbeatslgbixs\endcsname{none}
\expandafter\def\csname rev@rcount@tfmplanbeatslgbixslist\endcsname{none}
\expandafter\def\csname rev@rcount@tfmplanbeatslgbtotal\endcsname{none}
\expandafter\def\csname rev@rcount@tfmplanbeatslgbtotallist\endcsname{none}
\expandafter\def\csname rev@rcount@tfmplanbeatsworldixs\endcsname{one}
\expandafter\def\csname rev@rcount@tfmplanbeatsworldixslist\endcsname{M5}
\expandafter\def\csname rev@rcount@tfmplanbeatsworldtotal\endcsname{one}
\expandafter\def\csname rev@rcount@tfmplanbeatsworldtotallist\endcsname{Frat}
\expandafter\def\csname rev@rcount@tfmplanworldixsn\endcsname{eight}
\expandafter\def\csname rev@rcount@tfmplanworldtotaln\endcsname{eight}
\expandafter\def\csname rev@rcount@tftbeatslgbixs\endcsname{none}
\expandafter\def\csname rev@rcount@tftbeatslgbixslist\endcsname{none}
\expandafter\def\csname rev@rcount@tftbeatslgbtotal\endcsname{none}
\expandafter\def\csname rev@rcount@tftbeatslgbtotallist\endcsname{none}
\expandafter\def\csname rev@rcount@tftnativebetter\endcsname{seven}
\expandafter\def\csname rev@rcount@tftnativen\endcsname{seven}
\expandafter\def\csname rev@rcount@tsbeatstfmmean\endcsname{none}
\expandafter\def\csname rev@rcount@tsbeatstfmplan\endcsname{none}
\expandafter\def\csname rev@rcount@tsvstfmmeanlevel\endcsname{the total in cheese, the total in frozen entrees, the total in soft drinks, the total in snack crackers, the total on Frat and the total on M5}
\expandafter\def\csname rev@rcount@tsvstfmmeann\endcsname{16}
\expandafter\def\csname rev@rcount@tsvstfmplanlevel\endcsname{the total on Favorita and the total on M5}
\expandafter\def\csname rev@rcount@tsvstfmplann\endcsname{18}
\expandafter\def\csname rev@rcount@withoutlightgbmixsens\endcsname{eight}
\expandafter\def\csname rev@rcount@withoutlightgbmixsenslist\endcsname{analgesics, bottled juice, cheese, frozen entrees, soft drinks, snack crackers, Frat and Favorita}
\expandafter\def\csname rev@rcount@withoutlightgbmixsvar\endcsname{none}
\expandafter\def\csname rev@rcount@withoutlightgbmixsvarlist\endcsname{none}
\expandafter\def\csname rev@rcount@withoutlightgbmtotalens\endcsname{four}
\expandafter\def\csname rev@rcount@withoutlightgbmtotalenslist\endcsname{cheese, frozen entrees, soft drinks and Frat}
\expandafter\def\csname rev@rcount@withoutlightgbmtotalvar\endcsname{none}
\expandafter\def\csname rev@rcount@withoutlightgbmtotalvarlist\endcsname{none}
\expandafter\def\csname rev@rcount@withouttimesfmixsens\endcsname{five}
\expandafter\def\csname rev@rcount@withouttimesfmixsenslist\endcsname{bottled juice, cheese, Frat, M5 and Favorita}
\expandafter\def\csname rev@rcount@withouttimesfmixsvar\endcsname{none}
\expandafter\def\csname rev@rcount@withouttimesfmixsvarlist\endcsname{none}
\expandafter\def\csname rev@rcount@withouttimesfmtotalens\endcsname{one}
\expandafter\def\csname rev@rcount@withouttimesfmtotalenslist\endcsname{Frat}
\expandafter\def\csname rev@rcount@withouttimesfmtotalvar\endcsname{two}
\expandafter\def\csname rev@rcount@withouttimesfmtotalvarlist\endcsname{M5 and Favorita}
\expandafter\def\csname rev@rcount@withoutworldmodelixsens\endcsname{four}
\expandafter\def\csname rev@rcount@withoutworldmodelixsenslist\endcsname{bottled juice, frozen entrees, M5 and Favorita}
\expandafter\def\csname rev@rcount@withoutworldmodelixsvar\endcsname{none}
\expandafter\def\csname rev@rcount@withoutworldmodelixsvarlist\endcsname{none}
\expandafter\def\csname rev@rcount@withoutworldmodeltotalens\endcsname{three}
\expandafter\def\csname rev@rcount@withoutworldmodeltotalenslist\endcsname{bottled juice, frozen entrees and M5}
\expandafter\def\csname rev@rcount@withoutworldmodeltotalvar\endcsname{one}
\expandafter\def\csname rev@rcount@withoutworldmodeltotalvarlist\endcsname{Frat}
\expandafter\def\csname rev@rcount@worldbeatslgbixs\endcsname{none}
\expandafter\def\csname rev@rcount@worldbeatslgbixslist\endcsname{none}
\expandafter\def\csname rev@rcount@worldbeatslgbtotal\endcsname{none}
\expandafter\def\csname rev@rcount@worldbeatslgbtotallist\endcsname{none}
\expandafter\def\csname rev@rcount@worldbeatsliftcat\endcsname{four}
\expandafter\def\csname rev@rcount@worldbeatsliftixs\endcsname{one}
\expandafter\def\csname rev@rcount@worldbeatsliftixslist\endcsname{soft drinks}
\expandafter\def\csname rev@rcount@worldbeatslifttotal\endcsname{none}
\expandafter\def\csname rev@rcount@worldbeatslifttotallist\endcsname{none}
\expandafter\def\csname rev@rcount@worldbeatstfmplanixs\endcsname{one}
\expandafter\def\csname rev@rcount@worldbeatstfmplanixslist\endcsname{frozen entrees}
\expandafter\def\csname rev@rcount@worldbeatstfmplantotal\endcsname{two}
\expandafter\def\csname rev@rcount@worldbeatstfmplantotallist\endcsname{frozen entrees and M5}
\expandafter\def\csname rev@rdec@ana@categoryplanning@ens\endcsname{0.46}
\expandafter\def\csname rev@rdec@ana@categoryplanning@lgb\endcsname{0.48}
\expandafter\def\csname rev@rdec@ana@categoryplanning@lift\endcsname{0.49}
\expandafter\def\csname rev@rdec@ana@categoryplanning@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@ana@categoryplanning@tfmplan\endcsname{0.51}
\expandafter\def\csname rev@rdec@ana@categoryplanning@world\endcsname{0.48}
\expandafter\def\csname rev@rdec@ana@replenish05@chronos\endcsname{0.79}
\expandafter\def\csname rev@rdec@ana@replenish05@ens\endcsname{0.69}
\expandafter\def\csname rev@rdec@ana@replenish05@lgb\endcsname{0.68}
\expandafter\def\csname rev@rdec@ana@replenish05@lift\endcsname{0.72}
\expandafter\def\csname rev@rdec@ana@replenish05@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@ana@replenish05@tfm\endcsname{0.77}
\expandafter\def\csname rev@rdec@ana@replenish05@tfmplan\endcsname{0.73}
\expandafter\def\csname rev@rdec@ana@replenish05@tft\endcsname{0.72}
\expandafter\def\csname rev@rdec@ana@replenish05@world\endcsname{0.71}
\expandafter\def\csname rev@rdec@ana@replenish08@chronos\endcsname{0.78}
\expandafter\def\csname rev@rdec@ana@replenish08@ens\endcsname{0.68}
\expandafter\def\csname rev@rdec@ana@replenish08@lgb\endcsname{0.68}
\expandafter\def\csname rev@rdec@ana@replenish08@lift\endcsname{0.71}
\expandafter\def\csname rev@rdec@ana@replenish08@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@ana@replenish08@tfm\endcsname{0.76}
\expandafter\def\csname rev@rdec@ana@replenish08@tfmplan\endcsname{0.71}
\expandafter\def\csname rev@rdec@ana@replenish08@tft\endcsname{0.68}
\expandafter\def\csname rev@rdec@ana@replenish08@world\endcsname{0.70}
\expandafter\def\csname rev@rdec@ana@replenish095@chronos\endcsname{0.87}
\expandafter\def\csname rev@rdec@ana@replenish095@ens\endcsname{0.74}
\expandafter\def\csname rev@rdec@ana@replenish095@lgb\endcsname{0.74}
\expandafter\def\csname rev@rdec@ana@replenish095@lift\endcsname{0.76}
\expandafter\def\csname rev@rdec@ana@replenish095@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@ana@replenish095@tfm\endcsname{0.87}
\expandafter\def\csname rev@rdec@ana@replenish095@tfmplan\endcsname{0.77}
\expandafter\def\csname rev@rdec@ana@replenish095@tft\endcsname{0.76}
\expandafter\def\csname rev@rdec@ana@replenish095@world\endcsname{0.75}
\expandafter\def\csname rev@rdec@bjc@categoryplanning@ens\endcsname{0.38}
\expandafter\def\csname rev@rdec@bjc@categoryplanning@lgb\endcsname{0.40}
\expandafter\def\csname rev@rdec@bjc@categoryplanning@lift\endcsname{0.46}
\expandafter\def\csname rev@rdec@bjc@categoryplanning@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@bjc@categoryplanning@tfmplan\endcsname{0.45}
\expandafter\def\csname rev@rdec@bjc@categoryplanning@world\endcsname{0.48}
\expandafter\def\csname rev@rdec@bjc@replenish05@chronos\endcsname{0.60}
\expandafter\def\csname rev@rdec@bjc@replenish05@ens\endcsname{0.45}
\expandafter\def\csname rev@rdec@bjc@replenish05@lgb\endcsname{0.46}
\expandafter\def\csname rev@rdec@bjc@replenish05@lift\endcsname{0.49}
\expandafter\def\csname rev@rdec@bjc@replenish05@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@bjc@replenish05@tfm\endcsname{0.56}
\expandafter\def\csname rev@rdec@bjc@replenish05@tfmplan\endcsname{0.51}
\expandafter\def\csname rev@rdec@bjc@replenish05@tft\endcsname{0.51}
\expandafter\def\csname rev@rdec@bjc@replenish05@world\endcsname{0.48}
\expandafter\def\csname rev@rdec@bjc@replenish08@chronos\endcsname{0.64}
\expandafter\def\csname rev@rdec@bjc@replenish08@ens\endcsname{0.48}
\expandafter\def\csname rev@rdec@bjc@replenish08@lgb\endcsname{0.49}
\expandafter\def\csname rev@rdec@bjc@replenish08@lift\endcsname{0.51}
\expandafter\def\csname rev@rdec@bjc@replenish08@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@bjc@replenish08@tfm\endcsname{0.63}
\expandafter\def\csname rev@rdec@bjc@replenish08@tfmplan\endcsname{0.54}
\expandafter\def\csname rev@rdec@bjc@replenish08@tft\endcsname{0.53}
\expandafter\def\csname rev@rdec@bjc@replenish08@world\endcsname{0.49}
\expandafter\def\csname rev@rdec@bjc@replenish095@chronos\endcsname{0.77}
\expandafter\def\csname rev@rdec@bjc@replenish095@ens\endcsname{0.56}
\expandafter\def\csname rev@rdec@bjc@replenish095@lgb\endcsname{0.57}
\expandafter\def\csname rev@rdec@bjc@replenish095@lift\endcsname{0.58}
\expandafter\def\csname rev@rdec@bjc@replenish095@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@bjc@replenish095@tfm\endcsname{0.77}
\expandafter\def\csname rev@rdec@bjc@replenish095@tfmplan\endcsname{0.65}
\expandafter\def\csname rev@rdec@bjc@replenish095@tft\endcsname{0.65}
\expandafter\def\csname rev@rdec@bjc@replenish095@world\endcsname{0.55}
\expandafter\def\csname rev@rdec@che@categoryplanning@ens\endcsname{0.53}
\expandafter\def\csname rev@rdec@che@categoryplanning@lgb\endcsname{0.45}
\expandafter\def\csname rev@rdec@che@categoryplanning@lift\endcsname{0.69}
\expandafter\def\csname rev@rdec@che@categoryplanning@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@che@categoryplanning@tfmplan\endcsname{0.50}
\expandafter\def\csname rev@rdec@che@categoryplanning@world\endcsname{0.94}
\expandafter\def\csname rev@rdec@che@replenish05@chronos\endcsname{0.72}
\expandafter\def\csname rev@rdec@che@replenish05@ens\endcsname{0.50}
\expandafter\def\csname rev@rdec@che@replenish05@lgb\endcsname{0.51}
\expandafter\def\csname rev@rdec@che@replenish05@lift\endcsname{0.54}
\expandafter\def\csname rev@rdec@che@replenish05@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@che@replenish05@tfm\endcsname{0.71}
\expandafter\def\csname rev@rdec@che@replenish05@tfmplan\endcsname{0.57}
\expandafter\def\csname rev@rdec@che@replenish05@tft\endcsname{0.60}
\expandafter\def\csname rev@rdec@che@replenish05@world\endcsname{0.54}
\expandafter\def\csname rev@rdec@che@replenish08@chronos\endcsname{0.78}
\expandafter\def\csname rev@rdec@che@replenish08@ens\endcsname{0.52}
\expandafter\def\csname rev@rdec@che@replenish08@lgb\endcsname{0.52}
\expandafter\def\csname rev@rdec@che@replenish08@lift\endcsname{0.57}
\expandafter\def\csname rev@rdec@che@replenish08@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@che@replenish08@tfm\endcsname{0.77}
\expandafter\def\csname rev@rdec@che@replenish08@tfmplan\endcsname{0.62}
\expandafter\def\csname rev@rdec@che@replenish08@tft\endcsname{0.62}
\expandafter\def\csname rev@rdec@che@replenish08@world\endcsname{0.55}
\expandafter\def\csname rev@rdec@che@replenish095@chronos\endcsname{0.90}
\expandafter\def\csname rev@rdec@che@replenish095@ens\endcsname{0.59}
\expandafter\def\csname rev@rdec@che@replenish095@lgb\endcsname{0.57}
\expandafter\def\csname rev@rdec@che@replenish095@lift\endcsname{0.61}
\expandafter\def\csname rev@rdec@che@replenish095@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@che@replenish095@tfm\endcsname{0.89}
\expandafter\def\csname rev@rdec@che@replenish095@tfmplan\endcsname{0.73}
\expandafter\def\csname rev@rdec@che@replenish095@tft\endcsname{0.75}
\expandafter\def\csname rev@rdec@che@replenish095@world\endcsname{0.61}
\expandafter\def\csname rev@rdec@frat@categoryplanning@ens\endcsname{0.50}
\expandafter\def\csname rev@rdec@frat@categoryplanning@lgb\endcsname{0.51}
\expandafter\def\csname rev@rdec@frat@categoryplanning@lift\endcsname{0.56}
\expandafter\def\csname rev@rdec@frat@categoryplanning@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@frat@categoryplanning@tfmplan\endcsname{0.52}
\expandafter\def\csname rev@rdec@frat@categoryplanning@world\endcsname{0.57}
\expandafter\def\csname rev@rdec@frat@replenish05@chronos\endcsname{0.76}
\expandafter\def\csname rev@rdec@frat@replenish05@ens\endcsname{0.49}
\expandafter\def\csname rev@rdec@frat@replenish05@lgb\endcsname{0.51}
\expandafter\def\csname rev@rdec@frat@replenish05@lift\endcsname{0.52}
\expandafter\def\csname rev@rdec@frat@replenish05@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@frat@replenish05@tfm\endcsname{0.76}
\expandafter\def\csname rev@rdec@frat@replenish05@tfmplan\endcsname{0.53}
\expandafter\def\csname rev@rdec@frat@replenish05@tft\endcsname{0.56}
\expandafter\def\csname rev@rdec@frat@replenish05@world\endcsname{0.54}
\expandafter\def\csname rev@rdec@frat@replenish08@chronos\endcsname{0.88}
\expandafter\def\csname rev@rdec@frat@replenish08@ens\endcsname{0.50}
\expandafter\def\csname rev@rdec@frat@replenish08@lgb\endcsname{0.52}
\expandafter\def\csname rev@rdec@frat@replenish08@lift\endcsname{0.52}
\expandafter\def\csname rev@rdec@frat@replenish08@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@frat@replenish08@tfm\endcsname{0.88}
\expandafter\def\csname rev@rdec@frat@replenish08@tfmplan\endcsname{0.56}
\expandafter\def\csname rev@rdec@frat@replenish08@tft\endcsname{0.57}
\expandafter\def\csname rev@rdec@frat@replenish08@world\endcsname{0.53}
\expandafter\def\csname rev@rdec@frat@replenish095@chronos\endcsname{0.95}
\expandafter\def\csname rev@rdec@frat@replenish095@ens\endcsname{0.59}
\expandafter\def\csname rev@rdec@frat@replenish095@lgb\endcsname{0.59}
\expandafter\def\csname rev@rdec@frat@replenish095@lift\endcsname{0.60}
\expandafter\def\csname rev@rdec@frat@replenish095@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@frat@replenish095@tfm\endcsname{0.95}
\expandafter\def\csname rev@rdec@frat@replenish095@tfmplan\endcsname{0.65}
\expandafter\def\csname rev@rdec@frat@replenish095@tft\endcsname{0.67}
\expandafter\def\csname rev@rdec@frat@replenish095@world\endcsname{0.60}
\expandafter\def\csname rev@rdec@fre@categoryplanning@ens\endcsname{0.58}
\expandafter\def\csname rev@rdec@fre@categoryplanning@lgb\endcsname{0.50}
\expandafter\def\csname rev@rdec@fre@categoryplanning@lift\endcsname{0.67}
\expandafter\def\csname rev@rdec@fre@categoryplanning@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@fre@categoryplanning@tfmplan\endcsname{0.83}
\expandafter\def\csname rev@rdec@fre@categoryplanning@world\endcsname{0.56}
\expandafter\def\csname rev@rdec@fre@replenish05@chronos\endcsname{0.71}
\expandafter\def\csname rev@rdec@fre@replenish05@ens\endcsname{0.55}
\expandafter\def\csname rev@rdec@fre@replenish05@lgb\endcsname{0.52}
\expandafter\def\csname rev@rdec@fre@replenish05@lift\endcsname{0.62}
\expandafter\def\csname rev@rdec@fre@replenish05@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@fre@replenish05@tfm\endcsname{0.74}
\expandafter\def\csname rev@rdec@fre@replenish05@tfmplan\endcsname{0.74}
\expandafter\def\csname rev@rdec@fre@replenish05@tft\endcsname{0.61}
\expandafter\def\csname rev@rdec@fre@replenish05@world\endcsname{0.54}
\expandafter\def\csname rev@rdec@fre@replenish08@chronos\endcsname{0.85}
\expandafter\def\csname rev@rdec@fre@replenish08@ens\endcsname{0.51}
\expandafter\def\csname rev@rdec@fre@replenish08@lgb\endcsname{0.51}
\expandafter\def\csname rev@rdec@fre@replenish08@lift\endcsname{0.60}
\expandafter\def\csname rev@rdec@fre@replenish08@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@fre@replenish08@tfm\endcsname{0.84}
\expandafter\def\csname rev@rdec@fre@replenish08@tfmplan\endcsname{0.63}
\expandafter\def\csname rev@rdec@fre@replenish08@tft\endcsname{0.55}
\expandafter\def\csname rev@rdec@fre@replenish08@world\endcsname{0.52}
\expandafter\def\csname rev@rdec@fre@replenish095@chronos\endcsname{0.95}
\expandafter\def\csname rev@rdec@fre@replenish095@ens\endcsname{0.56}
\expandafter\def\csname rev@rdec@fre@replenish095@lgb\endcsname{0.58}
\expandafter\def\csname rev@rdec@fre@replenish095@lift\endcsname{0.63}
\expandafter\def\csname rev@rdec@fre@replenish095@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@fre@replenish095@tfm\endcsname{0.94}
\expandafter\def\csname rev@rdec@fre@replenish095@tfmplan\endcsname{0.65}
\expandafter\def\csname rev@rdec@fre@replenish095@tft\endcsname{0.64}
\expandafter\def\csname rev@rdec@fre@replenish095@world\endcsname{0.57}
\expandafter\def\csname rev@rdec@mfive@categoryplanning@ens\endcsname{0.64}
\expandafter\def\csname rev@rdec@mfive@categoryplanning@lgb\endcsname{0.65}
\expandafter\def\csname rev@rdec@mfive@categoryplanning@lift\endcsname{1.29}
\expandafter\def\csname rev@rdec@mfive@categoryplanning@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@mfive@categoryplanning@tfmplan\endcsname{0.84}
\expandafter\def\csname rev@rdec@mfive@categoryplanning@world\endcsname{0.63}
\expandafter\def\csname rev@rdec@mfive@replenish05@chronos\endcsname{0.78}
\expandafter\def\csname rev@rdec@mfive@replenish05@ens\endcsname{0.76}
\expandafter\def\csname rev@rdec@mfive@replenish05@lgb\endcsname{0.79}
\expandafter\def\csname rev@rdec@mfive@replenish05@lift\endcsname{0.89}
\expandafter\def\csname rev@rdec@mfive@replenish05@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@mfive@replenish05@tfm\endcsname{0.77}
\expandafter\def\csname rev@rdec@mfive@replenish05@tfmplan\endcsname{0.77}
\expandafter\def\csname rev@rdec@mfive@replenish05@world\endcsname{0.78}
\expandafter\def\csname rev@rdec@mfive@replenish08@chronos\endcsname{0.84}
\expandafter\def\csname rev@rdec@mfive@replenish08@ens\endcsname{0.82}
\expandafter\def\csname rev@rdec@mfive@replenish08@lgb\endcsname{0.85}
\expandafter\def\csname rev@rdec@mfive@replenish08@lift\endcsname{0.88}
\expandafter\def\csname rev@rdec@mfive@replenish08@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@mfive@replenish08@tfm\endcsname{0.83}
\expandafter\def\csname rev@rdec@mfive@replenish08@tfmplan\endcsname{0.83}
\expandafter\def\csname rev@rdec@mfive@replenish08@world\endcsname{0.83}
\expandafter\def\csname rev@rdec@mfive@replenish095@chronos\endcsname{0.92}
\expandafter\def\csname rev@rdec@mfive@replenish095@ens\endcsname{0.90}
\expandafter\def\csname rev@rdec@mfive@replenish095@lgb\endcsname{0.92}
\expandafter\def\csname rev@rdec@mfive@replenish095@lift\endcsname{0.93}
\expandafter\def\csname rev@rdec@mfive@replenish095@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@mfive@replenish095@tfm\endcsname{0.91}
\expandafter\def\csname rev@rdec@mfive@replenish095@tfmplan\endcsname{0.91}
\expandafter\def\csname rev@rdec@mfive@replenish095@world\endcsname{0.90}
\expandafter\def\csname rev@rdec@sdr@categoryplanning@ens\endcsname{0.72}
\expandafter\def\csname rev@rdec@sdr@categoryplanning@lgb\endcsname{0.74}
\expandafter\def\csname rev@rdec@sdr@categoryplanning@lift\endcsname{0.93}
\expandafter\def\csname rev@rdec@sdr@categoryplanning@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@sdr@categoryplanning@tfmplan\endcsname{0.87}
\expandafter\def\csname rev@rdec@sdr@categoryplanning@world\endcsname{0.78}
\expandafter\def\csname rev@rdec@sdr@replenish05@chronos\endcsname{0.80}
\expandafter\def\csname rev@rdec@sdr@replenish05@ens\endcsname{0.58}
\expandafter\def\csname rev@rdec@sdr@replenish05@lgb\endcsname{0.56}
\expandafter\def\csname rev@rdec@sdr@replenish05@lift\endcsname{0.69}
\expandafter\def\csname rev@rdec@sdr@replenish05@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@sdr@replenish05@tfm\endcsname{0.80}
\expandafter\def\csname rev@rdec@sdr@replenish05@tfmplan\endcsname{0.70}
\expandafter\def\csname rev@rdec@sdr@replenish05@tft\endcsname{0.67}
\expandafter\def\csname rev@rdec@sdr@replenish05@world\endcsname{0.62}
\expandafter\def\csname rev@rdec@sdr@replenish08@chronos\endcsname{0.91}
\expandafter\def\csname rev@rdec@sdr@replenish08@ens\endcsname{0.59}
\expandafter\def\csname rev@rdec@sdr@replenish08@lgb\endcsname{0.57}
\expandafter\def\csname rev@rdec@sdr@replenish08@lift\endcsname{0.64}
\expandafter\def\csname rev@rdec@sdr@replenish08@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@sdr@replenish08@tfm\endcsname{0.89}
\expandafter\def\csname rev@rdec@sdr@replenish08@tfmplan\endcsname{0.69}
\expandafter\def\csname rev@rdec@sdr@replenish08@tft\endcsname{0.70}
\expandafter\def\csname rev@rdec@sdr@replenish08@world\endcsname{0.61}
\expandafter\def\csname rev@rdec@sdr@replenish095@chronos\endcsname{0.93}
\expandafter\def\csname rev@rdec@sdr@replenish095@ens\endcsname{0.69}
\expandafter\def\csname rev@rdec@sdr@replenish095@lgb\endcsname{0.66}
\expandafter\def\csname rev@rdec@sdr@replenish095@lift\endcsname{0.71}
\expandafter\def\csname rev@rdec@sdr@replenish095@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@sdr@replenish095@tfm\endcsname{0.93}
\expandafter\def\csname rev@rdec@sdr@replenish095@tfmplan\endcsname{0.79}
\expandafter\def\csname rev@rdec@sdr@replenish095@tft\endcsname{0.81}
\expandafter\def\csname rev@rdec@sdr@replenish095@world\endcsname{0.70}
\expandafter\def\csname rev@rdec@sna@categoryplanning@ens\endcsname{0.60}
\expandafter\def\csname rev@rdec@sna@categoryplanning@lgb\endcsname{0.52}
\expandafter\def\csname rev@rdec@sna@categoryplanning@lift\endcsname{0.76}
\expandafter\def\csname rev@rdec@sna@categoryplanning@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@sna@categoryplanning@tfmplan\endcsname{0.62}
\expandafter\def\csname rev@rdec@sna@categoryplanning@world\endcsname{0.78}
\expandafter\def\csname rev@rdec@sna@replenish05@chronos\endcsname{2.03}
\expandafter\def\csname rev@rdec@sna@replenish05@ens\endcsname{0.71}
\expandafter\def\csname rev@rdec@sna@replenish05@lgb\endcsname{0.65}
\expandafter\def\csname rev@rdec@sna@replenish05@lift\endcsname{0.83}
\expandafter\def\csname rev@rdec@sna@replenish05@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@sna@replenish05@tfm\endcsname{0.92}
\expandafter\def\csname rev@rdec@sna@replenish05@tfmplan\endcsname{0.77}
\expandafter\def\csname rev@rdec@sna@replenish05@tft\endcsname{0.76}
\expandafter\def\csname rev@rdec@sna@replenish05@world\endcsname{0.83}
\expandafter\def\csname rev@rdec@sna@replenish08@chronos\endcsname{1.28}
\expandafter\def\csname rev@rdec@sna@replenish08@ens\endcsname{0.72}
\expandafter\def\csname rev@rdec@sna@replenish08@lgb\endcsname{0.71}
\expandafter\def\csname rev@rdec@sna@replenish08@lift\endcsname{0.77}
\expandafter\def\csname rev@rdec@sna@replenish08@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@sna@replenish08@tfm\endcsname{0.85}
\expandafter\def\csname rev@rdec@sna@replenish08@tfmplan\endcsname{0.76}
\expandafter\def\csname rev@rdec@sna@replenish08@tft\endcsname{0.76}
\expandafter\def\csname rev@rdec@sna@replenish08@world\endcsname{0.77}
\expandafter\def\csname rev@rdec@sna@replenish095@chronos\endcsname{1.00}
\expandafter\def\csname rev@rdec@sna@replenish095@ens\endcsname{0.76}
\expandafter\def\csname rev@rdec@sna@replenish095@lgb\endcsname{0.76}
\expandafter\def\csname rev@rdec@sna@replenish095@lift\endcsname{0.78}
\expandafter\def\csname rev@rdec@sna@replenish095@naive\endcsname{1.00}
\expandafter\def\csname rev@rdec@sna@replenish095@tfm\endcsname{0.88}
\expandafter\def\csname rev@rdec@sna@replenish095@tfmplan\endcsname{0.79}
\expandafter\def\csname rev@rdec@sna@replenish095@tft\endcsname{0.79}
\expandafter\def\csname rev@rdec@sna@replenish095@world\endcsname{0.77}
\expandafter\def\csname rev@rf@ana@chronos@all\endcsname{1.068}
\expandafter\def\csname rev@rf@ana@chronos@ixs\endcsname{0.802}
\expandafter\def\csname rev@rf@ana@chronos@total\endcsname{1.454}
\expandafter\def\csname rev@rf@ana@ens@all\endcsname{0.908}
\expandafter\def\csname rev@rf@ana@ens@ixs\endcsname{0.710}
\expandafter\def\csname rev@rf@ana@ens@total\endcsname{1.236}
\expandafter\def\csname rev@rf@ana@lgb@all\endcsname{0.987}
\expandafter\def\csname rev@rf@ana@lgb@ixs\endcsname{0.716}
\expandafter\def\csname rev@rf@ana@lgb@total\endcsname{1.407}
\expandafter\def\csname rev@rf@ana@lift@all\endcsname{0.956}
\expandafter\def\csname rev@rf@ana@lift@ixs\endcsname{0.714}
\expandafter\def\csname rev@rf@ana@lift@total\endcsname{1.280}
\expandafter\def\csname rev@rf@ana@tfm@all\endcsname{1.008}
\expandafter\def\csname rev@rf@ana@tfm@ixs\endcsname{0.790}
\expandafter\def\csname rev@rf@ana@tfm@total\endcsname{1.337}
\expandafter\def\csname rev@rf@ana@tfmplan@all\endcsname{0.889}
\expandafter\def\csname rev@rf@ana@tfmplan@ixs\endcsname{0.742}
\expandafter\def\csname rev@rf@ana@tfmplan@total\endcsname{1.149}
\expandafter\def\csname rev@rf@ana@tft@all\endcsname{0.806}
\expandafter\def\csname rev@rf@ana@tft@ixs\endcsname{0.770}
\expandafter\def\csname rev@rf@ana@tft@total\endcsname{0.878}
\expandafter\def\csname rev@rf@ana@world@all\endcsname{0.894}
\expandafter\def\csname rev@rf@ana@world@ixs\endcsname{0.712}
\expandafter\def\csname rev@rf@ana@world@total\endcsname{1.186}
\expandafter\def\csname rev@rf@bjc@chronos@all\endcsname{0.930}
\expandafter\def\csname rev@rf@bjc@chronos@ixs\endcsname{0.785}
\expandafter\def\csname rev@rf@bjc@chronos@total\endcsname{1.046}
\expandafter\def\csname rev@rf@bjc@ens@all\endcsname{0.958}
\expandafter\def\csname rev@rf@bjc@ens@ixs\endcsname{0.760}
\expandafter\def\csname rev@rf@bjc@ens@total\endcsname{1.111}
\expandafter\def\csname rev@rf@bjc@lgb@all\endcsname{0.989}
\expandafter\def\csname rev@rf@bjc@lgb@ixs\endcsname{0.756}
\expandafter\def\csname rev@rf@bjc@lgb@total\endcsname{1.171}
\expandafter\def\csname rev@rf@bjc@lift@all\endcsname{1.035}
\expandafter\def\csname rev@rf@bjc@lift@ixs\endcsname{0.807}
\expandafter\def\csname rev@rf@bjc@lift@total\endcsname{1.190}
\expandafter\def\csname rev@rf@bjc@tfm@all\endcsname{0.939}
\expandafter\def\csname rev@rf@bjc@tfm@ixs\endcsname{0.782}
\expandafter\def\csname rev@rf@bjc@tfm@total\endcsname{1.065}
\expandafter\def\csname rev@rf@bjc@tfmplan@all\endcsname{0.990}
\expandafter\def\csname rev@rf@bjc@tfmplan@ixs\endcsname{0.754}
\expandafter\def\csname rev@rf@bjc@tfmplan@total\endcsname{1.172}
\expandafter\def\csname rev@rf@bjc@tft@all\endcsname{0.906}
\expandafter\def\csname rev@rf@bjc@tft@ixs\endcsname{0.775}
\expandafter\def\csname rev@rf@bjc@tft@total\endcsname{1.015}
\expandafter\def\csname rev@rf@bjc@world@all\endcsname{0.943}
\expandafter\def\csname rev@rf@bjc@world@ixs\endcsname{0.849}
\expandafter\def\csname rev@rf@bjc@world@total\endcsname{1.019}
\expandafter\def\csname rev@rf@che@chronos@all\endcsname{0.877}
\expandafter\def\csname rev@rf@che@chronos@ixs\endcsname{0.807}
\expandafter\def\csname rev@rf@che@chronos@total\endcsname{1.009}
\expandafter\def\csname rev@rf@che@ens@all\endcsname{0.677}
\expandafter\def\csname rev@rf@che@ens@ixs\endcsname{0.675}
\expandafter\def\csname rev@rf@che@ens@total\endcsname{0.753}
\expandafter\def\csname rev@rf@che@lgb@all\endcsname{0.699}
\expandafter\def\csname rev@rf@che@lgb@ixs\endcsname{0.699}
\expandafter\def\csname rev@rf@che@lgb@total\endcsname{0.768}
\expandafter\def\csname rev@rf@che@lift@all\endcsname{0.877}
\expandafter\def\csname rev@rf@che@lift@ixs\endcsname{0.756}
\expandafter\def\csname rev@rf@che@lift@total\endcsname{0.997}
\expandafter\def\csname rev@rf@che@tfm@all\endcsname{0.829}
\expandafter\def\csname rev@rf@che@tfm@ixs\endcsname{0.792}
\expandafter\def\csname rev@rf@che@tfm@total\endcsname{0.933}
\expandafter\def\csname rev@rf@che@tfmplan@all\endcsname{0.564}
\expandafter\def\csname rev@rf@che@tfmplan@ixs\endcsname{0.704}
\expandafter\def\csname rev@rf@che@tfmplan@total\endcsname{0.531}
\expandafter\def\csname rev@rf@che@tft@all\endcsname{0.583}
\expandafter\def\csname rev@rf@che@tft@ixs\endcsname{0.731}
\expandafter\def\csname rev@rf@che@tft@total\endcsname{0.522}
\expandafter\def\csname rev@rf@che@world@all\endcsname{0.883}
\expandafter\def\csname rev@rf@che@world@ixs\endcsname{0.712}
\expandafter\def\csname rev@rf@che@world@total\endcsname{1.064}
\expandafter\def\csname rev@rf@frat@chronos@all\endcsname{1.024}
\expandafter\def\csname rev@rf@frat@chronos@ixs\endcsname{0.856}
\expandafter\def\csname rev@rf@frat@chronos@total\endcsname{1.222}
\expandafter\def\csname rev@rf@frat@ens@all\endcsname{0.591}
\expandafter\def\csname rev@rf@frat@ens@ixs\endcsname{0.604}
\expandafter\def\csname rev@rf@frat@ens@total\endcsname{0.586}
\expandafter\def\csname rev@rf@frat@lgb@all\endcsname{0.561}
\expandafter\def\csname rev@rf@frat@lgb@ixs\endcsname{0.613}
\expandafter\def\csname rev@rf@frat@lgb@total\endcsname{0.523}
\expandafter\def\csname rev@rf@frat@lift@all\endcsname{0.679}
\expandafter\def\csname rev@rf@frat@lift@ixs\endcsname{0.662}
\expandafter\def\csname rev@rf@frat@lift@total\endcsname{0.698}
\expandafter\def\csname rev@rf@frat@tfm@all\endcsname{0.965}
\expandafter\def\csname rev@rf@frat@tfm@ixs\endcsname{0.827}
\expandafter\def\csname rev@rf@frat@tfm@total\endcsname{1.137}
\expandafter\def\csname rev@rf@frat@tfmplan@all\endcsname{0.681}
\expandafter\def\csname rev@rf@frat@tfmplan@ixs\endcsname{0.644}
\expandafter\def\csname rev@rf@frat@tfmplan@total\endcsname{0.677}
\expandafter\def\csname rev@rf@frat@tft@all\endcsname{0.782}
\expandafter\def\csname rev@rf@frat@tft@ixs\endcsname{0.702}
\expandafter\def\csname rev@rf@frat@tft@total\endcsname{0.818}
\expandafter\def\csname rev@rf@frat@world@all\endcsname{0.684}
\expandafter\def\csname rev@rf@frat@world@ixs\endcsname{0.671}
\expandafter\def\csname rev@rf@frat@world@total\endcsname{0.681}
\expandafter\def\csname rev@rf@fre@chronos@all\endcsname{0.609}
\expandafter\def\csname rev@rf@fre@chronos@ixs\endcsname{0.692}
\expandafter\def\csname rev@rf@fre@chronos@total\endcsname{0.536}
\expandafter\def\csname rev@rf@fre@ens@all\endcsname{0.490}
\expandafter\def\csname rev@rf@fre@ens@ixs\endcsname{0.543}
\expandafter\def\csname rev@rf@fre@ens@total\endcsname{0.454}
\expandafter\def\csname rev@rf@fre@lgb@all\endcsname{0.475}
\expandafter\def\csname rev@rf@fre@lgb@ixs\endcsname{0.530}
\expandafter\def\csname rev@rf@fre@lgb@total\endcsname{0.438}
\expandafter\def\csname rev@rf@fre@lift@all\endcsname{0.469}
\expandafter\def\csname rev@rf@fre@lift@ixs\endcsname{0.563}
\expandafter\def\csname rev@rf@fre@lift@total\endcsname{0.404}
\expandafter\def\csname rev@rf@fre@tfm@all\endcsname{0.563}
\expandafter\def\csname rev@rf@fre@tfm@ixs\endcsname{0.682}
\expandafter\def\csname rev@rf@fre@tfm@total\endcsname{0.465}
\expandafter\def\csname rev@rf@fre@tfmplan@all\endcsname{0.566}
\expandafter\def\csname rev@rf@fre@tfmplan@ixs\endcsname{0.599}
\expandafter\def\csname rev@rf@fre@tfmplan@total\endcsname{0.537}
\expandafter\def\csname rev@rf@fre@tft@all\endcsname{0.474}
\expandafter\def\csname rev@rf@fre@tft@ixs\endcsname{0.557}
\expandafter\def\csname rev@rf@fre@tft@total\endcsname{0.414}
\expandafter\def\csname rev@rf@fre@world@all\endcsname{0.487}
\expandafter\def\csname rev@rf@fre@world@ixs\endcsname{0.574}
\expandafter\def\csname rev@rf@fre@world@total\endcsname{0.423}
\expandafter\def\csname rev@rf@mfive@chronos@all\endcsname{1.012}
\expandafter\def\csname rev@rf@mfive@chronos@ixs\endcsname{0.899}
\expandafter\def\csname rev@rf@mfive@chronos@total\endcsname{1.007}
\expandafter\def\csname rev@rf@mfive@ens@all\endcsname{0.544}
\expandafter\def\csname rev@rf@mfive@ens@ixs\endcsname{0.881}
\expandafter\def\csname rev@rf@mfive@ens@total\endcsname{0.240}
\expandafter\def\csname rev@rf@mfive@graph@all\endcsname{0.669}
\expandafter\def\csname rev@rf@mfive@graph@ixs\endcsname{0.907}
\expandafter\def\csname rev@rf@mfive@graph@total\endcsname{0.404}
\expandafter\def\csname rev@rf@mfive@lgb@all\endcsname{0.548}
\expandafter\def\csname rev@rf@mfive@lgb@ixs\endcsname{0.905}
\expandafter\def\csname rev@rf@mfive@lgb@total\endcsname{0.245}
\expandafter\def\csname rev@rf@mfive@lift@all\endcsname{0.719}
\expandafter\def\csname rev@rf@mfive@lift@ixs\endcsname{0.896}
\expandafter\def\csname rev@rf@mfive@lift@total\endcsname{0.424}
\expandafter\def\csname rev@rf@mfive@tfm@all\endcsname{0.729}
\expandafter\def\csname rev@rf@mfive@tfm@ixs\endcsname{0.885}
\expandafter\def\csname rev@rf@mfive@tfm@total\endcsname{0.558}
\expandafter\def\csname rev@rf@mfive@tfmplan@all\endcsname{0.719}
\expandafter\def\csname rev@rf@mfive@tfmplan@ixs\endcsname{0.883}
\expandafter\def\csname rev@rf@mfive@tfmplan@total\endcsname{0.556}
\expandafter\def\csname rev@rf@mfive@world@all\endcsname{0.627}
\expandafter\def\csname rev@rf@mfive@world@ixs\endcsname{0.896}
\expandafter\def\csname rev@rf@mfive@world@total\endcsname{0.363}
\expandafter\def\csname rev@rf@sdr@chronos@all\endcsname{1.161}
\expandafter\def\csname rev@rf@sdr@chronos@ixs\endcsname{0.912}
\expandafter\def\csname rev@rf@sdr@chronos@total\endcsname{1.385}
\expandafter\def\csname rev@rf@sdr@ens@all\endcsname{0.890}
\expandafter\def\csname rev@rf@sdr@ens@ixs\endcsname{0.674}
\expandafter\def\csname rev@rf@sdr@ens@total\endcsname{1.065}
\expandafter\def\csname rev@rf@sdr@lgb@all\endcsname{0.982}
\expandafter\def\csname rev@rf@sdr@lgb@ixs\endcsname{0.655}
\expandafter\def\csname rev@rf@sdr@lgb@total\endcsname{1.238}
\expandafter\def\csname rev@rf@sdr@lift@all\endcsname{0.850}
\expandafter\def\csname rev@rf@sdr@lift@ixs\endcsname{0.772}
\expandafter\def\csname rev@rf@sdr@lift@total\endcsname{0.920}
\expandafter\def\csname rev@rf@sdr@tfm@all\endcsname{1.070}
\expandafter\def\csname rev@rf@sdr@tfm@ixs\endcsname{0.895}
\expandafter\def\csname rev@rf@sdr@tfm@total\endcsname{1.241}
\expandafter\def\csname rev@rf@sdr@tfmplan@all\endcsname{0.974}
\expandafter\def\csname rev@rf@sdr@tfmplan@ixs\endcsname{0.780}
\expandafter\def\csname rev@rf@sdr@tfmplan@total\endcsname{1.140}
\expandafter\def\csname rev@rf@sdr@tft@all\endcsname{1.044}
\expandafter\def\csname rev@rf@sdr@tft@ixs\endcsname{0.849}
\expandafter\def\csname rev@rf@sdr@tft@total\endcsname{1.228}
\expandafter\def\csname rev@rf@sdr@world@all\endcsname{0.805}
\expandafter\def\csname rev@rf@sdr@world@ixs\endcsname{0.709}
\expandafter\def\csname rev@rf@sdr@world@total\endcsname{0.891}
\expandafter\def\csname rev@rf@sna@chronos@all\endcsname{0.460}
\expandafter\def\csname rev@rf@sna@chronos@ixs\endcsname{0.661}
\expandafter\def\csname rev@rf@sna@chronos@total\endcsname{0.327}
\expandafter\def\csname rev@rf@sna@ens@all\endcsname{0.430}
\expandafter\def\csname rev@rf@sna@ens@ixs\endcsname{0.585}
\expandafter\def\csname rev@rf@sna@ens@total\endcsname{0.334}
\expandafter\def\csname rev@rf@sna@lgb@all\endcsname{0.419}
\expandafter\def\csname rev@rf@sna@lgb@ixs\endcsname{0.603}
\expandafter\def\csname rev@rf@sna@lgb@total\endcsname{0.317}
\expandafter\def\csname rev@rf@sna@lift@all\endcsname{0.436}
\expandafter\def\csname rev@rf@sna@lift@ixs\endcsname{0.620}
\expandafter\def\csname rev@rf@sna@lift@total\endcsname{0.302}
\expandafter\def\csname rev@rf@sna@tfm@all\endcsname{0.468}
\expandafter\def\csname rev@rf@sna@tfm@ixs\endcsname{0.640}
\expandafter\def\csname rev@rf@sna@tfm@total\endcsname{0.365}
\expandafter\def\csname rev@rf@sna@tfmplan@all\endcsname{0.477}
\expandafter\def\csname rev@rf@sna@tfmplan@ixs\endcsname{0.624}
\expandafter\def\csname rev@rf@sna@tfmplan@total\endcsname{0.362}
\expandafter\def\csname rev@rf@sna@tft@all\endcsname{0.389}
\expandafter\def\csname rev@rf@sna@tft@ixs\endcsname{0.621}
\expandafter\def\csname rev@rf@sna@tft@total\endcsname{0.219}
\expandafter\def\csname rev@rf@sna@world@all\endcsname{0.531}
\expandafter\def\csname rev@rf@sna@world@ixs\endcsname{0.610}
\expandafter\def\csname rev@rf@sna@world@total\endcsname{0.484}
\expandafter\def\csname rev@rgrain@cat@ens@best\endcsname{five}
\expandafter\def\csname rev@rgrain@cat@ens@bestlist\endcsname{cheese, bottled juice, analgesics, Frat and Favorita}
\expandafter\def\csname rev@rgrain@cat@ens@inset\endcsname{nine}
\expandafter\def\csname rev@rgrain@cat@lgb@best\endcsname{two}
\expandafter\def\csname rev@rgrain@cat@lgb@bestlist\endcsname{soft drinks and frozen entrees}
\expandafter\def\csname rev@rgrain@cat@lgb@inset\endcsname{nine}
\expandafter\def\csname rev@rgrain@cat@lift@best\endcsname{one}
\expandafter\def\csname rev@rgrain@cat@lift@bestlist\endcsname{snack crackers}
\expandafter\def\csname rev@rgrain@cat@lift@inset\endcsname{eight}
\expandafter\def\csname rev@rgrain@cat@set@max\endcsname{9}
\expandafter\def\csname rev@rgrain@cat@set@median\endcsname{4}
\expandafter\def\csname rev@rgrain@cat@set@min\endcsname{2}
\expandafter\def\csname rev@rgrain@cat@tfmplan@best\endcsname{none}
\expandafter\def\csname rev@rgrain@cat@tfmplan@bestlist\endcsname{none}
\expandafter\def\csname rev@rgrain@cat@tfmplan@inset\endcsname{four}
\expandafter\def\csname rev@rgrain@cat@world@best\endcsname{one}
\expandafter\def\csname rev@rgrain@cat@world@bestlist\endcsname{M5}
\expandafter\def\csname rev@rgrain@cat@world@inset\endcsname{seven}
\expandafter\def\csname rev@rgrain@catstore@ens@best\endcsname{five}
\expandafter\def\csname rev@rgrain@catstore@ens@bestlist\endcsname{soft drinks, bottled juice, analgesics, Frat and Favorita}
\expandafter\def\csname rev@rgrain@catstore@ens@inset\endcsname{nine}
\expandafter\def\csname rev@rgrain@catstore@lgb@best\endcsname{four}
\expandafter\def\csname rev@rgrain@catstore@lgb@bestlist\endcsname{cheese, snack crackers, frozen entrees and M5}
\expandafter\def\csname rev@rgrain@catstore@lgb@inset\endcsname{nine}
\expandafter\def\csname rev@rgrain@catstore@lift@best\endcsname{none}
\expandafter\def\csname rev@rgrain@catstore@lift@bestlist\endcsname{none}
\expandafter\def\csname rev@rgrain@catstore@lift@inset\endcsname{five}
\expandafter\def\csname rev@rgrain@catstore@set@max\endcsname{9}
\expandafter\def\csname rev@rgrain@catstore@set@median\endcsname{4}
\expandafter\def\csname rev@rgrain@catstore@set@min\endcsname{2}
\expandafter\def\csname rev@rgrain@catstore@tfmplan@best\endcsname{none}
\expandafter\def\csname rev@rgrain@catstore@tfmplan@bestlist\endcsname{none}
\expandafter\def\csname rev@rgrain@catstore@tfmplan@inset\endcsname{three}
\expandafter\def\csname rev@rgrain@catstore@world@best\endcsname{none}
\expandafter\def\csname rev@rgrain@catstore@world@bestlist\endcsname{none}
\expandafter\def\csname rev@rgrain@catstore@world@inset\endcsname{five}
\expandafter\def\csname rev@rgrain@item@ens@best\endcsname{eight}
\expandafter\def\csname rev@rgrain@item@ens@bestlist\endcsname{cheese, snack crackers, bottled juice, analgesics, frozen entrees, Frat, M5 and Favorita}
\expandafter\def\csname rev@rgrain@item@ens@inset\endcsname{nine}
\expandafter\def\csname rev@rgrain@item@lgb@best\endcsname{one}
\expandafter\def\csname rev@rgrain@item@lgb@bestlist\endcsname{soft drinks}
\expandafter\def\csname rev@rgrain@item@lgb@inset\endcsname{six}
\expandafter\def\csname rev@rgrain@item@lift@best\endcsname{none}
\expandafter\def\csname rev@rgrain@item@lift@bestlist\endcsname{none}
\expandafter\def\csname rev@rgrain@item@lift@inset\endcsname{none}
\expandafter\def\csname rev@rgrain@item@set@max\endcsname{3}
\expandafter\def\csname rev@rgrain@item@set@median\endcsname{2}
\expandafter\def\csname rev@rgrain@item@set@min\endcsname{1}
\expandafter\def\csname rev@rgrain@item@tfmplan@best\endcsname{none}
\expandafter\def\csname rev@rgrain@item@tfmplan@bestlist\endcsname{none}
\expandafter\def\csname rev@rgrain@item@tfmplan@inset\endcsname{one}
\expandafter\def\csname rev@rgrain@item@world@best\endcsname{none}
\expandafter\def\csname rev@rgrain@item@world@bestlist\endcsname{none}
\expandafter\def\csname rev@rgrain@item@world@inset\endcsname{one}
\expandafter\def\csname rev@rgrain@ixs@ens@best\endcsname{seven}
\expandafter\def\csname rev@rgrain@ixs@ens@bestlist\endcsname{snack crackers, soft drinks, bottled juice, frozen entrees, Frat, M5 and Favorita}
\expandafter\def\csname rev@rgrain@ixs@ens@inset\endcsname{eight}
\expandafter\def\csname rev@rgrain@ixs@lgb@best\endcsname{two}
\expandafter\def\csname rev@rgrain@ixs@lgb@bestlist\endcsname{cheese and analgesics}
\expandafter\def\csname rev@rgrain@ixs@lgb@inset\endcsname{four}
\expandafter\def\csname rev@rgrain@ixs@lift@best\endcsname{none}
\expandafter\def\csname rev@rgrain@ixs@lift@bestlist\endcsname{none}
\expandafter\def\csname rev@rgrain@ixs@lift@inset\endcsname{none}
\expandafter\def\csname rev@rgrain@ixs@set@max\endcsname{2}
\expandafter\def\csname rev@rgrain@ixs@set@median\endcsname{1}
\expandafter\def\csname rev@rgrain@ixs@set@min\endcsname{1}
\expandafter\def\csname rev@rgrain@ixs@tfmplan@best\endcsname{none}
\expandafter\def\csname rev@rgrain@ixs@tfmplan@bestlist\endcsname{none}
\expandafter\def\csname rev@rgrain@ixs@tfmplan@inset\endcsname{none}
\expandafter\def\csname rev@rgrain@ixs@world@best\endcsname{none}
\expandafter\def\csname rev@rgrain@ixs@world@bestlist\endcsname{none}
\expandafter\def\csname rev@rgrain@ixs@world@inset\endcsname{none}
\expandafter\def\csname rev@rgrain@total@ens@best\endcsname{four}
\expandafter\def\csname rev@rgrain@total@ens@bestlist\endcsname{cheese, bottled juice, analgesics and Favorita}
\expandafter\def\csname rev@rgrain@total@ens@inset\endcsname{nine}
\expandafter\def\csname rev@rgrain@total@lgb@best\endcsname{two}
\expandafter\def\csname rev@rgrain@total@lgb@bestlist\endcsname{soft drinks and frozen entrees}
\expandafter\def\csname rev@rgrain@total@lgb@inset\endcsname{nine}
\expandafter\def\csname rev@rgrain@total@lift@best\endcsname{one}
\expandafter\def\csname rev@rgrain@total@lift@bestlist\endcsname{snack crackers}
\expandafter\def\csname rev@rgrain@total@lift@inset\endcsname{eight}
\expandafter\def\csname rev@rgrain@total@set@max\endcsname{9}
\expandafter\def\csname rev@rgrain@total@set@median\endcsname{4}
\expandafter\def\csname rev@rgrain@total@set@min\endcsname{3}
\expandafter\def\csname rev@rgrain@total@tfmplan@best\endcsname{one}
\expandafter\def\csname rev@rgrain@total@tfmplan@bestlist\endcsname{Frat}
\expandafter\def\csname rev@rgrain@total@tfmplan@inset\endcsname{four}
\expandafter\def\csname rev@rgrain@total@world@best\endcsname{one}
\expandafter\def\csname rev@rgrain@total@world@bestlist\endcsname{M5}
\expandafter\def\csname rev@rgrain@total@world@inset\endcsname{eight}
\expandafter\def\csname rev@rint@ana@chronos@ixs@coverage50\endcsname{0.77}
\expandafter\def\csname rev@rint@ana@chronos@ixs@coverage80\endcsname{0.90}
\expandafter\def\csname rev@rint@ana@chronos@ixs@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@ana@chronos@ixs@spl\endcsname{0.28}
\expandafter\def\csname rev@rint@ana@chronos@native@spl\endcsname{0.33}
\expandafter\def\csname rev@rint@ana@chronos@total@coverage50\endcsname{0.40}
\expandafter\def\csname rev@rint@ana@chronos@total@coverage80\endcsname{0.70}
\expandafter\def\csname rev@rint@ana@chronos@total@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rint@ana@chronos@total@spl\endcsname{0.34}
\expandafter\def\csname rev@rint@ana@ens@ixs@coverage50\endcsname{0.81}
\expandafter\def\csname rev@rint@ana@ens@ixs@coverage80\endcsname{0.91}
\expandafter\def\csname rev@rint@ana@ens@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@ana@ens@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@ana@ens@total@coverage50\endcsname{0.70}
\expandafter\def\csname rev@rint@ana@ens@total@coverage80\endcsname{0.85}
\expandafter\def\csname rev@rint@ana@ens@total@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rint@ana@ens@total@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@ana@lgb@ixs@coverage50\endcsname{0.82}
\expandafter\def\csname rev@rint@ana@lgb@ixs@coverage80\endcsname{0.91}
\expandafter\def\csname rev@rint@ana@lgb@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@ana@lgb@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rint@ana@lgb@total@coverage50\endcsname{0.72}
\expandafter\def\csname rev@rint@ana@lgb@total@coverage80\endcsname{0.88}
\expandafter\def\csname rev@rint@ana@lgb@total@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@ana@lgb@total@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@ana@lift@ixs@coverage50\endcsname{0.81}
\expandafter\def\csname rev@rint@ana@lift@ixs@coverage80\endcsname{0.91}
\expandafter\def\csname rev@rint@ana@lift@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@ana@lift@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@ana@lift@total@coverage50\endcsname{0.55}
\expandafter\def\csname rev@rint@ana@lift@total@coverage80\endcsname{0.80}
\expandafter\def\csname rev@rint@ana@lift@total@coverage95\endcsname{0.85}
\expandafter\def\csname rev@rint@ana@lift@total@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@ana@liftstock@ixs@coverage50\endcsname{0.80}
\expandafter\def\csname rev@rint@ana@liftstock@ixs@coverage80\endcsname{0.91}
\expandafter\def\csname rev@rint@ana@liftstock@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@ana@liftstock@ixs@spl\endcsname{0.26}
\expandafter\def\csname rev@rint@ana@liftstock@total@coverage50\endcsname{0.47}
\expandafter\def\csname rev@rint@ana@liftstock@total@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@ana@liftstock@total@coverage95\endcsname{0.75}
\expandafter\def\csname rev@rint@ana@liftstock@total@spl\endcsname{0.34}
\expandafter\def\csname rev@rint@ana@naive@ixs@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rint@ana@naive@ixs@coverage80\endcsname{0.84}
\expandafter\def\csname rev@rint@ana@naive@ixs@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@ana@naive@ixs@spl\endcsname{0.36}
\expandafter\def\csname rev@rint@ana@naive@total@coverage50\endcsname{0.53}
\expandafter\def\csname rev@rint@ana@naive@total@coverage80\endcsname{0.88}
\expandafter\def\csname rev@rint@ana@naive@total@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@ana@naive@total@spl\endcsname{0.68}
\expandafter\def\csname rev@rint@ana@tfm@ixs@coverage50\endcsname{0.79}
\expandafter\def\csname rev@rint@ana@tfm@ixs@coverage80\endcsname{0.91}
\expandafter\def\csname rev@rint@ana@tfm@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@ana@tfm@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@ana@tfm@total@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rint@ana@tfm@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@ana@tfm@total@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@ana@tfm@total@spl\endcsname{0.31}
\expandafter\def\csname rev@rint@ana@tfmplan@ixs@coverage50\endcsname{0.78}
\expandafter\def\csname rev@rint@ana@tfmplan@ixs@coverage80\endcsname{0.90}
\expandafter\def\csname rev@rint@ana@tfmplan@ixs@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@ana@tfmplan@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@ana@tfmplan@total@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rint@ana@tfmplan@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@ana@tfmplan@total@coverage95\endcsname{0.80}
\expandafter\def\csname rev@rint@ana@tfmplan@total@spl\endcsname{0.29}
\expandafter\def\csname rev@rint@ana@tft@ixs@coverage50\endcsname{0.80}
\expandafter\def\csname rev@rint@ana@tft@ixs@coverage80\endcsname{0.90}
\expandafter\def\csname rev@rint@ana@tft@ixs@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@ana@tft@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@ana@tft@native@spl\endcsname{0.18}
\expandafter\def\csname rev@rint@ana@tft@total@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rint@ana@tft@total@coverage80\endcsname{0.65}
\expandafter\def\csname rev@rint@ana@tft@total@coverage95\endcsname{0.82}
\expandafter\def\csname rev@rint@ana@tft@total@spl\endcsname{0.34}
\expandafter\def\csname rev@rint@ana@world@ixs@coverage50\endcsname{0.81}
\expandafter\def\csname rev@rint@ana@world@ixs@coverage80\endcsname{0.91}
\expandafter\def\csname rev@rint@ana@world@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@ana@world@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@ana@world@total@coverage50\endcsname{0.60}
\expandafter\def\csname rev@rint@ana@world@total@coverage80\endcsname{0.85}
\expandafter\def\csname rev@rint@ana@world@total@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@ana@world@total@spl\endcsname{0.29}
\expandafter\def\csname rev@rint@bjc@chronos@ixs@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rint@bjc@chronos@ixs@coverage80\endcsname{0.71}
\expandafter\def\csname rev@rint@bjc@chronos@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@chronos@ixs@spl\endcsname{0.29}
\expandafter\def\csname rev@rint@bjc@chronos@native@spl\endcsname{0.36}
\expandafter\def\csname rev@rint@bjc@chronos@total@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rint@bjc@chronos@total@coverage80\endcsname{0.65}
\expandafter\def\csname rev@rint@bjc@chronos@total@coverage95\endcsname{0.78}
\expandafter\def\csname rev@rint@bjc@chronos@total@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@bjc@ens@ixs@coverage50\endcsname{0.40}
\expandafter\def\csname rev@rint@bjc@ens@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@bjc@ens@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@ens@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rint@bjc@ens@total@coverage50\endcsname{0.55}
\expandafter\def\csname rev@rint@bjc@ens@total@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rint@bjc@ens@total@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@ens@total@spl\endcsname{0.15}
\expandafter\def\csname rev@rint@bjc@lgb@ixs@coverage50\endcsname{0.41}
\expandafter\def\csname rev@rint@bjc@lgb@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@bjc@lgb@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@lgb@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rint@bjc@lgb@total@coverage50\endcsname{0.62}
\expandafter\def\csname rev@rint@bjc@lgb@total@coverage80\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@lgb@total@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@bjc@lgb@total@spl\endcsname{0.15}
\expandafter\def\csname rev@rint@bjc@lift@ixs@coverage50\endcsname{0.37}
\expandafter\def\csname rev@rint@bjc@lift@ixs@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@bjc@lift@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@lift@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@bjc@lift@total@coverage50\endcsname{0.50}
\expandafter\def\csname rev@rint@bjc@lift@total@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@bjc@lift@total@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rint@bjc@lift@total@spl\endcsname{0.17}
\expandafter\def\csname rev@rint@bjc@liftstock@ixs@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rint@bjc@liftstock@ixs@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@bjc@liftstock@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@liftstock@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@bjc@liftstock@total@coverage50\endcsname{0.50}
\expandafter\def\csname rev@rint@bjc@liftstock@total@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rint@bjc@liftstock@total@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@bjc@liftstock@total@spl\endcsname{0.16}
\expandafter\def\csname rev@rint@bjc@naive@ixs@coverage50\endcsname{0.18}
\expandafter\def\csname rev@rint@bjc@naive@ixs@coverage80\endcsname{0.70}
\expandafter\def\csname rev@rint@bjc@naive@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@naive@ixs@spl\endcsname{0.44}
\expandafter\def\csname rev@rint@bjc@naive@total@coverage50\endcsname{0.60}
\expandafter\def\csname rev@rint@bjc@naive@total@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rint@bjc@naive@total@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rint@bjc@naive@total@spl\endcsname{0.43}
\expandafter\def\csname rev@rint@bjc@tfm@ixs@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rint@bjc@tfm@ixs@coverage80\endcsname{0.71}
\expandafter\def\csname rev@rint@bjc@tfm@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@tfm@ixs@spl\endcsname{0.29}
\expandafter\def\csname rev@rint@bjc@tfm@total@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rint@bjc@tfm@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@bjc@tfm@total@coverage95\endcsname{0.82}
\expandafter\def\csname rev@rint@bjc@tfm@total@spl\endcsname{0.26}
\expandafter\def\csname rev@rint@bjc@tfmplan@ixs@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rint@bjc@tfmplan@ixs@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@bjc@tfmplan@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@tfmplan@ixs@spl\endcsname{0.26}
\expandafter\def\csname rev@rint@bjc@tfmplan@total@coverage50\endcsname{0.42}
\expandafter\def\csname rev@rint@bjc@tfmplan@total@coverage80\endcsname{0.65}
\expandafter\def\csname rev@rint@bjc@tfmplan@total@coverage95\endcsname{0.75}
\expandafter\def\csname rev@rint@bjc@tfmplan@total@spl\endcsname{0.23}
\expandafter\def\csname rev@rint@bjc@tft@ixs@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rint@bjc@tft@ixs@coverage80\endcsname{0.71}
\expandafter\def\csname rev@rint@bjc@tft@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@tft@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@bjc@tft@native@spl\endcsname{0.22}
\expandafter\def\csname rev@rint@bjc@tft@total@coverage50\endcsname{0.47}
\expandafter\def\csname rev@rint@bjc@tft@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@bjc@tft@total@coverage95\endcsname{0.85}
\expandafter\def\csname rev@rint@bjc@tft@total@spl\endcsname{0.22}
\expandafter\def\csname rev@rint@bjc@world@ixs@coverage50\endcsname{0.39}
\expandafter\def\csname rev@rint@bjc@world@ixs@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@bjc@world@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@bjc@world@ixs@spl\endcsname{0.26}
\expandafter\def\csname rev@rint@bjc@world@total@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rint@bjc@world@total@coverage80\endcsname{0.80}
\expandafter\def\csname rev@rint@bjc@world@total@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@bjc@world@total@spl\endcsname{0.20}
\expandafter\def\csname rev@rint@che@chronos@ixs@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rint@che@chronos@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@che@chronos@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@che@chronos@ixs@spl\endcsname{0.30}
\expandafter\def\csname rev@rint@che@chronos@native@spl\endcsname{0.37}
\expandafter\def\csname rev@rint@che@chronos@total@coverage50\endcsname{0.42}
\expandafter\def\csname rev@rint@che@chronos@total@coverage80\endcsname{0.57}
\expandafter\def\csname rev@rint@che@chronos@total@coverage95\endcsname{0.75}
\expandafter\def\csname rev@rint@che@chronos@total@spl\endcsname{0.26}
\expandafter\def\csname rev@rint@che@ens@ixs@coverage50\endcsname{0.34}
\expandafter\def\csname rev@rint@che@ens@ixs@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@che@ens@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@che@ens@ixs@spl\endcsname{0.22}
\expandafter\def\csname rev@rint@che@ens@total@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rint@che@ens@total@coverage80\endcsname{0.68}
\expandafter\def\csname rev@rint@che@ens@total@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rint@che@ens@total@spl\endcsname{0.12}
\expandafter\def\csname rev@rint@che@lgb@ixs@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rint@che@lgb@ixs@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@che@lgb@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@che@lgb@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rint@che@lgb@total@coverage50\endcsname{0.60}
\expandafter\def\csname rev@rint@che@lgb@total@coverage80\endcsname{0.93}
\expandafter\def\csname rev@rint@che@lgb@total@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@che@lgb@total@spl\endcsname{0.16}
\expandafter\def\csname rev@rint@che@lift@ixs@coverage50\endcsname{0.31}
\expandafter\def\csname rev@rint@che@lift@ixs@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@che@lift@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@che@lift@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@che@lift@total@coverage50\endcsname{0.65}
\expandafter\def\csname rev@rint@che@lift@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@che@lift@total@coverage95\endcsname{0.80}
\expandafter\def\csname rev@rint@che@lift@total@spl\endcsname{0.35}
\expandafter\def\csname rev@rint@che@liftstock@ixs@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rint@che@liftstock@ixs@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@che@liftstock@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@che@liftstock@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rint@che@liftstock@total@coverage50\endcsname{0.40}
\expandafter\def\csname rev@rint@che@liftstock@total@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@che@liftstock@total@coverage95\endcsname{0.78}
\expandafter\def\csname rev@rint@che@liftstock@total@spl\endcsname{0.29}
\expandafter\def\csname rev@rint@che@naive@ixs@coverage50\endcsname{0.17}
\expandafter\def\csname rev@rint@che@naive@ixs@coverage80\endcsname{0.71}
\expandafter\def\csname rev@rint@che@naive@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@che@naive@ixs@spl\endcsname{0.43}
\expandafter\def\csname rev@rint@che@naive@total@coverage50\endcsname{0.57}
\expandafter\def\csname rev@rint@che@naive@total@coverage80\endcsname{0.88}
\expandafter\def\csname rev@rint@che@naive@total@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rint@che@naive@total@spl\endcsname{0.40}
\expandafter\def\csname rev@rint@che@tfm@ixs@coverage50\endcsname{0.34}
\expandafter\def\csname rev@rint@che@tfm@ixs@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@che@tfm@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@che@tfm@ixs@spl\endcsname{0.29}
\expandafter\def\csname rev@rint@che@tfm@total@coverage50\endcsname{0.47}
\expandafter\def\csname rev@rint@che@tfm@total@coverage80\endcsname{0.68}
\expandafter\def\csname rev@rint@che@tfm@total@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rint@che@tfm@total@spl\endcsname{0.22}
\expandafter\def\csname rev@rint@che@tfmplan@ixs@coverage50\endcsname{0.32}
\expandafter\def\csname rev@rint@che@tfmplan@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@che@tfmplan@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@che@tfmplan@ixs@spl\endcsname{0.26}
\expandafter\def\csname rev@rint@che@tfmplan@total@coverage50\endcsname{0.70}
\expandafter\def\csname rev@rint@che@tfmplan@total@coverage80\endcsname{0.78}
\expandafter\def\csname rev@rint@che@tfmplan@total@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rint@che@tfmplan@total@spl\endcsname{0.14}
\expandafter\def\csname rev@rint@che@tft@ixs@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rint@che@tft@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@che@tft@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@che@tft@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@che@tft@native@spl\endcsname{0.22}
\expandafter\def\csname rev@rint@che@tft@total@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rint@che@tft@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@che@tft@total@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@che@tft@total@spl\endcsname{0.15}
\expandafter\def\csname rev@rint@che@world@ixs@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rint@che@world@ixs@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@che@world@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@che@world@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@che@world@total@coverage50\endcsname{0.47}
\expandafter\def\csname rev@rint@che@world@total@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@che@world@total@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@che@world@total@spl\endcsname{0.20}
\expandafter\def\csname rev@rint@fav@ens@ixs@coverage50\endcsname{0.48}
\expandafter\def\csname rev@rint@fav@ens@ixs@coverage80\endcsname{0.79}
\expandafter\def\csname rev@rint@fav@ens@ixs@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@fav@ens@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rint@fav@ens@total@coverage50\endcsname{0.54}
\expandafter\def\csname rev@rint@fav@ens@total@coverage80\endcsname{0.83}
\expandafter\def\csname rev@rint@fav@ens@total@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@fav@ens@total@spl\endcsname{0.07}
\expandafter\def\csname rev@rint@fav@lgb@ixs@coverage50\endcsname{0.48}
\expandafter\def\csname rev@rint@fav@lgb@ixs@coverage80\endcsname{0.79}
\expandafter\def\csname rev@rint@fav@lgb@ixs@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@fav@lgb@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rint@fav@lgb@total@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rint@fav@lgb@total@coverage80\endcsname{0.86}
\expandafter\def\csname rev@rint@fav@lgb@total@coverage95\endcsname{1.00}
\expandafter\def\csname rev@rint@fav@lgb@total@spl\endcsname{0.07}
\expandafter\def\csname rev@rint@fav@lift@ixs@coverage50\endcsname{0.48}
\expandafter\def\csname rev@rint@fav@lift@ixs@coverage80\endcsname{0.79}
\expandafter\def\csname rev@rint@fav@lift@ixs@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@fav@lift@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@fav@lift@total@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rint@fav@lift@total@coverage80\endcsname{0.64}
\expandafter\def\csname rev@rint@fav@lift@total@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@fav@lift@total@spl\endcsname{0.11}
\expandafter\def\csname rev@rint@fav@naive@ixs@coverage50\endcsname{0.47}
\expandafter\def\csname rev@rint@fav@naive@ixs@coverage80\endcsname{0.79}
\expandafter\def\csname rev@rint@fav@naive@ixs@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@fav@naive@ixs@spl\endcsname{0.38}
\expandafter\def\csname rev@rint@fav@naive@total@coverage50\endcsname{0.42}
\expandafter\def\csname rev@rint@fav@naive@total@coverage80\endcsname{0.69}
\expandafter\def\csname rev@rint@fav@naive@total@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@fav@naive@total@spl\endcsname{0.13}
\expandafter\def\csname rev@rint@fav@tfmplan@ixs@coverage50\endcsname{0.47}
\expandafter\def\csname rev@rint@fav@tfmplan@ixs@coverage80\endcsname{0.79}
\expandafter\def\csname rev@rint@fav@tfmplan@ixs@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@fav@tfmplan@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rint@fav@tfmplan@total@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rint@fav@tfmplan@total@coverage80\endcsname{0.76}
\expandafter\def\csname rev@rint@fav@tfmplan@total@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rint@fav@tfmplan@total@spl\endcsname{0.09}
\expandafter\def\csname rev@rint@fav@world@ixs@coverage50\endcsname{0.48}
\expandafter\def\csname rev@rint@fav@world@ixs@coverage80\endcsname{0.79}
\expandafter\def\csname rev@rint@fav@world@ixs@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@fav@world@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@fav@world@total@coverage50\endcsname{0.43}
\expandafter\def\csname rev@rint@fav@world@total@coverage80\endcsname{0.70}
\expandafter\def\csname rev@rint@fav@world@total@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@fav@world@total@spl\endcsname{0.10}
\expandafter\def\csname rev@rint@frat@chronos@ixs@coverage50\endcsname{0.61}
\expandafter\def\csname rev@rint@frat@chronos@ixs@coverage80\endcsname{0.85}
\expandafter\def\csname rev@rint@frat@chronos@ixs@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rint@frat@chronos@ixs@spl\endcsname{0.30}
\expandafter\def\csname rev@rint@frat@chronos@native@spl\endcsname{0.38}
\expandafter\def\csname rev@rint@frat@chronos@total@coverage50\endcsname{0.54}
\expandafter\def\csname rev@rint@frat@chronos@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@frat@chronos@total@coverage95\endcsname{0.79}
\expandafter\def\csname rev@rint@frat@chronos@total@spl\endcsname{0.16}
\expandafter\def\csname rev@rint@frat@ens@ixs@coverage50\endcsname{0.64}
\expandafter\def\csname rev@rint@frat@ens@ixs@coverage80\endcsname{0.87}
\expandafter\def\csname rev@rint@frat@ens@ixs@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@frat@ens@ixs@spl\endcsname{0.20}
\expandafter\def\csname rev@rint@frat@ens@total@coverage50\endcsname{0.46}
\expandafter\def\csname rev@rint@frat@ens@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@frat@ens@total@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rint@frat@ens@total@spl\endcsname{0.11}
\expandafter\def\csname rev@rint@frat@lgb@ixs@coverage50\endcsname{0.64}
\expandafter\def\csname rev@rint@frat@lgb@ixs@coverage80\endcsname{0.87}
\expandafter\def\csname rev@rint@frat@lgb@ixs@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@frat@lgb@ixs@spl\endcsname{0.21}
\expandafter\def\csname rev@rint@frat@lgb@total@coverage50\endcsname{0.46}
\expandafter\def\csname rev@rint@frat@lgb@total@coverage80\endcsname{0.62}
\expandafter\def\csname rev@rint@frat@lgb@total@coverage95\endcsname{0.83}
\expandafter\def\csname rev@rint@frat@lgb@total@spl\endcsname{0.14}
\expandafter\def\csname rev@rint@frat@lift@ixs@coverage50\endcsname{0.65}
\expandafter\def\csname rev@rint@frat@lift@ixs@coverage80\endcsname{0.88}
\expandafter\def\csname rev@rint@frat@lift@ixs@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@frat@lift@ixs@spl\endcsname{0.21}
\expandafter\def\csname rev@rint@frat@lift@total@coverage50\endcsname{0.54}
\expandafter\def\csname rev@rint@frat@lift@total@coverage80\endcsname{0.83}
\expandafter\def\csname rev@rint@frat@lift@total@coverage95\endcsname{0.92}
\expandafter\def\csname rev@rint@frat@lift@total@spl\endcsname{0.12}
\expandafter\def\csname rev@rint@frat@naive@ixs@coverage50\endcsname{0.60}
\expandafter\def\csname rev@rint@frat@naive@ixs@coverage80\endcsname{0.85}
\expandafter\def\csname rev@rint@frat@naive@ixs@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rint@frat@naive@ixs@spl\endcsname{0.37}
\expandafter\def\csname rev@rint@frat@naive@total@coverage50\endcsname{0.46}
\expandafter\def\csname rev@rint@frat@naive@total@coverage80\endcsname{0.71}
\expandafter\def\csname rev@rint@frat@naive@total@coverage95\endcsname{0.79}
\expandafter\def\csname rev@rint@frat@naive@total@spl\endcsname{0.33}
\expandafter\def\csname rev@rint@frat@tfm@ixs@coverage50\endcsname{0.61}
\expandafter\def\csname rev@rint@frat@tfm@ixs@coverage80\endcsname{0.85}
\expandafter\def\csname rev@rint@frat@tfm@ixs@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rint@frat@tfm@ixs@spl\endcsname{0.30}
\expandafter\def\csname rev@rint@frat@tfm@total@coverage50\endcsname{0.42}
\expandafter\def\csname rev@rint@frat@tfm@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@frat@tfm@total@coverage95\endcsname{0.83}
\expandafter\def\csname rev@rint@frat@tfm@total@spl\endcsname{0.16}
\expandafter\def\csname rev@rint@frat@tfmplan@ixs@coverage50\endcsname{0.63}
\expandafter\def\csname rev@rint@frat@tfmplan@ixs@coverage80\endcsname{0.87}
\expandafter\def\csname rev@rint@frat@tfmplan@ixs@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@frat@tfmplan@ixs@spl\endcsname{0.22}
\expandafter\def\csname rev@rint@frat@tfmplan@total@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rint@frat@tfmplan@total@coverage80\endcsname{0.83}
\expandafter\def\csname rev@rint@frat@tfmplan@total@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rint@frat@tfmplan@total@spl\endcsname{0.09}
\expandafter\def\csname rev@rint@frat@tft@ixs@coverage50\endcsname{0.63}
\expandafter\def\csname rev@rint@frat@tft@ixs@coverage80\endcsname{0.87}
\expandafter\def\csname rev@rint@frat@tft@ixs@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@frat@tft@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rint@frat@tft@native@spl\endcsname{0.19}
\expandafter\def\csname rev@rint@frat@tft@total@coverage50\endcsname{0.50}
\expandafter\def\csname rev@rint@frat@tft@total@coverage80\endcsname{0.92}
\expandafter\def\csname rev@rint@frat@tft@total@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rint@frat@tft@total@spl\endcsname{0.10}
\expandafter\def\csname rev@rint@frat@world@ixs@coverage50\endcsname{0.64}
\expandafter\def\csname rev@rint@frat@world@ixs@coverage80\endcsname{0.87}
\expandafter\def\csname rev@rint@frat@world@ixs@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@frat@world@ixs@spl\endcsname{0.22}
\expandafter\def\csname rev@rint@frat@world@total@coverage50\endcsname{0.42}
\expandafter\def\csname rev@rint@frat@world@total@coverage80\endcsname{0.83}
\expandafter\def\csname rev@rint@frat@world@total@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rint@frat@world@total@spl\endcsname{0.15}
\expandafter\def\csname rev@rint@fre@chronos@ixs@coverage50\endcsname{0.32}
\expandafter\def\csname rev@rint@fre@chronos@ixs@coverage80\endcsname{0.68}
\expandafter\def\csname rev@rint@fre@chronos@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@fre@chronos@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rint@fre@chronos@native@spl\endcsname{0.31}
\expandafter\def\csname rev@rint@fre@chronos@total@coverage50\endcsname{0.42}
\expandafter\def\csname rev@rint@fre@chronos@total@coverage80\endcsname{0.88}
\expandafter\def\csname rev@rint@fre@chronos@total@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@fre@chronos@total@spl\endcsname{0.15}
\expandafter\def\csname rev@rint@fre@ens@ixs@coverage50\endcsname{0.39}
\expandafter\def\csname rev@rint@fre@ens@ixs@coverage80\endcsname{0.69}
\expandafter\def\csname rev@rint@fre@ens@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@fre@ens@ixs@spl\endcsname{0.18}
\expandafter\def\csname rev@rint@fre@ens@total@coverage50\endcsname{0.57}
\expandafter\def\csname rev@rint@fre@ens@total@coverage80\endcsname{0.90}
\expandafter\def\csname rev@rint@fre@ens@total@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@fre@ens@total@spl\endcsname{0.12}
\expandafter\def\csname rev@rint@fre@lgb@ixs@coverage50\endcsname{0.41}
\expandafter\def\csname rev@rint@fre@lgb@ixs@coverage80\endcsname{0.70}
\expandafter\def\csname rev@rint@fre@lgb@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@fre@lgb@ixs@spl\endcsname{0.17}
\expandafter\def\csname rev@rint@fre@lgb@total@coverage50\endcsname{0.60}
\expandafter\def\csname rev@rint@fre@lgb@total@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rint@fre@lgb@total@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rint@fre@lgb@total@spl\endcsname{0.10}
\expandafter\def\csname rev@rint@fre@lift@ixs@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rint@fre@lift@ixs@coverage80\endcsname{0.67}
\expandafter\def\csname rev@rint@fre@lift@ixs@coverage95\endcsname{0.92}
\expandafter\def\csname rev@rint@fre@lift@ixs@spl\endcsname{0.21}
\expandafter\def\csname rev@rint@fre@lift@total@coverage50\endcsname{0.47}
\expandafter\def\csname rev@rint@fre@lift@total@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@fre@lift@total@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rint@fre@lift@total@spl\endcsname{0.16}
\expandafter\def\csname rev@rint@fre@liftstock@ixs@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rint@fre@liftstock@ixs@coverage80\endcsname{0.68}
\expandafter\def\csname rev@rint@fre@liftstock@ixs@coverage95\endcsname{0.92}
\expandafter\def\csname rev@rint@fre@liftstock@ixs@spl\endcsname{0.20}
\expandafter\def\csname rev@rint@fre@liftstock@total@coverage50\endcsname{0.53}
\expandafter\def\csname rev@rint@fre@liftstock@total@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@fre@liftstock@total@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rint@fre@liftstock@total@spl\endcsname{0.15}
\expandafter\def\csname rev@rint@fre@naive@ixs@coverage50\endcsname{0.26}
\expandafter\def\csname rev@rint@fre@naive@ixs@coverage80\endcsname{0.66}
\expandafter\def\csname rev@rint@fre@naive@ixs@coverage95\endcsname{0.92}
\expandafter\def\csname rev@rint@fre@naive@ixs@spl\endcsname{0.32}
\expandafter\def\csname rev@rint@fre@naive@total@coverage50\endcsname{0.55}
\expandafter\def\csname rev@rint@fre@naive@total@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rint@fre@naive@total@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@fre@naive@total@spl\endcsname{0.23}
\expandafter\def\csname rev@rint@fre@tfm@ixs@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rint@fre@tfm@ixs@coverage80\endcsname{0.68}
\expandafter\def\csname rev@rint@fre@tfm@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@fre@tfm@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rint@fre@tfm@total@coverage50\endcsname{0.53}
\expandafter\def\csname rev@rint@fre@tfm@total@coverage80\endcsname{0.95}
\expandafter\def\csname rev@rint@fre@tfm@total@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@fre@tfm@total@spl\endcsname{0.14}
\expandafter\def\csname rev@rint@fre@tfmplan@ixs@coverage50\endcsname{0.32}
\expandafter\def\csname rev@rint@fre@tfmplan@ixs@coverage80\endcsname{0.66}
\expandafter\def\csname rev@rint@fre@tfmplan@ixs@coverage95\endcsname{0.91}
\expandafter\def\csname rev@rint@fre@tfmplan@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rint@fre@tfmplan@total@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rint@fre@tfmplan@total@coverage80\endcsname{0.88}
\expandafter\def\csname rev@rint@fre@tfmplan@total@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@fre@tfmplan@total@spl\endcsname{0.17}
\expandafter\def\csname rev@rint@fre@tft@ixs@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rint@fre@tft@ixs@coverage80\endcsname{0.67}
\expandafter\def\csname rev@rint@fre@tft@ixs@coverage95\endcsname{0.92}
\expandafter\def\csname rev@rint@fre@tft@ixs@spl\endcsname{0.21}
\expandafter\def\csname rev@rint@fre@tft@native@spl\endcsname{0.16}
\expandafter\def\csname rev@rint@fre@tft@total@coverage50\endcsname{0.65}
\expandafter\def\csname rev@rint@fre@tft@total@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rint@fre@tft@total@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@fre@tft@total@spl\endcsname{0.12}
\expandafter\def\csname rev@rint@fre@world@ixs@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rint@fre@world@ixs@coverage80\endcsname{0.69}
\expandafter\def\csname rev@rint@fre@world@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@fre@world@ixs@spl\endcsname{0.18}
\expandafter\def\csname rev@rint@fre@world@total@coverage50\endcsname{0.65}
\expandafter\def\csname rev@rint@fre@world@total@coverage80\endcsname{0.88}
\expandafter\def\csname rev@rint@fre@world@total@coverage95\endcsname{1.00}
\expandafter\def\csname rev@rint@fre@world@total@spl\endcsname{0.12}
\expandafter\def\csname rev@rint@mfive@chronos@ixs@coverage50\endcsname{0.83}
\expandafter\def\csname rev@rint@mfive@chronos@ixs@coverage80\endcsname{0.94}
\expandafter\def\csname rev@rint@mfive@chronos@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@mfive@chronos@ixs@spl\endcsname{0.33}
\expandafter\def\csname rev@rint@mfive@chronos@native@spl\endcsname{0.42}
\expandafter\def\csname rev@rint@mfive@chronos@total@coverage50\endcsname{0.57}
\expandafter\def\csname rev@rint@mfive@chronos@total@coverage80\endcsname{0.80}
\expandafter\def\csname rev@rint@mfive@chronos@total@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rint@mfive@chronos@total@spl\endcsname{0.30}
\expandafter\def\csname rev@rint@mfive@ens@ixs@coverage50\endcsname{0.85}
\expandafter\def\csname rev@rint@mfive@ens@ixs@coverage80\endcsname{0.94}
\expandafter\def\csname rev@rint@mfive@ens@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@mfive@ens@ixs@spl\endcsname{0.32}
\expandafter\def\csname rev@rint@mfive@ens@total@coverage50\endcsname{0.43}
\expandafter\def\csname rev@rint@mfive@ens@total@coverage80\endcsname{0.71}
\expandafter\def\csname rev@rint@mfive@ens@total@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@mfive@ens@total@spl\endcsname{0.18}
\expandafter\def\csname rev@rint@mfive@lgb@ixs@coverage50\endcsname{0.84}
\expandafter\def\csname rev@rint@mfive@lgb@ixs@coverage80\endcsname{0.94}
\expandafter\def\csname rev@rint@mfive@lgb@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@mfive@lgb@ixs@spl\endcsname{0.33}
\expandafter\def\csname rev@rint@mfive@lgb@total@coverage50\endcsname{0.46}
\expandafter\def\csname rev@rint@mfive@lgb@total@coverage80\endcsname{0.80}
\expandafter\def\csname rev@rint@mfive@lgb@total@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@mfive@lgb@total@spl\endcsname{0.14}
\expandafter\def\csname rev@rint@mfive@lift@ixs@coverage50\endcsname{0.84}
\expandafter\def\csname rev@rint@mfive@lift@ixs@coverage80\endcsname{0.94}
\expandafter\def\csname rev@rint@mfive@lift@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@mfive@lift@ixs@spl\endcsname{0.32}
\expandafter\def\csname rev@rint@mfive@lift@total@coverage50\endcsname{0.43}
\expandafter\def\csname rev@rint@mfive@lift@total@coverage80\endcsname{0.60}
\expandafter\def\csname rev@rint@mfive@lift@total@coverage95\endcsname{0.76}
\expandafter\def\csname rev@rint@mfive@lift@total@spl\endcsname{0.59}
\expandafter\def\csname rev@rint@mfive@naive@ixs@coverage50\endcsname{0.59}
\expandafter\def\csname rev@rint@mfive@naive@ixs@coverage80\endcsname{0.91}
\expandafter\def\csname rev@rint@mfive@naive@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@mfive@naive@ixs@spl\endcsname{0.45}
\expandafter\def\csname rev@rint@mfive@naive@total@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rint@mfive@naive@total@coverage80\endcsname{0.62}
\expandafter\def\csname rev@rint@mfive@naive@total@coverage95\endcsname{0.82}
\expandafter\def\csname rev@rint@mfive@naive@total@spl\endcsname{0.35}
\expandafter\def\csname rev@rint@mfive@tfm@ixs@coverage50\endcsname{0.84}
\expandafter\def\csname rev@rint@mfive@tfm@ixs@coverage80\endcsname{0.94}
\expandafter\def\csname rev@rint@mfive@tfm@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@mfive@tfm@ixs@spl\endcsname{0.32}
\expandafter\def\csname rev@rint@mfive@tfm@total@coverage50\endcsname{0.49}
\expandafter\def\csname rev@rint@mfive@tfm@total@coverage80\endcsname{0.77}
\expandafter\def\csname rev@rint@mfive@tfm@total@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rint@mfive@tfm@total@spl\endcsname{0.26}
\expandafter\def\csname rev@rint@mfive@tfmplan@ixs@coverage50\endcsname{0.84}
\expandafter\def\csname rev@rint@mfive@tfmplan@ixs@coverage80\endcsname{0.94}
\expandafter\def\csname rev@rint@mfive@tfmplan@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@mfive@tfmplan@ixs@spl\endcsname{0.32}
\expandafter\def\csname rev@rint@mfive@tfmplan@total@coverage50\endcsname{0.48}
\expandafter\def\csname rev@rint@mfive@tfmplan@total@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@mfive@tfmplan@total@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rint@mfive@tfmplan@total@spl\endcsname{0.26}
\expandafter\def\csname rev@rint@mfive@world@ixs@coverage50\endcsname{0.84}
\expandafter\def\csname rev@rint@mfive@world@ixs@coverage80\endcsname{0.94}
\expandafter\def\csname rev@rint@mfive@world@ixs@coverage95\endcsname{0.98}
\expandafter\def\csname rev@rint@mfive@world@ixs@spl\endcsname{0.33}
\expandafter\def\csname rev@rint@mfive@world@total@coverage50\endcsname{0.42}
\expandafter\def\csname rev@rint@mfive@world@total@coverage80\endcsname{0.76}
\expandafter\def\csname rev@rint@mfive@world@total@coverage95\endcsname{0.86}
\expandafter\def\csname rev@rint@mfive@world@total@spl\endcsname{0.19}
\expandafter\def\csname rev@rint@sdr@chronos@ixs@coverage50\endcsname{0.43}
\expandafter\def\csname rev@rint@sdr@chronos@ixs@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@sdr@chronos@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sdr@chronos@ixs@spl\endcsname{0.31}
\expandafter\def\csname rev@rint@sdr@chronos@native@spl\endcsname{0.35}
\expandafter\def\csname rev@rint@sdr@chronos@total@coverage50\endcsname{0.25}
\expandafter\def\csname rev@rint@sdr@chronos@total@coverage80\endcsname{0.60}
\expandafter\def\csname rev@rint@sdr@chronos@total@coverage95\endcsname{0.72}
\expandafter\def\csname rev@rint@sdr@chronos@total@spl\endcsname{0.30}
\expandafter\def\csname rev@rint@sdr@ens@ixs@coverage50\endcsname{0.50}
\expandafter\def\csname rev@rint@sdr@ens@ixs@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@sdr@ens@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@sdr@ens@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rint@sdr@ens@total@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rint@sdr@ens@total@coverage80\endcsname{0.68}
\expandafter\def\csname rev@rint@sdr@ens@total@coverage95\endcsname{0.80}
\expandafter\def\csname rev@rint@sdr@ens@total@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@sdr@lgb@ixs@coverage50\endcsname{0.51}
\expandafter\def\csname rev@rint@sdr@lgb@ixs@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@sdr@lgb@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sdr@lgb@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rint@sdr@lgb@total@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rint@sdr@lgb@total@coverage80\endcsname{0.65}
\expandafter\def\csname rev@rint@sdr@lgb@total@coverage95\endcsname{0.85}
\expandafter\def\csname rev@rint@sdr@lgb@total@spl\endcsname{0.26}
\expandafter\def\csname rev@rint@sdr@lift@ixs@coverage50\endcsname{0.48}
\expandafter\def\csname rev@rint@sdr@lift@ixs@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@sdr@lift@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sdr@lift@ixs@spl\endcsname{0.30}
\expandafter\def\csname rev@rint@sdr@lift@total@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rint@sdr@lift@total@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@sdr@lift@total@coverage95\endcsname{0.85}
\expandafter\def\csname rev@rint@sdr@lift@total@spl\endcsname{0.29}
\expandafter\def\csname rev@rint@sdr@liftstock@ixs@coverage50\endcsname{0.49}
\expandafter\def\csname rev@rint@sdr@liftstock@ixs@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@sdr@liftstock@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sdr@liftstock@ixs@spl\endcsname{0.29}
\expandafter\def\csname rev@rint@sdr@liftstock@total@coverage50\endcsname{0.40}
\expandafter\def\csname rev@rint@sdr@liftstock@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@sdr@liftstock@total@coverage95\endcsname{0.82}
\expandafter\def\csname rev@rint@sdr@liftstock@total@spl\endcsname{0.30}
\expandafter\def\csname rev@rint@sdr@naive@ixs@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rint@sdr@naive@ixs@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@sdr@naive@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@sdr@naive@ixs@spl\endcsname{0.40}
\expandafter\def\csname rev@rint@sdr@naive@total@coverage50\endcsname{0.60}
\expandafter\def\csname rev@rint@sdr@naive@total@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rint@sdr@naive@total@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rint@sdr@naive@total@spl\endcsname{0.31}
\expandafter\def\csname rev@rint@sdr@tfm@ixs@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rint@sdr@tfm@ixs@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@sdr@tfm@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sdr@tfm@ixs@spl\endcsname{0.31}
\expandafter\def\csname rev@rint@sdr@tfm@total@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rint@sdr@tfm@total@coverage80\endcsname{0.68}
\expandafter\def\csname rev@rint@sdr@tfm@total@coverage95\endcsname{0.80}
\expandafter\def\csname rev@rint@sdr@tfm@total@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@sdr@tfmplan@ixs@coverage50\endcsname{0.39}
\expandafter\def\csname rev@rint@sdr@tfmplan@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@sdr@tfmplan@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sdr@tfmplan@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@sdr@tfmplan@total@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rint@sdr@tfmplan@total@coverage80\endcsname{0.57}
\expandafter\def\csname rev@rint@sdr@tfmplan@total@coverage95\endcsname{0.78}
\expandafter\def\csname rev@rint@sdr@tfmplan@total@spl\endcsname{0.32}
\expandafter\def\csname rev@rint@sdr@tft@ixs@coverage50\endcsname{0.49}
\expandafter\def\csname rev@rint@sdr@tft@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@sdr@tft@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sdr@tft@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@sdr@tft@native@spl\endcsname{0.21}
\expandafter\def\csname rev@rint@sdr@tft@total@coverage50\endcsname{0.47}
\expandafter\def\csname rev@rint@sdr@tft@total@coverage80\endcsname{0.62}
\expandafter\def\csname rev@rint@sdr@tft@total@coverage95\endcsname{0.70}
\expandafter\def\csname rev@rint@sdr@tft@total@spl\endcsname{0.31}
\expandafter\def\csname rev@rint@sdr@world@ixs@coverage50\endcsname{0.49}
\expandafter\def\csname rev@rint@sdr@world@ixs@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@sdr@world@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@sdr@world@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@sdr@world@total@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rint@sdr@world@total@coverage80\endcsname{0.80}
\expandafter\def\csname rev@rint@sdr@world@total@coverage95\endcsname{0.82}
\expandafter\def\csname rev@rint@sdr@world@total@spl\endcsname{0.28}
\expandafter\def\csname rev@rint@sna@chronos@ixs@coverage50\endcsname{0.41}
\expandafter\def\csname rev@rint@sna@chronos@ixs@coverage80\endcsname{0.72}
\expandafter\def\csname rev@rint@sna@chronos@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sna@chronos@ixs@spl\endcsname{0.29}
\expandafter\def\csname rev@rint@sna@chronos@native@spl\endcsname{0.34}
\expandafter\def\csname rev@rint@sna@chronos@total@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rint@sna@chronos@total@coverage80\endcsname{0.53}
\expandafter\def\csname rev@rint@sna@chronos@total@coverage95\endcsname{0.62}
\expandafter\def\csname rev@rint@sna@chronos@total@spl\endcsname{3.88}
\expandafter\def\csname rev@rint@sna@ens@ixs@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rint@sna@ens@ixs@coverage80\endcsname{0.74}
\expandafter\def\csname rev@rint@sna@ens@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@sna@ens@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rint@sna@ens@total@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rint@sna@ens@total@coverage80\endcsname{0.60}
\expandafter\def\csname rev@rint@sna@ens@total@coverage95\endcsname{0.72}
\expandafter\def\csname rev@rint@sna@ens@total@spl\endcsname{0.53}
\expandafter\def\csname rev@rint@sna@lgb@ixs@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rint@sna@lgb@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@sna@lgb@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sna@lgb@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rint@sna@lgb@total@coverage50\endcsname{0.50}
\expandafter\def\csname rev@rint@sna@lgb@total@coverage80\endcsname{0.75}
\expandafter\def\csname rev@rint@sna@lgb@total@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rint@sna@lgb@total@spl\endcsname{0.42}
\expandafter\def\csname rev@rint@sna@lift@ixs@coverage50\endcsname{0.41}
\expandafter\def\csname rev@rint@sna@lift@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@sna@lift@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sna@lift@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@sna@lift@total@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rint@sna@lift@total@coverage80\endcsname{0.62}
\expandafter\def\csname rev@rint@sna@lift@total@coverage95\endcsname{0.68}
\expandafter\def\csname rev@rint@sna@lift@total@spl\endcsname{0.46}
\expandafter\def\csname rev@rint@sna@liftstock@ixs@coverage50\endcsname{0.41}
\expandafter\def\csname rev@rint@sna@liftstock@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@sna@liftstock@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@sna@liftstock@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@sna@liftstock@total@coverage50\endcsname{0.23}
\expandafter\def\csname rev@rint@sna@liftstock@total@coverage80\endcsname{0.47}
\expandafter\def\csname rev@rint@sna@liftstock@total@coverage95\endcsname{0.60}
\expandafter\def\csname rev@rint@sna@liftstock@total@spl\endcsname{0.85}
\expandafter\def\csname rev@rint@sna@naive@ixs@coverage50\endcsname{0.28}
\expandafter\def\csname rev@rint@sna@naive@ixs@coverage80\endcsname{0.68}
\expandafter\def\csname rev@rint@sna@naive@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rint@sna@naive@ixs@spl\endcsname{0.40}
\expandafter\def\csname rev@rint@sna@naive@total@coverage50\endcsname{0.53}
\expandafter\def\csname rev@rint@sna@naive@total@coverage80\endcsname{0.97}
\expandafter\def\csname rev@rint@sna@naive@total@coverage95\endcsname{0.97}
\expandafter\def\csname rev@rint@sna@naive@total@spl\endcsname{0.68}
\expandafter\def\csname rev@rint@sna@tfm@ixs@coverage50\endcsname{0.41}
\expandafter\def\csname rev@rint@sna@tfm@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@sna@tfm@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sna@tfm@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@sna@tfm@total@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rint@sna@tfm@total@coverage80\endcsname{0.57}
\expandafter\def\csname rev@rint@sna@tfm@total@coverage95\endcsname{0.68}
\expandafter\def\csname rev@rint@sna@tfm@total@spl\endcsname{0.89}
\expandafter\def\csname rev@rint@sna@tfmplan@ixs@coverage50\endcsname{0.40}
\expandafter\def\csname rev@rint@sna@tfmplan@ixs@coverage80\endcsname{0.71}
\expandafter\def\csname rev@rint@sna@tfmplan@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sna@tfmplan@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rint@sna@tfmplan@total@coverage50\endcsname{0.42}
\expandafter\def\csname rev@rint@sna@tfmplan@total@coverage80\endcsname{0.62}
\expandafter\def\csname rev@rint@sna@tfmplan@total@coverage95\endcsname{0.78}
\expandafter\def\csname rev@rint@sna@tfmplan@total@spl\endcsname{0.50}
\expandafter\def\csname rev@rint@sna@tft@ixs@coverage50\endcsname{0.41}
\expandafter\def\csname rev@rint@sna@tft@ixs@coverage80\endcsname{0.71}
\expandafter\def\csname rev@rint@sna@tft@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rint@sna@tft@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rint@sna@tft@native@spl\endcsname{0.22}
\expandafter\def\csname rev@rint@sna@tft@total@coverage50\endcsname{0.28}
\expandafter\def\csname rev@rint@sna@tft@total@coverage80\endcsname{0.55}
\expandafter\def\csname rev@rint@sna@tft@total@coverage95\endcsname{0.68}
\expandafter\def\csname rev@rint@sna@tft@total@spl\endcsname{0.57}
\expandafter\def\csname rev@rint@sna@world@ixs@coverage50\endcsname{0.42}
\expandafter\def\csname rev@rint@sna@world@ixs@coverage80\endcsname{0.73}
\expandafter\def\csname rev@rint@sna@world@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rint@sna@world@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rint@sna@world@total@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rint@sna@world@total@coverage80\endcsname{0.57}
\expandafter\def\csname rev@rint@sna@world@total@coverage95\endcsname{0.60}
\expandafter\def\csname rev@rint@sna@world@total@spl\endcsname{0.80}
\expandafter\def\csname rev@rintold@ana@chronos@ixs@coverage50\endcsname{0.11}
\expandafter\def\csname rev@rintold@ana@chronos@ixs@coverage80\endcsname{0.56}
\expandafter\def\csname rev@rintold@ana@chronos@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@ana@chronos@ixs@spl\endcsname{0.28}
\expandafter\def\csname rev@rintold@ana@chronos@total@coverage50\endcsname{0.23}
\expandafter\def\csname rev@rintold@ana@chronos@total@coverage80\endcsname{0.42}
\expandafter\def\csname rev@rintold@ana@chronos@total@coverage95\endcsname{0.45}
\expandafter\def\csname rev@rintold@ana@chronos@total@spl\endcsname{0.50}
\expandafter\def\csname rev@rintold@ana@ens@ixs@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@ana@ens@ixs@coverage80\endcsname{0.58}
\expandafter\def\csname rev@rintold@ana@ens@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@ana@ens@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@ana@ens@total@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rintold@ana@ens@total@coverage80\endcsname{0.47}
\expandafter\def\csname rev@rintold@ana@ens@total@coverage95\endcsname{0.53}
\expandafter\def\csname rev@rintold@ana@ens@total@spl\endcsname{0.44}
\expandafter\def\csname rev@rintold@ana@lgb@ixs@coverage50\endcsname{0.17}
\expandafter\def\csname rev@rintold@ana@lgb@ixs@coverage80\endcsname{0.59}
\expandafter\def\csname rev@rintold@ana@lgb@ixs@coverage95\endcsname{0.91}
\expandafter\def\csname rev@rintold@ana@lgb@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rintold@ana@lgb@total@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rintold@ana@lgb@total@coverage80\endcsname{0.47}
\expandafter\def\csname rev@rintold@ana@lgb@total@coverage95\endcsname{0.47}
\expandafter\def\csname rev@rintold@ana@lgb@total@spl\endcsname{0.49}
\expandafter\def\csname rev@rintold@ana@lift@ixs@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@ana@lift@ixs@coverage80\endcsname{0.59}
\expandafter\def\csname rev@rintold@ana@lift@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@ana@lift@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@ana@lift@total@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rintold@ana@lift@total@coverage80\endcsname{0.45}
\expandafter\def\csname rev@rintold@ana@lift@total@coverage95\endcsname{0.55}
\expandafter\def\csname rev@rintold@ana@lift@total@spl\endcsname{0.47}
\expandafter\def\csname rev@rintold@ana@naive@ixs@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rintold@ana@naive@ixs@coverage80\endcsname{0.63}
\expandafter\def\csname rev@rintold@ana@naive@ixs@coverage95\endcsname{0.92}
\expandafter\def\csname rev@rintold@ana@naive@ixs@spl\endcsname{0.36}
\expandafter\def\csname rev@rintold@ana@naive@total@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rintold@ana@naive@total@coverage80\endcsname{0.47}
\expandafter\def\csname rev@rintold@ana@naive@total@coverage95\endcsname{0.47}
\expandafter\def\csname rev@rintold@ana@naive@total@spl\endcsname{0.94}
\expandafter\def\csname rev@rintold@ana@tfm@ixs@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@ana@tfm@ixs@coverage80\endcsname{0.57}
\expandafter\def\csname rev@rintold@ana@tfm@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@ana@tfm@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@ana@tfm@total@coverage50\endcsname{0.25}
\expandafter\def\csname rev@rintold@ana@tfm@total@coverage80\endcsname{0.38}
\expandafter\def\csname rev@rintold@ana@tfm@total@coverage95\endcsname{0.45}
\expandafter\def\csname rev@rintold@ana@tfm@total@spl\endcsname{0.49}
\expandafter\def\csname rev@rintold@ana@tfmplan@ixs@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@ana@tfmplan@ixs@coverage80\endcsname{0.56}
\expandafter\def\csname rev@rintold@ana@tfmplan@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@ana@tfmplan@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@ana@tfmplan@total@coverage50\endcsname{0.20}
\expandafter\def\csname rev@rintold@ana@tfmplan@total@coverage80\endcsname{0.40}
\expandafter\def\csname rev@rintold@ana@tfmplan@total@coverage95\endcsname{0.47}
\expandafter\def\csname rev@rintold@ana@tfmplan@total@spl\endcsname{0.47}
\expandafter\def\csname rev@rintold@ana@tft@ixs@coverage50\endcsname{0.14}
\expandafter\def\csname rev@rintold@ana@tft@ixs@coverage80\endcsname{0.57}
\expandafter\def\csname rev@rintold@ana@tft@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@ana@tft@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@ana@tft@total@coverage50\endcsname{0.28}
\expandafter\def\csname rev@rintold@ana@tft@total@coverage80\endcsname{0.38}
\expandafter\def\csname rev@rintold@ana@tft@total@coverage95\endcsname{0.40}
\expandafter\def\csname rev@rintold@ana@tft@total@spl\endcsname{0.52}
\expandafter\def\csname rev@rintold@ana@world@ixs@coverage50\endcsname{0.14}
\expandafter\def\csname rev@rintold@ana@world@ixs@coverage80\endcsname{0.58}
\expandafter\def\csname rev@rintold@ana@world@ixs@coverage95\endcsname{0.91}
\expandafter\def\csname rev@rintold@ana@world@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@ana@world@total@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rintold@ana@world@total@coverage80\endcsname{0.47}
\expandafter\def\csname rev@rintold@ana@world@total@coverage95\endcsname{0.53}
\expandafter\def\csname rev@rintold@ana@world@total@spl\endcsname{0.47}
\expandafter\def\csname rev@rintold@bjc@chronos@ixs@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@bjc@chronos@ixs@coverage80\endcsname{0.55}
\expandafter\def\csname rev@rintold@bjc@chronos@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@bjc@chronos@ixs@spl\endcsname{0.29}
\expandafter\def\csname rev@rintold@bjc@chronos@total@coverage50\endcsname{0.15}
\expandafter\def\csname rev@rintold@bjc@chronos@total@coverage80\endcsname{0.25}
\expandafter\def\csname rev@rintold@bjc@chronos@total@coverage95\endcsname{0.33}
\expandafter\def\csname rev@rintold@bjc@chronos@total@spl\endcsname{0.45}
\expandafter\def\csname rev@rintold@bjc@ens@ixs@coverage50\endcsname{0.11}
\expandafter\def\csname rev@rintold@bjc@ens@ixs@coverage80\endcsname{0.56}
\expandafter\def\csname rev@rintold@bjc@ens@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@bjc@ens@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rintold@bjc@ens@total@coverage50\endcsname{0.28}
\expandafter\def\csname rev@rintold@bjc@ens@total@coverage80\endcsname{0.38}
\expandafter\def\csname rev@rintold@bjc@ens@total@coverage95\endcsname{0.38}
\expandafter\def\csname rev@rintold@bjc@ens@total@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@bjc@lgb@ixs@coverage50\endcsname{0.14}
\expandafter\def\csname rev@rintold@bjc@lgb@ixs@coverage80\endcsname{0.57}
\expandafter\def\csname rev@rintold@bjc@lgb@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@bjc@lgb@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rintold@bjc@lgb@total@coverage50\endcsname{0.28}
\expandafter\def\csname rev@rintold@bjc@lgb@total@coverage80\endcsname{0.33}
\expandafter\def\csname rev@rintold@bjc@lgb@total@coverage95\endcsname{0.38}
\expandafter\def\csname rev@rintold@bjc@lgb@total@spl\endcsname{0.30}
\expandafter\def\csname rev@rintold@bjc@lift@ixs@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@bjc@lift@ixs@coverage80\endcsname{0.56}
\expandafter\def\csname rev@rintold@bjc@lift@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@bjc@lift@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@bjc@lift@total@coverage50\endcsname{0.20}
\expandafter\def\csname rev@rintold@bjc@lift@total@coverage80\endcsname{0.35}
\expandafter\def\csname rev@rintold@bjc@lift@total@coverage95\endcsname{0.38}
\expandafter\def\csname rev@rintold@bjc@lift@total@spl\endcsname{0.31}
\expandafter\def\csname rev@rintold@bjc@naive@ixs@coverage50\endcsname{0.15}
\expandafter\def\csname rev@rintold@bjc@naive@ixs@coverage80\endcsname{0.62}
\expandafter\def\csname rev@rintold@bjc@naive@ixs@coverage95\endcsname{0.91}
\expandafter\def\csname rev@rintold@bjc@naive@ixs@spl\endcsname{0.44}
\expandafter\def\csname rev@rintold@bjc@naive@total@coverage50\endcsname{0.20}
\expandafter\def\csname rev@rintold@bjc@naive@total@coverage80\endcsname{0.35}
\expandafter\def\csname rev@rintold@bjc@naive@total@coverage95\endcsname{0.42}
\expandafter\def\csname rev@rintold@bjc@naive@total@spl\endcsname{0.74}
\expandafter\def\csname rev@rintold@bjc@tfm@ixs@coverage50\endcsname{0.11}
\expandafter\def\csname rev@rintold@bjc@tfm@ixs@coverage80\endcsname{0.55}
\expandafter\def\csname rev@rintold@bjc@tfm@ixs@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rintold@bjc@tfm@ixs@spl\endcsname{0.29}
\expandafter\def\csname rev@rintold@bjc@tfm@total@coverage50\endcsname{0.17}
\expandafter\def\csname rev@rintold@bjc@tfm@total@coverage80\endcsname{0.28}
\expandafter\def\csname rev@rintold@bjc@tfm@total@coverage95\endcsname{0.35}
\expandafter\def\csname rev@rintold@bjc@tfm@total@spl\endcsname{0.43}
\expandafter\def\csname rev@rintold@bjc@tfmplan@ixs@coverage50\endcsname{0.08}
\expandafter\def\csname rev@rintold@bjc@tfmplan@ixs@coverage80\endcsname{0.55}
\expandafter\def\csname rev@rintold@bjc@tfmplan@ixs@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rintold@bjc@tfmplan@ixs@spl\endcsname{0.26}
\expandafter\def\csname rev@rintold@bjc@tfmplan@total@coverage50\endcsname{0.25}
\expandafter\def\csname rev@rintold@bjc@tfmplan@total@coverage80\endcsname{0.38}
\expandafter\def\csname rev@rintold@bjc@tfmplan@total@coverage95\endcsname{0.40}
\expandafter\def\csname rev@rintold@bjc@tfmplan@total@spl\endcsname{0.37}
\expandafter\def\csname rev@rintold@bjc@tft@ixs@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@bjc@tft@ixs@coverage80\endcsname{0.55}
\expandafter\def\csname rev@rintold@bjc@tft@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@bjc@tft@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@bjc@tft@total@coverage50\endcsname{0.20}
\expandafter\def\csname rev@rintold@bjc@tft@total@coverage80\endcsname{0.25}
\expandafter\def\csname rev@rintold@bjc@tft@total@coverage95\endcsname{0.35}
\expandafter\def\csname rev@rintold@bjc@tft@total@spl\endcsname{0.39}
\expandafter\def\csname rev@rintold@bjc@world@ixs@coverage50\endcsname{0.11}
\expandafter\def\csname rev@rintold@bjc@world@ixs@coverage80\endcsname{0.56}
\expandafter\def\csname rev@rintold@bjc@world@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@bjc@world@ixs@spl\endcsname{0.26}
\expandafter\def\csname rev@rintold@bjc@world@total@coverage50\endcsname{0.17}
\expandafter\def\csname rev@rintold@bjc@world@total@coverage80\endcsname{0.30}
\expandafter\def\csname rev@rintold@bjc@world@total@coverage95\endcsname{0.42}
\expandafter\def\csname rev@rintold@bjc@world@total@spl\endcsname{0.36}
\expandafter\def\csname rev@rintold@che@chronos@ixs@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@che@chronos@ixs@coverage80\endcsname{0.61}
\expandafter\def\csname rev@rintold@che@chronos@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@che@chronos@ixs@spl\endcsname{0.30}
\expandafter\def\csname rev@rintold@che@chronos@total@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@che@chronos@total@coverage80\endcsname{0.20}
\expandafter\def\csname rev@rintold@che@chronos@total@coverage95\endcsname{0.25}
\expandafter\def\csname rev@rintold@che@chronos@total@spl\endcsname{0.44}
\expandafter\def\csname rev@rintold@che@ens@ixs@coverage50\endcsname{0.09}
\expandafter\def\csname rev@rintold@che@ens@ixs@coverage80\endcsname{0.61}
\expandafter\def\csname rev@rintold@che@ens@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@che@ens@ixs@spl\endcsname{0.22}
\expandafter\def\csname rev@rintold@che@ens@total@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@che@ens@total@coverage80\endcsname{0.25}
\expandafter\def\csname rev@rintold@che@ens@total@coverage95\endcsname{0.33}
\expandafter\def\csname rev@rintold@che@ens@total@spl\endcsname{0.20}
\expandafter\def\csname rev@rintold@che@lgb@ixs@coverage50\endcsname{0.14}
\expandafter\def\csname rev@rintold@che@lgb@ixs@coverage80\endcsname{0.62}
\expandafter\def\csname rev@rintold@che@lgb@ixs@coverage95\endcsname{0.91}
\expandafter\def\csname rev@rintold@che@lgb@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rintold@che@lgb@total@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rintold@che@lgb@total@coverage80\endcsname{0.50}
\expandafter\def\csname rev@rintold@che@lgb@total@coverage95\endcsname{0.55}
\expandafter\def\csname rev@rintold@che@lgb@total@spl\endcsname{0.29}
\expandafter\def\csname rev@rintold@che@lift@ixs@coverage50\endcsname{0.07}
\expandafter\def\csname rev@rintold@che@lift@ixs@coverage80\endcsname{0.61}
\expandafter\def\csname rev@rintold@che@lift@ixs@coverage95\endcsname{0.91}
\expandafter\def\csname rev@rintold@che@lift@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@che@lift@total@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rintold@che@lift@total@coverage80\endcsname{0.70}
\expandafter\def\csname rev@rintold@che@lift@total@coverage95\endcsname{0.70}
\expandafter\def\csname rev@rintold@che@lift@total@spl\endcsname{0.42}
\expandafter\def\csname rev@rintold@che@naive@ixs@coverage50\endcsname{0.14}
\expandafter\def\csname rev@rintold@che@naive@ixs@coverage80\endcsname{0.64}
\expandafter\def\csname rev@rintold@che@naive@ixs@coverage95\endcsname{0.92}
\expandafter\def\csname rev@rintold@che@naive@ixs@spl\endcsname{0.43}
\expandafter\def\csname rev@rintold@che@naive@total@coverage50\endcsname{0.28}
\expandafter\def\csname rev@rintold@che@naive@total@coverage80\endcsname{0.40}
\expandafter\def\csname rev@rintold@che@naive@total@coverage95\endcsname{0.45}
\expandafter\def\csname rev@rintold@che@naive@total@spl\endcsname{0.64}
\expandafter\def\csname rev@rintold@che@tfm@ixs@coverage50\endcsname{0.11}
\expandafter\def\csname rev@rintold@che@tfm@ixs@coverage80\endcsname{0.61}
\expandafter\def\csname rev@rintold@che@tfm@ixs@coverage95\endcsname{0.91}
\expandafter\def\csname rev@rintold@che@tfm@ixs@spl\endcsname{0.29}
\expandafter\def\csname rev@rintold@che@tfm@total@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@che@tfm@total@coverage80\endcsname{0.23}
\expandafter\def\csname rev@rintold@che@tfm@total@coverage95\endcsname{0.33}
\expandafter\def\csname rev@rintold@che@tfm@total@spl\endcsname{0.39}
\expandafter\def\csname rev@rintold@che@tfmplan@ixs@coverage50\endcsname{0.08}
\expandafter\def\csname rev@rintold@che@tfmplan@ixs@coverage80\endcsname{0.61}
\expandafter\def\csname rev@rintold@che@tfmplan@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@che@tfmplan@ixs@spl\endcsname{0.26}
\expandafter\def\csname rev@rintold@che@tfmplan@total@coverage50\endcsname{0.23}
\expandafter\def\csname rev@rintold@che@tfmplan@total@coverage80\endcsname{0.40}
\expandafter\def\csname rev@rintold@che@tfmplan@total@coverage95\endcsname{0.42}
\expandafter\def\csname rev@rintold@che@tfmplan@total@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@che@tft@ixs@coverage50\endcsname{0.11}
\expandafter\def\csname rev@rintold@che@tft@ixs@coverage80\endcsname{0.61}
\expandafter\def\csname rev@rintold@che@tft@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@che@tft@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@che@tft@total@coverage50\endcsname{0.23}
\expandafter\def\csname rev@rintold@che@tft@total@coverage80\endcsname{0.35}
\expandafter\def\csname rev@rintold@che@tft@total@coverage95\endcsname{0.38}
\expandafter\def\csname rev@rintold@che@tft@total@spl\endcsname{0.29}
\expandafter\def\csname rev@rintold@che@world@ixs@coverage50\endcsname{0.06}
\expandafter\def\csname rev@rintold@che@world@ixs@coverage80\endcsname{0.61}
\expandafter\def\csname rev@rintold@che@world@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@che@world@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@che@world@total@coverage50\endcsname{0.15}
\expandafter\def\csname rev@rintold@che@world@total@coverage80\endcsname{0.33}
\expandafter\def\csname rev@rintold@che@world@total@coverage95\endcsname{0.42}
\expandafter\def\csname rev@rintold@che@world@total@spl\endcsname{0.38}
\expandafter\def\csname rev@rintold@frat@chronos@ixs@coverage50\endcsname{0.49}
\expandafter\def\csname rev@rintold@frat@chronos@ixs@coverage80\endcsname{0.79}
\expandafter\def\csname rev@rintold@frat@chronos@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rintold@frat@chronos@ixs@spl\endcsname{0.30}
\expandafter\def\csname rev@rintold@frat@chronos@total@coverage50\endcsname{0.17}
\expandafter\def\csname rev@rintold@frat@chronos@total@coverage80\endcsname{0.17}
\expandafter\def\csname rev@rintold@frat@chronos@total@coverage95\endcsname{0.17}
\expandafter\def\csname rev@rintold@frat@chronos@total@spl\endcsname{0.26}
\expandafter\def\csname rev@rintold@frat@ens@ixs@coverage50\endcsname{0.50}
\expandafter\def\csname rev@rintold@frat@ens@ixs@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rintold@frat@ens@ixs@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rintold@frat@ens@ixs@spl\endcsname{0.20}
\expandafter\def\csname rev@rintold@frat@ens@total@coverage50\endcsname{0.08}
\expandafter\def\csname rev@rintold@frat@ens@total@coverage80\endcsname{0.17}
\expandafter\def\csname rev@rintold@frat@ens@total@coverage95\endcsname{0.21}
\expandafter\def\csname rev@rintold@frat@ens@total@spl\endcsname{0.20}
\expandafter\def\csname rev@rintold@frat@lgb@ixs@coverage50\endcsname{0.50}
\expandafter\def\csname rev@rintold@frat@lgb@ixs@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rintold@frat@lgb@ixs@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rintold@frat@lgb@ixs@spl\endcsname{0.21}
\expandafter\def\csname rev@rintold@frat@lgb@total@coverage50\endcsname{0.17}
\expandafter\def\csname rev@rintold@frat@lgb@total@coverage80\endcsname{0.21}
\expandafter\def\csname rev@rintold@frat@lgb@total@coverage95\endcsname{0.25}
\expandafter\def\csname rev@rintold@frat@lgb@total@spl\endcsname{0.22}
\expandafter\def\csname rev@rintold@frat@lift@ixs@coverage50\endcsname{0.51}
\expandafter\def\csname rev@rintold@frat@lift@ixs@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rintold@frat@lift@ixs@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rintold@frat@lift@ixs@spl\endcsname{0.21}
\expandafter\def\csname rev@rintold@frat@lift@total@coverage50\endcsname{0.04}
\expandafter\def\csname rev@rintold@frat@lift@total@coverage80\endcsname{0.04}
\expandafter\def\csname rev@rintold@frat@lift@total@coverage95\endcsname{0.08}
\expandafter\def\csname rev@rintold@frat@lift@total@spl\endcsname{0.24}
\expandafter\def\csname rev@rintold@frat@naive@ixs@coverage50\endcsname{0.51}
\expandafter\def\csname rev@rintold@frat@naive@ixs@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rintold@frat@naive@ixs@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rintold@frat@naive@ixs@spl\endcsname{0.37}
\expandafter\def\csname rev@rintold@frat@naive@total@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@frat@naive@total@coverage80\endcsname{0.21}
\expandafter\def\csname rev@rintold@frat@naive@total@coverage95\endcsname{0.29}
\expandafter\def\csname rev@rintold@frat@naive@total@spl\endcsname{0.47}
\expandafter\def\csname rev@rintold@frat@tfm@ixs@coverage50\endcsname{0.49}
\expandafter\def\csname rev@rintold@frat@tfm@ixs@coverage80\endcsname{0.79}
\expandafter\def\csname rev@rintold@frat@tfm@ixs@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rintold@frat@tfm@ixs@spl\endcsname{0.30}
\expandafter\def\csname rev@rintold@frat@tfm@total@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@frat@tfm@total@coverage80\endcsname{0.21}
\expandafter\def\csname rev@rintold@frat@tfm@total@coverage95\endcsname{0.25}
\expandafter\def\csname rev@rintold@frat@tfm@total@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@frat@tfmplan@ixs@coverage50\endcsname{0.49}
\expandafter\def\csname rev@rintold@frat@tfmplan@ixs@coverage80\endcsname{0.81}
\expandafter\def\csname rev@rintold@frat@tfmplan@ixs@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rintold@frat@tfmplan@ixs@spl\endcsname{0.22}
\expandafter\def\csname rev@rintold@frat@tfmplan@total@coverage50\endcsname{0.08}
\expandafter\def\csname rev@rintold@frat@tfmplan@total@coverage80\endcsname{0.08}
\expandafter\def\csname rev@rintold@frat@tfmplan@total@coverage95\endcsname{0.08}
\expandafter\def\csname rev@rintold@frat@tfmplan@total@spl\endcsname{0.19}
\expandafter\def\csname rev@rintold@frat@tft@ixs@coverage50\endcsname{0.50}
\expandafter\def\csname rev@rintold@frat@tft@ixs@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rintold@frat@tft@ixs@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rintold@frat@tft@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rintold@frat@tft@total@coverage50\endcsname{0.08}
\expandafter\def\csname rev@rintold@frat@tft@total@coverage80\endcsname{0.17}
\expandafter\def\csname rev@rintold@frat@tft@total@coverage95\endcsname{0.21}
\expandafter\def\csname rev@rintold@frat@tft@total@spl\endcsname{0.21}
\expandafter\def\csname rev@rintold@frat@world@ixs@coverage50\endcsname{0.50}
\expandafter\def\csname rev@rintold@frat@world@ixs@coverage80\endcsname{0.82}
\expandafter\def\csname rev@rintold@frat@world@ixs@coverage95\endcsname{0.96}
\expandafter\def\csname rev@rintold@frat@world@ixs@spl\endcsname{0.22}
\expandafter\def\csname rev@rintold@frat@world@total@coverage50\endcsname{0.00}
\expandafter\def\csname rev@rintold@frat@world@total@coverage80\endcsname{0.04}
\expandafter\def\csname rev@rintold@frat@world@total@coverage95\endcsname{0.08}
\expandafter\def\csname rev@rintold@frat@world@total@spl\endcsname{0.28}
\expandafter\def\csname rev@rintold@fre@chronos@ixs@coverage50\endcsname{0.09}
\expandafter\def\csname rev@rintold@fre@chronos@ixs@coverage80\endcsname{0.54}
\expandafter\def\csname rev@rintold@fre@chronos@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@fre@chronos@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rintold@fre@chronos@total@coverage50\endcsname{0.15}
\expandafter\def\csname rev@rintold@fre@chronos@total@coverage80\endcsname{0.23}
\expandafter\def\csname rev@rintold@fre@chronos@total@coverage95\endcsname{0.30}
\expandafter\def\csname rev@rintold@fre@chronos@total@spl\endcsname{0.31}
\expandafter\def\csname rev@rintold@fre@ens@ixs@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@fre@ens@ixs@coverage80\endcsname{0.55}
\expandafter\def\csname rev@rintold@fre@ens@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@fre@ens@ixs@spl\endcsname{0.18}
\expandafter\def\csname rev@rintold@fre@ens@total@coverage50\endcsname{0.40}
\expandafter\def\csname rev@rintold@fre@ens@total@coverage80\endcsname{0.50}
\expandafter\def\csname rev@rintold@fre@ens@total@coverage95\endcsname{0.55}
\expandafter\def\csname rev@rintold@fre@ens@total@spl\endcsname{0.24}
\expandafter\def\csname rev@rintold@fre@lgb@ixs@coverage50\endcsname{0.14}
\expandafter\def\csname rev@rintold@fre@lgb@ixs@coverage80\endcsname{0.56}
\expandafter\def\csname rev@rintold@fre@lgb@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@fre@lgb@ixs@spl\endcsname{0.17}
\expandafter\def\csname rev@rintold@fre@lgb@total@coverage50\endcsname{0.23}
\expandafter\def\csname rev@rintold@fre@lgb@total@coverage80\endcsname{0.38}
\expandafter\def\csname rev@rintold@fre@lgb@total@coverage95\endcsname{0.47}
\expandafter\def\csname rev@rintold@fre@lgb@total@spl\endcsname{0.21}
\expandafter\def\csname rev@rintold@fre@lift@ixs@coverage50\endcsname{0.09}
\expandafter\def\csname rev@rintold@fre@lift@ixs@coverage80\endcsname{0.54}
\expandafter\def\csname rev@rintold@fre@lift@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@fre@lift@ixs@spl\endcsname{0.21}
\expandafter\def\csname rev@rintold@fre@lift@total@coverage50\endcsname{0.28}
\expandafter\def\csname rev@rintold@fre@lift@total@coverage80\endcsname{0.40}
\expandafter\def\csname rev@rintold@fre@lift@total@coverage95\endcsname{0.45}
\expandafter\def\csname rev@rintold@fre@lift@total@spl\endcsname{0.29}
\expandafter\def\csname rev@rintold@fre@naive@ixs@coverage50\endcsname{0.26}
\expandafter\def\csname rev@rintold@fre@naive@ixs@coverage80\endcsname{0.59}
\expandafter\def\csname rev@rintold@fre@naive@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@fre@naive@ixs@spl\endcsname{0.32}
\expandafter\def\csname rev@rintold@fre@naive@total@coverage50\endcsname{0.20}
\expandafter\def\csname rev@rintold@fre@naive@total@coverage80\endcsname{0.30}
\expandafter\def\csname rev@rintold@fre@naive@total@coverage95\endcsname{0.35}
\expandafter\def\csname rev@rintold@fre@naive@total@spl\endcsname{0.40}
\expandafter\def\csname rev@rintold@fre@tfm@ixs@coverage50\endcsname{0.11}
\expandafter\def\csname rev@rintold@fre@tfm@ixs@coverage80\endcsname{0.53}
\expandafter\def\csname rev@rintold@fre@tfm@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@fre@tfm@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rintold@fre@tfm@total@coverage50\endcsname{0.17}
\expandafter\def\csname rev@rintold@fre@tfm@total@coverage80\endcsname{0.30}
\expandafter\def\csname rev@rintold@fre@tfm@total@coverage95\endcsname{0.35}
\expandafter\def\csname rev@rintold@fre@tfm@total@spl\endcsname{0.29}
\expandafter\def\csname rev@rintold@fre@tfmplan@ixs@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@fre@tfmplan@ixs@coverage80\endcsname{0.54}
\expandafter\def\csname rev@rintold@fre@tfmplan@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@fre@tfmplan@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rintold@fre@tfmplan@total@coverage50\endcsname{0.33}
\expandafter\def\csname rev@rintold@fre@tfmplan@total@coverage80\endcsname{0.42}
\expandafter\def\csname rev@rintold@fre@tfmplan@total@coverage95\endcsname{0.45}
\expandafter\def\csname rev@rintold@fre@tfmplan@total@spl\endcsname{0.33}
\expandafter\def\csname rev@rintold@fre@tft@ixs@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@fre@tft@ixs@coverage80\endcsname{0.54}
\expandafter\def\csname rev@rintold@fre@tft@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@fre@tft@ixs@spl\endcsname{0.21}
\expandafter\def\csname rev@rintold@fre@tft@total@coverage50\endcsname{0.35}
\expandafter\def\csname rev@rintold@fre@tft@total@coverage80\endcsname{0.53}
\expandafter\def\csname rev@rintold@fre@tft@total@coverage95\endcsname{0.60}
\expandafter\def\csname rev@rintold@fre@tft@total@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@fre@world@ixs@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@fre@world@ixs@coverage80\endcsname{0.56}
\expandafter\def\csname rev@rintold@fre@world@ixs@coverage95\endcsname{0.91}
\expandafter\def\csname rev@rintold@fre@world@ixs@spl\endcsname{0.18}
\expandafter\def\csname rev@rintold@fre@world@total@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rintold@fre@world@total@coverage80\endcsname{0.53}
\expandafter\def\csname rev@rintold@fre@world@total@coverage95\endcsname{0.60}
\expandafter\def\csname rev@rintold@fre@world@total@spl\endcsname{0.24}
\expandafter\def\csname rev@rintold@mfive@chronos@ixs@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rintold@mfive@chronos@ixs@coverage80\endcsname{0.78}
\expandafter\def\csname rev@rintold@mfive@chronos@ixs@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rintold@mfive@chronos@ixs@spl\endcsname{0.33}
\expandafter\def\csname rev@rintold@mfive@chronos@total@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@mfive@chronos@total@coverage80\endcsname{0.18}
\expandafter\def\csname rev@rintold@mfive@chronos@total@coverage95\endcsname{0.25}
\expandafter\def\csname rev@rintold@mfive@chronos@total@spl\endcsname{0.40}
\expandafter\def\csname rev@rintold@mfive@ens@ixs@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rintold@mfive@ens@ixs@coverage80\endcsname{0.77}
\expandafter\def\csname rev@rintold@mfive@ens@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rintold@mfive@ens@ixs@spl\endcsname{0.32}
\expandafter\def\csname rev@rintold@mfive@ens@total@coverage50\endcsname{0.14}
\expandafter\def\csname rev@rintold@mfive@ens@total@coverage80\endcsname{0.23}
\expandafter\def\csname rev@rintold@mfive@ens@total@coverage95\endcsname{0.27}
\expandafter\def\csname rev@rintold@mfive@ens@total@spl\endcsname{0.28}
\expandafter\def\csname rev@rintold@mfive@lgb@ixs@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rintold@mfive@lgb@ixs@coverage80\endcsname{0.77}
\expandafter\def\csname rev@rintold@mfive@lgb@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rintold@mfive@lgb@ixs@spl\endcsname{0.33}
\expandafter\def\csname rev@rintold@mfive@lgb@total@coverage50\endcsname{0.15}
\expandafter\def\csname rev@rintold@mfive@lgb@total@coverage80\endcsname{0.23}
\expandafter\def\csname rev@rintold@mfive@lgb@total@coverage95\endcsname{0.30}
\expandafter\def\csname rev@rintold@mfive@lgb@total@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@mfive@lift@ixs@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rintold@mfive@lift@ixs@coverage80\endcsname{0.77}
\expandafter\def\csname rev@rintold@mfive@lift@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rintold@mfive@lift@ixs@spl\endcsname{0.32}
\expandafter\def\csname rev@rintold@mfive@lift@total@coverage50\endcsname{0.18}
\expandafter\def\csname rev@rintold@mfive@lift@total@coverage80\endcsname{0.19}
\expandafter\def\csname rev@rintold@mfive@lift@total@coverage95\endcsname{0.20}
\expandafter\def\csname rev@rintold@mfive@lift@total@spl\endcsname{0.73}
\expandafter\def\csname rev@rintold@mfive@naive@ixs@coverage50\endcsname{0.47}
\expandafter\def\csname rev@rintold@mfive@naive@ixs@coverage80\endcsname{0.78}
\expandafter\def\csname rev@rintold@mfive@naive@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rintold@mfive@naive@ixs@spl\endcsname{0.45}
\expandafter\def\csname rev@rintold@mfive@naive@total@coverage50\endcsname{0.08}
\expandafter\def\csname rev@rintold@mfive@naive@total@coverage80\endcsname{0.14}
\expandafter\def\csname rev@rintold@mfive@naive@total@coverage95\endcsname{0.19}
\expandafter\def\csname rev@rintold@mfive@naive@total@spl\endcsname{0.59}
\expandafter\def\csname rev@rintold@mfive@tfm@ixs@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rintold@mfive@tfm@ixs@coverage80\endcsname{0.78}
\expandafter\def\csname rev@rintold@mfive@tfm@ixs@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rintold@mfive@tfm@ixs@spl\endcsname{0.32}
\expandafter\def\csname rev@rintold@mfive@tfm@total@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@mfive@tfm@total@coverage80\endcsname{0.19}
\expandafter\def\csname rev@rintold@mfive@tfm@total@coverage95\endcsname{0.26}
\expandafter\def\csname rev@rintold@mfive@tfm@total@spl\endcsname{0.40}
\expandafter\def\csname rev@rintold@mfive@tfmplan@ixs@coverage50\endcsname{0.45}
\expandafter\def\csname rev@rintold@mfive@tfmplan@ixs@coverage80\endcsname{0.78}
\expandafter\def\csname rev@rintold@mfive@tfmplan@ixs@coverage95\endcsname{0.95}
\expandafter\def\csname rev@rintold@mfive@tfmplan@ixs@spl\endcsname{0.32}
\expandafter\def\csname rev@rintold@mfive@tfmplan@total@coverage50\endcsname{0.17}
\expandafter\def\csname rev@rintold@mfive@tfmplan@total@coverage80\endcsname{0.23}
\expandafter\def\csname rev@rintold@mfive@tfmplan@total@coverage95\endcsname{0.25}
\expandafter\def\csname rev@rintold@mfive@tfmplan@total@spl\endcsname{0.38}
\expandafter\def\csname rev@rintold@mfive@world@ixs@coverage50\endcsname{0.44}
\expandafter\def\csname rev@rintold@mfive@world@ixs@coverage80\endcsname{0.77}
\expandafter\def\csname rev@rintold@mfive@world@ixs@coverage95\endcsname{0.94}
\expandafter\def\csname rev@rintold@mfive@world@ixs@spl\endcsname{0.33}
\expandafter\def\csname rev@rintold@mfive@world@total@coverage50\endcsname{0.11}
\expandafter\def\csname rev@rintold@mfive@world@total@coverage80\endcsname{0.18}
\expandafter\def\csname rev@rintold@mfive@world@total@coverage95\endcsname{0.19}
\expandafter\def\csname rev@rintold@mfive@world@total@spl\endcsname{0.30}
\expandafter\def\csname rev@rintold@sdr@chronos@ixs@coverage50\endcsname{0.21}
\expandafter\def\csname rev@rintold@sdr@chronos@ixs@coverage80\endcsname{0.62}
\expandafter\def\csname rev@rintold@sdr@chronos@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@sdr@chronos@ixs@spl\endcsname{0.31}
\expandafter\def\csname rev@rintold@sdr@chronos@total@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@sdr@chronos@total@coverage80\endcsname{0.23}
\expandafter\def\csname rev@rintold@sdr@chronos@total@coverage95\endcsname{0.28}
\expandafter\def\csname rev@rintold@sdr@chronos@total@spl\endcsname{0.46}
\expandafter\def\csname rev@rintold@sdr@ens@ixs@coverage50\endcsname{0.27}
\expandafter\def\csname rev@rintold@sdr@ens@ixs@coverage80\endcsname{0.64}
\expandafter\def\csname rev@rintold@sdr@ens@ixs@coverage95\endcsname{0.92}
\expandafter\def\csname rev@rintold@sdr@ens@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rintold@sdr@ens@total@coverage50\endcsname{0.17}
\expandafter\def\csname rev@rintold@sdr@ens@total@coverage80\endcsname{0.33}
\expandafter\def\csname rev@rintold@sdr@ens@total@coverage95\endcsname{0.40}
\expandafter\def\csname rev@rintold@sdr@ens@total@spl\endcsname{0.42}
\expandafter\def\csname rev@rintold@sdr@lgb@ixs@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rintold@sdr@lgb@ixs@coverage80\endcsname{0.65}
\expandafter\def\csname rev@rintold@sdr@lgb@ixs@coverage95\endcsname{0.91}
\expandafter\def\csname rev@rintold@sdr@lgb@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rintold@sdr@lgb@total@coverage50\endcsname{0.15}
\expandafter\def\csname rev@rintold@sdr@lgb@total@coverage80\endcsname{0.35}
\expandafter\def\csname rev@rintold@sdr@lgb@total@coverage95\endcsname{0.38}
\expandafter\def\csname rev@rintold@sdr@lgb@total@spl\endcsname{0.40}
\expandafter\def\csname rev@rintold@sdr@lift@ixs@coverage50\endcsname{0.27}
\expandafter\def\csname rev@rintold@sdr@lift@ixs@coverage80\endcsname{0.64}
\expandafter\def\csname rev@rintold@sdr@lift@ixs@coverage95\endcsname{0.92}
\expandafter\def\csname rev@rintold@sdr@lift@ixs@spl\endcsname{0.30}
\expandafter\def\csname rev@rintold@sdr@lift@total@coverage50\endcsname{0.20}
\expandafter\def\csname rev@rintold@sdr@lift@total@coverage80\endcsname{0.28}
\expandafter\def\csname rev@rintold@sdr@lift@total@coverage95\endcsname{0.30}
\expandafter\def\csname rev@rintold@sdr@lift@total@spl\endcsname{0.49}
\expandafter\def\csname rev@rintold@sdr@naive@ixs@coverage50\endcsname{0.29}
\expandafter\def\csname rev@rintold@sdr@naive@ixs@coverage80\endcsname{0.70}
\expandafter\def\csname rev@rintold@sdr@naive@ixs@coverage95\endcsname{0.93}
\expandafter\def\csname rev@rintold@sdr@naive@ixs@spl\endcsname{0.40}
\expandafter\def\csname rev@rintold@sdr@naive@total@coverage50\endcsname{0.38}
\expandafter\def\csname rev@rintold@sdr@naive@total@coverage80\endcsname{0.50}
\expandafter\def\csname rev@rintold@sdr@naive@total@coverage95\endcsname{0.57}
\expandafter\def\csname rev@rintold@sdr@naive@total@spl\endcsname{0.49}
\expandafter\def\csname rev@rintold@sdr@tfm@ixs@coverage50\endcsname{0.22}
\expandafter\def\csname rev@rintold@sdr@tfm@ixs@coverage80\endcsname{0.62}
\expandafter\def\csname rev@rintold@sdr@tfm@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@sdr@tfm@ixs@spl\endcsname{0.31}
\expandafter\def\csname rev@rintold@sdr@tfm@total@coverage50\endcsname{0.20}
\expandafter\def\csname rev@rintold@sdr@tfm@total@coverage80\endcsname{0.30}
\expandafter\def\csname rev@rintold@sdr@tfm@total@coverage95\endcsname{0.30}
\expandafter\def\csname rev@rintold@sdr@tfm@total@spl\endcsname{0.43}
\expandafter\def\csname rev@rintold@sdr@tfmplan@ixs@coverage50\endcsname{0.17}
\expandafter\def\csname rev@rintold@sdr@tfmplan@ixs@coverage80\endcsname{0.62}
\expandafter\def\csname rev@rintold@sdr@tfmplan@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@sdr@tfmplan@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@sdr@tfmplan@total@coverage50\endcsname{0.07}
\expandafter\def\csname rev@rintold@sdr@tfmplan@total@coverage80\endcsname{0.28}
\expandafter\def\csname rev@rintold@sdr@tfmplan@total@coverage95\endcsname{0.30}
\expandafter\def\csname rev@rintold@sdr@tfmplan@total@spl\endcsname{0.49}
\expandafter\def\csname rev@rintold@sdr@tft@ixs@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rintold@sdr@tft@ixs@coverage80\endcsname{0.63}
\expandafter\def\csname rev@rintold@sdr@tft@ixs@coverage95\endcsname{0.91}
\expandafter\def\csname rev@rintold@sdr@tft@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@sdr@tft@total@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@sdr@tft@total@coverage80\endcsname{0.28}
\expandafter\def\csname rev@rintold@sdr@tft@total@coverage95\endcsname{0.28}
\expandafter\def\csname rev@rintold@sdr@tft@total@spl\endcsname{0.47}
\expandafter\def\csname rev@rintold@sdr@world@ixs@coverage50\endcsname{0.28}
\expandafter\def\csname rev@rintold@sdr@world@ixs@coverage80\endcsname{0.64}
\expandafter\def\csname rev@rintold@sdr@world@ixs@coverage95\endcsname{0.92}
\expandafter\def\csname rev@rintold@sdr@world@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@sdr@world@total@coverage50\endcsname{0.23}
\expandafter\def\csname rev@rintold@sdr@world@total@coverage80\endcsname{0.33}
\expandafter\def\csname rev@rintold@sdr@world@total@coverage95\endcsname{0.40}
\expandafter\def\csname rev@rintold@sdr@world@total@spl\endcsname{0.46}
\expandafter\def\csname rev@rintold@sna@chronos@ixs@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@sna@chronos@ixs@coverage80\endcsname{0.54}
\expandafter\def\csname rev@rintold@sna@chronos@ixs@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rintold@sna@chronos@ixs@spl\endcsname{0.29}
\expandafter\def\csname rev@rintold@sna@chronos@total@coverage50\endcsname{0.15}
\expandafter\def\csname rev@rintold@sna@chronos@total@coverage80\endcsname{0.25}
\expandafter\def\csname rev@rintold@sna@chronos@total@coverage95\endcsname{0.25}
\expandafter\def\csname rev@rintold@sna@chronos@total@spl\endcsname{4.07}
\expandafter\def\csname rev@rintold@sna@ens@ixs@coverage50\endcsname{0.09}
\expandafter\def\csname rev@rintold@sna@ens@ixs@coverage80\endcsname{0.55}
\expandafter\def\csname rev@rintold@sna@ens@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@sna@ens@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rintold@sna@ens@total@coverage50\endcsname{0.12}
\expandafter\def\csname rev@rintold@sna@ens@total@coverage80\endcsname{0.17}
\expandafter\def\csname rev@rintold@sna@ens@total@coverage95\endcsname{0.25}
\expandafter\def\csname rev@rintold@sna@ens@total@spl\endcsname{0.66}
\expandafter\def\csname rev@rintold@sna@lgb@ixs@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@sna@lgb@ixs@coverage80\endcsname{0.54}
\expandafter\def\csname rev@rintold@sna@lgb@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@sna@lgb@ixs@spl\endcsname{0.23}
\expandafter\def\csname rev@rintold@sna@lgb@total@coverage50\endcsname{0.30}
\expandafter\def\csname rev@rintold@sna@lgb@total@coverage80\endcsname{0.40}
\expandafter\def\csname rev@rintold@sna@lgb@total@coverage95\endcsname{0.42}
\expandafter\def\csname rev@rintold@sna@lgb@total@spl\endcsname{0.56}
\expandafter\def\csname rev@rintold@sna@lift@ixs@coverage50\endcsname{0.08}
\expandafter\def\csname rev@rintold@sna@lift@ixs@coverage80\endcsname{0.54}
\expandafter\def\csname rev@rintold@sna@lift@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@sna@lift@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@sna@lift@total@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@sna@lift@total@coverage80\endcsname{0.17}
\expandafter\def\csname rev@rintold@sna@lift@total@coverage95\endcsname{0.23}
\expandafter\def\csname rev@rintold@sna@lift@total@spl\endcsname{0.58}
\expandafter\def\csname rev@rintold@sna@naive@ixs@coverage50\endcsname{0.27}
\expandafter\def\csname rev@rintold@sna@naive@ixs@coverage80\endcsname{0.59}
\expandafter\def\csname rev@rintold@sna@naive@ixs@coverage95\endcsname{0.87}
\expandafter\def\csname rev@rintold@sna@naive@ixs@spl\endcsname{0.40}
\expandafter\def\csname rev@rintold@sna@naive@total@coverage50\endcsname{0.28}
\expandafter\def\csname rev@rintold@sna@naive@total@coverage80\endcsname{0.47}
\expandafter\def\csname rev@rintold@sna@naive@total@coverage95\endcsname{0.50}
\expandafter\def\csname rev@rintold@sna@naive@total@spl\endcsname{1.16}
\expandafter\def\csname rev@rintold@sna@tfm@ixs@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@sna@tfm@ixs@coverage80\endcsname{0.53}
\expandafter\def\csname rev@rintold@sna@tfm@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@sna@tfm@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@sna@tfm@total@coverage50\endcsname{0.20}
\expandafter\def\csname rev@rintold@sna@tfm@total@coverage80\endcsname{0.28}
\expandafter\def\csname rev@rintold@sna@tfm@total@coverage95\endcsname{0.30}
\expandafter\def\csname rev@rintold@sna@tfm@total@spl\endcsname{1.07}
\expandafter\def\csname rev@rintold@sna@tfmplan@ixs@coverage50\endcsname{0.09}
\expandafter\def\csname rev@rintold@sna@tfmplan@ixs@coverage80\endcsname{0.53}
\expandafter\def\csname rev@rintold@sna@tfmplan@ixs@coverage95\endcsname{0.89}
\expandafter\def\csname rev@rintold@sna@tfmplan@ixs@spl\endcsname{0.25}
\expandafter\def\csname rev@rintold@sna@tfmplan@total@coverage50\endcsname{0.15}
\expandafter\def\csname rev@rintold@sna@tfmplan@total@coverage80\endcsname{0.23}
\expandafter\def\csname rev@rintold@sna@tfmplan@total@coverage95\endcsname{0.25}
\expandafter\def\csname rev@rintold@sna@tfmplan@total@spl\endcsname{0.64}
\expandafter\def\csname rev@rintold@sna@tft@ixs@coverage50\endcsname{0.11}
\expandafter\def\csname rev@rintold@sna@tft@ixs@coverage80\endcsname{0.54}
\expandafter\def\csname rev@rintold@sna@tft@ixs@coverage95\endcsname{0.88}
\expandafter\def\csname rev@rintold@sna@tft@ixs@spl\endcsname{0.27}
\expandafter\def\csname rev@rintold@sna@tft@total@coverage50\endcsname{0.10}
\expandafter\def\csname rev@rintold@sna@tft@total@coverage80\endcsname{0.17}
\expandafter\def\csname rev@rintold@sna@tft@total@coverage95\endcsname{0.23}
\expandafter\def\csname rev@rintold@sna@tft@total@spl\endcsname{0.69}
\expandafter\def\csname rev@rintold@sna@world@ixs@coverage50\endcsname{0.08}
\expandafter\def\csname rev@rintold@sna@world@ixs@coverage80\endcsname{0.55}
\expandafter\def\csname rev@rintold@sna@world@ixs@coverage95\endcsname{0.90}
\expandafter\def\csname rev@rintold@sna@world@ixs@spl\endcsname{0.24}
\expandafter\def\csname rev@rintold@sna@world@total@coverage50\endcsname{0.07}
\expandafter\def\csname rev@rintold@sna@world@total@coverage80\endcsname{0.17}
\expandafter\def\csname rev@rintold@sna@world@total@coverage95\endcsname{0.23}
\expandafter\def\csname rev@rintold@sna@world@total@spl\endcsname{0.95}
\expandafter\def\csname rev@rmech@che@rolling@lift@bottomchange\endcsname{26}
\expandafter\def\csname rev@rmech@che@rolling@lift@persisth1\endcsname{105}
\expandafter\def\csname rev@rmech@che@rolling@lift@persisth2\endcsname{0}
\expandafter\def\csname rev@rmech@che@rolling@lift@persisth3\endcsname{0}
\expandafter\def\csname rev@rmech@che@rolling@lift@persisth4\endcsname{0}
\expandafter\def\csname rev@rmech@che@rolling@lift@persisth5\endcsname{0}
\expandafter\def\csname rev@rmech@che@rolling@lift@persisth6\endcsname{0}
\expandafter\def\csname rev@rmech@che@rolling@lift@persisth7\endcsname{0}
\expandafter\def\csname rev@rmech@che@rolling@lift@persisth8\endcsname{0}
\expandafter\def\csname rev@rmech@che@rolling@lift@totalchange\endcsname{44}
\expandafter\def\csname rev@rmech@che@rolling@world@bottomchange\endcsname{29}
\expandafter\def\csname rev@rmech@che@rolling@world@persisth1\endcsname{134}
\expandafter\def\csname rev@rmech@che@rolling@world@persisth2\endcsname{2}
\expandafter\def\csname rev@rmech@che@rolling@world@persisth3\endcsname{8}
\expandafter\def\csname rev@rmech@che@rolling@world@persisth4\endcsname{10}
\expandafter\def\csname rev@rmech@che@rolling@world@persisth5\endcsname{9}
\expandafter\def\csname rev@rmech@che@rolling@world@persisth6\endcsname{8}
\expandafter\def\csname rev@rmech@che@rolling@world@persisth7\endcsname{5}
\expandafter\def\csname rev@rmech@che@rolling@world@persisth8\endcsname{4}
\expandafter\def\csname rev@rmech@che@rolling@world@probeafterr2\endcsname{0.92}
\expandafter\def\csname rev@rmech@che@rolling@world@probebeforer2\endcsname{0.91}
\expandafter\def\csname rev@rmech@che@rolling@world@totalchange\endcsname{54}
\expandafter\def\csname rev@rmech@frat@final@lift@bottomchange\endcsname{34}
\expandafter\def\csname rev@rmech@frat@final@lift@persisth1\endcsname{42}
\expandafter\def\csname rev@rmech@frat@final@lift@persisth2\endcsname{0}
\expandafter\def\csname rev@rmech@frat@final@lift@persisth3\endcsname{0}
\expandafter\def\csname rev@rmech@frat@final@lift@persisth4\endcsname{0}
\expandafter\def\csname rev@rmech@frat@final@lift@persisth5\endcsname{0}
\expandafter\def\csname rev@rmech@frat@final@lift@persisth6\endcsname{0}
\expandafter\def\csname rev@rmech@frat@final@lift@persisth7\endcsname{0}
\expandafter\def\csname rev@rmech@frat@final@lift@persisth8\endcsname{0}
\expandafter\def\csname rev@rmech@frat@final@lift@totalchange\endcsname{16}
\expandafter\def\csname rev@rmech@frat@final@world@bottomchange\endcsname{36}
\expandafter\def\csname rev@rmech@frat@final@world@persisth1\endcsname{37}
\expandafter\def\csname rev@rmech@frat@final@world@persisth2\endcsname{\textminus{}2}
\expandafter\def\csname rev@rmech@frat@final@world@persisth3\endcsname{\textminus{}3}
\expandafter\def\csname rev@rmech@frat@final@world@persisth4\endcsname{\textminus{}2}
\expandafter\def\csname rev@rmech@frat@final@world@persisth5\endcsname{\textminus{}1}
\expandafter\def\csname rev@rmech@frat@final@world@persisth6\endcsname{\textminus{}1}
\expandafter\def\csname rev@rmech@frat@final@world@persisth7\endcsname{\textminus{}1}
\expandafter\def\csname rev@rmech@frat@final@world@persisth8\endcsname{\textminus{}1}
\expandafter\def\csname rev@rmech@frat@final@world@totalchange\endcsname{10}
\expandafter\def\csname rev@rmech@mfive@final@lift@bottomchange\endcsname{1}
\expandafter\def\csname rev@rmech@mfive@final@lift@totalchange\endcsname{5}
\expandafter\def\csname rev@rmech@mfive@final@world@bottomchange\endcsname{2}
\expandafter\def\csname rev@rmech@mfive@final@world@totalchange\endcsname{33}
\expandafter\def\csname rev@rmech@mfive@rolling@lift@bottomchange\endcsname{2}
\expandafter\def\csname rev@rmech@mfive@rolling@lift@totalchange\endcsname{29}
\expandafter\def\csname rev@rmech@mfive@rolling@world@bottomchange\endcsname{2}
\expandafter\def\csname rev@rmech@mfive@rolling@world@probeafterr2\endcsname{0.64}
\expandafter\def\csname rev@rmech@mfive@rolling@world@probebeforer2\endcsname{0.64}
\expandafter\def\csname rev@rmech@mfive@rolling@world@totalchange\endcsname{30}
\expandafter\def\csname rev@rmech@sdr@rolling@world@bottomchange\endcsname{38}
\expandafter\def\csname rev@rmech@sdr@rolling@world@persisth1\endcsname{681}
\expandafter\def\csname rev@rmech@sdr@rolling@world@persisth2\endcsname{52}
\expandafter\def\csname rev@rmech@sdr@rolling@world@persisth3\endcsname{28}
\expandafter\def\csname rev@rmech@sdr@rolling@world@persisth4\endcsname{15}
\expandafter\def\csname rev@rmech@sdr@rolling@world@persisth5\endcsname{15}
\expandafter\def\csname rev@rmech@sdr@rolling@world@persisth6\endcsname{13}
\expandafter\def\csname rev@rmech@sdr@rolling@world@persisth7\endcsname{12}
\expandafter\def\csname rev@rmech@sdr@rolling@world@persisth8\endcsname{12}
\expandafter\def\csname rev@rmech@sdr@rolling@world@probeafterr2\endcsname{0.87}
\expandafter\def\csname rev@rmech@sdr@rolling@world@probebeforer2\endcsname{0.86}
\expandafter\def\csname rev@rmech@sdr@rolling@world@totalchange\endcsname{2}
\expandafter\def\csname rev@rmech@sna@rolling@lift@bottomchange\endcsname{27}
\expandafter\def\csname rev@rmech@sna@rolling@lift@persisth1\endcsname{182}
\expandafter\def\csname rev@rmech@sna@rolling@lift@persisth2\endcsname{0}
\expandafter\def\csname rev@rmech@sna@rolling@lift@persisth3\endcsname{0}
\expandafter\def\csname rev@rmech@sna@rolling@lift@persisth4\endcsname{0}
\expandafter\def\csname rev@rmech@sna@rolling@lift@persisth5\endcsname{0}
\expandafter\def\csname rev@rmech@sna@rolling@lift@persisth6\endcsname{0}
\expandafter\def\csname rev@rmech@sna@rolling@lift@persisth7\endcsname{0}
\expandafter\def\csname rev@rmech@sna@rolling@lift@persisth8\endcsname{0}
\expandafter\def\csname rev@rmech@sna@rolling@lift@totalchange\endcsname{26}
\expandafter\def\csname rev@rmech@sna@rolling@world@bottomchange\endcsname{26}
\expandafter\def\csname rev@rmech@sna@rolling@world@persisth1\endcsname{230}
\expandafter\def\csname rev@rmech@sna@rolling@world@persisth2\endcsname{15}
\expandafter\def\csname rev@rmech@sna@rolling@world@persisth3\endcsname{15}
\expandafter\def\csname rev@rmech@sna@rolling@world@persisth4\endcsname{14}
\expandafter\def\csname rev@rmech@sna@rolling@world@persisth5\endcsname{5}
\expandafter\def\csname rev@rmech@sna@rolling@world@persisth6\endcsname{5}
\expandafter\def\csname rev@rmech@sna@rolling@world@persisth7\endcsname{4}
\expandafter\def\csname rev@rmech@sna@rolling@world@persisth8\endcsname{4}
\expandafter\def\csname rev@rmech@sna@rolling@world@probeafterr2\endcsname{0.87}
\expandafter\def\csname rev@rmech@sna@rolling@world@probebeforer2\endcsname{0.86}
\expandafter\def\csname rev@rmech@sna@rolling@world@totalchange\endcsname{24}
\expandafter\def\csname rev@rpair@ana@chronos@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@chronos@lgb@ixs@hi\endcsname{0.125}
\expandafter\def\csname rev@rpair@ana@chronos@lgb@ixs@lo\endcsname{0.075}
\expandafter\def\csname rev@rpair@ana@chronos@lgb@ixs@meandiff\endcsname{0.098}
\expandafter\def\csname rev@rpair@ana@chronos@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@chronos@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@chronos@lgb@total@hi\endcsname{0.317}
\expandafter\def\csname rev@rpair@ana@chronos@lgb@total@lo\endcsname{\textminus 0.083}
\expandafter\def\csname rev@rpair@ana@chronos@lgb@total@meandiff\endcsname{0.110}
\expandafter\def\csname rev@rpair@ana@chronos@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@chronos@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@chronos@world@ixs@hi\endcsname{0.098}
\expandafter\def\csname rev@rpair@ana@chronos@world@ixs@lo\endcsname{0.052}
\expandafter\def\csname rev@rpair@ana@chronos@world@ixs@meandiff\endcsname{0.073}
\expandafter\def\csname rev@rpair@ana@chronos@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@chronos@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@chronos@world@total@hi\endcsname{0.362}
\expandafter\def\csname rev@rpair@ana@chronos@world@total@lo\endcsname{\textminus 0.061}
\expandafter\def\csname rev@rpair@ana@chronos@world@total@meandiff\endcsname{0.154}
\expandafter\def\csname rev@rpair@ana@chronos@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@ens@lgb@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@ana@ens@lgb@ixs@hi\endcsname{0.010}
\expandafter\def\csname rev@rpair@ana@ens@lgb@ixs@lo\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rpair@ana@ens@lgb@ixs@meandiff\endcsname{0.003}
\expandafter\def\csname rev@rpair@ana@ens@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@ens@lgb@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@ana@ens@lgb@total@hi\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rpair@ana@ens@lgb@total@lo\endcsname{\textminus 0.162}
\expandafter\def\csname rev@rpair@ana@ens@lgb@total@meandiff\endcsname{\textminus 0.087}
\expandafter\def\csname rev@rpair@ana@ens@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@ens@world@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@ana@ens@world@ixs@hi\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rpair@ana@ens@world@ixs@lo\endcsname{\textminus 0.029}
\expandafter\def\csname rev@rpair@ana@ens@world@ixs@meandiff\endcsname{\textminus 0.022}
\expandafter\def\csname rev@rpair@ana@ens@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@ens@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@ana@ens@world@total@hi\endcsname{0.029}
\expandafter\def\csname rev@rpair@ana@ens@world@total@lo\endcsname{\textminus 0.117}
\expandafter\def\csname rev@rpair@ana@ens@world@total@meandiff\endcsname{\textminus 0.043}
\expandafter\def\csname rev@rpair@ana@ens@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@naive@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@naive@ixs@hi\endcsname{\textminus 0.323}
\expandafter\def\csname rev@rpair@ana@lgb@naive@ixs@lo\endcsname{\textminus 0.377}
\expandafter\def\csname rev@rpair@ana@lgb@naive@ixs@meandiff\endcsname{\textminus 0.351}
\expandafter\def\csname rev@rpair@ana@lgb@naive@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@naive@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@ana@lgb@naive@total@hi\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rpair@ana@lgb@naive@total@lo\endcsname{\textminus 2.507}
\expandafter\def\csname rev@rpair@ana@lgb@naive@total@meandiff\endcsname{\textminus 0.927}
\expandafter\def\csname rev@rpair@ana@lgb@naive@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@tfm@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@tfm@ixs@hi\endcsname{\textminus 0.065}
\expandafter\def\csname rev@rpair@ana@lgb@tfm@ixs@lo\endcsname{\textminus 0.114}
\expandafter\def\csname rev@rpair@ana@lgb@tfm@ixs@meandiff\endcsname{\textminus 0.087}
\expandafter\def\csname rev@rpair@ana@lgb@tfm@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@tfm@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@lgb@tfm@total@hi\endcsname{0.116}
\expandafter\def\csname rev@rpair@ana@lgb@tfm@total@lo\endcsname{\textminus 0.178}
\expandafter\def\csname rev@rpair@ana@lgb@tfm@total@meandiff\endcsname{\textminus 0.031}
\expandafter\def\csname rev@rpair@ana@lgb@tfm@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@tfmplan@ixs@awins\endcsname{5}
\expandafter\def\csname rev@rpair@ana@lgb@tfmplan@ixs@hi\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rpair@ana@lgb@tfmplan@ixs@lo\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rpair@ana@lgb@tfmplan@ixs@meandiff\endcsname{\textminus 0.033}
\expandafter\def\csname rev@rpair@ana@lgb@tfmplan@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@tfmplan@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@lgb@tfmplan@total@hi\endcsname{0.150}
\expandafter\def\csname rev@rpair@ana@lgb@tfmplan@total@lo\endcsname{\textminus 0.087}
\expandafter\def\csname rev@rpair@ana@lgb@tfmplan@total@meandiff\endcsname{0.021}
\expandafter\def\csname rev@rpair@ana@lgb@tfmplan@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@tft@ixs@awins\endcsname{5}
\expandafter\def\csname rev@rpair@ana@lgb@tft@ixs@hi\endcsname{\textminus 0.032}
\expandafter\def\csname rev@rpair@ana@lgb@tft@ixs@lo\endcsname{\textminus 0.060}
\expandafter\def\csname rev@rpair@ana@lgb@tft@ixs@meandiff\endcsname{\textminus 0.047}
\expandafter\def\csname rev@rpair@ana@lgb@tft@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@tft@total@awins\endcsname{3}
\expandafter\def\csname rev@rpair@ana@lgb@tft@total@hi\endcsname{0.079}
\expandafter\def\csname rev@rpair@ana@lgb@tft@total@lo\endcsname{\textminus 0.486}
\expandafter\def\csname rev@rpair@ana@lgb@tft@total@meandiff\endcsname{\textminus 0.188}
\expandafter\def\csname rev@rpair@ana@lgb@tft@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@world@ixs@awins\endcsname{5}
\expandafter\def\csname rev@rpair@ana@lgb@world@ixs@hi\endcsname{\textminus 0.018}
\expandafter\def\csname rev@rpair@ana@lgb@world@ixs@lo\endcsname{\textminus 0.031}
\expandafter\def\csname rev@rpair@ana@lgb@world@ixs@meandiff\endcsname{\textminus 0.025}
\expandafter\def\csname rev@rpair@ana@lgb@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lgb@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@ana@lgb@world@total@hi\endcsname{0.146}
\expandafter\def\csname rev@rpair@ana@lgb@world@total@lo\endcsname{\textminus 0.097}
\expandafter\def\csname rev@rpair@ana@lgb@world@total@meandiff\endcsname{0.043}
\expandafter\def\csname rev@rpair@ana@lgb@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lift@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@lift@lgb@ixs@hi\endcsname{0.042}
\expandafter\def\csname rev@rpair@ana@lift@lgb@ixs@lo\endcsname{0.021}
\expandafter\def\csname rev@rpair@ana@lift@lgb@ixs@meandiff\endcsname{0.031}
\expandafter\def\csname rev@rpair@ana@lift@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lift@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@lift@lgb@total@hi\endcsname{0.158}
\expandafter\def\csname rev@rpair@ana@lift@lgb@total@lo\endcsname{\textminus 0.119}
\expandafter\def\csname rev@rpair@ana@lift@lgb@total@meandiff\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rpair@ana@lift@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lift@world@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@ana@lift@world@ixs@hi\endcsname{0.013}
\expandafter\def\csname rev@rpair@ana@lift@world@ixs@lo\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rpair@ana@lift@world@ixs@meandiff\endcsname{0.006}
\expandafter\def\csname rev@rpair@ana@lift@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@lift@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@lift@world@total@hi\endcsname{0.105}
\expandafter\def\csname rev@rpair@ana@lift@world@total@lo\endcsname{\textminus 0.022}
\expandafter\def\csname rev@rpair@ana@lift@world@total@meandiff\endcsname{0.043}
\expandafter\def\csname rev@rpair@ana@lift@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@naive@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@naive@world@ixs@hi\endcsname{0.347}
\expandafter\def\csname rev@rpair@ana@naive@world@ixs@lo\endcsname{0.304}
\expandafter\def\csname rev@rpair@ana@naive@world@ixs@meandiff\endcsname{0.326}
\expandafter\def\csname rev@rpair@ana@naive@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@naive@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@naive@world@total@hi\endcsname{2.542}
\expandafter\def\csname rev@rpair@ana@naive@world@total@lo\endcsname{0.029}
\expandafter\def\csname rev@rpair@ana@naive@world@total@meandiff\endcsname{0.970}
\expandafter\def\csname rev@rpair@ana@naive@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@tfm@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@tfm@world@ixs@hi\endcsname{0.085}
\expandafter\def\csname rev@rpair@ana@tfm@world@ixs@lo\endcsname{0.042}
\expandafter\def\csname rev@rpair@ana@tfm@world@ixs@meandiff\endcsname{0.062}
\expandafter\def\csname rev@rpair@ana@tfm@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@tfm@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@tfm@world@total@hi\endcsname{0.226}
\expandafter\def\csname rev@rpair@ana@tfm@world@total@lo\endcsname{\textminus 0.086}
\expandafter\def\csname rev@rpair@ana@tfm@world@total@meandiff\endcsname{0.074}
\expandafter\def\csname rev@rpair@ana@tfm@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@tfmplan@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@tfmplan@world@ixs@hi\endcsname{0.020}
\expandafter\def\csname rev@rpair@ana@tfmplan@world@ixs@lo\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rpair@ana@tfmplan@world@ixs@meandiff\endcsname{0.008}
\expandafter\def\csname rev@rpair@ana@tfmplan@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@tfmplan@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@tfmplan@world@total@hi\endcsname{0.150}
\expandafter\def\csname rev@rpair@ana@tfmplan@world@total@lo\endcsname{\textminus 0.111}
\expandafter\def\csname rev@rpair@ana@tfmplan@world@total@meandiff\endcsname{0.023}
\expandafter\def\csname rev@rpair@ana@tfmplan@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@tft@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@tft@world@ixs@hi\endcsname{0.035}
\expandafter\def\csname rev@rpair@ana@tft@world@ixs@lo\endcsname{0.007}
\expandafter\def\csname rev@rpair@ana@tft@world@ixs@meandiff\endcsname{0.022}
\expandafter\def\csname rev@rpair@ana@tft@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@ana@tft@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@ana@tft@world@total@hi\endcsname{0.563}
\expandafter\def\csname rev@rpair@ana@tft@world@total@lo\endcsname{\textminus 0.080}
\expandafter\def\csname rev@rpair@ana@tft@world@total@meandiff\endcsname{0.231}
\expandafter\def\csname rev@rpair@ana@tft@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@chronos@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@chronos@lgb@ixs@hi\endcsname{0.192}
\expandafter\def\csname rev@rpair@bjc@chronos@lgb@ixs@lo\endcsname{0.075}
\expandafter\def\csname rev@rpair@bjc@chronos@lgb@ixs@meandiff\endcsname{0.123}
\expandafter\def\csname rev@rpair@bjc@chronos@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@chronos@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@chronos@lgb@total@hi\endcsname{0.832}
\expandafter\def\csname rev@rpair@bjc@chronos@lgb@total@lo\endcsname{0.056}
\expandafter\def\csname rev@rpair@bjc@chronos@lgb@total@meandiff\endcsname{0.367}
\expandafter\def\csname rev@rpair@bjc@chronos@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@chronos@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@chronos@world@ixs@hi\endcsname{0.147}
\expandafter\def\csname rev@rpair@bjc@chronos@world@ixs@lo\endcsname{0.005}
\expandafter\def\csname rev@rpair@bjc@chronos@world@ixs@meandiff\endcsname{0.071}
\expandafter\def\csname rev@rpair@bjc@chronos@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@chronos@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@chronos@world@total@hi\endcsname{0.794}
\expandafter\def\csname rev@rpair@bjc@chronos@world@total@lo\endcsname{\textminus 0.041}
\expandafter\def\csname rev@rpair@bjc@chronos@world@total@meandiff\endcsname{0.284}
\expandafter\def\csname rev@rpair@bjc@chronos@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@ens@lgb@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@bjc@ens@lgb@ixs@hi\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rpair@bjc@ens@lgb@ixs@lo\endcsname{\textminus 0.026}
\expandafter\def\csname rev@rpair@bjc@ens@lgb@ixs@meandiff\endcsname{\textminus 0.020}
\expandafter\def\csname rev@rpair@bjc@ens@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@ens@lgb@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@bjc@ens@lgb@total@hi\endcsname{0.107}
\expandafter\def\csname rev@rpair@bjc@ens@lgb@total@lo\endcsname{\textminus 0.109}
\expandafter\def\csname rev@rpair@bjc@ens@lgb@total@meandiff\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rpair@bjc@ens@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@ens@world@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@ens@world@ixs@hi\endcsname{\textminus 0.032}
\expandafter\def\csname rev@rpair@bjc@ens@world@ixs@lo\endcsname{\textminus 0.132}
\expandafter\def\csname rev@rpair@bjc@ens@world@ixs@meandiff\endcsname{\textminus 0.071}
\expandafter\def\csname rev@rpair@bjc@ens@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@ens@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@ens@world@total@hi\endcsname{0.072}
\expandafter\def\csname rev@rpair@bjc@ens@world@total@lo\endcsname{\textminus 0.271}
\expandafter\def\csname rev@rpair@bjc@ens@world@total@meandiff\endcsname{\textminus 0.088}
\expandafter\def\csname rev@rpair@bjc@ens@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@naive@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@naive@ixs@hi\endcsname{\textminus 0.412}
\expandafter\def\csname rev@rpair@bjc@lgb@naive@ixs@lo\endcsname{\textminus 0.542}
\expandafter\def\csname rev@rpair@bjc@lgb@naive@ixs@meandiff\endcsname{\textminus 0.474}
\expandafter\def\csname rev@rpair@bjc@lgb@naive@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@naive@total@awins\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@naive@total@hi\endcsname{\textminus 0.521}
\expandafter\def\csname rev@rpair@bjc@lgb@naive@total@lo\endcsname{\textminus 1.252}
\expandafter\def\csname rev@rpair@bjc@lgb@naive@total@meandiff\endcsname{\textminus 0.860}
\expandafter\def\csname rev@rpair@bjc@lgb@naive@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@tfm@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@tfm@ixs@hi\endcsname{\textminus 0.063}
\expandafter\def\csname rev@rpair@bjc@lgb@tfm@ixs@lo\endcsname{\textminus 0.173}
\expandafter\def\csname rev@rpair@bjc@lgb@tfm@ixs@meandiff\endcsname{\textminus 0.108}
\expandafter\def\csname rev@rpair@bjc@lgb@tfm@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@tfm@total@awins\endcsname{3}
\expandafter\def\csname rev@rpair@bjc@lgb@tfm@total@hi\endcsname{\textminus 0.043}
\expandafter\def\csname rev@rpair@bjc@lgb@tfm@total@lo\endcsname{\textminus 0.836}
\expandafter\def\csname rev@rpair@bjc@lgb@tfm@total@meandiff\endcsname{\textminus 0.368}
\expandafter\def\csname rev@rpair@bjc@lgb@tfm@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@tfmplan@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@bjc@lgb@tfmplan@ixs@hi\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rpair@bjc@lgb@tfmplan@ixs@lo\endcsname{\textminus 0.076}
\expandafter\def\csname rev@rpair@bjc@lgb@tfmplan@ixs@meandiff\endcsname{\textminus 0.031}
\expandafter\def\csname rev@rpair@bjc@lgb@tfmplan@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@tfmplan@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@bjc@lgb@tfmplan@total@hi\endcsname{\textminus 0.000}
\expandafter\def\csname rev@rpair@bjc@lgb@tfmplan@total@lo\endcsname{\textminus 0.568}
\expandafter\def\csname rev@rpair@bjc@lgb@tfmplan@total@meandiff\endcsname{\textminus 0.237}
\expandafter\def\csname rev@rpair@bjc@lgb@tfmplan@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@tft@ixs@awins\endcsname{5}
\expandafter\def\csname rev@rpair@bjc@lgb@tft@ixs@hi\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rpair@bjc@lgb@tft@ixs@lo\endcsname{\textminus 0.119}
\expandafter\def\csname rev@rpair@bjc@lgb@tft@ixs@meandiff\endcsname{\textminus 0.071}
\expandafter\def\csname rev@rpair@bjc@lgb@tft@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@tft@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@bjc@lgb@tft@total@hi\endcsname{\textminus 0.035}
\expandafter\def\csname rev@rpair@bjc@lgb@tft@total@lo\endcsname{\textminus 0.568}
\expandafter\def\csname rev@rpair@bjc@lgb@tft@total@meandiff\endcsname{\textminus 0.263}
\expandafter\def\csname rev@rpair@bjc@lgb@tft@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@world@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@bjc@lgb@world@ixs@hi\endcsname{\textminus 0.013}
\expandafter\def\csname rev@rpair@bjc@lgb@world@ixs@lo\endcsname{\textminus 0.110}
\expandafter\def\csname rev@rpair@bjc@lgb@world@ixs@meandiff\endcsname{\textminus 0.051}
\expandafter\def\csname rev@rpair@bjc@lgb@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lgb@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@lgb@world@total@hi\endcsname{0.003}
\expandafter\def\csname rev@rpair@bjc@lgb@world@total@lo\endcsname{\textminus 0.186}
\expandafter\def\csname rev@rpair@bjc@lgb@world@total@meandiff\endcsname{\textminus 0.083}
\expandafter\def\csname rev@rpair@bjc@lgb@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lift@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@lift@lgb@ixs@hi\endcsname{0.024}
\expandafter\def\csname rev@rpair@bjc@lift@lgb@ixs@lo\endcsname{0.001}
\expandafter\def\csname rev@rpair@bjc@lift@lgb@ixs@meandiff\endcsname{0.011}
\expandafter\def\csname rev@rpair@bjc@lift@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lift@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@lift@lgb@total@hi\endcsname{0.205}
\expandafter\def\csname rev@rpair@bjc@lift@lgb@total@lo\endcsname{\textminus 0.083}
\expandafter\def\csname rev@rpair@bjc@lift@lgb@total@meandiff\endcsname{0.055}
\expandafter\def\csname rev@rpair@bjc@lift@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lift@world@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@bjc@lift@world@ixs@hi\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rpair@bjc@lift@world@ixs@lo\endcsname{\textminus 0.094}
\expandafter\def\csname rev@rpair@bjc@lift@world@ixs@meandiff\endcsname{\textminus 0.040}
\expandafter\def\csname rev@rpair@bjc@lift@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@lift@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@lift@world@total@hi\endcsname{0.162}
\expandafter\def\csname rev@rpair@bjc@lift@world@total@lo\endcsname{\textminus 0.242}
\expandafter\def\csname rev@rpair@bjc@lift@world@total@meandiff\endcsname{\textminus 0.028}
\expandafter\def\csname rev@rpair@bjc@lift@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@naive@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@naive@world@ixs@hi\endcsname{0.497}
\expandafter\def\csname rev@rpair@bjc@naive@world@ixs@lo\endcsname{0.348}
\expandafter\def\csname rev@rpair@bjc@naive@world@ixs@meandiff\endcsname{0.423}
\expandafter\def\csname rev@rpair@bjc@naive@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@naive@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@naive@world@total@hi\endcsname{1.218}
\expandafter\def\csname rev@rpair@bjc@naive@world@total@lo\endcsname{0.400}
\expandafter\def\csname rev@rpair@bjc@naive@world@total@meandiff\endcsname{0.777}
\expandafter\def\csname rev@rpair@bjc@naive@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@tfm@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@tfm@world@ixs@hi\endcsname{0.135}
\expandafter\def\csname rev@rpair@bjc@tfm@world@ixs@lo\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rpair@bjc@tfm@world@ixs@meandiff\endcsname{0.056}
\expandafter\def\csname rev@rpair@bjc@tfm@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@tfm@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@tfm@world@total@hi\endcsname{0.787}
\expandafter\def\csname rev@rpair@bjc@tfm@world@total@lo\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rpair@bjc@tfm@world@total@meandiff\endcsname{0.285}
\expandafter\def\csname rev@rpair@bjc@tfm@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@tfmplan@world@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@bjc@tfmplan@world@ixs@hi\endcsname{0.040}
\expandafter\def\csname rev@rpair@bjc@tfmplan@world@ixs@lo\endcsname{\textminus 0.091}
\expandafter\def\csname rev@rpair@bjc@tfmplan@world@ixs@meandiff\endcsname{\textminus 0.020}
\expandafter\def\csname rev@rpair@bjc@tfmplan@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@tfmplan@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@tfmplan@world@total@hi\endcsname{0.512}
\expandafter\def\csname rev@rpair@bjc@tfmplan@world@total@lo\endcsname{\textminus 0.092}
\expandafter\def\csname rev@rpair@bjc@tfmplan@world@total@meandiff\endcsname{0.154}
\expandafter\def\csname rev@rpair@bjc@tfmplan@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@tft@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@tft@world@ixs@hi\endcsname{0.079}
\expandafter\def\csname rev@rpair@bjc@tft@world@ixs@lo\endcsname{\textminus 0.050}
\expandafter\def\csname rev@rpair@bjc@tft@world@ixs@meandiff\endcsname{0.020}
\expandafter\def\csname rev@rpair@bjc@tft@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@bjc@tft@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@bjc@tft@world@total@hi\endcsname{0.546}
\expandafter\def\csname rev@rpair@bjc@tft@world@total@lo\endcsname{\textminus 0.089}
\expandafter\def\csname rev@rpair@bjc@tft@world@total@meandiff\endcsname{0.180}
\expandafter\def\csname rev@rpair@bjc@tft@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@chronos@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@che@chronos@lgb@ixs@hi\endcsname{0.188}
\expandafter\def\csname rev@rpair@che@chronos@lgb@ixs@lo\endcsname{0.092}
\expandafter\def\csname rev@rpair@che@chronos@lgb@ixs@meandiff\endcsname{0.139}
\expandafter\def\csname rev@rpair@che@chronos@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@chronos@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@che@chronos@lgb@total@hi\endcsname{0.477}
\expandafter\def\csname rev@rpair@che@chronos@lgb@total@lo\endcsname{0.194}
\expandafter\def\csname rev@rpair@che@chronos@lgb@total@meandiff\endcsname{0.334}
\expandafter\def\csname rev@rpair@che@chronos@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@chronos@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@che@chronos@world@ixs@hi\endcsname{0.143}
\expandafter\def\csname rev@rpair@che@chronos@world@ixs@lo\endcsname{\textminus 3.090}
\expandafter\def\csname rev@rpair@che@chronos@world@ixs@meandiff\endcsname{\textminus 0.951}
\expandafter\def\csname rev@rpair@che@chronos@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@chronos@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@che@chronos@world@total@hi\endcsname{0.453}
\expandafter\def\csname rev@rpair@che@chronos@world@total@lo\endcsname{\textminus 0.077}
\expandafter\def\csname rev@rpair@che@chronos@world@total@meandiff\endcsname{0.205}
\expandafter\def\csname rev@rpair@che@chronos@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@ens@lgb@ixs@awins\endcsname{3}
\expandafter\def\csname rev@rpair@che@ens@lgb@ixs@hi\endcsname{0.989}
\expandafter\def\csname rev@rpair@che@ens@lgb@ixs@lo\endcsname{\textminus 0.035}
\expandafter\def\csname rev@rpair@che@ens@lgb@ixs@meandiff\endcsname{0.311}
\expandafter\def\csname rev@rpair@che@ens@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@ens@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@che@ens@lgb@total@hi\endcsname{0.060}
\expandafter\def\csname rev@rpair@che@ens@lgb@total@lo\endcsname{\textminus 0.243}
\expandafter\def\csname rev@rpair@che@ens@lgb@total@meandiff\endcsname{\textminus 0.085}
\expandafter\def\csname rev@rpair@che@ens@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@ens@world@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@che@ens@world@ixs@hi\endcsname{\textminus 0.042}
\expandafter\def\csname rev@rpair@che@ens@world@ixs@lo\endcsname{\textminus 2.223}
\expandafter\def\csname rev@rpair@che@ens@world@ixs@meandiff\endcsname{\textminus 0.779}
\expandafter\def\csname rev@rpair@che@ens@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@ens@world@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@che@ens@world@total@hi\endcsname{\textminus 0.034}
\expandafter\def\csname rev@rpair@che@ens@world@total@lo\endcsname{\textminus 0.508}
\expandafter\def\csname rev@rpair@che@ens@world@total@meandiff\endcsname{\textminus 0.214}
\expandafter\def\csname rev@rpair@che@ens@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@naive@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@naive@ixs@hi\endcsname{\textminus 0.460}
\expandafter\def\csname rev@rpair@che@lgb@naive@ixs@lo\endcsname{\textminus 0.519}
\expandafter\def\csname rev@rpair@che@lgb@naive@ixs@meandiff\endcsname{\textminus 0.494}
\expandafter\def\csname rev@rpair@che@lgb@naive@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@naive@total@awins\endcsname{5}
\expandafter\def\csname rev@rpair@che@lgb@naive@total@hi\endcsname{\textminus 0.390}
\expandafter\def\csname rev@rpair@che@lgb@naive@total@lo\endcsname{\textminus 1.153}
\expandafter\def\csname rev@rpair@che@lgb@naive@total@meandiff\endcsname{\textminus 0.719}
\expandafter\def\csname rev@rpair@che@lgb@naive@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@tfm@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@tfm@ixs@hi\endcsname{\textminus 0.081}
\expandafter\def\csname rev@rpair@che@lgb@tfm@ixs@lo\endcsname{\textminus 0.174}
\expandafter\def\csname rev@rpair@che@lgb@tfm@ixs@meandiff\endcsname{\textminus 0.126}
\expandafter\def\csname rev@rpair@che@lgb@tfm@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@tfm@total@awins\endcsname{3}
\expandafter\def\csname rev@rpair@che@lgb@tfm@total@hi\endcsname{\textminus 0.091}
\expandafter\def\csname rev@rpair@che@lgb@tfm@total@lo\endcsname{\textminus 0.437}
\expandafter\def\csname rev@rpair@che@lgb@tfm@total@meandiff\endcsname{\textminus 0.262}
\expandafter\def\csname rev@rpair@che@lgb@tfm@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@tfmplan@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@che@lgb@tfmplan@ixs@hi\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rpair@che@lgb@tfmplan@ixs@lo\endcsname{\textminus 0.073}
\expandafter\def\csname rev@rpair@che@lgb@tfmplan@ixs@meandiff\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rpair@che@lgb@tfmplan@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@tfmplan@total@awins\endcsname{3}
\expandafter\def\csname rev@rpair@che@lgb@tfmplan@total@hi\endcsname{0.040}
\expandafter\def\csname rev@rpair@che@lgb@tfmplan@total@lo\endcsname{\textminus 0.303}
\expandafter\def\csname rev@rpair@che@lgb@tfmplan@total@meandiff\endcsname{\textminus 0.128}
\expandafter\def\csname rev@rpair@che@lgb@tfmplan@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@tft@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@che@lgb@tft@ixs@hi\endcsname{\textminus 0.031}
\expandafter\def\csname rev@rpair@che@lgb@tft@ixs@lo\endcsname{\textminus 0.115}
\expandafter\def\csname rev@rpair@che@lgb@tft@ixs@meandiff\endcsname{\textminus 0.074}
\expandafter\def\csname rev@rpair@che@lgb@tft@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@tft@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@che@lgb@tft@total@hi\endcsname{0.107}
\expandafter\def\csname rev@rpair@che@lgb@tft@total@lo\endcsname{\textminus 0.160}
\expandafter\def\csname rev@rpair@che@lgb@tft@total@meandiff\endcsname{\textminus 0.025}
\expandafter\def\csname rev@rpair@che@lgb@tft@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@world@ixs@awins\endcsname{3}
\expandafter\def\csname rev@rpair@che@lgb@world@ixs@hi\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rpair@che@lgb@world@ixs@lo\endcsname{\textminus 3.216}
\expandafter\def\csname rev@rpair@che@lgb@world@ixs@meandiff\endcsname{\textminus 1.090}
\expandafter\def\csname rev@rpair@che@lgb@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lgb@world@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@che@lgb@world@total@hi\endcsname{0.020}
\expandafter\def\csname rev@rpair@che@lgb@world@total@lo\endcsname{\textminus 0.310}
\expandafter\def\csname rev@rpair@che@lgb@world@total@meandiff\endcsname{\textminus 0.129}
\expandafter\def\csname rev@rpair@che@lgb@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lift@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@che@lift@lgb@ixs@hi\endcsname{1.433}
\expandafter\def\csname rev@rpair@che@lift@lgb@ixs@lo\endcsname{0.012}
\expandafter\def\csname rev@rpair@che@lift@lgb@ixs@meandiff\endcsname{0.496}
\expandafter\def\csname rev@rpair@che@lift@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lift@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@che@lift@lgb@total@hi\endcsname{0.337}
\expandafter\def\csname rev@rpair@che@lift@lgb@total@lo\endcsname{0.019}
\expandafter\def\csname rev@rpair@che@lift@lgb@total@meandiff\endcsname{0.161}
\expandafter\def\csname rev@rpair@che@lift@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lift@world@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@che@lift@world@ixs@hi\endcsname{0.009}
\expandafter\def\csname rev@rpair@che@lift@world@ixs@lo\endcsname{\textminus 1.779}
\expandafter\def\csname rev@rpair@che@lift@world@ixs@meandiff\endcsname{\textminus 0.594}
\expandafter\def\csname rev@rpair@che@lift@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@lift@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@che@lift@world@total@hi\endcsname{0.298}
\expandafter\def\csname rev@rpair@che@lift@world@total@lo\endcsname{\textminus 0.150}
\expandafter\def\csname rev@rpair@che@lift@world@total@meandiff\endcsname{0.032}
\expandafter\def\csname rev@rpair@che@lift@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@naive@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@che@naive@world@ixs@hi\endcsname{0.482}
\expandafter\def\csname rev@rpair@che@naive@world@ixs@lo\endcsname{\textminus 2.712}
\expandafter\def\csname rev@rpair@che@naive@world@ixs@meandiff\endcsname{\textminus 0.596}
\expandafter\def\csname rev@rpair@che@naive@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@naive@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@che@naive@world@total@hi\endcsname{1.089}
\expandafter\def\csname rev@rpair@che@naive@world@total@lo\endcsname{0.207}
\expandafter\def\csname rev@rpair@che@naive@world@total@meandiff\endcsname{0.590}
\expandafter\def\csname rev@rpair@che@naive@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@tfm@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@che@tfm@world@ixs@hi\endcsname{0.128}
\expandafter\def\csname rev@rpair@che@tfm@world@ixs@lo\endcsname{\textminus 3.105}
\expandafter\def\csname rev@rpair@che@tfm@world@ixs@meandiff\endcsname{\textminus 0.964}
\expandafter\def\csname rev@rpair@che@tfm@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@tfm@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@che@tfm@world@total@hi\endcsname{0.404}
\expandafter\def\csname rev@rpair@che@tfm@world@total@lo\endcsname{\textminus 0.178}
\expandafter\def\csname rev@rpair@che@tfm@world@total@meandiff\endcsname{0.134}
\expandafter\def\csname rev@rpair@che@tfm@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@tfmplan@world@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@che@tfmplan@world@ixs@hi\endcsname{0.027}
\expandafter\def\csname rev@rpair@che@tfmplan@world@ixs@lo\endcsname{\textminus 3.186}
\expandafter\def\csname rev@rpair@che@tfmplan@world@ixs@meandiff\endcsname{\textminus 1.054}
\expandafter\def\csname rev@rpair@che@tfmplan@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@tfmplan@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@che@tfmplan@world@total@hi\endcsname{0.221}
\expandafter\def\csname rev@rpair@che@tfmplan@world@total@lo\endcsname{\textminus 0.270}
\expandafter\def\csname rev@rpair@che@tfmplan@world@total@meandiff\endcsname{\textminus 0.000}
\expandafter\def\csname rev@rpair@che@tfmplan@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@tft@world@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@che@tft@world@ixs@hi\endcsname{0.067}
\expandafter\def\csname rev@rpair@che@tft@world@ixs@lo\endcsname{\textminus 3.143}
\expandafter\def\csname rev@rpair@che@tft@world@ixs@meandiff\endcsname{\textminus 1.016}
\expandafter\def\csname rev@rpair@che@tft@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@che@tft@world@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@che@tft@world@total@hi\endcsname{0.077}
\expandafter\def\csname rev@rpair@che@tft@world@total@lo\endcsname{\textminus 0.297}
\expandafter\def\csname rev@rpair@che@tft@world@total@meandiff\endcsname{\textminus 0.104}
\expandafter\def\csname rev@rpair@che@tft@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@frat@chronos@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@chronos@lgb@ixs@hi\endcsname{0.241}
\expandafter\def\csname rev@rpair@frat@chronos@lgb@ixs@lo\endcsname{0.150}
\expandafter\def\csname rev@rpair@frat@chronos@lgb@ixs@meandiff\endcsname{0.208}
\expandafter\def\csname rev@rpair@frat@chronos@lgb@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@chronos@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@chronos@lgb@total@hi\endcsname{0.405}
\expandafter\def\csname rev@rpair@frat@chronos@lgb@total@lo\endcsname{0.085}
\expandafter\def\csname rev@rpair@frat@chronos@lgb@total@meandiff\endcsname{0.245}
\expandafter\def\csname rev@rpair@frat@chronos@lgb@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@chronos@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@chronos@world@ixs@hi\endcsname{0.228}
\expandafter\def\csname rev@rpair@frat@chronos@world@ixs@lo\endcsname{0.119}
\expandafter\def\csname rev@rpair@frat@chronos@world@ixs@meandiff\endcsname{0.183}
\expandafter\def\csname rev@rpair@frat@chronos@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@chronos@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@chronos@world@total@hi\endcsname{0.323}
\expandafter\def\csname rev@rpair@frat@chronos@world@total@lo\endcsname{\textminus 0.028}
\expandafter\def\csname rev@rpair@frat@chronos@world@total@meandiff\endcsname{0.147}
\expandafter\def\csname rev@rpair@frat@chronos@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@ens@lgb@ixs@awins\endcsname{3}
\expandafter\def\csname rev@rpair@frat@ens@lgb@ixs@hi\endcsname{\textminus 0.013}
\expandafter\def\csname rev@rpair@frat@ens@lgb@ixs@lo\endcsname{\textminus 0.028}
\expandafter\def\csname rev@rpair@frat@ens@lgb@ixs@meandiff\endcsname{\textminus 0.021}
\expandafter\def\csname rev@rpair@frat@ens@lgb@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@ens@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@ens@lgb@total@hi\endcsname{0.027}
\expandafter\def\csname rev@rpair@frat@ens@lgb@total@lo\endcsname{\textminus 0.059}
\expandafter\def\csname rev@rpair@frat@ens@lgb@total@meandiff\endcsname{\textminus 0.023}
\expandafter\def\csname rev@rpair@frat@ens@lgb@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@ens@world@ixs@awins\endcsname{3}
\expandafter\def\csname rev@rpair@frat@ens@world@ixs@hi\endcsname{\textminus 0.031}
\expandafter\def\csname rev@rpair@frat@ens@world@ixs@lo\endcsname{\textminus 0.061}
\expandafter\def\csname rev@rpair@frat@ens@world@ixs@meandiff\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rpair@frat@ens@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@ens@world@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@frat@ens@world@total@hi\endcsname{\textminus 0.062}
\expandafter\def\csname rev@rpair@frat@ens@world@total@lo\endcsname{\textminus 0.168}
\expandafter\def\csname rev@rpair@frat@ens@world@total@meandiff\endcsname{\textminus 0.120}
\expandafter\def\csname rev@rpair@frat@ens@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@naive@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@naive@ixs@hi\endcsname{\textminus 0.440}
\expandafter\def\csname rev@rpair@frat@lgb@naive@ixs@lo\endcsname{\textminus 0.591}
\expandafter\def\csname rev@rpair@frat@lgb@naive@ixs@meandiff\endcsname{\textminus 0.507}
\expandafter\def\csname rev@rpair@frat@lgb@naive@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@naive@total@awins\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@naive@total@hi\endcsname{\textminus 0.439}
\expandafter\def\csname rev@rpair@frat@lgb@naive@total@lo\endcsname{\textminus 0.810}
\expandafter\def\csname rev@rpair@frat@lgb@naive@total@meandiff\endcsname{\textminus 0.604}
\expandafter\def\csname rev@rpair@frat@lgb@naive@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@tfm@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@tfm@ixs@hi\endcsname{\textminus 0.152}
\expandafter\def\csname rev@rpair@frat@lgb@tfm@ixs@lo\endcsname{\textminus 0.242}
\expandafter\def\csname rev@rpair@frat@lgb@tfm@ixs@meandiff\endcsname{\textminus 0.205}
\expandafter\def\csname rev@rpair@frat@lgb@tfm@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@tfm@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@lgb@tfm@total@hi\endcsname{\textminus 0.052}
\expandafter\def\csname rev@rpair@frat@lgb@tfm@total@lo\endcsname{\textminus 0.311}
\expandafter\def\csname rev@rpair@frat@lgb@tfm@total@meandiff\endcsname{\textminus 0.181}
\expandafter\def\csname rev@rpair@frat@lgb@tfm@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@tfmplan@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@frat@lgb@tfmplan@ixs@hi\endcsname{0.004}
\expandafter\def\csname rev@rpair@frat@lgb@tfmplan@ixs@lo\endcsname{\textminus 0.029}
\expandafter\def\csname rev@rpair@frat@lgb@tfmplan@ixs@meandiff\endcsname{\textminus 0.009}
\expandafter\def\csname rev@rpair@frat@lgb@tfmplan@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@tfmplan@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@lgb@tfmplan@total@hi\endcsname{0.106}
\expandafter\def\csname rev@rpair@frat@lgb@tfmplan@total@lo\endcsname{\textminus 0.038}
\expandafter\def\csname rev@rpair@frat@lgb@tfmplan@total@meandiff\endcsname{0.033}
\expandafter\def\csname rev@rpair@frat@lgb@tfmplan@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@tft@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@tft@ixs@hi\endcsname{\textminus 0.048}
\expandafter\def\csname rev@rpair@frat@lgb@tft@ixs@lo\endcsname{\textminus 0.110}
\expandafter\def\csname rev@rpair@frat@lgb@tft@ixs@meandiff\endcsname{\textminus 0.082}
\expandafter\def\csname rev@rpair@frat@lgb@tft@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@tft@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@frat@lgb@tft@total@hi\endcsname{0.026}
\expandafter\def\csname rev@rpair@frat@lgb@tft@total@lo\endcsname{\textminus 0.206}
\expandafter\def\csname rev@rpair@frat@lgb@tft@total@meandiff\endcsname{\textminus 0.065}
\expandafter\def\csname rev@rpair@frat@lgb@tft@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@world@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@frat@lgb@world@ixs@hi\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rpair@frat@lgb@world@ixs@lo\endcsname{\textminus 0.039}
\expandafter\def\csname rev@rpair@frat@lgb@world@ixs@meandiff\endcsname{\textminus 0.025}
\expandafter\def\csname rev@rpair@frat@lgb@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lgb@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@frat@lgb@world@total@hi\endcsname{\textminus 0.026}
\expandafter\def\csname rev@rpair@frat@lgb@world@total@lo\endcsname{\textminus 0.169}
\expandafter\def\csname rev@rpair@frat@lgb@world@total@meandiff\endcsname{\textminus 0.097}
\expandafter\def\csname rev@rpair@frat@lgb@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lift@lgb@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@frat@lift@lgb@ixs@hi\endcsname{0.048}
\expandafter\def\csname rev@rpair@frat@lift@lgb@ixs@lo\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rpair@frat@lift@lgb@ixs@meandiff\endcsname{0.020}
\expandafter\def\csname rev@rpair@frat@lift@lgb@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lift@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@lift@lgb@total@hi\endcsname{0.190}
\expandafter\def\csname rev@rpair@frat@lift@lgb@total@lo\endcsname{\textminus 0.052}
\expandafter\def\csname rev@rpair@frat@lift@lgb@total@meandiff\endcsname{0.045}
\expandafter\def\csname rev@rpair@frat@lift@lgb@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lift@world@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@frat@lift@world@ixs@hi\endcsname{0.013}
\expandafter\def\csname rev@rpair@frat@lift@world@ixs@lo\endcsname{\textminus 0.019}
\expandafter\def\csname rev@rpair@frat@lift@world@ixs@meandiff\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rpair@frat@lift@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@lift@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@lift@world@total@hi\endcsname{0.035}
\expandafter\def\csname rev@rpair@frat@lift@world@total@lo\endcsname{\textminus 0.145}
\expandafter\def\csname rev@rpair@frat@lift@world@total@meandiff\endcsname{\textminus 0.053}
\expandafter\def\csname rev@rpair@frat@lift@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@naive@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@naive@world@ixs@hi\endcsname{0.552}
\expandafter\def\csname rev@rpair@frat@naive@world@ixs@lo\endcsname{0.428}
\expandafter\def\csname rev@rpair@frat@naive@world@ixs@meandiff\endcsname{0.482}
\expandafter\def\csname rev@rpair@frat@naive@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@naive@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@naive@world@total@hi\endcsname{0.601}
\expandafter\def\csname rev@rpair@frat@naive@world@total@lo\endcsname{0.413}
\expandafter\def\csname rev@rpair@frat@naive@world@total@meandiff\endcsname{0.506}
\expandafter\def\csname rev@rpair@frat@naive@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@tfm@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@tfm@world@ixs@hi\endcsname{0.223}
\expandafter\def\csname rev@rpair@frat@tfm@world@ixs@lo\endcsname{0.120}
\expandafter\def\csname rev@rpair@frat@tfm@world@ixs@meandiff\endcsname{0.180}
\expandafter\def\csname rev@rpair@frat@tfm@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@tfm@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@tfm@world@total@hi\endcsname{0.271}
\expandafter\def\csname rev@rpair@frat@tfm@world@total@lo\endcsname{\textminus 0.105}
\expandafter\def\csname rev@rpair@frat@tfm@world@total@meandiff\endcsname{0.084}
\expandafter\def\csname rev@rpair@frat@tfm@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@tfmplan@world@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@frat@tfmplan@world@ixs@hi\endcsname{0.008}
\expandafter\def\csname rev@rpair@frat@tfmplan@world@ixs@lo\endcsname{\textminus 0.040}
\expandafter\def\csname rev@rpair@frat@tfmplan@world@ixs@meandiff\endcsname{\textminus 0.016}
\expandafter\def\csname rev@rpair@frat@tfmplan@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@tfmplan@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@frat@tfmplan@world@total@hi\endcsname{\textminus 0.041}
\expandafter\def\csname rev@rpair@frat@tfmplan@world@total@lo\endcsname{\textminus 0.234}
\expandafter\def\csname rev@rpair@frat@tfmplan@world@total@meandiff\endcsname{\textminus 0.131}
\expandafter\def\csname rev@rpair@frat@tfmplan@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@tft@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@tft@world@ixs@hi\endcsname{0.077}
\expandafter\def\csname rev@rpair@frat@tft@world@ixs@lo\endcsname{0.037}
\expandafter\def\csname rev@rpair@frat@tft@world@ixs@meandiff\endcsname{0.057}
\expandafter\def\csname rev@rpair@frat@tft@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@frat@tft@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@frat@tft@world@total@hi\endcsname{0.042}
\expandafter\def\csname rev@rpair@frat@tft@world@total@lo\endcsname{\textminus 0.106}
\expandafter\def\csname rev@rpair@frat@tft@world@total@meandiff\endcsname{\textminus 0.032}
\expandafter\def\csname rev@rpair@frat@tft@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@fre@chronos@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@chronos@lgb@ixs@hi\endcsname{0.177}
\expandafter\def\csname rev@rpair@fre@chronos@lgb@ixs@lo\endcsname{0.112}
\expandafter\def\csname rev@rpair@fre@chronos@lgb@ixs@meandiff\endcsname{0.145}
\expandafter\def\csname rev@rpair@fre@chronos@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@chronos@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@chronos@lgb@total@hi\endcsname{0.342}
\expandafter\def\csname rev@rpair@fre@chronos@lgb@total@lo\endcsname{0.142}
\expandafter\def\csname rev@rpair@fre@chronos@lgb@total@meandiff\endcsname{0.257}
\expandafter\def\csname rev@rpair@fre@chronos@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@chronos@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@chronos@world@ixs@hi\endcsname{0.154}
\expandafter\def\csname rev@rpair@fre@chronos@world@ixs@lo\endcsname{0.083}
\expandafter\def\csname rev@rpair@fre@chronos@world@ixs@meandiff\endcsname{0.121}
\expandafter\def\csname rev@rpair@fre@chronos@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@chronos@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@chronos@world@total@hi\endcsname{0.325}
\expandafter\def\csname rev@rpair@fre@chronos@world@total@lo\endcsname{0.157}
\expandafter\def\csname rev@rpair@fre@chronos@world@total@meandiff\endcsname{0.240}
\expandafter\def\csname rev@rpair@fre@chronos@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@ens@lgb@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@fre@ens@lgb@ixs@hi\endcsname{0.010}
\expandafter\def\csname rev@rpair@fre@ens@lgb@ixs@lo\endcsname{\textminus 0.013}
\expandafter\def\csname rev@rpair@fre@ens@lgb@ixs@meandiff\endcsname{\textminus 0.002}
\expandafter\def\csname rev@rpair@fre@ens@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@ens@lgb@total@awins\endcsname{3}
\expandafter\def\csname rev@rpair@fre@ens@lgb@total@hi\endcsname{0.081}
\expandafter\def\csname rev@rpair@fre@ens@lgb@total@lo\endcsname{\textminus 0.027}
\expandafter\def\csname rev@rpair@fre@ens@lgb@total@meandiff\endcsname{0.021}
\expandafter\def\csname rev@rpair@fre@ens@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@ens@world@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@fre@ens@world@ixs@hi\endcsname{\textminus 0.005}
\expandafter\def\csname rev@rpair@fre@ens@world@ixs@lo\endcsname{\textminus 0.047}
\expandafter\def\csname rev@rpair@fre@ens@world@ixs@meandiff\endcsname{\textminus 0.025}
\expandafter\def\csname rev@rpair@fre@ens@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@ens@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@fre@ens@world@total@hi\endcsname{0.046}
\expandafter\def\csname rev@rpair@fre@ens@world@total@lo\endcsname{\textminus 0.030}
\expandafter\def\csname rev@rpair@fre@ens@world@total@meandiff\endcsname{0.005}
\expandafter\def\csname rev@rpair@fre@ens@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@naive@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@naive@ixs@hi\endcsname{\textminus 0.281}
\expandafter\def\csname rev@rpair@fre@lgb@naive@ixs@lo\endcsname{\textminus 0.318}
\expandafter\def\csname rev@rpair@fre@lgb@naive@ixs@meandiff\endcsname{\textminus 0.301}
\expandafter\def\csname rev@rpair@fre@lgb@naive@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@naive@total@awins\endcsname{4}
\expandafter\def\csname rev@rpair@fre@lgb@naive@total@hi\endcsname{\textminus 0.120}
\expandafter\def\csname rev@rpair@fre@lgb@naive@total@lo\endcsname{\textminus 0.464}
\expandafter\def\csname rev@rpair@fre@lgb@naive@total@meandiff\endcsname{\textminus 0.299}
\expandafter\def\csname rev@rpair@fre@lgb@naive@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@tfm@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@tfm@ixs@hi\endcsname{\textminus 0.110}
\expandafter\def\csname rev@rpair@fre@lgb@tfm@ixs@lo\endcsname{\textminus 0.167}
\expandafter\def\csname rev@rpair@fre@lgb@tfm@ixs@meandiff\endcsname{\textminus 0.140}
\expandafter\def\csname rev@rpair@fre@lgb@tfm@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@tfm@total@awins\endcsname{5}
\expandafter\def\csname rev@rpair@fre@lgb@tfm@total@hi\endcsname{\textminus 0.083}
\expandafter\def\csname rev@rpair@fre@lgb@tfm@total@lo\endcsname{\textminus 0.250}
\expandafter\def\csname rev@rpair@fre@lgb@tfm@total@meandiff\endcsname{\textminus 0.179}
\expandafter\def\csname rev@rpair@fre@lgb@tfm@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@tfmplan@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@tfmplan@ixs@hi\endcsname{\textminus 0.049}
\expandafter\def\csname rev@rpair@fre@lgb@tfmplan@ixs@lo\endcsname{\textminus 0.108}
\expandafter\def\csname rev@rpair@fre@lgb@tfmplan@ixs@meandiff\endcsname{\textminus 0.077}
\expandafter\def\csname rev@rpair@fre@lgb@tfmplan@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@tfmplan@total@awins\endcsname{5}
\expandafter\def\csname rev@rpair@fre@lgb@tfmplan@total@hi\endcsname{\textminus 0.049}
\expandafter\def\csname rev@rpair@fre@lgb@tfmplan@total@lo\endcsname{\textminus 0.278}
\expandafter\def\csname rev@rpair@fre@lgb@tfmplan@total@meandiff\endcsname{\textminus 0.160}
\expandafter\def\csname rev@rpair@fre@lgb@tfmplan@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@tft@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@tft@ixs@hi\endcsname{\textminus 0.055}
\expandafter\def\csname rev@rpair@fre@lgb@tft@ixs@lo\endcsname{\textminus 0.100}
\expandafter\def\csname rev@rpair@fre@lgb@tft@ixs@meandiff\endcsname{\textminus 0.079}
\expandafter\def\csname rev@rpair@fre@lgb@tft@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@tft@total@awins\endcsname{4}
\expandafter\def\csname rev@rpair@fre@lgb@tft@total@hi\endcsname{\textminus 0.024}
\expandafter\def\csname rev@rpair@fre@lgb@tft@total@lo\endcsname{\textminus 0.097}
\expandafter\def\csname rev@rpair@fre@lgb@tft@total@meandiff\endcsname{\textminus 0.059}
\expandafter\def\csname rev@rpair@fre@lgb@tft@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@world@ixs@awins\endcsname{5}
\expandafter\def\csname rev@rpair@fre@lgb@world@ixs@hi\endcsname{0.003}
\expandafter\def\csname rev@rpair@fre@lgb@world@ixs@lo\endcsname{\textminus 0.050}
\expandafter\def\csname rev@rpair@fre@lgb@world@ixs@meandiff\endcsname{\textminus 0.024}
\expandafter\def\csname rev@rpair@fre@lgb@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lgb@world@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@fre@lgb@world@total@hi\endcsname{0.055}
\expandafter\def\csname rev@rpair@fre@lgb@world@total@lo\endcsname{\textminus 0.089}
\expandafter\def\csname rev@rpair@fre@lgb@world@total@meandiff\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rpair@fre@lgb@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lift@lgb@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@fre@lift@lgb@ixs@hi\endcsname{0.071}
\expandafter\def\csname rev@rpair@fre@lift@lgb@ixs@lo\endcsname{0.002}
\expandafter\def\csname rev@rpair@fre@lift@lgb@ixs@meandiff\endcsname{0.039}
\expandafter\def\csname rev@rpair@fre@lift@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lift@lgb@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@fre@lift@lgb@total@hi\endcsname{0.198}
\expandafter\def\csname rev@rpair@fre@lift@lgb@total@lo\endcsname{\textminus 0.083}
\expandafter\def\csname rev@rpair@fre@lift@lgb@total@meandiff\endcsname{0.066}
\expandafter\def\csname rev@rpair@fre@lift@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lift@world@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@fre@lift@world@ixs@hi\endcsname{0.043}
\expandafter\def\csname rev@rpair@fre@lift@world@ixs@lo\endcsname{\textminus 0.021}
\expandafter\def\csname rev@rpair@fre@lift@world@ixs@meandiff\endcsname{0.015}
\expandafter\def\csname rev@rpair@fre@lift@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@lift@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@fre@lift@world@total@hi\endcsname{0.144}
\expandafter\def\csname rev@rpair@fre@lift@world@total@lo\endcsname{\textminus 0.049}
\expandafter\def\csname rev@rpair@fre@lift@world@total@meandiff\endcsname{0.049}
\expandafter\def\csname rev@rpair@fre@lift@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@naive@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@naive@world@ixs@hi\endcsname{0.304}
\expandafter\def\csname rev@rpair@fre@naive@world@ixs@lo\endcsname{0.251}
\expandafter\def\csname rev@rpair@fre@naive@world@ixs@meandiff\endcsname{0.277}
\expandafter\def\csname rev@rpair@fre@naive@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@naive@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@naive@world@total@hi\endcsname{0.393}
\expandafter\def\csname rev@rpair@fre@naive@world@total@lo\endcsname{0.170}
\expandafter\def\csname rev@rpair@fre@naive@world@total@meandiff\endcsname{0.282}
\expandafter\def\csname rev@rpair@fre@naive@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@tfm@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@tfm@world@ixs@hi\endcsname{0.144}
\expandafter\def\csname rev@rpair@fre@tfm@world@ixs@lo\endcsname{0.079}
\expandafter\def\csname rev@rpair@fre@tfm@world@ixs@meandiff\endcsname{0.116}
\expandafter\def\csname rev@rpair@fre@tfm@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@tfm@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@tfm@world@total@hi\endcsname{0.222}
\expandafter\def\csname rev@rpair@fre@tfm@world@total@lo\endcsname{0.104}
\expandafter\def\csname rev@rpair@fre@tfm@world@total@meandiff\endcsname{0.163}
\expandafter\def\csname rev@rpair@fre@tfm@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@tfmplan@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@tfmplan@world@ixs@hi\endcsname{0.086}
\expandafter\def\csname rev@rpair@fre@tfmplan@world@ixs@lo\endcsname{0.024}
\expandafter\def\csname rev@rpair@fre@tfmplan@world@ixs@meandiff\endcsname{0.053}
\expandafter\def\csname rev@rpair@fre@tfmplan@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@tfmplan@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@tfmplan@world@total@hi\endcsname{0.225}
\expandafter\def\csname rev@rpair@fre@tfmplan@world@total@lo\endcsname{0.065}
\expandafter\def\csname rev@rpair@fre@tfmplan@world@total@meandiff\endcsname{0.143}
\expandafter\def\csname rev@rpair@fre@tfmplan@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@tft@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@fre@tft@world@ixs@hi\endcsname{0.073}
\expandafter\def\csname rev@rpair@fre@tft@world@ixs@lo\endcsname{0.034}
\expandafter\def\csname rev@rpair@fre@tft@world@ixs@meandiff\endcsname{0.055}
\expandafter\def\csname rev@rpair@fre@tft@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@fre@tft@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@fre@tft@world@total@hi\endcsname{0.110}
\expandafter\def\csname rev@rpair@fre@tft@world@total@lo\endcsname{\textminus 0.024}
\expandafter\def\csname rev@rpair@fre@tft@world@total@meandiff\endcsname{0.042}
\expandafter\def\csname rev@rpair@fre@tft@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@mfive@chronos@lgb@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@mfive@chronos@lgb@ixs@hi\endcsname{0.014}
\expandafter\def\csname rev@rpair@mfive@chronos@lgb@ixs@lo\endcsname{\textminus 0.019}
\expandafter\def\csname rev@rpair@mfive@chronos@lgb@ixs@meandiff\endcsname{\textminus 0.004}
\expandafter\def\csname rev@rpair@mfive@chronos@lgb@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@chronos@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@mfive@chronos@lgb@total@hi\endcsname{0.798}
\expandafter\def\csname rev@rpair@mfive@chronos@lgb@total@lo\endcsname{0.480}
\expandafter\def\csname rev@rpair@mfive@chronos@lgb@total@meandiff\endcsname{0.639}
\expandafter\def\csname rev@rpair@mfive@chronos@lgb@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@chronos@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@mfive@chronos@world@ixs@hi\endcsname{0.012}
\expandafter\def\csname rev@rpair@mfive@chronos@world@ixs@lo\endcsname{0.003}
\expandafter\def\csname rev@rpair@mfive@chronos@world@ixs@meandiff\endcsname{0.007}
\expandafter\def\csname rev@rpair@mfive@chronos@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@chronos@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@mfive@chronos@world@total@hi\endcsname{0.954}
\expandafter\def\csname rev@rpair@mfive@chronos@world@total@lo\endcsname{0.495}
\expandafter\def\csname rev@rpair@mfive@chronos@world@total@meandiff\endcsname{0.724}
\expandafter\def\csname rev@rpair@mfive@chronos@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@ens@lgb@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@ens@lgb@ixs@hi\endcsname{\textminus 0.016}
\expandafter\def\csname rev@rpair@mfive@ens@lgb@ixs@lo\endcsname{\textminus 0.038}
\expandafter\def\csname rev@rpair@mfive@ens@lgb@ixs@meandiff\endcsname{\textminus 0.027}
\expandafter\def\csname rev@rpair@mfive@ens@lgb@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@ens@lgb@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@mfive@ens@lgb@total@hi\endcsname{0.173}
\expandafter\def\csname rev@rpair@mfive@ens@lgb@total@lo\endcsname{\textminus 0.127}
\expandafter\def\csname rev@rpair@mfive@ens@lgb@total@meandiff\endcsname{0.013}
\expandafter\def\csname rev@rpair@mfive@ens@lgb@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@ens@world@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@ens@world@ixs@hi\endcsname{\textminus 0.014}
\expandafter\def\csname rev@rpair@mfive@ens@world@ixs@lo\endcsname{\textminus 0.019}
\expandafter\def\csname rev@rpair@mfive@ens@world@ixs@meandiff\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rpair@mfive@ens@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@ens@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@mfive@ens@world@total@hi\endcsname{0.238}
\expandafter\def\csname rev@rpair@mfive@ens@world@total@lo\endcsname{\textminus 0.063}
\expandafter\def\csname rev@rpair@mfive@ens@world@total@meandiff\endcsname{0.098}
\expandafter\def\csname rev@rpair@mfive@ens@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@naive@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@naive@ixs@hi\endcsname{\textminus 0.262}
\expandafter\def\csname rev@rpair@mfive@lgb@naive@ixs@lo\endcsname{\textminus 0.343}
\expandafter\def\csname rev@rpair@mfive@lgb@naive@ixs@meandiff\endcsname{\textminus 0.301}
\expandafter\def\csname rev@rpair@mfive@lgb@naive@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@naive@total@awins\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@naive@total@hi\endcsname{\textminus 0.223}
\expandafter\def\csname rev@rpair@mfive@lgb@naive@total@lo\endcsname{\textminus 0.653}
\expandafter\def\csname rev@rpair@mfive@lgb@naive@total@meandiff\endcsname{\textminus 0.394}
\expandafter\def\csname rev@rpair@mfive@lgb@naive@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@tfm@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@mfive@lgb@tfm@ixs@hi\endcsname{0.036}
\expandafter\def\csname rev@rpair@mfive@lgb@tfm@ixs@lo\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rpair@mfive@lgb@tfm@ixs@meandiff\endcsname{0.019}
\expandafter\def\csname rev@rpair@mfive@lgb@tfm@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@tfm@total@awins\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@tfm@total@hi\endcsname{\textminus 0.131}
\expandafter\def\csname rev@rpair@mfive@lgb@tfm@total@lo\endcsname{\textminus 0.518}
\expandafter\def\csname rev@rpair@mfive@lgb@tfm@total@meandiff\endcsname{\textminus 0.307}
\expandafter\def\csname rev@rpair@mfive@lgb@tfm@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@tfmplan@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@mfive@lgb@tfmplan@ixs@hi\endcsname{0.035}
\expandafter\def\csname rev@rpair@mfive@lgb@tfmplan@ixs@lo\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rpair@mfive@lgb@tfmplan@ixs@meandiff\endcsname{0.019}
\expandafter\def\csname rev@rpair@mfive@lgb@tfmplan@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@tfmplan@total@awins\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@tfmplan@total@hi\endcsname{\textminus 0.162}
\expandafter\def\csname rev@rpair@mfive@lgb@tfmplan@total@lo\endcsname{\textminus 0.522}
\expandafter\def\csname rev@rpair@mfive@lgb@tfmplan@total@meandiff\endcsname{\textminus 0.341}
\expandafter\def\csname rev@rpair@mfive@lgb@tfmplan@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@mfive@lgb@world@ixs@hi\endcsname{0.024}
\expandafter\def\csname rev@rpair@mfive@lgb@world@ixs@lo\endcsname{\textminus 0.003}
\expandafter\def\csname rev@rpair@mfive@lgb@world@ixs@meandiff\endcsname{0.010}
\expandafter\def\csname rev@rpair@mfive@lgb@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lgb@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@mfive@lgb@world@total@hi\endcsname{0.343}
\expandafter\def\csname rev@rpair@mfive@lgb@world@total@lo\endcsname{\textminus 0.247}
\expandafter\def\csname rev@rpair@mfive@lgb@world@total@meandiff\endcsname{0.085}
\expandafter\def\csname rev@rpair@mfive@lgb@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lift@lgb@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@mfive@lift@lgb@ixs@hi\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rpair@mfive@lift@lgb@ixs@lo\endcsname{\textminus 0.028}
\expandafter\def\csname rev@rpair@mfive@lift@lgb@ixs@meandiff\endcsname{\textminus 0.016}
\expandafter\def\csname rev@rpair@mfive@lift@lgb@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lift@lgb@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@mfive@lift@lgb@total@hi\endcsname{1.419}
\expandafter\def\csname rev@rpair@mfive@lift@lgb@total@lo\endcsname{\textminus 0.092}
\expandafter\def\csname rev@rpair@mfive@lift@lgb@total@meandiff\endcsname{0.470}
\expandafter\def\csname rev@rpair@mfive@lift@lgb@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lift@world@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@mfive@lift@world@ixs@hi\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rpair@mfive@lift@world@ixs@lo\endcsname{\textminus 0.010}
\expandafter\def\csname rev@rpair@mfive@lift@world@ixs@meandiff\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rpair@mfive@lift@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@lift@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@mfive@lift@world@total@hi\endcsname{1.744}
\expandafter\def\csname rev@rpair@mfive@lift@world@total@lo\endcsname{\textminus 0.147}
\expandafter\def\csname rev@rpair@mfive@lift@world@total@meandiff\endcsname{0.555}
\expandafter\def\csname rev@rpair@mfive@lift@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@naive@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@mfive@naive@world@ixs@hi\endcsname{0.344}
\expandafter\def\csname rev@rpair@mfive@naive@world@ixs@lo\endcsname{0.278}
\expandafter\def\csname rev@rpair@mfive@naive@world@ixs@meandiff\endcsname{0.312}
\expandafter\def\csname rev@rpair@mfive@naive@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@naive@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@mfive@naive@world@total@hi\endcsname{0.576}
\expandafter\def\csname rev@rpair@mfive@naive@world@total@lo\endcsname{0.382}
\expandafter\def\csname rev@rpair@mfive@naive@world@total@meandiff\endcsname{0.479}
\expandafter\def\csname rev@rpair@mfive@naive@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@tfm@world@ixs@awins\endcsname{3}
\expandafter\def\csname rev@rpair@mfive@tfm@world@ixs@hi\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rpair@mfive@tfm@world@ixs@lo\endcsname{\textminus 0.015}
\expandafter\def\csname rev@rpair@mfive@tfm@world@ixs@meandiff\endcsname{\textminus 0.009}
\expandafter\def\csname rev@rpair@mfive@tfm@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@tfm@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@mfive@tfm@world@total@hi\endcsname{0.492}
\expandafter\def\csname rev@rpair@mfive@tfm@world@total@lo\endcsname{0.288}
\expandafter\def\csname rev@rpair@mfive@tfm@world@total@meandiff\endcsname{0.392}
\expandafter\def\csname rev@rpair@mfive@tfm@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@tfmplan@world@ixs@awins\endcsname{3}
\expandafter\def\csname rev@rpair@mfive@tfmplan@world@ixs@hi\endcsname{\textminus 0.001}
\expandafter\def\csname rev@rpair@mfive@tfmplan@world@ixs@lo\endcsname{\textminus 0.014}
\expandafter\def\csname rev@rpair@mfive@tfmplan@world@ixs@meandiff\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rpair@mfive@tfmplan@world@ixs@n\endcsname{4}
\expandafter\def\csname rev@rpair@mfive@tfmplan@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@mfive@tfmplan@world@total@hi\endcsname{0.590}
\expandafter\def\csname rev@rpair@mfive@tfmplan@world@total@lo\endcsname{0.263}
\expandafter\def\csname rev@rpair@mfive@tfmplan@world@total@meandiff\endcsname{0.426}
\expandafter\def\csname rev@rpair@mfive@tfmplan@world@total@n\endcsname{4}
\expandafter\def\csname rev@rpair@sdr@chronos@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@chronos@lgb@ixs@hi\endcsname{0.218}
\expandafter\def\csname rev@rpair@sdr@chronos@lgb@ixs@lo\endcsname{0.126}
\expandafter\def\csname rev@rpair@sdr@chronos@lgb@ixs@meandiff\endcsname{0.174}
\expandafter\def\csname rev@rpair@sdr@chronos@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@chronos@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@chronos@lgb@total@hi\endcsname{0.630}
\expandafter\def\csname rev@rpair@sdr@chronos@lgb@total@lo\endcsname{0.194}
\expandafter\def\csname rev@rpair@sdr@chronos@lgb@total@meandiff\endcsname{0.439}
\expandafter\def\csname rev@rpair@sdr@chronos@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@chronos@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@chronos@world@ixs@hi\endcsname{0.159}
\expandafter\def\csname rev@rpair@sdr@chronos@world@ixs@lo\endcsname{0.078}
\expandafter\def\csname rev@rpair@sdr@chronos@world@ixs@meandiff\endcsname{0.120}
\expandafter\def\csname rev@rpair@sdr@chronos@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@chronos@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@chronos@world@total@hi\endcsname{0.526}
\expandafter\def\csname rev@rpair@sdr@chronos@world@total@lo\endcsname{0.141}
\expandafter\def\csname rev@rpair@sdr@chronos@world@total@meandiff\endcsname{0.390}
\expandafter\def\csname rev@rpair@sdr@chronos@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@ens@lgb@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@sdr@ens@lgb@ixs@hi\endcsname{0.010}
\expandafter\def\csname rev@rpair@sdr@ens@lgb@ixs@lo\endcsname{\textminus 0.032}
\expandafter\def\csname rev@rpair@sdr@ens@lgb@ixs@meandiff\endcsname{\textminus 0.009}
\expandafter\def\csname rev@rpair@sdr@ens@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@ens@lgb@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@sdr@ens@lgb@total@hi\endcsname{0.058}
\expandafter\def\csname rev@rpair@sdr@ens@lgb@total@lo\endcsname{\textminus 0.051}
\expandafter\def\csname rev@rpair@sdr@ens@lgb@total@meandiff\endcsname{0.003}
\expandafter\def\csname rev@rpair@sdr@ens@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@ens@world@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@sdr@ens@world@ixs@hi\endcsname{\textminus 0.031}
\expandafter\def\csname rev@rpair@sdr@ens@world@ixs@lo\endcsname{\textminus 0.102}
\expandafter\def\csname rev@rpair@sdr@ens@world@ixs@meandiff\endcsname{\textminus 0.064}
\expandafter\def\csname rev@rpair@sdr@ens@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@ens@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@ens@world@total@hi\endcsname{0.057}
\expandafter\def\csname rev@rpair@sdr@ens@world@total@lo\endcsname{\textminus 0.140}
\expandafter\def\csname rev@rpair@sdr@ens@world@total@meandiff\endcsname{\textminus 0.046}
\expandafter\def\csname rev@rpair@sdr@ens@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@naive@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@naive@ixs@hi\endcsname{\textminus 0.332}
\expandafter\def\csname rev@rpair@sdr@lgb@naive@ixs@lo\endcsname{\textminus 0.498}
\expandafter\def\csname rev@rpair@sdr@lgb@naive@ixs@meandiff\endcsname{\textminus 0.415}
\expandafter\def\csname rev@rpair@sdr@lgb@naive@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@naive@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@sdr@lgb@naive@total@hi\endcsname{\textminus 0.057}
\expandafter\def\csname rev@rpair@sdr@lgb@naive@total@lo\endcsname{\textminus 0.351}
\expandafter\def\csname rev@rpair@sdr@lgb@naive@total@meandiff\endcsname{\textminus 0.204}
\expandafter\def\csname rev@rpair@sdr@lgb@naive@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@tfm@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@tfm@ixs@hi\endcsname{\textminus 0.124}
\expandafter\def\csname rev@rpair@sdr@lgb@tfm@ixs@lo\endcsname{\textminus 0.207}
\expandafter\def\csname rev@rpair@sdr@lgb@tfm@ixs@meandiff\endcsname{\textminus 0.165}
\expandafter\def\csname rev@rpair@sdr@lgb@tfm@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@tfm@total@awins\endcsname{5}
\expandafter\def\csname rev@rpair@sdr@lgb@tfm@total@hi\endcsname{\textminus 0.140}
\expandafter\def\csname rev@rpair@sdr@lgb@tfm@total@lo\endcsname{\textminus 0.486}
\expandafter\def\csname rev@rpair@sdr@lgb@tfm@total@meandiff\endcsname{\textminus 0.326}
\expandafter\def\csname rev@rpair@sdr@lgb@tfm@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@tfmplan@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@sdr@lgb@tfmplan@ixs@hi\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rpair@sdr@lgb@tfmplan@ixs@lo\endcsname{\textminus 0.120}
\expandafter\def\csname rev@rpair@sdr@lgb@tfmplan@ixs@meandiff\endcsname{\textminus 0.063}
\expandafter\def\csname rev@rpair@sdr@lgb@tfmplan@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@tfmplan@total@awins\endcsname{3}
\expandafter\def\csname rev@rpair@sdr@lgb@tfmplan@total@hi\endcsname{\textminus 0.042}
\expandafter\def\csname rev@rpair@sdr@lgb@tfmplan@total@lo\endcsname{\textminus 0.249}
\expandafter\def\csname rev@rpair@sdr@lgb@tfmplan@total@meandiff\endcsname{\textminus 0.146}
\expandafter\def\csname rev@rpair@sdr@lgb@tfmplan@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@tft@ixs@awins\endcsname{5}
\expandafter\def\csname rev@rpair@sdr@lgb@tft@ixs@hi\endcsname{\textminus 0.052}
\expandafter\def\csname rev@rpair@sdr@lgb@tft@ixs@lo\endcsname{\textminus 0.137}
\expandafter\def\csname rev@rpair@sdr@lgb@tft@ixs@meandiff\endcsname{\textminus 0.094}
\expandafter\def\csname rev@rpair@sdr@lgb@tft@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@tft@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@lgb@tft@total@hi\endcsname{\textminus 0.057}
\expandafter\def\csname rev@rpair@sdr@lgb@tft@total@lo\endcsname{\textminus 0.222}
\expandafter\def\csname rev@rpair@sdr@lgb@tft@total@meandiff\endcsname{\textminus 0.140}
\expandafter\def\csname rev@rpair@sdr@lgb@tft@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@world@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@sdr@lgb@world@ixs@hi\endcsname{\textminus 0.010}
\expandafter\def\csname rev@rpair@sdr@lgb@world@ixs@lo\endcsname{\textminus 0.101}
\expandafter\def\csname rev@rpair@sdr@lgb@world@ixs@meandiff\endcsname{\textminus 0.055}
\expandafter\def\csname rev@rpair@sdr@lgb@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lgb@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@lgb@world@total@hi\endcsname{0.073}
\expandafter\def\csname rev@rpair@sdr@lgb@world@total@lo\endcsname{\textminus 0.145}
\expandafter\def\csname rev@rpair@sdr@lgb@world@total@meandiff\endcsname{\textminus 0.048}
\expandafter\def\csname rev@rpair@sdr@lgb@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lift@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@lift@lgb@ixs@hi\endcsname{0.193}
\expandafter\def\csname rev@rpair@sdr@lift@lgb@ixs@lo\endcsname{0.065}
\expandafter\def\csname rev@rpair@sdr@lift@lgb@ixs@meandiff\endcsname{0.127}
\expandafter\def\csname rev@rpair@sdr@lift@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lift@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@lift@lgb@total@hi\endcsname{0.267}
\expandafter\def\csname rev@rpair@sdr@lift@lgb@total@lo\endcsname{0.009}
\expandafter\def\csname rev@rpair@sdr@lift@lgb@total@meandiff\endcsname{0.134}
\expandafter\def\csname rev@rpair@sdr@lift@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lift@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@lift@world@ixs@hi\endcsname{0.101}
\expandafter\def\csname rev@rpair@sdr@lift@world@ixs@lo\endcsname{0.043}
\expandafter\def\csname rev@rpair@sdr@lift@world@ixs@meandiff\endcsname{0.072}
\expandafter\def\csname rev@rpair@sdr@lift@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@lift@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@lift@world@total@hi\endcsname{0.187}
\expandafter\def\csname rev@rpair@sdr@lift@world@total@lo\endcsname{\textminus 0.037}
\expandafter\def\csname rev@rpair@sdr@lift@world@total@meandiff\endcsname{0.086}
\expandafter\def\csname rev@rpair@sdr@lift@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@naive@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@naive@world@ixs@hi\endcsname{0.448}
\expandafter\def\csname rev@rpair@sdr@naive@world@ixs@lo\endcsname{0.253}
\expandafter\def\csname rev@rpair@sdr@naive@world@ixs@meandiff\endcsname{0.360}
\expandafter\def\csname rev@rpair@sdr@naive@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@naive@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@naive@world@total@hi\endcsname{0.313}
\expandafter\def\csname rev@rpair@sdr@naive@world@total@lo\endcsname{\textminus 0.008}
\expandafter\def\csname rev@rpair@sdr@naive@world@total@meandiff\endcsname{0.156}
\expandafter\def\csname rev@rpair@sdr@naive@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@tfm@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@tfm@world@ixs@hi\endcsname{0.149}
\expandafter\def\csname rev@rpair@sdr@tfm@world@ixs@lo\endcsname{0.072}
\expandafter\def\csname rev@rpair@sdr@tfm@world@ixs@meandiff\endcsname{0.111}
\expandafter\def\csname rev@rpair@sdr@tfm@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@tfm@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@tfm@world@total@hi\endcsname{0.399}
\expandafter\def\csname rev@rpair@sdr@tfm@world@total@lo\endcsname{0.088}
\expandafter\def\csname rev@rpair@sdr@tfm@world@total@meandiff\endcsname{0.278}
\expandafter\def\csname rev@rpair@sdr@tfm@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@tfmplan@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@tfmplan@world@ixs@hi\endcsname{0.067}
\expandafter\def\csname rev@rpair@sdr@tfmplan@world@ixs@lo\endcsname{\textminus 0.047}
\expandafter\def\csname rev@rpair@sdr@tfmplan@world@ixs@meandiff\endcsname{0.009}
\expandafter\def\csname rev@rpair@sdr@tfmplan@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@tfmplan@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@tfmplan@world@total@hi\endcsname{0.228}
\expandafter\def\csname rev@rpair@sdr@tfmplan@world@total@lo\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rpair@sdr@tfmplan@world@total@meandiff\endcsname{0.098}
\expandafter\def\csname rev@rpair@sdr@tfmplan@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@tft@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@tft@world@ixs@hi\endcsname{0.090}
\expandafter\def\csname rev@rpair@sdr@tft@world@ixs@lo\endcsname{\textminus 0.016}
\expandafter\def\csname rev@rpair@sdr@tft@world@ixs@meandiff\endcsname{0.040}
\expandafter\def\csname rev@rpair@sdr@tft@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sdr@tft@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sdr@tft@world@total@hi\endcsname{0.205}
\expandafter\def\csname rev@rpair@sdr@tft@world@total@lo\endcsname{0.001}
\expandafter\def\csname rev@rpair@sdr@tft@world@total@meandiff\endcsname{0.092}
\expandafter\def\csname rev@rpair@sdr@tft@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@chronos@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@chronos@lgb@ixs@hi\endcsname{0.152}
\expandafter\def\csname rev@rpair@sna@chronos@lgb@ixs@lo\endcsname{0.110}
\expandafter\def\csname rev@rpair@sna@chronos@lgb@ixs@meandiff\endcsname{0.130}
\expandafter\def\csname rev@rpair@sna@chronos@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@chronos@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@chronos@lgb@total@hi\endcsname{9.652}
\expandafter\def\csname rev@rpair@sna@chronos@lgb@total@lo\endcsname{0.108}
\expandafter\def\csname rev@rpair@sna@chronos@lgb@total@meandiff\endcsname{3.313}
\expandafter\def\csname rev@rpair@sna@chronos@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@chronos@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@chronos@world@ixs@hi\endcsname{0.129}
\expandafter\def\csname rev@rpair@sna@chronos@world@ixs@lo\endcsname{0.096}
\expandafter\def\csname rev@rpair@sna@chronos@world@ixs@meandiff\endcsname{0.113}
\expandafter\def\csname rev@rpair@sna@chronos@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@chronos@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@chronos@world@total@hi\endcsname{8.674}
\expandafter\def\csname rev@rpair@sna@chronos@world@total@lo\endcsname{0.032}
\expandafter\def\csname rev@rpair@sna@chronos@world@total@meandiff\endcsname{2.957}
\expandafter\def\csname rev@rpair@sna@chronos@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@ens@lgb@ixs@awins\endcsname{3}
\expandafter\def\csname rev@rpair@sna@ens@lgb@ixs@hi\endcsname{\textminus 0.006}
\expandafter\def\csname rev@rpair@sna@ens@lgb@ixs@lo\endcsname{\textminus 0.024}
\expandafter\def\csname rev@rpair@sna@ens@lgb@ixs@meandiff\endcsname{\textminus 0.015}
\expandafter\def\csname rev@rpair@sna@ens@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@ens@lgb@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@sna@ens@lgb@total@hi\endcsname{0.271}
\expandafter\def\csname rev@rpair@sna@ens@lgb@total@lo\endcsname{\textminus 0.057}
\expandafter\def\csname rev@rpair@sna@ens@lgb@total@meandiff\endcsname{0.083}
\expandafter\def\csname rev@rpair@sna@ens@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@ens@world@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@sna@ens@world@ixs@hi\endcsname{\textminus 0.023}
\expandafter\def\csname rev@rpair@sna@ens@world@ixs@lo\endcsname{\textminus 0.044}
\expandafter\def\csname rev@rpair@sna@ens@world@ixs@meandiff\endcsname{\textminus 0.033}
\expandafter\def\csname rev@rpair@sna@ens@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@ens@world@total@awins\endcsname{3}
\expandafter\def\csname rev@rpair@sna@ens@world@total@hi\endcsname{0.002}
\expandafter\def\csname rev@rpair@sna@ens@world@total@lo\endcsname{\textminus 0.737}
\expandafter\def\csname rev@rpair@sna@ens@world@total@meandiff\endcsname{\textminus 0.273}
\expandafter\def\csname rev@rpair@sna@ens@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@naive@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@naive@ixs@hi\endcsname{\textminus 0.288}
\expandafter\def\csname rev@rpair@sna@lgb@naive@ixs@lo\endcsname{\textminus 0.592}
\expandafter\def\csname rev@rpair@sna@lgb@naive@ixs@meandiff\endcsname{\textminus 0.432}
\expandafter\def\csname rev@rpair@sna@lgb@naive@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@naive@total@awins\endcsname{4}
\expandafter\def\csname rev@rpair@sna@lgb@naive@total@hi\endcsname{\textminus 0.022}
\expandafter\def\csname rev@rpair@sna@lgb@naive@total@lo\endcsname{\textminus 1.595}
\expandafter\def\csname rev@rpair@sna@lgb@naive@total@meandiff\endcsname{\textminus 0.693}
\expandafter\def\csname rev@rpair@sna@lgb@naive@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@tfm@ixs@awins\endcsname{5}
\expandafter\def\csname rev@rpair@sna@lgb@tfm@ixs@hi\endcsname{\textminus 0.070}
\expandafter\def\csname rev@rpair@sna@lgb@tfm@ixs@lo\endcsname{\textminus 0.129}
\expandafter\def\csname rev@rpair@sna@lgb@tfm@ixs@meandiff\endcsname{\textminus 0.099}
\expandafter\def\csname rev@rpair@sna@lgb@tfm@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@tfm@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@sna@lgb@tfm@total@hi\endcsname{\textminus 0.032}
\expandafter\def\csname rev@rpair@sna@lgb@tfm@total@lo\endcsname{\textminus 1.270}
\expandafter\def\csname rev@rpair@sna@lgb@tfm@total@meandiff\endcsname{\textminus 0.484}
\expandafter\def\csname rev@rpair@sna@lgb@tfm@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@tfmplan@ixs@awins\endcsname{4}
\expandafter\def\csname rev@rpair@sna@lgb@tfmplan@ixs@hi\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rpair@sna@lgb@tfmplan@ixs@lo\endcsname{\textminus 0.047}
\expandafter\def\csname rev@rpair@sna@lgb@tfmplan@ixs@meandiff\endcsname{\textminus 0.028}
\expandafter\def\csname rev@rpair@sna@lgb@tfmplan@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@tfmplan@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@sna@lgb@tfmplan@total@hi\endcsname{0.069}
\expandafter\def\csname rev@rpair@sna@lgb@tfmplan@total@lo\endcsname{\textminus 0.250}
\expandafter\def\csname rev@rpair@sna@lgb@tfmplan@total@meandiff\endcsname{\textminus 0.084}
\expandafter\def\csname rev@rpair@sna@lgb@tfmplan@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@tft@ixs@awins\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@tft@ixs@hi\endcsname{\textminus 0.050}
\expandafter\def\csname rev@rpair@sna@lgb@tft@ixs@lo\endcsname{\textminus 0.109}
\expandafter\def\csname rev@rpair@sna@lgb@tft@ixs@meandiff\endcsname{\textminus 0.076}
\expandafter\def\csname rev@rpair@sna@lgb@tft@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@tft@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@sna@lgb@tft@total@hi\endcsname{0.127}
\expandafter\def\csname rev@rpair@sna@lgb@tft@total@lo\endcsname{\textminus 0.688}
\expandafter\def\csname rev@rpair@sna@lgb@tft@total@meandiff\endcsname{\textminus 0.203}
\expandafter\def\csname rev@rpair@sna@lgb@tft@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@world@ixs@awins\endcsname{2}
\expandafter\def\csname rev@rpair@sna@lgb@world@ixs@hi\endcsname{\textminus 0.009}
\expandafter\def\csname rev@rpair@sna@lgb@world@ixs@lo\endcsname{\textminus 0.025}
\expandafter\def\csname rev@rpair@sna@lgb@world@ixs@meandiff\endcsname{\textminus 0.017}
\expandafter\def\csname rev@rpair@sna@lgb@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lgb@world@total@awins\endcsname{3}
\expandafter\def\csname rev@rpair@sna@lgb@world@total@hi\endcsname{0.051}
\expandafter\def\csname rev@rpair@sna@lgb@world@total@lo\endcsname{\textminus 1.004}
\expandafter\def\csname rev@rpair@sna@lgb@world@total@meandiff\endcsname{\textminus 0.356}
\expandafter\def\csname rev@rpair@sna@lgb@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lift@lgb@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@lift@lgb@ixs@hi\endcsname{0.038}
\expandafter\def\csname rev@rpair@sna@lift@lgb@ixs@lo\endcsname{0.006}
\expandafter\def\csname rev@rpair@sna@lift@lgb@ixs@meandiff\endcsname{0.021}
\expandafter\def\csname rev@rpair@sna@lift@lgb@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lift@lgb@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@lift@lgb@total@hi\endcsname{0.357}
\expandafter\def\csname rev@rpair@sna@lift@lgb@total@lo\endcsname{\textminus 0.618}
\expandafter\def\csname rev@rpair@sna@lift@lgb@total@meandiff\endcsname{\textminus 0.071}
\expandafter\def\csname rev@rpair@sna@lift@lgb@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lift@world@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@sna@lift@world@ixs@hi\endcsname{0.019}
\expandafter\def\csname rev@rpair@sna@lift@world@ixs@lo\endcsname{\textminus 0.009}
\expandafter\def\csname rev@rpair@sna@lift@world@ixs@meandiff\endcsname{0.003}
\expandafter\def\csname rev@rpair@sna@lift@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@lift@world@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@sna@lift@world@total@hi\endcsname{0.071}
\expandafter\def\csname rev@rpair@sna@lift@world@total@lo\endcsname{\textminus 0.927}
\expandafter\def\csname rev@rpair@sna@lift@world@total@meandiff\endcsname{\textminus 0.427}
\expandafter\def\csname rev@rpair@sna@lift@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@naive@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@naive@world@ixs@hi\endcsname{0.568}
\expandafter\def\csname rev@rpair@sna@naive@world@ixs@lo\endcsname{0.274}
\expandafter\def\csname rev@rpair@sna@naive@world@ixs@meandiff\endcsname{0.415}
\expandafter\def\csname rev@rpair@sna@naive@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@naive@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@naive@world@total@hi\endcsname{1.471}
\expandafter\def\csname rev@rpair@sna@naive@world@total@lo\endcsname{\textminus 0.602}
\expandafter\def\csname rev@rpair@sna@naive@world@total@meandiff\endcsname{0.337}
\expandafter\def\csname rev@rpair@sna@naive@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@tfm@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@tfm@world@ixs@hi\endcsname{0.109}
\expandafter\def\csname rev@rpair@sna@tfm@world@ixs@lo\endcsname{0.055}
\expandafter\def\csname rev@rpair@sna@tfm@world@ixs@meandiff\endcsname{0.082}
\expandafter\def\csname rev@rpair@sna@tfm@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@tfm@world@total@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@tfm@world@total@hi\endcsname{0.285}
\expandafter\def\csname rev@rpair@sna@tfm@world@total@lo\endcsname{\textminus 0.014}
\expandafter\def\csname rev@rpair@sna@tfm@world@total@meandiff\endcsname{0.128}
\expandafter\def\csname rev@rpair@sna@tfm@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@tfmplan@world@ixs@awins\endcsname{1}
\expandafter\def\csname rev@rpair@sna@tfmplan@world@ixs@hi\endcsname{0.028}
\expandafter\def\csname rev@rpair@sna@tfmplan@world@ixs@lo\endcsname{\textminus 0.011}
\expandafter\def\csname rev@rpair@sna@tfmplan@world@ixs@meandiff\endcsname{0.011}
\expandafter\def\csname rev@rpair@sna@tfmplan@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@tfmplan@world@total@awins\endcsname{2}
\expandafter\def\csname rev@rpair@sna@tfmplan@world@total@hi\endcsname{0.050}
\expandafter\def\csname rev@rpair@sna@tfmplan@world@total@lo\endcsname{\textminus 0.802}
\expandafter\def\csname rev@rpair@sna@tfmplan@world@total@meandiff\endcsname{\textminus 0.272}
\expandafter\def\csname rev@rpair@sna@tfmplan@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@tft@world@ixs@awins\endcsname{0}
\expandafter\def\csname rev@rpair@sna@tft@world@ixs@hi\endcsname{0.089}
\expandafter\def\csname rev@rpair@sna@tft@world@ixs@lo\endcsname{0.035}
\expandafter\def\csname rev@rpair@sna@tft@world@ixs@meandiff\endcsname{0.059}
\expandafter\def\csname rev@rpair@sna@tft@world@ixs@n\endcsname{6}
\expandafter\def\csname rev@rpair@sna@tft@world@total@awins\endcsname{1}
\expandafter\def\csname rev@rpair@sna@tft@world@total@hi\endcsname{\textminus 0.007}
\expandafter\def\csname rev@rpair@sna@tft@world@total@lo\endcsname{\textminus 0.342}
\expandafter\def\csname rev@rpair@sna@tft@world@total@meandiff\endcsname{\textminus 0.153}
\expandafter\def\csname rev@rpair@sna@tft@world@total@n\endcsname{6}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@a@afterpromoerr\endcsname{0.569}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@a@afterpromofa\endcsname{0.91}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@a@itembystore\endcsname{0.712}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@a@overall\endcsname{0.713}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@a@total\endcsname{0.806}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@b@afterpromoerr\endcsname{0.566}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@b@afterpromofa\endcsname{0.90}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@b@itembystore\endcsname{0.708}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@b@overall\endcsname{0.728}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@b@total\endcsname{0.844}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@c@afterpromoerr\endcsname{0.566}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@c@afterpromofa\endcsname{0.90}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@c@itembystore\endcsname{0.708}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@c@overall\endcsname{0.728}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@c@total\endcsname{0.844}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@mean@afterpromoerr\endcsname{0.567}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@mean@afterpromofa\endcsname{0.90}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@mean@itembystore\endcsname{0.710}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@mean@overall\endcsname{0.723}
\expandafter\def\csname rev@rpan@dev@ana@liftstock@mean@total\endcsname{0.831}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@a@afterpromoerr\endcsname{0.566}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@a@afterpromofa\endcsname{0.98}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@a@itembystore\endcsname{0.702}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@a@overall\endcsname{0.628}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@a@total\endcsname{0.626}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@b@afterpromoerr\endcsname{0.571}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@b@afterpromofa\endcsname{0.99}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@b@itembystore\endcsname{0.706}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@b@overall\endcsname{0.653}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@b@total\endcsname{0.683}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@c@afterpromoerr\endcsname{0.571}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@c@afterpromofa\endcsname{0.99}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@c@itembystore\endcsname{0.706}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@c@overall\endcsname{0.653}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@c@total\endcsname{0.683}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@mean@afterpromoerr\endcsname{0.569}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@mean@afterpromofa\endcsname{0.99}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@mean@itembystore\endcsname{0.705}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@mean@overall\endcsname{0.645}
\expandafter\def\csname rev@rpan@dev@ana@worldmodel@mean@total\endcsname{0.664}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@a@afterpromoerr\endcsname{0.556}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@a@afterpromofa\endcsname{1.05}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@a@itembystore\endcsname{0.868}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@a@overall\endcsname{1.015}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@a@total\endcsname{1.155}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@b@afterpromoerr\endcsname{0.547}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@b@afterpromofa\endcsname{1.03}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@b@itembystore\endcsname{0.871}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@b@overall\endcsname{1.040}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@b@total\endcsname{1.200}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@c@afterpromoerr\endcsname{0.547}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@c@afterpromofa\endcsname{1.03}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@c@itembystore\endcsname{0.871}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@c@overall\endcsname{1.040}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@c@total\endcsname{1.200}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@mean@afterpromoerr\endcsname{0.550}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@mean@afterpromofa\endcsname{1.04}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@mean@itembystore\endcsname{0.870}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@mean@overall\endcsname{1.032}
\expandafter\def\csname rev@rpan@dev@bjc@liftstock@mean@total\endcsname{1.185}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@a@afterpromoerr\endcsname{0.532}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@a@afterpromofa\endcsname{1.07}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@a@itembystore\endcsname{0.898}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@a@overall\endcsname{1.039}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@a@total\endcsname{1.174}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@b@afterpromoerr\endcsname{0.526}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@b@afterpromofa\endcsname{1.02}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@b@itembystore\endcsname{0.892}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@b@overall\endcsname{1.092}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@b@total\endcsname{1.270}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@c@afterpromoerr\endcsname{0.526}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@c@afterpromofa\endcsname{1.02}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@c@itembystore\endcsname{0.892}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@c@overall\endcsname{1.092}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@c@total\endcsname{1.270}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@mean@afterpromoerr\endcsname{0.528}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@mean@afterpromofa\endcsname{1.04}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@mean@itembystore\endcsname{0.894}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@mean@overall\endcsname{1.074}
\expandafter\def\csname rev@rpan@dev@bjc@worldmodel@mean@total\endcsname{1.238}
\expandafter\def\csname rev@rpan@dev@che@liftstock@a@afterpromoerr\endcsname{0.394}
\expandafter\def\csname rev@rpan@dev@che@liftstock@a@afterpromofa\endcsname{1.01}
\expandafter\def\csname rev@rpan@dev@che@liftstock@a@itembystore\endcsname{0.720}
\expandafter\def\csname rev@rpan@dev@che@liftstock@a@overall\endcsname{1.058}
\expandafter\def\csname rev@rpan@dev@che@liftstock@a@total\endcsname{1.345}
\expandafter\def\csname rev@rpan@dev@che@liftstock@b@afterpromoerr\endcsname{0.391}
\expandafter\def\csname rev@rpan@dev@che@liftstock@b@afterpromofa\endcsname{1.01}
\expandafter\def\csname rev@rpan@dev@che@liftstock@b@itembystore\endcsname{0.743}
\expandafter\def\csname rev@rpan@dev@che@liftstock@b@overall\endcsname{1.113}
\expandafter\def\csname rev@rpan@dev@che@liftstock@b@total\endcsname{1.417}
\expandafter\def\csname rev@rpan@dev@che@liftstock@c@afterpromoerr\endcsname{0.391}
\expandafter\def\csname rev@rpan@dev@che@liftstock@c@afterpromofa\endcsname{1.01}
\expandafter\def\csname rev@rpan@dev@che@liftstock@c@itembystore\endcsname{0.743}
\expandafter\def\csname rev@rpan@dev@che@liftstock@c@overall\endcsname{1.113}
\expandafter\def\csname rev@rpan@dev@che@liftstock@c@total\endcsname{1.417}
\expandafter\def\csname rev@rpan@dev@che@liftstock@mean@afterpromoerr\endcsname{0.392}
\expandafter\def\csname rev@rpan@dev@che@liftstock@mean@afterpromofa\endcsname{1.01}
\expandafter\def\csname rev@rpan@dev@che@liftstock@mean@itembystore\endcsname{0.735}
\expandafter\def\csname rev@rpan@dev@che@liftstock@mean@overall\endcsname{1.095}
\expandafter\def\csname rev@rpan@dev@che@liftstock@mean@total\endcsname{1.393}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@a@afterpromoerr\endcsname{0.411}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@a@afterpromofa\endcsname{1.08}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@a@itembystore\endcsname{0.804}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@a@overall\endcsname{1.345}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@a@total\endcsname{1.758}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@b@afterpromoerr\endcsname{0.402}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@b@afterpromofa\endcsname{1.04}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@b@itembystore\endcsname{0.792}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@b@overall\endcsname{1.281}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@b@total\endcsname{1.666}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@c@afterpromoerr\endcsname{0.402}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@c@afterpromofa\endcsname{1.04}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@c@itembystore\endcsname{0.792}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@c@overall\endcsname{1.281}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@c@total\endcsname{1.666}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@mean@afterpromoerr\endcsname{0.405}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@mean@afterpromofa\endcsname{1.05}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@mean@itembystore\endcsname{0.796}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@mean@overall\endcsname{1.302}
\expandafter\def\csname rev@rpan@dev@che@worldmodel@mean@total\endcsname{1.697}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@a@afterpromoerr\endcsname{0.402}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@a@afterpromofa\endcsname{0.61}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@a@itembystore\endcsname{0.504}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@a@overall\endcsname{0.377}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@a@total\endcsname{0.290}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@b@afterpromoerr\endcsname{0.398}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@b@afterpromofa\endcsname{0.71}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@b@itembystore\endcsname{0.497}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@b@overall\endcsname{0.388}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@b@total\endcsname{0.320}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@c@afterpromoerr\endcsname{0.398}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@c@afterpromofa\endcsname{0.71}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@c@itembystore\endcsname{0.497}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@c@overall\endcsname{0.388}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@c@total\endcsname{0.320}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@mean@afterpromoerr\endcsname{0.399}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@mean@afterpromofa\endcsname{0.68}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@mean@itembystore\endcsname{0.499}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@mean@overall\endcsname{0.384}
\expandafter\def\csname rev@rpan@dev@fre@liftstock@mean@total\endcsname{0.310}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@a@afterpromoerr\endcsname{0.389}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@a@afterpromofa\endcsname{0.75}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@a@itembystore\endcsname{0.502}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@a@overall\endcsname{0.398}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@a@total\endcsname{0.333}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@b@afterpromoerr\endcsname{0.391}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@b@afterpromofa\endcsname{0.66}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@b@itembystore\endcsname{0.502}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@b@overall\endcsname{0.387}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@b@total\endcsname{0.310}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@c@afterpromoerr\endcsname{0.391}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@c@afterpromofa\endcsname{0.66}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@c@itembystore\endcsname{0.502}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@c@overall\endcsname{0.387}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@c@total\endcsname{0.310}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@mean@afterpromoerr\endcsname{0.390}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@mean@afterpromofa\endcsname{0.69}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@mean@itembystore\endcsname{0.502}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@mean@overall\endcsname{0.391}
\expandafter\def\csname rev@rpan@dev@fre@worldmodel@mean@total\endcsname{0.318}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@a@afterpromoerr\endcsname{0.148}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@a@afterpromofa\endcsname{0.93}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@a@itembystore\endcsname{0.630}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@a@overall\endcsname{0.866}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@a@total\endcsname{1.073}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@b@afterpromoerr\endcsname{0.168}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@b@afterpromofa\endcsname{0.98}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@b@itembystore\endcsname{0.635}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@b@overall\endcsname{0.871}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@b@total\endcsname{1.076}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@c@afterpromoerr\endcsname{0.168}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@c@afterpromofa\endcsname{0.98}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@c@itembystore\endcsname{0.635}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@c@overall\endcsname{0.871}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@c@total\endcsname{1.076}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@mean@afterpromoerr\endcsname{0.161}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@mean@afterpromofa\endcsname{0.97}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@mean@itembystore\endcsname{0.633}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@mean@overall\endcsname{0.870}
\expandafter\def\csname rev@rpan@dev@sdr@liftstock@mean@total\endcsname{1.075}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@a@afterpromoerr\endcsname{0.128}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@a@afterpromofa\endcsname{1.00}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@a@itembystore\endcsname{0.627}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@a@overall\endcsname{0.812}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@a@total\endcsname{0.984}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@b@afterpromoerr\endcsname{0.174}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@b@afterpromofa\endcsname{0.97}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@b@itembystore\endcsname{0.618}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@b@overall\endcsname{0.829}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@b@total\endcsname{1.006}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@c@afterpromoerr\endcsname{0.174}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@c@afterpromofa\endcsname{0.97}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@c@itembystore\endcsname{0.618}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@c@overall\endcsname{0.829}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@c@total\endcsname{1.006}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@mean@afterpromoerr\endcsname{0.159}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@mean@afterpromofa\endcsname{0.98}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@mean@itembystore\endcsname{0.621}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@mean@overall\endcsname{0.823}
\expandafter\def\csname rev@rpan@dev@sdr@worldmodel@mean@total\endcsname{0.998}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@a@afterpromoerr\endcsname{0.468}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@a@afterpromofa\endcsname{0.93}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@a@itembystore\endcsname{0.739}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@a@overall\endcsname{0.712}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@a@total\endcsname{0.651}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@b@afterpromoerr\endcsname{0.488}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@b@afterpromofa\endcsname{0.93}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@b@itembystore\endcsname{0.790}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@b@overall\endcsname{0.756}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@b@total\endcsname{0.701}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@c@afterpromoerr\endcsname{0.488}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@c@afterpromofa\endcsname{0.93}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@c@itembystore\endcsname{0.790}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@c@overall\endcsname{0.756}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@c@total\endcsname{0.701}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@mean@afterpromoerr\endcsname{0.481}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@mean@afterpromofa\endcsname{0.93}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@mean@itembystore\endcsname{0.773}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@mean@overall\endcsname{0.741}
\expandafter\def\csname rev@rpan@dev@sna@liftstock@mean@total\endcsname{0.684}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@a@afterpromoerr\endcsname{0.431}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@a@afterpromofa\endcsname{1.04}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@a@itembystore\endcsname{0.707}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@a@overall\endcsname{0.911}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@a@total\endcsname{0.983}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@b@afterpromoerr\endcsname{0.477}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@b@afterpromofa\endcsname{1.02}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@b@itembystore\endcsname{0.795}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@b@overall\endcsname{0.749}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@b@total\endcsname{0.683}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@c@afterpromoerr\endcsname{0.477}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@c@afterpromofa\endcsname{1.02}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@c@itembystore\endcsname{0.795}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@c@overall\endcsname{0.749}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@c@total\endcsname{0.683}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@mean@afterpromoerr\endcsname{0.462}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@mean@afterpromofa\endcsname{1.03}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@mean@itembystore\endcsname{0.766}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@mean@overall\endcsname{0.803}
\expandafter\def\csname rev@rpan@dev@sna@worldmodel@mean@total\endcsname{0.783}
\expandafter\def\csname rev@rpan@rol@ana@lift@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@ana@lift@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@ana@lift@roll@itembystore\endcsname{0.677}
\expandafter\def\csname rev@rpan@rol@ana@lift@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@ana@lift@roll@total\endcsname{0.868}
\expandafter\def\csname rev@rpan@rol@ana@liftstock@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@ana@liftstock@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@ana@liftstock@roll@itembystore\endcsname{0.674}
\expandafter\def\csname rev@rpan@rol@ana@liftstock@roll@overall\endcsname{0.764}
\expandafter\def\csname rev@rpan@rol@ana@liftstock@roll@total\endcsname{0.948}
\expandafter\def\csname rev@rpan@rol@ana@lightgbm@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@ana@lightgbm@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@ana@lightgbm@roll@itembystore\endcsname{0.647}
\expandafter\def\csname rev@rpan@rol@ana@lightgbm@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@ana@lightgbm@roll@total\endcsname{0.869}
\expandafter\def\csname rev@rpan@rol@ana@worldmodel@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@ana@worldmodel@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@ana@worldmodel@roll@itembystore\endcsname{0.672}
\expandafter\def\csname rev@rpan@rol@ana@worldmodel@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@ana@worldmodel@roll@total\endcsname{0.826}
\expandafter\def\csname rev@rpan@rol@bjc@lift@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@bjc@lift@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@bjc@lift@roll@itembystore\endcsname{0.616}
\expandafter\def\csname rev@rpan@rol@bjc@lift@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@bjc@lift@roll@total\endcsname{0.585}
\expandafter\def\csname rev@rpan@rol@bjc@liftstock@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@bjc@liftstock@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@bjc@liftstock@roll@itembystore\endcsname{0.622}
\expandafter\def\csname rev@rpan@rol@bjc@liftstock@roll@overall\endcsname{0.578}
\expandafter\def\csname rev@rpan@rol@bjc@liftstock@roll@total\endcsname{0.540}
\expandafter\def\csname rev@rpan@rol@bjc@lightgbm@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@bjc@lightgbm@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@bjc@lightgbm@roll@itembystore\endcsname{0.605}
\expandafter\def\csname rev@rpan@rol@bjc@lightgbm@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@bjc@lightgbm@roll@total\endcsname{0.530}
\expandafter\def\csname rev@rpan@rol@bjc@worldmodel@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@bjc@worldmodel@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@bjc@worldmodel@roll@itembystore\endcsname{0.656}
\expandafter\def\csname rev@rpan@rol@bjc@worldmodel@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@bjc@worldmodel@roll@total\endcsname{0.613}
\expandafter\def\csname rev@rpan@rol@che@lift@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@che@lift@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@che@lift@roll@itembystore\endcsname{1.119}
\expandafter\def\csname rev@rpan@rol@che@lift@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@che@lift@roll@total\endcsname{0.617}
\expandafter\def\csname rev@rpan@rol@che@liftstock@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@che@liftstock@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@che@liftstock@roll@itembystore\endcsname{1.324}
\expandafter\def\csname rev@rpan@rol@che@liftstock@roll@overall\endcsname{0.805}
\expandafter\def\csname rev@rpan@rol@che@liftstock@roll@total\endcsname{0.556}
\expandafter\def\csname rev@rpan@rol@che@lightgbm@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@che@lightgbm@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@che@lightgbm@roll@itembystore\endcsname{0.623}
\expandafter\def\csname rev@rpan@rol@che@lightgbm@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@che@lightgbm@roll@total\endcsname{0.456}
\expandafter\def\csname rev@rpan@rol@che@worldmodel@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@che@worldmodel@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@che@worldmodel@roll@itembystore\endcsname{1.713}
\expandafter\def\csname rev@rpan@rol@che@worldmodel@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@che@worldmodel@roll@total\endcsname{0.585}
\expandafter\def\csname rev@rpan@rol@fre@lift@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@fre@lift@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@fre@lift@roll@itembystore\endcsname{0.449}
\expandafter\def\csname rev@rpan@rol@fre@lift@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@fre@lift@roll@total\endcsname{0.387}
\expandafter\def\csname rev@rpan@rol@fre@liftstock@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@fre@liftstock@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@fre@liftstock@roll@itembystore\endcsname{0.447}
\expandafter\def\csname rev@rpan@rol@fre@liftstock@roll@overall\endcsname{0.397}
\expandafter\def\csname rev@rpan@rol@fre@liftstock@roll@total\endcsname{0.376}
\expandafter\def\csname rev@rpan@rol@fre@lightgbm@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@fre@lightgbm@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@fre@lightgbm@roll@itembystore\endcsname{0.410}
\expandafter\def\csname rev@rpan@rol@fre@lightgbm@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@fre@lightgbm@roll@total\endcsname{0.321}
\expandafter\def\csname rev@rpan@rol@fre@worldmodel@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@fre@worldmodel@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@fre@worldmodel@roll@itembystore\endcsname{0.433}
\expandafter\def\csname rev@rpan@rol@fre@worldmodel@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@fre@worldmodel@roll@total\endcsname{0.338}
\expandafter\def\csname rev@rpan@rol@sdr@lift@roll@afterpromoerr\endcsname{0.206}
\expandafter\def\csname rev@rpan@rol@sdr@lift@roll@afterpromofa\endcsname{1.28}
\expandafter\def\csname rev@rpan@rol@sdr@lift@roll@itembystore\endcsname{0.672}
\expandafter\def\csname rev@rpan@rol@sdr@lift@roll@overall\endcsname{0.850}
\expandafter\def\csname rev@rpan@rol@sdr@lift@roll@total\endcsname{0.965}
\expandafter\def\csname rev@rpan@rol@sdr@liftstock@roll@afterpromoerr\endcsname{0.208}
\expandafter\def\csname rev@rpan@rol@sdr@liftstock@roll@afterpromofa\endcsname{1.27}
\expandafter\def\csname rev@rpan@rol@sdr@liftstock@roll@itembystore\endcsname{0.650}
\expandafter\def\csname rev@rpan@rol@sdr@liftstock@roll@overall\endcsname{0.817}
\expandafter\def\csname rev@rpan@rol@sdr@liftstock@roll@total\endcsname{0.931}
\expandafter\def\csname rev@rpan@rol@sdr@lightgbm@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@sdr@lightgbm@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@sdr@lightgbm@roll@itembystore\endcsname{0.545}
\expandafter\def\csname rev@rpan@rol@sdr@lightgbm@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@sdr@lightgbm@roll@total\endcsname{0.831}
\expandafter\def\csname rev@rpan@rol@sdr@worldmodel@roll@afterpromoerr\endcsname{0.151}
\expandafter\def\csname rev@rpan@rol@sdr@worldmodel@roll@afterpromofa\endcsname{1.19}
\expandafter\def\csname rev@rpan@rol@sdr@worldmodel@roll@itembystore\endcsname{0.600}
\expandafter\def\csname rev@rpan@rol@sdr@worldmodel@roll@overall\endcsname{0.760}
\expandafter\def\csname rev@rpan@rol@sdr@worldmodel@roll@total\endcsname{0.879}
\expandafter\def\csname rev@rpan@rol@sna@lift@roll@afterpromoerr\endcsname{0.420}
\expandafter\def\csname rev@rpan@rol@sna@lift@roll@afterpromofa\endcsname{1.03}
\expandafter\def\csname rev@rpan@rol@sna@lift@roll@itembystore\endcsname{0.598}
\expandafter\def\csname rev@rpan@rol@sna@lift@roll@overall\endcsname{1.023}
\expandafter\def\csname rev@rpan@rol@sna@lift@roll@total\endcsname{1.026}
\expandafter\def\csname rev@rpan@rol@sna@liftstock@roll@afterpromoerr\endcsname{0.420}
\expandafter\def\csname rev@rpan@rol@sna@liftstock@roll@afterpromofa\endcsname{1.16}
\expandafter\def\csname rev@rpan@rol@sna@liftstock@roll@itembystore\endcsname{0.595}
\expandafter\def\csname rev@rpan@rol@sna@liftstock@roll@overall\endcsname{1.166}
\expandafter\def\csname rev@rpan@rol@sna@liftstock@roll@total\endcsname{1.510}
\expandafter\def\csname rev@rpan@rol@sna@lightgbm@roll@afterpromoerr\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@sna@lightgbm@roll@afterpromofa\endcsname{nan}
\expandafter\def\csname rev@rpan@rol@sna@lightgbm@roll@itembystore\endcsname{0.578}
\expandafter\def\csname rev@rpan@rol@sna@lightgbm@roll@overall\endcsname{n/a}
\expandafter\def\csname rev@rpan@rol@sna@lightgbm@roll@total\endcsname{1.097}
\expandafter\def\csname rev@rpan@rol@sna@worldmodel@roll@afterpromoerr\endcsname{0.416}
\expandafter\def\csname rev@rpan@rol@sna@worldmodel@roll@afterpromofa\endcsname{1.17}
\expandafter\def\csname rev@rpan@rol@sna@worldmodel@roll@itembystore\endcsname{0.595}
\expandafter\def\csname rev@rpan@rol@sna@worldmodel@roll@overall\endcsname{1.095}
\expandafter\def\csname rev@rpan@rol@sna@worldmodel@roll@total\endcsname{1.454}
\expandafter\def\csname rev@rper@dom@lgb@price@occlude@ixs\endcsname{20}
\expandafter\def\csname rev@rper@dom@lgb@price@occlude@total\endcsname{115}
\expandafter\def\csname rev@rper@dom@lgb@price@occlude@units\endcsname{\textminus{}49}
\expandafter\def\csname rev@rper@dom@lgb@price@permute@ixs\endcsname{32}
\expandafter\def\csname rev@rper@dom@lgb@price@permute@total\endcsname{31}
\expandafter\def\csname rev@rper@dom@lgb@price@permute@units\endcsname{\textminus{}26}
\expandafter\def\csname rev@rper@dom@lgb@promo@occlude@ixs\endcsname{3}
\expandafter\def\csname rev@rper@dom@lgb@promo@occlude@total\endcsname{34}
\expandafter\def\csname rev@rper@dom@lgb@promo@occlude@units\endcsname{\textminus{}26}
\expandafter\def\csname rev@rper@dom@lgb@promo@permute@ixs\endcsname{3}
\expandafter\def\csname rev@rper@dom@lgb@promo@permute@total\endcsname{3}
\expandafter\def\csname rev@rper@dom@lgb@promo@permute@units\endcsname{\textminus{}16}
\expandafter\def\csname rev@rper@dom@lgb@wholeplan@occlude@ixs\endcsname{26}
\expandafter\def\csname rev@rper@dom@lgb@wholeplan@occlude@total\endcsname{149}
\expandafter\def\csname rev@rper@dom@lgb@wholeplan@occlude@units\endcsname{\textminus{}58}
\expandafter\def\csname rev@rper@dom@lift@historylast13@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@dom@lift@historylast13@occlude@total\endcsname{45}
\expandafter\def\csname rev@rper@dom@lift@historylast26@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@dom@lift@historylast26@occlude@total\endcsname{0}
\expandafter\def\csname rev@rper@dom@lift@historylast4@occlude@ixs\endcsname{6}
\expandafter\def\csname rev@rper@dom@lift@historylast4@occlude@total\endcsname{72}
\expandafter\def\csname rev@rper@dom@lift@price@occlude@ixs\endcsname{6}
\expandafter\def\csname rev@rper@dom@lift@price@occlude@total\endcsname{59}
\expandafter\def\csname rev@rper@dom@lift@price@occlude@units\endcsname{\textminus{}41}
\expandafter\def\csname rev@rper@dom@lift@price@permute@ixs\endcsname{15}
\expandafter\def\csname rev@rper@dom@lift@price@permute@total\endcsname{19}
\expandafter\def\csname rev@rper@dom@lift@price@permute@units\endcsname{\textminus{}24}
\expandafter\def\csname rev@rper@dom@lift@promo@occlude@ixs\endcsname{2}
\expandafter\def\csname rev@rper@dom@lift@promo@occlude@total\endcsname{38}
\expandafter\def\csname rev@rper@dom@lift@promo@occlude@units\endcsname{\textminus{}40}
\expandafter\def\csname rev@rper@dom@lift@promo@permute@ixs\endcsname{7}
\expandafter\def\csname rev@rper@dom@lift@promo@permute@total\endcsname{3}
\expandafter\def\csname rev@rper@dom@lift@promo@permute@units\endcsname{\textminus{}27}
\expandafter\def\csname rev@rper@dom@lift@wholeplan@occlude@ixs\endcsname{13}
\expandafter\def\csname rev@rper@dom@lift@wholeplan@occlude@total\endcsname{97}
\expandafter\def\csname rev@rper@dom@lift@wholeplan@occlude@units\endcsname{\textminus{}58}
\expandafter\def\csname rev@rper@dom@world@historylast13@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@dom@world@historylast13@occlude@total\endcsname{37}
\expandafter\def\csname rev@rper@dom@world@historylast26@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@dom@world@historylast26@occlude@total\endcsname{0}
\expandafter\def\csname rev@rper@dom@world@historylast4@occlude@ixs\endcsname{5}
\expandafter\def\csname rev@rper@dom@world@historylast4@occlude@total\endcsname{42}
\expandafter\def\csname rev@rper@dom@world@price@occlude@ixs\endcsname{8}
\expandafter\def\csname rev@rper@dom@world@price@occlude@total\endcsname{75}
\expandafter\def\csname rev@rper@dom@world@price@occlude@units\endcsname{\textminus{}45}
\expandafter\def\csname rev@rper@dom@world@price@permute@ixs\endcsname{24}
\expandafter\def\csname rev@rper@dom@world@price@permute@total\endcsname{30}
\expandafter\def\csname rev@rper@dom@world@price@permute@units\endcsname{\textminus{}26}
\expandafter\def\csname rev@rper@dom@world@promo@occlude@ixs\endcsname{4}
\expandafter\def\csname rev@rper@dom@world@promo@occlude@total\endcsname{41}
\expandafter\def\csname rev@rper@dom@world@promo@occlude@units\endcsname{\textminus{}34}
\expandafter\def\csname rev@rper@dom@world@promo@permute@ixs\endcsname{6}
\expandafter\def\csname rev@rper@dom@world@promo@permute@total\endcsname{7}
\expandafter\def\csname rev@rper@dom@world@promo@permute@units\endcsname{\textminus{}22}
\expandafter\def\csname rev@rper@dom@world@wholeplan@occlude@ixs\endcsname{15}
\expandafter\def\csname rev@rper@dom@world@wholeplan@occlude@total\endcsname{116}
\expandafter\def\csname rev@rper@dom@world@wholeplan@occlude@units\endcsname{\textminus{}59}
\expandafter\def\csname rev@rper@frat@lgb@display@occlude@ixs\endcsname{2}
\expandafter\def\csname rev@rper@frat@lgb@display@occlude@total\endcsname{4}
\expandafter\def\csname rev@rper@frat@lgb@display@occlude@units\endcsname{\textminus{}17}
\expandafter\def\csname rev@rper@frat@lgb@display@permute@ixs\endcsname{3}
\expandafter\def\csname rev@rper@frat@lgb@display@permute@total\endcsname{\textminus{}5}
\expandafter\def\csname rev@rper@frat@lgb@display@permute@units\endcsname{\textminus{}11}
\expandafter\def\csname rev@rper@frat@lgb@feature@occlude@ixs\endcsname{4}
\expandafter\def\csname rev@rper@frat@lgb@feature@occlude@total\endcsname{16}
\expandafter\def\csname rev@rper@frat@lgb@feature@occlude@units\endcsname{\textminus{}29}
\expandafter\def\csname rev@rper@frat@lgb@feature@permute@ixs\endcsname{5}
\expandafter\def\csname rev@rper@frat@lgb@feature@permute@total\endcsname{\textminus{}7}
\expandafter\def\csname rev@rper@frat@lgb@feature@permute@units\endcsname{\textminus{}21}
\expandafter\def\csname rev@rper@frat@lgb@price@occlude@ixs\endcsname{18}
\expandafter\def\csname rev@rper@frat@lgb@price@occlude@total\endcsname{138}
\expandafter\def\csname rev@rper@frat@lgb@price@occlude@units\endcsname{\textminus{}34}
\expandafter\def\csname rev@rper@frat@lgb@price@permute@ixs\endcsname{17}
\expandafter\def\csname rev@rper@frat@lgb@price@permute@total\endcsname{2}
\expandafter\def\csname rev@rper@frat@lgb@price@permute@units\endcsname{\textminus{}15}
\expandafter\def\csname rev@rper@frat@lgb@promo@occlude@ixs\endcsname{4}
\expandafter\def\csname rev@rper@frat@lgb@promo@occlude@total\endcsname{34}
\expandafter\def\csname rev@rper@frat@lgb@promo@occlude@units\endcsname{\textminus{}18}
\expandafter\def\csname rev@rper@frat@lgb@promo@permute@ixs\endcsname{3}
\expandafter\def\csname rev@rper@frat@lgb@promo@permute@total\endcsname{\textminus{}12}
\expandafter\def\csname rev@rper@frat@lgb@promo@permute@units\endcsname{\textminus{}10}
\expandafter\def\csname rev@rper@frat@lgb@tpronly@occlude@ixs\endcsname{1}
\expandafter\def\csname rev@rper@frat@lgb@tpronly@occlude@total\endcsname{3}
\expandafter\def\csname rev@rper@frat@lgb@tpronly@occlude@units\endcsname{10}
\expandafter\def\csname rev@rper@frat@lgb@tpronly@permute@ixs\endcsname{1}
\expandafter\def\csname rev@rper@frat@lgb@tpronly@permute@total\endcsname{1}
\expandafter\def\csname rev@rper@frat@lgb@tpronly@permute@units\endcsname{6}
\expandafter\def\csname rev@rper@frat@lgb@wholeplan@occlude@ixs\endcsname{40}
\expandafter\def\csname rev@rper@frat@lgb@wholeplan@occlude@total\endcsname{262}
\expandafter\def\csname rev@rper@frat@lgb@wholeplan@occlude@units\endcsname{\textminus{}46}
\expandafter\def\csname rev@rper@frat@lift@display@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@frat@lift@display@occlude@total\endcsname{9}
\expandafter\def\csname rev@rper@frat@lift@display@occlude@units\endcsname{\textminus{}19}
\expandafter\def\csname rev@rper@frat@lift@display@permute@ixs\endcsname{1}
\expandafter\def\csname rev@rper@frat@lift@display@permute@total\endcsname{\textminus{}5}
\expandafter\def\csname rev@rper@frat@lift@display@permute@units\endcsname{\textminus{}12}
\expandafter\def\csname rev@rper@frat@lift@feature@occlude@ixs\endcsname{2}
\expandafter\def\csname rev@rper@frat@lift@feature@occlude@total\endcsname{23}
\expandafter\def\csname rev@rper@frat@lift@feature@occlude@units\endcsname{\textminus{}28}
\expandafter\def\csname rev@rper@frat@lift@feature@permute@ixs\endcsname{2}
\expandafter\def\csname rev@rper@frat@lift@feature@permute@total\endcsname{0}
\expandafter\def\csname rev@rper@frat@lift@feature@permute@units\endcsname{\textminus{}20}
\expandafter\def\csname rev@rper@frat@lift@historylast13@occlude@ixs\endcsname{2}
\expandafter\def\csname rev@rper@frat@lift@historylast13@occlude@total\endcsname{\textminus{}7}
\expandafter\def\csname rev@rper@frat@lift@historylast26@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@frat@lift@historylast26@occlude@total\endcsname{0}
\expandafter\def\csname rev@rper@frat@lift@historylast4@occlude@ixs\endcsname{16}
\expandafter\def\csname rev@rper@frat@lift@historylast4@occlude@total\endcsname{92}
\expandafter\def\csname rev@rper@frat@lift@price@occlude@ixs\endcsname{16}
\expandafter\def\csname rev@rper@frat@lift@price@occlude@total\endcsname{152}
\expandafter\def\csname rev@rper@frat@lift@price@occlude@units\endcsname{\textminus{}36}
\expandafter\def\csname rev@rper@frat@lift@price@permute@ixs\endcsname{13}
\expandafter\def\csname rev@rper@frat@lift@price@permute@total\endcsname{16}
\expandafter\def\csname rev@rper@frat@lift@price@permute@units\endcsname{\textminus{}18}
\expandafter\def\csname rev@rper@frat@lift@promo@occlude@ixs\endcsname{6}
\expandafter\def\csname rev@rper@frat@lift@promo@occlude@total\endcsname{99}
\expandafter\def\csname rev@rper@frat@lift@promo@occlude@units\endcsname{\textminus{}30}
\expandafter\def\csname rev@rper@frat@lift@promo@permute@ixs\endcsname{5}
\expandafter\def\csname rev@rper@frat@lift@promo@permute@total\endcsname{2}
\expandafter\def\csname rev@rper@frat@lift@promo@permute@units\endcsname{\textminus{}16}
\expandafter\def\csname rev@rper@frat@lift@tpronly@occlude@ixs\endcsname{1}
\expandafter\def\csname rev@rper@frat@lift@tpronly@occlude@total\endcsname{10}
\expandafter\def\csname rev@rper@frat@lift@tpronly@occlude@units\endcsname{16}
\expandafter\def\csname rev@rper@frat@lift@tpronly@permute@ixs\endcsname{1}
\expandafter\def\csname rev@rper@frat@lift@tpronly@permute@total\endcsname{4}
\expandafter\def\csname rev@rper@frat@lift@tpronly@permute@units\endcsname{10}
\expandafter\def\csname rev@rper@frat@lift@wholeplan@occlude@ixs\endcsname{36}
\expandafter\def\csname rev@rper@frat@lift@wholeplan@occlude@total\endcsname{268}
\expandafter\def\csname rev@rper@frat@lift@wholeplan@occlude@units\endcsname{\textminus{}47}
\expandafter\def\csname rev@rper@frat@world@display@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@frat@world@display@occlude@total\endcsname{4}
\expandafter\def\csname rev@rper@frat@world@display@occlude@units\endcsname{\textminus{}18}
\expandafter\def\csname rev@rper@frat@world@display@permute@ixs\endcsname{1}
\expandafter\def\csname rev@rper@frat@world@display@permute@total\endcsname{\textminus{}6}
\expandafter\def\csname rev@rper@frat@world@display@permute@units\endcsname{\textminus{}10}
\expandafter\def\csname rev@rper@frat@world@feature@occlude@ixs\endcsname{1}
\expandafter\def\csname rev@rper@frat@world@feature@occlude@total\endcsname{7}
\expandafter\def\csname rev@rper@frat@world@feature@occlude@units\endcsname{\textminus{}28}
\expandafter\def\csname rev@rper@frat@world@feature@permute@ixs\endcsname{2}
\expandafter\def\csname rev@rper@frat@world@feature@permute@total\endcsname{\textminus{}9}
\expandafter\def\csname rev@rper@frat@world@feature@permute@units\endcsname{\textminus{}19}
\expandafter\def\csname rev@rper@frat@world@historylast13@occlude@ixs\endcsname{7}
\expandafter\def\csname rev@rper@frat@world@historylast13@occlude@total\endcsname{42}
\expandafter\def\csname rev@rper@frat@world@historylast26@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@frat@world@historylast26@occlude@total\endcsname{0}
\expandafter\def\csname rev@rper@frat@world@historylast4@occlude@ixs\endcsname{18}
\expandafter\def\csname rev@rper@frat@world@historylast4@occlude@total\endcsname{100}
\expandafter\def\csname rev@rper@frat@world@price@occlude@ixs\endcsname{17}
\expandafter\def\csname rev@rper@frat@world@price@occlude@total\endcsname{126}
\expandafter\def\csname rev@rper@frat@world@price@occlude@units\endcsname{\textminus{}38}
\expandafter\def\csname rev@rper@frat@world@price@permute@ixs\endcsname{20}
\expandafter\def\csname rev@rper@frat@world@price@permute@total\endcsname{\textminus{}2}
\expandafter\def\csname rev@rper@frat@world@price@permute@units\endcsname{\textminus{}19}
\expandafter\def\csname rev@rper@frat@world@promo@occlude@ixs\endcsname{\textminus{}1}
\expandafter\def\csname rev@rper@frat@world@promo@occlude@total\endcsname{20}
\expandafter\def\csname rev@rper@frat@world@promo@occlude@units\endcsname{\textminus{}16}
\expandafter\def\csname rev@rper@frat@world@promo@permute@ixs\endcsname{0}
\expandafter\def\csname rev@rper@frat@world@promo@permute@total\endcsname{\textminus{}14}
\expandafter\def\csname rev@rper@frat@world@promo@permute@units\endcsname{\textminus{}9}
\expandafter\def\csname rev@rper@frat@world@tpronly@occlude@ixs\endcsname{1}
\expandafter\def\csname rev@rper@frat@world@tpronly@occlude@total\endcsname{9}
\expandafter\def\csname rev@rper@frat@world@tpronly@occlude@units\endcsname{14}
\expandafter\def\csname rev@rper@frat@world@tpronly@permute@ixs\endcsname{1}
\expandafter\def\csname rev@rper@frat@world@tpronly@permute@total\endcsname{2}
\expandafter\def\csname rev@rper@frat@world@tpronly@permute@units\endcsname{9}
\expandafter\def\csname rev@rper@frat@world@wholeplan@occlude@ixs\endcsname{36}
\expandafter\def\csname rev@rper@frat@world@wholeplan@occlude@total\endcsname{229}
\expandafter\def\csname rev@rper@frat@world@wholeplan@occlude@units\endcsname{\textminus{}49}
\expandafter\def\csname rev@rper@mfive@lgb@event@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@lgb@event@occlude@total\endcsname{0}
\expandafter\def\csname rev@rper@mfive@lgb@event@occlude@units\endcsname{2}
\expandafter\def\csname rev@rper@mfive@lgb@event@permute@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@lgb@event@permute@total\endcsname{5}
\expandafter\def\csname rev@rper@mfive@lgb@event@permute@units\endcsname{2}
\expandafter\def\csname rev@rper@mfive@lgb@price@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@lgb@price@occlude@total\endcsname{\textminus{}1}
\expandafter\def\csname rev@rper@mfive@lgb@price@occlude@units\endcsname{18}
\expandafter\def\csname rev@rper@mfive@lgb@price@permute@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@lgb@price@permute@total\endcsname{0}
\expandafter\def\csname rev@rper@mfive@lgb@price@permute@units\endcsname{2}
\expandafter\def\csname rev@rper@mfive@lgb@snap@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@lgb@snap@occlude@total\endcsname{16}
\expandafter\def\csname rev@rper@mfive@lgb@snap@occlude@units\endcsname{\textminus{}6}
\expandafter\def\csname rev@rper@mfive@lgb@snap@permute@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@lgb@snap@permute@total\endcsname{2}
\expandafter\def\csname rev@rper@mfive@lgb@snap@permute@units\endcsname{\textminus{}4}
\expandafter\def\csname rev@rper@mfive@lgb@wholeplan@occlude@ixs\endcsname{1}
\expandafter\def\csname rev@rper@mfive@lgb@wholeplan@occlude@total\endcsname{15}
\expandafter\def\csname rev@rper@mfive@lgb@wholeplan@occlude@units\endcsname{\textminus{}4}
\expandafter\def\csname rev@rper@mfive@lift@event@occlude@ixs\endcsname{1}
\expandafter\def\csname rev@rper@mfive@lift@event@occlude@total\endcsname{18}
\expandafter\def\csname rev@rper@mfive@lift@event@occlude@units\endcsname{20}
\expandafter\def\csname rev@rper@mfive@lift@event@permute@ixs\endcsname{1}
\expandafter\def\csname rev@rper@mfive@lift@event@permute@total\endcsname{19}
\expandafter\def\csname rev@rper@mfive@lift@event@permute@units\endcsname{18}
\expandafter\def\csname rev@rper@mfive@lift@historylast28@occlude@ixs\endcsname{24}
\expandafter\def\csname rev@rper@mfive@lift@historylast28@occlude@total\endcsname{255}
\expandafter\def\csname rev@rper@mfive@lift@historylast56@occlude@ixs\endcsname{6}
\expandafter\def\csname rev@rper@mfive@lift@historylast56@occlude@total\endcsname{42}
\expandafter\def\csname rev@rper@mfive@lift@price@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@lift@price@occlude@total\endcsname{\textminus{}26}
\expandafter\def\csname rev@rper@mfive@lift@price@occlude@units\endcsname{\textminus{}60}
\expandafter\def\csname rev@rper@mfive@lift@price@permute@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@lift@price@permute@total\endcsname{11}
\expandafter\def\csname rev@rper@mfive@lift@price@permute@units\endcsname{\textminus{}37}
\expandafter\def\csname rev@rper@mfive@lift@snap@occlude@ixs\endcsname{2}
\expandafter\def\csname rev@rper@mfive@lift@snap@occlude@total\endcsname{30}
\expandafter\def\csname rev@rper@mfive@lift@snap@occlude@units\endcsname{\textminus{}14}
\expandafter\def\csname rev@rper@mfive@lift@snap@permute@ixs\endcsname{2}
\expandafter\def\csname rev@rper@mfive@lift@snap@permute@total\endcsname{14}
\expandafter\def\csname rev@rper@mfive@lift@snap@permute@units\endcsname{\textminus{}10}
\expandafter\def\csname rev@rper@mfive@lift@wholeplan@occlude@ixs\endcsname{1}
\expandafter\def\csname rev@rper@mfive@lift@wholeplan@occlude@total\endcsname{14}
\expandafter\def\csname rev@rper@mfive@lift@wholeplan@occlude@units\endcsname{\textminus{}19}
\expandafter\def\csname rev@rper@mfive@world@event@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@world@event@occlude@total\endcsname{16}
\expandafter\def\csname rev@rper@mfive@world@event@occlude@units\endcsname{15}
\expandafter\def\csname rev@rper@mfive@world@event@permute@ixs\endcsname{1}
\expandafter\def\csname rev@rper@mfive@world@event@permute@total\endcsname{18}
\expandafter\def\csname rev@rper@mfive@world@event@permute@units\endcsname{11}
\expandafter\def\csname rev@rper@mfive@world@historylast28@occlude@ixs\endcsname{42}
\expandafter\def\csname rev@rper@mfive@world@historylast28@occlude@total\endcsname{615}
\expandafter\def\csname rev@rper@mfive@world@historylast56@occlude@ixs\endcsname{11}
\expandafter\def\csname rev@rper@mfive@world@historylast56@occlude@total\endcsname{219}
\expandafter\def\csname rev@rper@mfive@world@price@occlude@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@world@price@occlude@total\endcsname{3}
\expandafter\def\csname rev@rper@mfive@world@price@occlude@units\endcsname{\textminus{}35}
\expandafter\def\csname rev@rper@mfive@world@price@permute@ixs\endcsname{0}
\expandafter\def\csname rev@rper@mfive@world@price@permute@total\endcsname{0}
\expandafter\def\csname rev@rper@mfive@world@price@permute@units\endcsname{\textminus{}13}
\expandafter\def\csname rev@rper@mfive@world@snap@occlude@ixs\endcsname{1}
\expandafter\def\csname rev@rper@mfive@world@snap@occlude@total\endcsname{58}
\expandafter\def\csname rev@rper@mfive@world@snap@occlude@units\endcsname{\textminus{}14}
\expandafter\def\csname rev@rper@mfive@world@snap@permute@ixs\endcsname{1}
\expandafter\def\csname rev@rper@mfive@world@snap@permute@total\endcsname{20}
\expandafter\def\csname rev@rper@mfive@world@snap@permute@units\endcsname{\textminus{}9}
\expandafter\def\csname rev@rper@mfive@world@wholeplan@occlude@ixs\endcsname{1}
\expandafter\def\csname rev@rper@mfive@world@wholeplan@occlude@total\endcsname{45}
\expandafter\def\csname rev@rper@mfive@world@wholeplan@occlude@units\endcsname{\textminus{}8}
\expandafter\def\csname rev@rrank@dom@ens@catidxstoreid@mediannoderatio\endcsname{0.99}
\expandafter\def\csname rev@rrank@dom@ens@catidxstoreid@spearman\endcsname{0.41}
\expandafter\def\csname rev@rrank@dom@ens@catidxstoreid@topdecilehit\endcsname{0.35}
\expandafter\def\csname rev@rrank@dom@ens@catidxstoreid@totalratio\endcsname{0.98}
\expandafter\def\csname rev@rrank@dom@ens@ixs@mediannoderatio\endcsname{1.03}
\expandafter\def\csname rev@rrank@dom@ens@ixs@promospearman\endcsname{0.66}
\expandafter\def\csname rev@rrank@dom@ens@ixs@spearman\endcsname{0.61}
\expandafter\def\csname rev@rrank@dom@ens@ixs@topdecilehit\endcsname{0.57}
\expandafter\def\csname rev@rrank@dom@ens@ixs@totalratio\endcsname{0.98}
\expandafter\def\csname rev@rrank@dom@ensfour@catidxstoreid@mediannoderatio\endcsname{1.37}
\expandafter\def\csname rev@rrank@dom@ensfour@catidxstoreid@spearman\endcsname{0.22}
\expandafter\def\csname rev@rrank@dom@ensfour@catidxstoreid@topdecilehit\endcsname{0.25}
\expandafter\def\csname rev@rrank@dom@ensfour@catidxstoreid@totalratio\endcsname{1.49}
\expandafter\def\csname rev@rrank@dom@ensfour@ixs@mediannoderatio\endcsname{1.11}
\expandafter\def\csname rev@rrank@dom@ensfour@ixs@promospearman\endcsname{0.65}
\expandafter\def\csname rev@rrank@dom@ensfour@ixs@spearman\endcsname{0.58}
\expandafter\def\csname rev@rrank@dom@ensfour@ixs@topdecilehit\endcsname{0.53}
\expandafter\def\csname rev@rrank@dom@ensfour@ixs@totalratio\endcsname{1.49}
\expandafter\def\csname rev@rrank@dom@enstimestral@catidxstoreid@mediannoderatio\endcsname{1.50}
\expandafter\def\csname rev@rrank@dom@enstimestral@catidxstoreid@spearman\endcsname{0.20}
\expandafter\def\csname rev@rrank@dom@enstimestral@catidxstoreid@topdecilehit\endcsname{0.24}
\expandafter\def\csname rev@rrank@dom@enstimestral@catidxstoreid@totalratio\endcsname{1.66}
\expandafter\def\csname rev@rrank@dom@enstimestral@ixs@mediannoderatio\endcsname{1.13}
\expandafter\def\csname rev@rrank@dom@enstimestral@ixs@promospearman\endcsname{0.66}
\expandafter\def\csname rev@rrank@dom@enstimestral@ixs@spearman\endcsname{0.58}
\expandafter\def\csname rev@rrank@dom@enstimestral@ixs@topdecilehit\endcsname{0.53}
\expandafter\def\csname rev@rrank@dom@enstimestral@ixs@totalratio\endcsname{1.66}
\expandafter\def\csname rev@rrank@dom@lgb@catidxstoreid@mediannoderatio\endcsname{0.97}
\expandafter\def\csname rev@rrank@dom@lgb@catidxstoreid@spearman\endcsname{0.42}
\expandafter\def\csname rev@rrank@dom@lgb@catidxstoreid@topdecilehit\endcsname{0.33}
\expandafter\def\csname rev@rrank@dom@lgb@catidxstoreid@totalratio\endcsname{0.96}
\expandafter\def\csname rev@rrank@dom@lgb@ixs@mediannoderatio\endcsname{1.03}
\expandafter\def\csname rev@rrank@dom@lgb@ixs@promospearman\endcsname{0.67}
\expandafter\def\csname rev@rrank@dom@lgb@ixs@spearman\endcsname{0.58}
\expandafter\def\csname rev@rrank@dom@lgb@ixs@topdecilehit\endcsname{0.56}
\expandafter\def\csname rev@rrank@dom@lgb@ixs@totalratio\endcsname{0.96}
\expandafter\def\csname rev@rrank@dom@tfmplan@catidxstoreid@mediannoderatio\endcsname{0.98}
\expandafter\def\csname rev@rrank@dom@tfmplan@catidxstoreid@spearman\endcsname{0.37}
\expandafter\def\csname rev@rrank@dom@tfmplan@catidxstoreid@topdecilehit\endcsname{0.29}
\expandafter\def\csname rev@rrank@dom@tfmplan@catidxstoreid@totalratio\endcsname{0.97}
\expandafter\def\csname rev@rrank@dom@tfmplan@ixs@mediannoderatio\endcsname{0.98}
\expandafter\def\csname rev@rrank@dom@tfmplan@ixs@promospearman\endcsname{0.55}
\expandafter\def\csname rev@rrank@dom@tfmplan@ixs@spearman\endcsname{0.52}
\expandafter\def\csname rev@rrank@dom@tfmplan@ixs@topdecilehit\endcsname{0.48}
\expandafter\def\csname rev@rrank@dom@tfmplan@ixs@totalratio\endcsname{0.97}
\expandafter\def\csname rev@rrank@dom@tsmean@catidxstoreid@mediannoderatio\endcsname{1.31}
\expandafter\def\csname rev@rrank@dom@tsmean@catidxstoreid@spearman\endcsname{0.28}
\expandafter\def\csname rev@rrank@dom@tsmean@catidxstoreid@topdecilehit\endcsname{0.26}
\expandafter\def\csname rev@rrank@dom@tsmean@catidxstoreid@totalratio\endcsname{1.36}
\expandafter\def\csname rev@rrank@dom@tsmean@ixs@mediannoderatio\endcsname{1.12}
\expandafter\def\csname rev@rrank@dom@tsmean@ixs@promospearman\endcsname{0.49}
\expandafter\def\csname rev@rrank@dom@tsmean@ixs@spearman\endcsname{0.37}
\expandafter\def\csname rev@rrank@dom@tsmean@ixs@topdecilehit\endcsname{0.42}
\expandafter\def\csname rev@rrank@dom@tsmean@ixs@totalratio\endcsname{1.36}
\expandafter\def\csname rev@rrank@dom@tsplan@catidxstoreid@mediannoderatio\endcsname{2.49}
\expandafter\def\csname rev@rrank@dom@tsplan@catidxstoreid@spearman\endcsname{0.13}
\expandafter\def\csname rev@rrank@dom@tsplan@catidxstoreid@topdecilehit\endcsname{0.22}
\expandafter\def\csname rev@rrank@dom@tsplan@catidxstoreid@totalratio\endcsname{3.00}
\expandafter\def\csname rev@rrank@dom@tsplan@ixs@mediannoderatio\endcsname{1.25}
\expandafter\def\csname rev@rrank@dom@tsplan@ixs@promospearman\endcsname{0.58}
\expandafter\def\csname rev@rrank@dom@tsplan@ixs@spearman\endcsname{0.52}
\expandafter\def\csname rev@rrank@dom@tsplan@ixs@topdecilehit\endcsname{0.48}
\expandafter\def\csname rev@rrank@dom@tsplan@ixs@totalratio\endcsname{3.00}
\expandafter\def\csname rev@rrank@dom@world@catidxstoreid@mediannoderatio\endcsname{1.01}
\expandafter\def\csname rev@rrank@dom@world@catidxstoreid@spearman\endcsname{0.32}
\expandafter\def\csname rev@rrank@dom@world@catidxstoreid@topdecilehit\endcsname{0.28}
\expandafter\def\csname rev@rrank@dom@world@catidxstoreid@totalratio\endcsname{1.01}
\expandafter\def\csname rev@rrank@dom@world@ixs@mediannoderatio\endcsname{1.02}
\expandafter\def\csname rev@rrank@dom@world@ixs@promospearman\endcsname{0.64}
\expandafter\def\csname rev@rrank@dom@world@ixs@spearman\endcsname{0.57}
\expandafter\def\csname rev@rrank@dom@world@ixs@topdecilehit\endcsname{0.53}
\expandafter\def\csname rev@rrank@dom@world@ixs@totalratio\endcsname{1.01}
\expandafter\def\csname rev@rrank@fav@ens@ixs@mediannoderatio\endcsname{0.99}
\expandafter\def\csname rev@rrank@fav@ens@ixs@promospearman\endcsname{0.58}
\expandafter\def\csname rev@rrank@fav@ens@ixs@spearman\endcsname{0.46}
\expandafter\def\csname rev@rrank@fav@ens@ixs@topdecilehit\endcsname{0.51}
\expandafter\def\csname rev@rrank@fav@ens@ixs@totalratio\endcsname{0.97}
\expandafter\def\csname rev@rrank@fav@ens@storeidxfamily@mediannoderatio\endcsname{0.97}
\expandafter\def\csname rev@rrank@fav@ens@storeidxfamily@spearman\endcsname{0.45}
\expandafter\def\csname rev@rrank@fav@ens@storeidxfamily@topdecilehit\endcsname{0.45}
\expandafter\def\csname rev@rrank@fav@ens@storeidxfamily@totalratio\endcsname{0.97}
\expandafter\def\csname rev@rrank@fav@ensfour@ixs@mediannoderatio\endcsname{1.00}
\expandafter\def\csname rev@rrank@fav@ensfour@ixs@promospearman\endcsname{0.59}
\expandafter\def\csname rev@rrank@fav@ensfour@ixs@spearman\endcsname{0.47}
\expandafter\def\csname rev@rrank@fav@ensfour@ixs@topdecilehit\endcsname{0.52}
\expandafter\def\csname rev@rrank@fav@ensfour@ixs@totalratio\endcsname{0.99}
\expandafter\def\csname rev@rrank@fav@ensfour@storeidxfamily@mediannoderatio\endcsname{0.99}
\expandafter\def\csname rev@rrank@fav@ensfour@storeidxfamily@spearman\endcsname{0.45}
\expandafter\def\csname rev@rrank@fav@ensfour@storeidxfamily@topdecilehit\endcsname{0.43}
\expandafter\def\csname rev@rrank@fav@ensfour@storeidxfamily@totalratio\endcsname{0.99}
\expandafter\def\csname rev@rrank@fav@enstimestral@ixs@mediannoderatio\endcsname{1.01}
\expandafter\def\csname rev@rrank@fav@enstimestral@ixs@promospearman\endcsname{0.58}
\expandafter\def\csname rev@rrank@fav@enstimestral@ixs@spearman\endcsname{0.46}
\expandafter\def\csname rev@rrank@fav@enstimestral@ixs@topdecilehit\endcsname{0.51}
\expandafter\def\csname rev@rrank@fav@enstimestral@ixs@totalratio\endcsname{1.00}
\expandafter\def\csname rev@rrank@fav@enstimestral@storeidxfamily@mediannoderatio\endcsname{1.00}
\expandafter\def\csname rev@rrank@fav@enstimestral@storeidxfamily@spearman\endcsname{0.44}
\expandafter\def\csname rev@rrank@fav@enstimestral@storeidxfamily@topdecilehit\endcsname{0.44}
\expandafter\def\csname rev@rrank@fav@enstimestral@storeidxfamily@totalratio\endcsname{1.00}
\expandafter\def\csname rev@rrank@fav@lgb@ixs@mediannoderatio\endcsname{0.98}
\expandafter\def\csname rev@rrank@fav@lgb@ixs@promospearman\endcsname{0.55}
\expandafter\def\csname rev@rrank@fav@lgb@ixs@spearman\endcsname{0.38}
\expandafter\def\csname rev@rrank@fav@lgb@ixs@topdecilehit\endcsname{0.46}
\expandafter\def\csname rev@rrank@fav@lgb@ixs@totalratio\endcsname{0.96}
\expandafter\def\csname rev@rrank@fav@lgb@storeidxfamily@mediannoderatio\endcsname{0.96}
\expandafter\def\csname rev@rrank@fav@lgb@storeidxfamily@spearman\endcsname{0.40}
\expandafter\def\csname rev@rrank@fav@lgb@storeidxfamily@topdecilehit\endcsname{0.41}
\expandafter\def\csname rev@rrank@fav@lgb@storeidxfamily@totalratio\endcsname{0.96}
\expandafter\def\csname rev@rrank@fav@tfmplan@ixs@mediannoderatio\endcsname{0.97}
\expandafter\def\csname rev@rrank@fav@tfmplan@ixs@promospearman\endcsname{0.55}
\expandafter\def\csname rev@rrank@fav@tfmplan@ixs@spearman\endcsname{0.44}
\expandafter\def\csname rev@rrank@fav@tfmplan@ixs@topdecilehit\endcsname{0.49}
\expandafter\def\csname rev@rrank@fav@tfmplan@ixs@totalratio\endcsname{0.96}
\expandafter\def\csname rev@rrank@fav@tfmplan@storeidxfamily@mediannoderatio\endcsname{0.96}
\expandafter\def\csname rev@rrank@fav@tfmplan@storeidxfamily@spearman\endcsname{0.35}
\expandafter\def\csname rev@rrank@fav@tfmplan@storeidxfamily@topdecilehit\endcsname{0.38}
\expandafter\def\csname rev@rrank@fav@tfmplan@storeidxfamily@totalratio\endcsname{0.96}
\expandafter\def\csname rev@rrank@fav@tsmean@ixs@mediannoderatio\endcsname{1.05}
\expandafter\def\csname rev@rrank@fav@tsmean@ixs@promospearman\endcsname{0.48}
\expandafter\def\csname rev@rrank@fav@tsmean@ixs@spearman\endcsname{0.35}
\expandafter\def\csname rev@rrank@fav@tsmean@ixs@topdecilehit\endcsname{0.43}
\expandafter\def\csname rev@rrank@fav@tsmean@ixs@totalratio\endcsname{1.04}
\expandafter\def\csname rev@rrank@fav@tsmean@storeidxfamily@mediannoderatio\endcsname{1.04}
\expandafter\def\csname rev@rrank@fav@tsmean@storeidxfamily@spearman\endcsname{0.36}
\expandafter\def\csname rev@rrank@fav@tsmean@storeidxfamily@topdecilehit\endcsname{0.40}
\expandafter\def\csname rev@rrank@fav@tsmean@storeidxfamily@totalratio\endcsname{1.04}
\expandafter\def\csname rev@rrank@fav@tsplan@ixs@mediannoderatio\endcsname{1.02}
\expandafter\def\csname rev@rrank@fav@tsplan@ixs@promospearman\endcsname{0.53}
\expandafter\def\csname rev@rrank@fav@tsplan@ixs@spearman\endcsname{0.44}
\expandafter\def\csname rev@rrank@fav@tsplan@ixs@topdecilehit\endcsname{0.50}
\expandafter\def\csname rev@rrank@fav@tsplan@ixs@totalratio\endcsname{1.03}
\expandafter\def\csname rev@rrank@fav@tsplan@storeidxfamily@mediannoderatio\endcsname{1.02}
\expandafter\def\csname rev@rrank@fav@tsplan@storeidxfamily@spearman\endcsname{0.40}
\expandafter\def\csname rev@rrank@fav@tsplan@storeidxfamily@topdecilehit\endcsname{0.38}
\expandafter\def\csname rev@rrank@fav@tsplan@storeidxfamily@totalratio\endcsname{1.03}
\expandafter\def\csname rev@rrank@fav@world@ixs@mediannoderatio\endcsname{1.02}
\expandafter\def\csname rev@rrank@fav@world@ixs@promospearman\endcsname{0.55}
\expandafter\def\csname rev@rrank@fav@world@ixs@spearman\endcsname{0.43}
\expandafter\def\csname rev@rrank@fav@world@ixs@topdecilehit\endcsname{0.49}
\expandafter\def\csname rev@rrank@fav@world@ixs@totalratio\endcsname{1.00}
\expandafter\def\csname rev@rrank@fav@world@storeidxfamily@mediannoderatio\endcsname{1.00}
\expandafter\def\csname rev@rrank@fav@world@storeidxfamily@spearman\endcsname{0.36}
\expandafter\def\csname rev@rrank@fav@world@storeidxfamily@topdecilehit\endcsname{0.40}
\expandafter\def\csname rev@rrank@fav@world@storeidxfamily@totalratio\endcsname{1.00}
\expandafter\def\csname rev@rrank@frat@ens@catidxstoreid@mediannoderatio\endcsname{0.99}
\expandafter\def\csname rev@rrank@frat@ens@catidxstoreid@spearman\endcsname{0.80}
\expandafter\def\csname rev@rrank@frat@ens@catidxstoreid@topdecilehit\endcsname{0.57}
\expandafter\def\csname rev@rrank@frat@ens@catidxstoreid@totalratio\endcsname{1.00}
\expandafter\def\csname rev@rrank@frat@ens@ixs@mediannoderatio\endcsname{1.01}
\expandafter\def\csname rev@rrank@frat@ens@ixs@promospearman\endcsname{0.74}
\expandafter\def\csname rev@rrank@frat@ens@ixs@spearman\endcsname{0.83}
\expandafter\def\csname rev@rrank@frat@ens@ixs@topdecilehit\endcsname{0.68}
\expandafter\def\csname rev@rrank@frat@ens@ixs@totalratio\endcsname{1.00}
\expandafter\def\csname rev@rrank@frat@ensfour@catidxstoreid@mediannoderatio\endcsname{1.03}
\expandafter\def\csname rev@rrank@frat@ensfour@catidxstoreid@spearman\endcsname{0.78}
\expandafter\def\csname rev@rrank@frat@ensfour@catidxstoreid@topdecilehit\endcsname{0.49}
\expandafter\def\csname rev@rrank@frat@ensfour@catidxstoreid@totalratio\endcsname{1.04}
\expandafter\def\csname rev@rrank@frat@ensfour@ixs@mediannoderatio\endcsname{1.03}
\expandafter\def\csname rev@rrank@frat@ensfour@ixs@promospearman\endcsname{0.73}
\expandafter\def\csname rev@rrank@frat@ensfour@ixs@spearman\endcsname{0.82}
\expandafter\def\csname rev@rrank@frat@ensfour@ixs@topdecilehit\endcsname{0.67}
\expandafter\def\csname rev@rrank@frat@ensfour@ixs@totalratio\endcsname{1.04}
\expandafter\def\csname rev@rrank@frat@enstimestral@catidxstoreid@mediannoderatio\endcsname{1.05}
\expandafter\def\csname rev@rrank@frat@enstimestral@catidxstoreid@spearman\endcsname{0.78}
\expandafter\def\csname rev@rrank@frat@enstimestral@catidxstoreid@topdecilehit\endcsname{0.46}
\expandafter\def\csname rev@rrank@frat@enstimestral@catidxstoreid@totalratio\endcsname{1.06}
\expandafter\def\csname rev@rrank@frat@enstimestral@ixs@mediannoderatio\endcsname{1.06}
\expandafter\def\csname rev@rrank@frat@enstimestral@ixs@promospearman\endcsname{0.73}
\expandafter\def\csname rev@rrank@frat@enstimestral@ixs@spearman\endcsname{0.82}
\expandafter\def\csname rev@rrank@frat@enstimestral@ixs@topdecilehit\endcsname{0.66}
\expandafter\def\csname rev@rrank@frat@enstimestral@ixs@totalratio\endcsname{1.06}
\expandafter\def\csname rev@rrank@frat@lgb@catidxstoreid@mediannoderatio\endcsname{1.01}
\expandafter\def\csname rev@rrank@frat@lgb@catidxstoreid@spearman\endcsname{0.78}
\expandafter\def\csname rev@rrank@frat@lgb@catidxstoreid@topdecilehit\endcsname{0.53}
\expandafter\def\csname rev@rrank@frat@lgb@catidxstoreid@totalratio\endcsname{1.00}
\expandafter\def\csname rev@rrank@frat@lgb@ixs@mediannoderatio\endcsname{1.04}
\expandafter\def\csname rev@rrank@frat@lgb@ixs@promospearman\endcsname{0.73}
\expandafter\def\csname rev@rrank@frat@lgb@ixs@spearman\endcsname{0.81}
\expandafter\def\csname rev@rrank@frat@lgb@ixs@topdecilehit\endcsname{0.66}
\expandafter\def\csname rev@rrank@frat@lgb@ixs@totalratio\endcsname{1.00}
\expandafter\def\csname rev@rrank@frat@tfmplan@catidxstoreid@mediannoderatio\endcsname{0.97}
\expandafter\def\csname rev@rrank@frat@tfmplan@catidxstoreid@spearman\endcsname{0.74}
\expandafter\def\csname rev@rrank@frat@tfmplan@catidxstoreid@topdecilehit\endcsname{0.62}
\expandafter\def\csname rev@rrank@frat@tfmplan@catidxstoreid@totalratio\endcsname{0.98}
\expandafter\def\csname rev@rrank@frat@tfmplan@ixs@mediannoderatio\endcsname{0.95}
\expandafter\def\csname rev@rrank@frat@tfmplan@ixs@promospearman\endcsname{0.69}
\expandafter\def\csname rev@rrank@frat@tfmplan@ixs@spearman\endcsname{0.77}
\expandafter\def\csname rev@rrank@frat@tfmplan@ixs@topdecilehit\endcsname{0.62}
\expandafter\def\csname rev@rrank@frat@tfmplan@ixs@totalratio\endcsname{0.98}
\expandafter\def\csname rev@rrank@frat@tsbig@catidxstoreid@mediannoderatio\endcsname{1.11}
\expandafter\def\csname rev@rrank@frat@tsbig@catidxstoreid@spearman\endcsname{0.66}
\expandafter\def\csname rev@rrank@frat@tsbig@catidxstoreid@topdecilehit\endcsname{0.40}
\expandafter\def\csname rev@rrank@frat@tsbig@catidxstoreid@totalratio\endcsname{1.23}
\expandafter\def\csname rev@rrank@frat@tsbig@ixs@mediannoderatio\endcsname{1.07}
\expandafter\def\csname rev@rrank@frat@tsbig@ixs@promospearman\endcsname{0.70}
\expandafter\def\csname rev@rrank@frat@tsbig@ixs@spearman\endcsname{0.75}
\expandafter\def\csname rev@rrank@frat@tsbig@ixs@topdecilehit\endcsname{0.59}
\expandafter\def\csname rev@rrank@frat@tsbig@ixs@totalratio\endcsname{1.23}
\expandafter\def\csname rev@rrank@frat@tsmean@catidxstoreid@mediannoderatio\endcsname{1.01}
\expandafter\def\csname rev@rrank@frat@tsmean@catidxstoreid@spearman\endcsname{0.43}
\expandafter\def\csname rev@rrank@frat@tsmean@catidxstoreid@topdecilehit\endcsname{0.29}
\expandafter\def\csname rev@rrank@frat@tsmean@catidxstoreid@totalratio\endcsname{1.02}
\expandafter\def\csname rev@rrank@frat@tsmean@ixs@mediannoderatio\endcsname{0.99}
\expandafter\def\csname rev@rrank@frat@tsmean@ixs@promospearman\endcsname{0.50}
\expandafter\def\csname rev@rrank@frat@tsmean@ixs@spearman\endcsname{0.59}
\expandafter\def\csname rev@rrank@frat@tsmean@ixs@topdecilehit\endcsname{0.48}
\expandafter\def\csname rev@rrank@frat@tsmean@ixs@totalratio\endcsname{1.02}
\expandafter\def\csname rev@rrank@frat@tsplan@catidxstoreid@mediannoderatio\endcsname{1.12}
\expandafter\def\csname rev@rrank@frat@tsplan@catidxstoreid@spearman\endcsname{0.67}
\expandafter\def\csname rev@rrank@frat@tsplan@catidxstoreid@topdecilehit\endcsname{0.43}
\expandafter\def\csname rev@rrank@frat@tsplan@catidxstoreid@totalratio\endcsname{1.17}
\expandafter\def\csname rev@rrank@frat@tsplan@ixs@mediannoderatio\endcsname{1.08}
\expandafter\def\csname rev@rrank@frat@tsplan@ixs@promospearman\endcsname{0.67}
\expandafter\def\csname rev@rrank@frat@tsplan@ixs@spearman\endcsname{0.75}
\expandafter\def\csname rev@rrank@frat@tsplan@ixs@topdecilehit\endcsname{0.59}
\expandafter\def\csname rev@rrank@frat@tsplan@ixs@totalratio\endcsname{1.17}
\expandafter\def\csname rev@rrank@frat@world@catidxstoreid@mediannoderatio\endcsname{1.01}
\expandafter\def\csname rev@rrank@frat@world@catidxstoreid@spearman\endcsname{0.75}
\expandafter\def\csname rev@rrank@frat@world@catidxstoreid@topdecilehit\endcsname{0.46}
\expandafter\def\csname rev@rrank@frat@world@catidxstoreid@totalratio\endcsname{1.01}
\expandafter\def\csname rev@rrank@frat@world@ixs@mediannoderatio\endcsname{1.02}
\expandafter\def\csname rev@rrank@frat@world@ixs@promospearman\endcsname{0.71}
\expandafter\def\csname rev@rrank@frat@world@ixs@spearman\endcsname{0.80}
\expandafter\def\csname rev@rrank@frat@world@ixs@topdecilehit\endcsname{0.65}
\expandafter\def\csname rev@rrank@frat@world@ixs@totalratio\endcsname{1.01}
\expandafter\def\csname rev@rrank@mfive@ens@ixs@mediannoderatio\endcsname{0.94}
\expandafter\def\csname rev@rrank@mfive@ens@ixs@spearman\endcsname{0.42}
\expandafter\def\csname rev@rrank@mfive@ens@ixs@topdecilehit\endcsname{0.53}
\expandafter\def\csname rev@rrank@mfive@ens@ixs@totalratio\endcsname{0.94}
\expandafter\def\csname rev@rrank@mfive@ens@storeidxcatid@mediannoderatio\endcsname{0.96}
\expandafter\def\csname rev@rrank@mfive@ens@storeidxcatid@spearman\endcsname{0.48}
\expandafter\def\csname rev@rrank@mfive@ens@storeidxcatid@topdecilehit\endcsname{0.42}
\expandafter\def\csname rev@rrank@mfive@ens@storeidxcatid@totalratio\endcsname{0.94}
\expandafter\def\csname rev@rrank@mfive@ensfour@ixs@mediannoderatio\endcsname{0.96}
\expandafter\def\csname rev@rrank@mfive@ensfour@ixs@spearman\endcsname{0.43}
\expandafter\def\csname rev@rrank@mfive@ensfour@ixs@topdecilehit\endcsname{0.53}
\expandafter\def\csname rev@rrank@mfive@ensfour@ixs@totalratio\endcsname{0.96}
\expandafter\def\csname rev@rrank@mfive@ensfour@storeidxcatid@mediannoderatio\endcsname{0.98}
\expandafter\def\csname rev@rrank@mfive@ensfour@storeidxcatid@spearman\endcsname{0.41}
\expandafter\def\csname rev@rrank@mfive@ensfour@storeidxcatid@topdecilehit\endcsname{0.50}
\expandafter\def\csname rev@rrank@mfive@ensfour@storeidxcatid@totalratio\endcsname{0.96}
\expandafter\def\csname rev@rrank@mfive@enstimestral@ixs@mediannoderatio\endcsname{0.98}
\expandafter\def\csname rev@rrank@mfive@enstimestral@ixs@spearman\endcsname{0.43}
\expandafter\def\csname rev@rrank@mfive@enstimestral@ixs@topdecilehit\endcsname{0.53}
\expandafter\def\csname rev@rrank@mfive@enstimestral@ixs@totalratio\endcsname{0.98}
\expandafter\def\csname rev@rrank@mfive@enstimestral@storeidxcatid@mediannoderatio\endcsname{1.00}
\expandafter\def\csname rev@rrank@mfive@enstimestral@storeidxcatid@spearman\endcsname{0.49}
\expandafter\def\csname rev@rrank@mfive@enstimestral@storeidxcatid@topdecilehit\endcsname{0.50}
\expandafter\def\csname rev@rrank@mfive@enstimestral@storeidxcatid@totalratio\endcsname{0.98}
\expandafter\def\csname rev@rrank@mfive@lgb@ixs@mediannoderatio\endcsname{0.94}
\expandafter\def\csname rev@rrank@mfive@lgb@ixs@spearman\endcsname{0.36}
\expandafter\def\csname rev@rrank@mfive@lgb@ixs@topdecilehit\endcsname{0.48}
\expandafter\def\csname rev@rrank@mfive@lgb@ixs@totalratio\endcsname{0.92}
\expandafter\def\csname rev@rrank@mfive@lgb@storeidxcatid@mediannoderatio\endcsname{0.95}
\expandafter\def\csname rev@rrank@mfive@lgb@storeidxcatid@spearman\endcsname{0.49}
\expandafter\def\csname rev@rrank@mfive@lgb@storeidxcatid@topdecilehit\endcsname{0.25}
\expandafter\def\csname rev@rrank@mfive@lgb@storeidxcatid@totalratio\endcsname{0.92}
\expandafter\def\csname rev@rrank@mfive@tfmplan@ixs@mediannoderatio\endcsname{0.90}
\expandafter\def\csname rev@rrank@mfive@tfmplan@ixs@spearman\endcsname{0.36}
\expandafter\def\csname rev@rrank@mfive@tfmplan@ixs@topdecilehit\endcsname{0.47}
\expandafter\def\csname rev@rrank@mfive@tfmplan@ixs@totalratio\endcsname{0.92}
\expandafter\def\csname rev@rrank@mfive@tfmplan@storeidxcatid@mediannoderatio\endcsname{0.93}
\expandafter\def\csname rev@rrank@mfive@tfmplan@storeidxcatid@spearman\endcsname{0.28}
\expandafter\def\csname rev@rrank@mfive@tfmplan@storeidxcatid@topdecilehit\endcsname{0.25}
\expandafter\def\csname rev@rrank@mfive@tfmplan@storeidxcatid@totalratio\endcsname{0.92}
\expandafter\def\csname rev@rrank@mfive@tsmean@ixs@mediannoderatio\endcsname{1.03}
\expandafter\def\csname rev@rrank@mfive@tsmean@ixs@spearman\endcsname{0.40}
\expandafter\def\csname rev@rrank@mfive@tsmean@ixs@topdecilehit\endcsname{0.51}
\expandafter\def\csname rev@rrank@mfive@tsmean@ixs@totalratio\endcsname{1.03}
\expandafter\def\csname rev@rrank@mfive@tsmean@storeidxcatid@mediannoderatio\endcsname{1.04}
\expandafter\def\csname rev@rrank@mfive@tsmean@storeidxcatid@spearman\endcsname{0.36}
\expandafter\def\csname rev@rrank@mfive@tsmean@storeidxcatid@topdecilehit\endcsname{0.33}
\expandafter\def\csname rev@rrank@mfive@tsmean@storeidxcatid@totalratio\endcsname{1.03}
\expandafter\def\csname rev@rrank@mfive@tsplan@ixs@mediannoderatio\endcsname{1.01}
\expandafter\def\csname rev@rrank@mfive@tsplan@ixs@spearman\endcsname{0.40}
\expandafter\def\csname rev@rrank@mfive@tsplan@ixs@topdecilehit\endcsname{0.51}
\expandafter\def\csname rev@rrank@mfive@tsplan@ixs@totalratio\endcsname{1.03}
\expandafter\def\csname rev@rrank@mfive@tsplan@storeidxcatid@mediannoderatio\endcsname{1.03}
\expandafter\def\csname rev@rrank@mfive@tsplan@storeidxcatid@spearman\endcsname{0.32}
\expandafter\def\csname rev@rrank@mfive@tsplan@storeidxcatid@topdecilehit\endcsname{0.25}
\expandafter\def\csname rev@rrank@mfive@tsplan@storeidxcatid@totalratio\endcsname{1.03}
\expandafter\def\csname rev@rrank@mfive@world@ixs@mediannoderatio\endcsname{0.98}
\expandafter\def\csname rev@rrank@mfive@world@ixs@spearman\endcsname{0.41}
\expandafter\def\csname rev@rrank@mfive@world@ixs@topdecilehit\endcsname{0.52}
\expandafter\def\csname rev@rrank@mfive@world@ixs@totalratio\endcsname{0.98}
\expandafter\def\csname rev@rrank@mfive@world@storeidxcatid@mediannoderatio\endcsname{1.00}
\expandafter\def\csname rev@rrank@mfive@world@storeidxcatid@spearman\endcsname{0.50}
\expandafter\def\csname rev@rrank@mfive@world@storeidxcatid@topdecilehit\endcsname{0.25}
\expandafter\def\csname rev@rrank@mfive@world@storeidxcatid@totalratio\endcsname{0.98}
\expandafter\def\csname rev@rrec@ana@etsbottomup@ixs\endcsname{0.766}
\expandafter\def\csname rev@rrec@ana@etsbottomup@total\endcsname{1.037}
\expandafter\def\csname rev@rrec@ana@etsols@ixs\endcsname{0.792}
\expandafter\def\csname rev@rrec@ana@etsols@total\endcsname{1.082}
\expandafter\def\csname rev@rrec@ana@etstopdown@ixs\endcsname{0.747}
\expandafter\def\csname rev@rrec@ana@etstopdown@total\endcsname{0.889}
\expandafter\def\csname rev@rrec@ana@etswlsstruct@ixs\endcsname{0.772}
\expandafter\def\csname rev@rrec@ana@etswlsstruct@total\endcsname{1.001}
\expandafter\def\csname rev@rrec@ana@etswlsvar@ixs\endcsname{0.806}
\expandafter\def\csname rev@rrec@ana@etswlsvar@total\endcsname{1.536}
\expandafter\def\csname rev@rrec@ana@lightgbmwithetswlsvar@ixs\endcsname{0.678}
\expandafter\def\csname rev@rrec@ana@lightgbmwithetswlsvar@total\endcsname{1.201}
\expandafter\def\csname rev@rrec@ana@worldmodelwithetswlsvar@ixs\endcsname{0.725}
\expandafter\def\csname rev@rrec@ana@worldmodelwithetswlsvar@total\endcsname{1.887}
\expandafter\def\csname rev@rrec@bjc@etsbottomup@ixs\endcsname{0.786}
\expandafter\def\csname rev@rrec@bjc@etsbottomup@total\endcsname{1.021}
\expandafter\def\csname rev@rrec@bjc@etsols@ixs\endcsname{0.820}
\expandafter\def\csname rev@rrec@bjc@etsols@total\endcsname{1.057}
\expandafter\def\csname rev@rrec@bjc@etstopdown@ixs\endcsname{0.798}
\expandafter\def\csname rev@rrec@bjc@etstopdown@total\endcsname{0.936}
\expandafter\def\csname rev@rrec@bjc@etswlsstruct@ixs\endcsname{0.793}
\expandafter\def\csname rev@rrec@bjc@etswlsstruct@total\endcsname{1.034}
\expandafter\def\csname rev@rrec@bjc@etswlsvar@ixs\endcsname{0.793}
\expandafter\def\csname rev@rrec@bjc@etswlsvar@total\endcsname{1.035}
\expandafter\def\csname rev@rrec@bjc@lightgbmwithetswlsvar@ixs\endcsname{0.691}
\expandafter\def\csname rev@rrec@bjc@lightgbmwithetswlsvar@total\endcsname{1.015}
\expandafter\def\csname rev@rrec@bjc@worldmodelwithetswlsvar@ixs\endcsname{0.738}
\expandafter\def\csname rev@rrec@bjc@worldmodelwithetswlsvar@total\endcsname{1.047}
\expandafter\def\csname rev@rrec@che@etsbottomup@ixs\endcsname{0.791}
\expandafter\def\csname rev@rrec@che@etsbottomup@total\endcsname{0.718}
\expandafter\def\csname rev@rrec@che@etsols@ixs\endcsname{0.830}
\expandafter\def\csname rev@rrec@che@etsols@total\endcsname{0.752}
\expandafter\def\csname rev@rrec@che@etstopdown@ixs\endcsname{0.836}
\expandafter\def\csname rev@rrec@che@etstopdown@total\endcsname{0.776}
\expandafter\def\csname rev@rrec@che@etswlsstruct@ixs\endcsname{0.801}
\expandafter\def\csname rev@rrec@che@etswlsstruct@total\endcsname{0.702}
\expandafter\def\csname rev@rrec@che@etswlsvar@ixs\endcsname{1.066}
\expandafter\def\csname rev@rrec@che@etswlsvar@total\endcsname{1.884}
\expandafter\def\csname rev@rrec@che@lightgbmwithetswlsvar@ixs\endcsname{0.900}
\expandafter\def\csname rev@rrec@che@lightgbmwithetswlsvar@total\endcsname{1.526}
\expandafter\def\csname rev@rrec@che@worldmodelwithetswlsvar@ixs\endcsname{1.112}
\expandafter\def\csname rev@rrec@che@worldmodelwithetswlsvar@total\endcsname{1.714}
\expandafter\def\csname rev@rrec@frat@etsbottomup@ixs\endcsname{0.909}
\expandafter\def\csname rev@rrec@frat@etsbottomup@total\endcsname{0.566}
\expandafter\def\csname rev@rrec@frat@etsmintshrink@ixs\endcsname{0.926}
\expandafter\def\csname rev@rrec@frat@etsmintshrink@total\endcsname{0.610}
\expandafter\def\csname rev@rrec@frat@etsmintshrinkbeforefix@ixs\endcsname{0.926}
\expandafter\def\csname rev@rrec@frat@etsmintshrinkbeforefix@total\endcsname{247.170}
\expandafter\def\csname rev@rrec@frat@etsols@ixs\endcsname{0.953}
\expandafter\def\csname rev@rrec@frat@etsols@total\endcsname{0.520}
\expandafter\def\csname rev@rrec@frat@etstopdown@ixs\endcsname{0.806}
\expandafter\def\csname rev@rrec@frat@etstopdown@total\endcsname{0.487}
\expandafter\def\csname rev@rrec@frat@etswlsstruct@ixs\endcsname{0.912}
\expandafter\def\csname rev@rrec@frat@etswlsstruct@total\endcsname{0.538}
\expandafter\def\csname rev@rrec@frat@etswlsvar@ixs\endcsname{0.903}
\expandafter\def\csname rev@rrec@frat@etswlsvar@total\endcsname{0.511}
\expandafter\def\csname rev@rrec@frat@lightgbmwithetswlsvar@ixs\endcsname{0.581}
\expandafter\def\csname rev@rrec@frat@lightgbmwithetswlsvar@total\endcsname{0.304}
\expandafter\def\csname rev@rrec@frat@worldmodelwithetswlsvar@ixs\endcsname{0.602}
\expandafter\def\csname rev@rrec@frat@worldmodelwithetswlsvar@total\endcsname{0.343}
\expandafter\def\csname rev@rrec@fre@etsbottomup@ixs\endcsname{0.598}
\expandafter\def\csname rev@rrec@fre@etsbottomup@total\endcsname{0.495}
\expandafter\def\csname rev@rrec@fre@etsols@ixs\endcsname{0.645}
\expandafter\def\csname rev@rrec@fre@etsols@total\endcsname{0.549}
\expandafter\def\csname rev@rrec@fre@etstopdown@ixs\endcsname{0.612}
\expandafter\def\csname rev@rrec@fre@etstopdown@total\endcsname{0.543}
\expandafter\def\csname rev@rrec@fre@etswlsstruct@ixs\endcsname{0.603}
\expandafter\def\csname rev@rrec@fre@etswlsstruct@total\endcsname{0.482}
\expandafter\def\csname rev@rrec@fre@etswlsvar@ixs\endcsname{0.618}
\expandafter\def\csname rev@rrec@fre@etswlsvar@total\endcsname{0.725}
\expandafter\def\csname rev@rrec@fre@lightgbmwithetswlsvar@ixs\endcsname{0.464}
\expandafter\def\csname rev@rrec@fre@lightgbmwithetswlsvar@total\endcsname{0.519}
\expandafter\def\csname rev@rrec@fre@worldmodelwithetswlsvar@ixs\endcsname{0.489}
\expandafter\def\csname rev@rrec@fre@worldmodelwithetswlsvar@total\endcsname{0.544}
\expandafter\def\csname rev@rrec@mfive@etsbottomup@ixs\endcsname{0.898}
\expandafter\def\csname rev@rrec@mfive@etsbottomup@total\endcsname{1.271}
\expandafter\def\csname rev@rrec@mfive@etsols@ixs\endcsname{0.888}
\expandafter\def\csname rev@rrec@mfive@etsols@total\endcsname{0.902}
\expandafter\def\csname rev@rrec@mfive@etstopdown@ixs\endcsname{0.917}
\expandafter\def\csname rev@rrec@mfive@etstopdown@total\endcsname{0.902}
\expandafter\def\csname rev@rrec@mfive@etswlsstruct@ixs\endcsname{0.885}
\expandafter\def\csname rev@rrec@mfive@etswlsstruct@total\endcsname{0.908}
\expandafter\def\csname rev@rrec@mfive@etswlsvar@ixs\endcsname{0.884}
\expandafter\def\csname rev@rrec@mfive@etswlsvar@total\endcsname{0.946}
\expandafter\def\csname rev@rrec@mfive@lightgbmwithetswlsvar@ixs\endcsname{0.855}
\expandafter\def\csname rev@rrec@mfive@lightgbmwithetswlsvar@total\endcsname{0.763}
\expandafter\def\csname rev@rrec@mfive@worldmodelwithetswlsvar@ixs\endcsname{0.849}
\expandafter\def\csname rev@rrec@mfive@worldmodelwithetswlsvar@total\endcsname{0.754}
\expandafter\def\csname rev@rrec@sdr@etsbottomup@ixs\endcsname{0.736}
\expandafter\def\csname rev@rrec@sdr@etsbottomup@total\endcsname{0.907}
\expandafter\def\csname rev@rrec@sdr@etsols@ixs\endcsname{0.770}
\expandafter\def\csname rev@rrec@sdr@etsols@total\endcsname{0.876}
\expandafter\def\csname rev@rrec@sdr@etstopdown@ixs\endcsname{0.730}
\expandafter\def\csname rev@rrec@sdr@etstopdown@total\endcsname{0.884}
\expandafter\def\csname rev@rrec@sdr@etswlsstruct@ixs\endcsname{0.745}
\expandafter\def\csname rev@rrec@sdr@etswlsstruct@total\endcsname{0.880}
\expandafter\def\csname rev@rrec@sdr@etswlsvar@ixs\endcsname{0.846}
\expandafter\def\csname rev@rrec@sdr@etswlsvar@total\endcsname{2.719}
\expandafter\def\csname rev@rrec@sdr@lightgbmwithetswlsvar@ixs\endcsname{0.796}
\expandafter\def\csname rev@rrec@sdr@lightgbmwithetswlsvar@total\endcsname{2.493}
\expandafter\def\csname rev@rrec@sdr@worldmodelwithetswlsvar@ixs\endcsname{0.801}
\expandafter\def\csname rev@rrec@sdr@worldmodelwithetswlsvar@total\endcsname{2.474}
\expandafter\def\csname rev@rrec@sna@etsbottomup@ixs\endcsname{0.739}
\expandafter\def\csname rev@rrec@sna@etsbottomup@total\endcsname{2.810}
\expandafter\def\csname rev@rrec@sna@etsols@ixs\endcsname{0.812}
\expandafter\def\csname rev@rrec@sna@etsols@total\endcsname{2.747}
\expandafter\def\csname rev@rrec@sna@etstopdown@ixs\endcsname{0.794}
\expandafter\def\csname rev@rrec@sna@etstopdown@total\endcsname{1.517}
\expandafter\def\csname rev@rrec@sna@etswlsstruct@ixs\endcsname{0.773}
\expandafter\def\csname rev@rrec@sna@etswlsstruct@total\endcsname{2.652}
\expandafter\def\csname rev@rrec@sna@etswlsvar@ixs\endcsname{0.988}
\expandafter\def\csname rev@rrec@sna@etswlsvar@total\endcsname{2.604}
\expandafter\def\csname rev@rrec@sna@lightgbmwithetswlsvar@ixs\endcsname{0.791}
\expandafter\def\csname rev@rrec@sna@lightgbmwithetswlsvar@total\endcsname{2.143}
\expandafter\def\csname rev@rrec@sna@worldmodelwithetswlsvar@ixs\endcsname{0.854}
\expandafter\def\csname rev@rrec@sna@worldmodelwithetswlsvar@total\endcsname{2.331}
\expandafter\def\csname rev@rreg@clean@lightgbm@v\endcsname{1.8}
\expandafter\def\csname rev@rreg@clean@lightgbmpriceblind@v\endcsname{7.6}
\expandafter\def\csname rev@rreg@clean@n@v\endcsname{304}
\expandafter\def\csname rev@rreg@clean@world@hi\endcsname{2.1}
\expandafter\def\csname rev@rreg@clean@world@lo\endcsname{1.7}
\expandafter\def\csname rev@rreg@clean@worldleverblind@v\endcsname{77}
\expandafter\def\csname rev@rreg@clean@worldpriceblind@v\endcsname{9.5}
\expandafter\def\csname rev@rreg@confounded@lightgbm@v\endcsname{1.6}
\expandafter\def\csname rev@rreg@confounded@lightgbmpriceblind@v\endcsname{10.2}
\expandafter\def\csname rev@rreg@confounded@n@v\endcsname{424}
\expandafter\def\csname rev@rreg@confounded@world@hi\endcsname{2.5}
\expandafter\def\csname rev@rreg@confounded@world@lo\endcsname{2.0}
\expandafter\def\csname rev@rreg@confounded@worldleverblind@v\endcsname{98}
\expandafter\def\csname rev@rreg@confounded@worldpriceblind@v\endcsname{10.1}
\expandafter\def\csname rev@rsf@dom@ens@ixs\endcsname{0.612}
\expandafter\def\csname rev@rsf@dom@ens@total\endcsname{0.672}
\expandafter\def\csname rev@rsf@dom@ensfour@ixs\endcsname{0.821}
\expandafter\def\csname rev@rsf@dom@ensfour@total\endcsname{2.858}
\expandafter\def\csname rev@rsf@dom@enstimestral@ixs\endcsname{0.916}
\expandafter\def\csname rev@rsf@dom@enstimestral@total\endcsname{3.729}
\expandafter\def\csname rev@rsf@dom@lgb@ixs\endcsname{0.568}
\expandafter\def\csname rev@rsf@dom@lgb@total\endcsname{0.684}
\expandafter\def\csname rev@rsf@dom@tfmplan@ixs\endcsname{0.613}
\expandafter\def\csname rev@rsf@dom@tfmplan@total\endcsname{0.807}
\expandafter\def\csname rev@rsf@dom@tsmean@ixs\endcsname{0.728}
\expandafter\def\csname rev@rsf@dom@tsmean@total\endcsname{2.121}
\expandafter\def\csname rev@rsf@dom@tsplan@ixs\endcsname{1.565}
\expandafter\def\csname rev@rsf@dom@tsplan@total\endcsname{10.788}
\expandafter\def\csname rev@rsf@dom@world@ixs\endcsname{0.778}
\expandafter\def\csname rev@rsf@dom@world@total\endcsname{0.782}
\expandafter\def\csname rev@rsf@fav@ens@ixs\endcsname{0.694}
\expandafter\def\csname rev@rsf@fav@ens@total\endcsname{0.303}
\expandafter\def\csname rev@rsf@fav@ensfour@ixs\endcsname{0.694}
\expandafter\def\csname rev@rsf@fav@ensfour@total\endcsname{0.313}
\expandafter\def\csname rev@rsf@fav@enstimestral@ixs\endcsname{0.697}
\expandafter\def\csname rev@rsf@fav@enstimestral@total\endcsname{0.298}
\expandafter\def\csname rev@rsf@fav@lgb@ixs\endcsname{0.719}
\expandafter\def\csname rev@rsf@fav@lgb@total\endcsname{0.309}
\expandafter\def\csname rev@rsf@fav@tfmplan@ixs\endcsname{0.712}
\expandafter\def\csname rev@rsf@fav@tfmplan@total\endcsname{0.397}
\expandafter\def\csname rev@rsf@fav@tsmean@ixs\endcsname{0.771}
\expandafter\def\csname rev@rsf@fav@tsmean@total\endcsname{0.430}
\expandafter\def\csname rev@rsf@fav@tsplan@ixs\endcsname{0.731}
\expandafter\def\csname rev@rsf@fav@tsplan@total\endcsname{0.403}
\expandafter\def\csname rev@rsf@fav@world@ixs\endcsname{0.726}
\expandafter\def\csname rev@rsf@fav@world@total\endcsname{0.341}
\expandafter\def\csname rev@rsf@frat@ens@ixs\endcsname{0.549}
\expandafter\def\csname rev@rsf@frat@ens@total\endcsname{0.337}
\expandafter\def\csname rev@rsf@frat@ensfour@ixs\endcsname{0.595}
\expandafter\def\csname rev@rsf@frat@ensfour@total\endcsname{0.407}
\expandafter\def\csname rev@rsf@frat@enstimestral@ixs\endcsname{0.623}
\expandafter\def\csname rev@rsf@frat@enstimestral@total\endcsname{0.501}
\expandafter\def\csname rev@rsf@frat@lgb@ixs\endcsname{0.570}
\expandafter\def\csname rev@rsf@frat@lgb@total\endcsname{0.360}
\expandafter\def\csname rev@rsf@frat@tfmplan@ixs\endcsname{0.578}
\expandafter\def\csname rev@rsf@frat@tfmplan@total\endcsname{0.327}
\expandafter\def\csname rev@rsf@frat@tsbig@ixs\endcsname{1.036}
\expandafter\def\csname rev@rsf@frat@tsbig@total\endcsname{1.392}
\expandafter\def\csname rev@rsf@frat@tsmean@ixs\endcsname{0.792}
\expandafter\def\csname rev@rsf@frat@tsmean@total\endcsname{0.484}
\expandafter\def\csname rev@rsf@frat@tsplan@ixs\endcsname{0.864}
\expandafter\def\csname rev@rsf@frat@tsplan@total\endcsname{1.048}
\expandafter\def\csname rev@rsf@frat@world@ixs\endcsname{0.595}
\expandafter\def\csname rev@rsf@frat@world@total\endcsname{0.457}
\expandafter\def\csname rev@rsf@mfive@ens@ixs\endcsname{0.834}
\expandafter\def\csname rev@rsf@mfive@ens@total\endcsname{0.706}
\expandafter\def\csname rev@rsf@mfive@ensfour@ixs\endcsname{0.842}
\expandafter\def\csname rev@rsf@mfive@ensfour@total\endcsname{0.699}
\expandafter\def\csname rev@rsf@mfive@enstimestral@ixs\endcsname{0.846}
\expandafter\def\csname rev@rsf@mfive@enstimestral@total\endcsname{0.609}
\expandafter\def\csname rev@rsf@mfive@lgb@ixs\endcsname{0.861}
\expandafter\def\csname rev@rsf@mfive@lgb@total\endcsname{0.693}
\expandafter\def\csname rev@rsf@mfive@tfmplan@ixs\endcsname{0.842}
\expandafter\def\csname rev@rsf@mfive@tfmplan@total\endcsname{1.035}
\expandafter\def\csname rev@rsf@mfive@tsmean@ixs\endcsname{0.861}
\expandafter\def\csname rev@rsf@mfive@tsmean@total\endcsname{1.014}
\expandafter\def\csname rev@rsf@mfive@tsplan@ixs\endcsname{0.894}
\expandafter\def\csname rev@rsf@mfive@tsplan@total\endcsname{1.025}
\expandafter\def\csname rev@rsf@mfive@world@ixs\endcsname{0.851}
\expandafter\def\csname rev@rsf@mfive@world@total\endcsname{0.609}
\expandafter\def\csname rev@rsg@liftmatched@ixs\endcsname{0.602}
\expandafter\def\csname rev@rsg@liftmatched@overall\endcsname{0.560}
\expandafter\def\csname rev@rsg@liftmatched@total\endcsname{0.473}
\expandafter\def\csname rev@rtail@ana@tsmean@forecast@hi\endcsname{1.31}
\expandafter\def\csname rev@rtail@ana@tsmean@forecast@lo\endcsname{1.12}
\expandafter\def\csname rev@rtail@ana@tsmean@median@hi\endcsname{0.76}
\expandafter\def\csname rev@rtail@ana@tsmean@median@lo\endcsname{0.70}
\expandafter\def\csname rev@rtail@ana@tsmean@q99@hi\endcsname{11}
\expandafter\def\csname rev@rtail@ana@tsmean@q99@lo\endcsname{8.0}
\expandafter\def\csname rev@rtail@ana@tsplan@forecast@hi\endcsname{5.84}
\expandafter\def\csname rev@rtail@ana@tsplan@forecast@lo\endcsname{3.15}
\expandafter\def\csname rev@rtail@ana@tsplan@median@hi\endcsname{0.91}
\expandafter\def\csname rev@rtail@ana@tsplan@median@lo\endcsname{0.80}
\expandafter\def\csname rev@rtail@ana@tsplan@q99@hi\endcsname{107}
\expandafter\def\csname rev@rtail@ana@tsplan@q99@lo\endcsname{57}
\expandafter\def\csname rev@rtail@ana@tsplan@share@hi\endcsname{88}
\expandafter\def\csname rev@rtail@ana@tsplan@share@lo\endcsname{75}
\expandafter\def\csname rev@rtail@frat@tsmean@forecast@hi\endcsname{1.09}
\expandafter\def\csname rev@rtail@frat@tsmean@forecast@lo\endcsname{0.98}
\expandafter\def\csname rev@rtail@frat@tsmean@median@hi\endcsname{0.86}
\expandafter\def\csname rev@rtail@frat@tsmean@median@lo\endcsname{0.81}
\expandafter\def\csname rev@rtail@frat@tsmean@q99@hi\endcsname{4.6}
\expandafter\def\csname rev@rtail@frat@tsmean@q99@lo\endcsname{3.7}
\expandafter\def\csname rev@rtail@frat@tsplan@forecast@hi\endcsname{1.20}
\expandafter\def\csname rev@rtail@frat@tsplan@forecast@lo\endcsname{1.15}
\expandafter\def\csname rev@rtail@frat@tsplan@median@hi\endcsname{1.07}
\expandafter\def\csname rev@rtail@frat@tsplan@median@lo\endcsname{1.01}
\expandafter\def\csname rev@rtail@frat@tsplan@q99@hi\endcsname{6.9}
\expandafter\def\csname rev@rtail@frat@tsplan@q99@lo\endcsname{3.4}
\expandafter\def\csname rev@rtail@sdr@tsmean@forecast@hi\endcsname{1.39}
\expandafter\def\csname rev@rtail@sdr@tsmean@forecast@lo\endcsname{0.91}
\expandafter\def\csname rev@rtail@sdr@tsmean@median@hi\endcsname{0.64}
\expandafter\def\csname rev@rtail@sdr@tsmean@median@lo\endcsname{0.48}
\expandafter\def\csname rev@rtail@sdr@tsmean@q99@hi\endcsname{14}
\expandafter\def\csname rev@rtail@sdr@tsmean@q99@lo\endcsname{7.1}
\expandafter\def\csname rev@rtail@sdr@tsplan@forecast@hi\endcsname{3.36}
\expandafter\def\csname rev@rtail@sdr@tsplan@forecast@lo\endcsname{1.61}
\expandafter\def\csname rev@rtail@sdr@tsplan@median@hi\endcsname{1.27}
\expandafter\def\csname rev@rtail@sdr@tsplan@median@lo\endcsname{0.84}
\expandafter\def\csname rev@rtail@sdr@tsplan@q99@hi\endcsname{53}
\expandafter\def\csname rev@rtail@sdr@tsplan@q99@lo\endcsname{14}
\expandafter\def\csname rev@rtail@sdr@tsplan@share@hi\endcsname{86}
\expandafter\def\csname rev@rtail@sdr@tsplan@share@lo\endcsname{49}
\expandafter\def\csname rev@rv@ana@chronos@all\endcsname{0.837}
\expandafter\def\csname rev@rv@ana@chronos@ixs\endcsname{0.745}
\expandafter\def\csname rev@rv@ana@chronos@total\endcsname{0.979}
\expandafter\def\csname rev@rv@ana@ens@all\endcsname{0.670}
\expandafter\def\csname rev@rv@ana@ens@ixs\endcsname{0.650}
\expandafter\def\csname rev@rv@ana@ens@total\endcsname{0.782}
\expandafter\def\csname rev@rv@ana@ensfour@ixs\endcsname{0.993}
\expandafter\def\csname rev@rv@ana@ensfour@total\endcsname{7.795}
\expandafter\def\csname rev@rv@ana@enstimestral@ixs\endcsname{1.110}
\expandafter\def\csname rev@rv@ana@enstimestral@total\endcsname{10.386}
\expandafter\def\csname rev@rv@ana@lgb@all\endcsname{0.704}
\expandafter\def\csname rev@rv@ana@lgb@ixs\endcsname{0.647}
\expandafter\def\csname rev@rv@ana@lgb@total\endcsname{0.869}
\expandafter\def\csname rev@rv@ana@lift@all\endcsname{0.733}
\expandafter\def\csname rev@rv@ana@lift@ixs\endcsname{0.677}
\expandafter\def\csname rev@rv@ana@lift@total\endcsname{0.868}
\expandafter\def\csname rev@rv@ana@naive@all\endcsname{1.419}
\expandafter\def\csname rev@rv@ana@naive@ixs\endcsname{0.997}
\expandafter\def\csname rev@rv@ana@naive@total\endcsname{1.796}
\expandafter\def\csname rev@rv@ana@tfm@all\endcsname{0.789}
\expandafter\def\csname rev@rv@ana@tfm@ixs\endcsname{0.734}
\expandafter\def\csname rev@rv@ana@tfm@total\endcsname{0.900}
\expandafter\def\csname rev@rv@ana@tfmplan@all\endcsname{0.724}
\expandafter\def\csname rev@rv@ana@tfmplan@ixs\endcsname{0.679}
\expandafter\def\csname rev@rv@ana@tfmplan@total\endcsname{0.848}
\expandafter\def\csname rev@rv@ana@tft@all\endcsname{0.820}
\expandafter\def\csname rev@rv@ana@tft@ixs\endcsname{0.693}
\expandafter\def\csname rev@rv@ana@tft@total\endcsname{1.057}
\expandafter\def\csname rev@rv@ana@tsmean@ixs\endcsname{0.770}
\expandafter\def\csname rev@rv@ana@tsmean@total\endcsname{2.421}
\expandafter\def\csname rev@rv@ana@tsplan@ixs\endcsname{2.111}
\expandafter\def\csname rev@rv@ana@tsplan@total\endcsname{31.256}
\expandafter\def\csname rev@rv@ana@world@all\endcsname{0.706}
\expandafter\def\csname rev@rv@ana@world@ixs\endcsname{0.672}
\expandafter\def\csname rev@rv@ana@world@total\endcsname{0.826}
\expandafter\def\csname rev@rv@bjc@chronos@all\endcsname{0.815}
\expandafter\def\csname rev@rv@bjc@chronos@ixs\endcsname{0.728}
\expandafter\def\csname rev@rv@bjc@chronos@total\endcsname{0.897}
\expandafter\def\csname rev@rv@bjc@ens@all\endcsname{0.534}
\expandafter\def\csname rev@rv@bjc@ens@ixs\endcsname{0.585}
\expandafter\def\csname rev@rv@bjc@ens@total\endcsname{0.525}
\expandafter\def\csname rev@rv@bjc@ensfour@ixs\endcsname{0.776}
\expandafter\def\csname rev@rv@bjc@ensfour@total\endcsname{1.611}
\expandafter\def\csname rev@rv@bjc@enstimestral@ixs\endcsname{0.851}
\expandafter\def\csname rev@rv@bjc@enstimestral@total\endcsname{2.141}
\expandafter\def\csname rev@rv@bjc@lgb@all\endcsname{0.544}
\expandafter\def\csname rev@rv@bjc@lgb@ixs\endcsname{0.605}
\expandafter\def\csname rev@rv@bjc@lgb@total\endcsname{0.530}
\expandafter\def\csname rev@rv@bjc@lift@all\endcsname{0.603}
\expandafter\def\csname rev@rv@bjc@lift@ixs\endcsname{0.616}
\expandafter\def\csname rev@rv@bjc@lift@total\endcsname{0.585}
\expandafter\def\csname rev@rv@bjc@naive@all\endcsname{1.296}
\expandafter\def\csname rev@rv@bjc@naive@ixs\endcsname{1.079}
\expandafter\def\csname rev@rv@bjc@naive@total\endcsname{1.390}
\expandafter\def\csname rev@rv@bjc@tfm@all\endcsname{0.807}
\expandafter\def\csname rev@rv@bjc@tfm@ixs\endcsname{0.712}
\expandafter\def\csname rev@rv@bjc@tfm@total\endcsname{0.898}
\expandafter\def\csname rev@rv@bjc@tfmplan@all\endcsname{0.691}
\expandafter\def\csname rev@rv@bjc@tfmplan@ixs\endcsname{0.636}
\expandafter\def\csname rev@rv@bjc@tfmplan@total\endcsname{0.766}
\expandafter\def\csname rev@rv@bjc@tft@all\endcsname{0.727}
\expandafter\def\csname rev@rv@bjc@tft@ixs\endcsname{0.676}
\expandafter\def\csname rev@rv@bjc@tft@total\endcsname{0.793}
\expandafter\def\csname rev@rv@bjc@tsmean@ixs\endcsname{0.765}
\expandafter\def\csname rev@rv@bjc@tsmean@total\endcsname{1.357}
\expandafter\def\csname rev@rv@bjc@tsplan@ixs\endcsname{1.459}
\expandafter\def\csname rev@rv@bjc@tsplan@total\endcsname{6.257}
\expandafter\def\csname rev@rv@bjc@world@all\endcsname{0.637}
\expandafter\def\csname rev@rv@bjc@world@ixs\endcsname{0.656}
\expandafter\def\csname rev@rv@bjc@world@total\endcsname{0.613}
\expandafter\def\csname rev@rv@che@chronos@all\endcsname{0.754}
\expandafter\def\csname rev@rv@che@chronos@ixs\endcsname{0.762}
\expandafter\def\csname rev@rv@che@chronos@total\endcsname{0.790}
\expandafter\def\csname rev@rv@che@ens@all\endcsname{0.584}
\expandafter\def\csname rev@rv@che@ens@ixs\endcsname{0.934}
\expandafter\def\csname rev@rv@che@ens@total\endcsname{0.371}
\expandafter\def\csname rev@rv@che@ensfour@ixs\endcsname{1.152}
\expandafter\def\csname rev@rv@che@ensfour@total\endcsname{1.067}
\expandafter\def\csname rev@rv@che@enstimestral@ixs\endcsname{1.356}
\expandafter\def\csname rev@rv@che@enstimestral@total\endcsname{1.534}
\expandafter\def\csname rev@rv@che@lgb@all\endcsname{0.518}
\expandafter\def\csname rev@rv@che@lgb@ixs\endcsname{0.623}
\expandafter\def\csname rev@rv@che@lgb@total\endcsname{0.456}
\expandafter\def\csname rev@rv@che@lift@all\endcsname{0.775}
\expandafter\def\csname rev@rv@che@lift@ixs\endcsname{1.119}
\expandafter\def\csname rev@rv@che@lift@total\endcsname{0.617}
\expandafter\def\csname rev@rv@che@naive@all\endcsname{1.164}
\expandafter\def\csname rev@rv@che@naive@ixs\endcsname{1.117}
\expandafter\def\csname rev@rv@che@naive@total\endcsname{1.175}
\expandafter\def\csname rev@rv@che@tfm@all\endcsname{0.709}
\expandafter\def\csname rev@rv@che@tfm@ixs\endcsname{0.749}
\expandafter\def\csname rev@rv@che@tfm@total\endcsname{0.718}
\expandafter\def\csname rev@rv@che@tfmplan@all\endcsname{0.592}
\expandafter\def\csname rev@rv@che@tfmplan@ixs\endcsname{0.659}
\expandafter\def\csname rev@rv@che@tfmplan@total\endcsname{0.584}
\expandafter\def\csname rev@rv@che@tft@all\endcsname{0.561}
\expandafter\def\csname rev@rv@che@tft@ixs\endcsname{0.696}
\expandafter\def\csname rev@rv@che@tft@total\endcsname{0.481}
\expandafter\def\csname rev@rv@che@tsmean@ixs\endcsname{0.771}
\expandafter\def\csname rev@rv@che@tsmean@total\endcsname{0.814}
\expandafter\def\csname rev@rv@che@tsplan@ixs\endcsname{1.956}
\expandafter\def\csname rev@rv@che@tsplan@total\endcsname{4.606}
\expandafter\def\csname rev@rv@che@world@all\endcsname{1.003}
\expandafter\def\csname rev@rv@che@world@ixs\endcsname{1.713}
\expandafter\def\csname rev@rv@che@world@total\endcsname{0.585}
\expandafter\def\csname rev@rv@fav@ens@all\endcsname{0.437}
\expandafter\def\csname rev@rv@fav@ens@ixs\endcsname{0.694}
\expandafter\def\csname rev@rv@fav@ens@total\endcsname{0.303}
\expandafter\def\csname rev@rv@fav@ensfour@ixs\endcsname{0.694}
\expandafter\def\csname rev@rv@fav@ensfour@total\endcsname{0.313}
\expandafter\def\csname rev@rv@fav@enstimestral@ixs\endcsname{0.697}
\expandafter\def\csname rev@rv@fav@enstimestral@total\endcsname{0.298}
\expandafter\def\csname rev@rv@fav@lgb@all\endcsname{0.452}
\expandafter\def\csname rev@rv@fav@lgb@ixs\endcsname{0.719}
\expandafter\def\csname rev@rv@fav@lgb@total\endcsname{0.309}
\expandafter\def\csname rev@rv@fav@lift@all\endcsname{0.551}
\expandafter\def\csname rev@rv@fav@lift@ixs\endcsname{0.744}
\expandafter\def\csname rev@rv@fav@lift@total\endcsname{0.452}
\expandafter\def\csname rev@rv@fav@naive@all\endcsname{0.662}
\expandafter\def\csname rev@rv@fav@naive@ixs\endcsname{0.992}
\expandafter\def\csname rev@rv@fav@naive@total\endcsname{0.501}
\expandafter\def\csname rev@rv@fav@tfmplan@all\endcsname{0.501}
\expandafter\def\csname rev@rv@fav@tfmplan@ixs\endcsname{0.712}
\expandafter\def\csname rev@rv@fav@tfmplan@total\endcsname{0.397}
\expandafter\def\csname rev@rv@fav@tsmean@ixs\endcsname{0.771}
\expandafter\def\csname rev@rv@fav@tsmean@total\endcsname{0.430}
\expandafter\def\csname rev@rv@fav@tsplan@ixs\endcsname{0.731}
\expandafter\def\csname rev@rv@fav@tsplan@total\endcsname{0.403}
\expandafter\def\csname rev@rv@fav@world@all\endcsname{0.480}
\expandafter\def\csname rev@rv@fav@world@ixs\endcsname{0.726}
\expandafter\def\csname rev@rv@fav@world@total\endcsname{0.341}
\expandafter\def\csname rev@rv@frat@chronos@all\endcsname{0.722}
\expandafter\def\csname rev@rv@frat@chronos@ixs\endcsname{0.778}
\expandafter\def\csname rev@rv@frat@chronos@total\endcsname{0.605}
\expandafter\def\csname rev@rv@frat@ens@all\endcsname{0.464}
\expandafter\def\csname rev@rv@frat@ens@ixs\endcsname{0.549}
\expandafter\def\csname rev@rv@frat@ens@total\endcsname{0.337}
\expandafter\def\csname rev@rv@frat@ensfour@ixs\endcsname{0.595}
\expandafter\def\csname rev@rv@frat@ensfour@total\endcsname{0.407}
\expandafter\def\csname rev@rv@frat@enstimestral@ixs\endcsname{0.623}
\expandafter\def\csname rev@rv@frat@enstimestral@total\endcsname{0.501}
\expandafter\def\csname rev@rv@frat@lgb@all\endcsname{0.481}
\expandafter\def\csname rev@rv@frat@lgb@ixs\endcsname{0.570}
\expandafter\def\csname rev@rv@frat@lgb@total\endcsname{0.360}
\expandafter\def\csname rev@rv@frat@lift@all\endcsname{0.524}
\expandafter\def\csname rev@rv@frat@lift@ixs\endcsname{0.590}
\expandafter\def\csname rev@rv@frat@lift@total\endcsname{0.405}
\expandafter\def\csname rev@rv@frat@naive@all\endcsname{1.038}
\expandafter\def\csname rev@rv@frat@naive@ixs\endcsname{1.077}
\expandafter\def\csname rev@rv@frat@naive@total\endcsname{0.964}
\expandafter\def\csname rev@rv@frat@tfm@all\endcsname{0.691}
\expandafter\def\csname rev@rv@frat@tfm@ixs\endcsname{0.775}
\expandafter\def\csname rev@rv@frat@tfm@total\endcsname{0.541}
\expandafter\def\csname rev@rv@frat@tfmplan@all\endcsname{0.482}
\expandafter\def\csname rev@rv@frat@tfmplan@ixs\endcsname{0.578}
\expandafter\def\csname rev@rv@frat@tfmplan@total\endcsname{0.327}
\expandafter\def\csname rev@rv@frat@tft@all\endcsname{0.571}
\expandafter\def\csname rev@rv@frat@tft@ixs\endcsname{0.652}
\expandafter\def\csname rev@rv@frat@tft@total\endcsname{0.425}
\expandafter\def\csname rev@rv@frat@tsmean@ixs\endcsname{0.792}
\expandafter\def\csname rev@rv@frat@tsmean@total\endcsname{0.484}
\expandafter\def\csname rev@rv@frat@tsplan@ixs\endcsname{0.864}
\expandafter\def\csname rev@rv@frat@tsplan@total\endcsname{1.048}
\expandafter\def\csname rev@rv@frat@world@all\endcsname{0.546}
\expandafter\def\csname rev@rv@frat@world@ixs\endcsname{0.595}
\expandafter\def\csname rev@rv@frat@world@total\endcsname{0.457}
\expandafter\def\csname rev@rv@fre@chronos@all\endcsname{0.574}
\expandafter\def\csname rev@rv@fre@chronos@ixs\endcsname{0.554}
\expandafter\def\csname rev@rv@fre@chronos@total\endcsname{0.578}
\expandafter\def\csname rev@rv@fre@ens@all\endcsname{0.361}
\expandafter\def\csname rev@rv@fre@ens@ixs\endcsname{0.408}
\expandafter\def\csname rev@rv@fre@ens@total\endcsname{0.342}
\expandafter\def\csname rev@rv@fre@ensfour@ixs\endcsname{0.537}
\expandafter\def\csname rev@rv@fre@ensfour@total\endcsname{0.699}
\expandafter\def\csname rev@rv@fre@enstimestral@ixs\endcsname{0.578}
\expandafter\def\csname rev@rv@fre@enstimestral@total\endcsname{0.807}
\expandafter\def\csname rev@rv@fre@lgb@all\endcsname{0.346}
\expandafter\def\csname rev@rv@fre@lgb@ixs\endcsname{0.410}
\expandafter\def\csname rev@rv@fre@lgb@total\endcsname{0.321}
\expandafter\def\csname rev@rv@fre@lift@all\endcsname{0.406}
\expandafter\def\csname rev@rv@fre@lift@ixs\endcsname{0.449}
\expandafter\def\csname rev@rv@fre@lift@total\endcsname{0.387}
\expandafter\def\csname rev@rv@fre@naive@all\endcsname{0.664}
\expandafter\def\csname rev@rv@fre@naive@ixs\endcsname{0.710}
\expandafter\def\csname rev@rv@fre@naive@total\endcsname{0.620}
\expandafter\def\csname rev@rv@fre@tfm@all\endcsname{0.522}
\expandafter\def\csname rev@rv@fre@tfm@ixs\endcsname{0.549}
\expandafter\def\csname rev@rv@fre@tfm@total\endcsname{0.500}
\expandafter\def\csname rev@rv@fre@tfmplan@all\endcsname{0.484}
\expandafter\def\csname rev@rv@fre@tfmplan@ixs\endcsname{0.487}
\expandafter\def\csname rev@rv@fre@tfmplan@total\endcsname{0.481}
\expandafter\def\csname rev@rv@fre@tft@all\endcsname{0.420}
\expandafter\def\csname rev@rv@fre@tft@ixs\endcsname{0.488}
\expandafter\def\csname rev@rv@fre@tft@total\endcsname{0.380}
\expandafter\def\csname rev@rv@fre@tsmean@ixs\endcsname{0.590}
\expandafter\def\csname rev@rv@fre@tsmean@total\endcsname{0.540}
\expandafter\def\csname rev@rv@fre@tsplan@ixs\endcsname{1.048}
\expandafter\def\csname rev@rv@fre@tsplan@total\endcsname{2.158}
\expandafter\def\csname rev@rv@fre@world@all\endcsname{0.366}
\expandafter\def\csname rev@rv@fre@world@ixs\endcsname{0.433}
\expandafter\def\csname rev@rv@fre@world@total\endcsname{0.338}
\expandafter\def\csname rev@rv@mfive@chronos@all\endcsname{1.184}
\expandafter\def\csname rev@rv@mfive@chronos@ixs\endcsname{0.858}
\expandafter\def\csname rev@rv@mfive@chronos@total\endcsname{1.333}
\expandafter\def\csname rev@rv@mfive@ens@all\endcsname{0.759}
\expandafter\def\csname rev@rv@mfive@ens@ixs\endcsname{0.834}
\expandafter\def\csname rev@rv@mfive@ens@total\endcsname{0.706}
\expandafter\def\csname rev@rv@mfive@ensfour@ixs\endcsname{0.842}
\expandafter\def\csname rev@rv@mfive@ensfour@total\endcsname{0.699}
\expandafter\def\csname rev@rv@mfive@enstimestral@ixs\endcsname{0.846}
\expandafter\def\csname rev@rv@mfive@enstimestral@total\endcsname{0.609}
\expandafter\def\csname rev@rv@mfive@lgb@all\endcsname{0.751}
\expandafter\def\csname rev@rv@mfive@lgb@ixs\endcsname{0.861}
\expandafter\def\csname rev@rv@mfive@lgb@total\endcsname{0.693}
\expandafter\def\csname rev@rv@mfive@lift@all\endcsname{1.291}
\expandafter\def\csname rev@rv@mfive@lift@ixs\endcsname{0.845}
\expandafter\def\csname rev@rv@mfive@lift@total\endcsname{1.163}
\expandafter\def\csname rev@rv@mfive@naive@all\endcsname{1.146}
\expandafter\def\csname rev@rv@mfive@naive@ixs\endcsname{1.163}
\expandafter\def\csname rev@rv@mfive@naive@total\endcsname{1.087}
\expandafter\def\csname rev@rv@mfive@tfm@all\endcsname{0.964}
\expandafter\def\csname rev@rv@mfive@tfm@ixs\endcsname{0.842}
\expandafter\def\csname rev@rv@mfive@tfm@total\endcsname{1.000}
\expandafter\def\csname rev@rv@mfive@tfmplan@all\endcsname{0.982}
\expandafter\def\csname rev@rv@mfive@tfmplan@ixs\endcsname{0.842}
\expandafter\def\csname rev@rv@mfive@tfmplan@total\endcsname{1.035}
\expandafter\def\csname rev@rv@mfive@tsmean@ixs\endcsname{0.861}
\expandafter\def\csname rev@rv@mfive@tsmean@total\endcsname{1.014}
\expandafter\def\csname rev@rv@mfive@tsplan@ixs\endcsname{0.894}
\expandafter\def\csname rev@rv@mfive@tsplan@total\endcsname{1.025}
\expandafter\def\csname rev@rv@mfive@world@all\endcsname{0.745}
\expandafter\def\csname rev@rv@mfive@world@ixs\endcsname{0.851}
\expandafter\def\csname rev@rv@mfive@world@total\endcsname{0.609}
\expandafter\def\csname rev@rv@sdr@chronos@all\endcsname{1.057}
\expandafter\def\csname rev@rv@sdr@chronos@ixs\endcsname{0.720}
\expandafter\def\csname rev@rv@sdr@chronos@total\endcsname{1.270}
\expandafter\def\csname rev@rv@sdr@ens@all\endcsname{0.706}
\expandafter\def\csname rev@rv@sdr@ens@ixs\endcsname{0.536}
\expandafter\def\csname rev@rv@sdr@ens@total\endcsname{0.834}
\expandafter\def\csname rev@rv@sdr@ensfour@ixs\endcsname{0.588}
\expandafter\def\csname rev@rv@sdr@ensfour@total\endcsname{1.287}
\expandafter\def\csname rev@rv@sdr@enstimestral@ixs\endcsname{0.616}
\expandafter\def\csname rev@rv@sdr@enstimestral@total\endcsname{1.574}
\expandafter\def\csname rev@rv@sdr@lgb@all\endcsname{0.709}
\expandafter\def\csname rev@rv@sdr@lgb@ixs\endcsname{0.545}
\expandafter\def\csname rev@rv@sdr@lgb@total\endcsname{0.831}
\expandafter\def\csname rev@rv@sdr@lift@all\endcsname{0.850}
\expandafter\def\csname rev@rv@sdr@lift@ixs\endcsname{0.672}
\expandafter\def\csname rev@rv@sdr@lift@total\endcsname{0.965}
\expandafter\def\csname rev@rv@sdr@naive@all\endcsname{1.006}
\expandafter\def\csname rev@rv@sdr@naive@ixs\endcsname{0.960}
\expandafter\def\csname rev@rv@sdr@naive@total\endcsname{1.035}
\expandafter\def\csname rev@rv@sdr@tfm@all\endcsname{0.972}
\expandafter\def\csname rev@rv@sdr@tfm@ixs\endcsname{0.711}
\expandafter\def\csname rev@rv@sdr@tfm@total\endcsname{1.157}
\expandafter\def\csname rev@rv@sdr@tfmplan@all\endcsname{0.825}
\expandafter\def\csname rev@rv@sdr@tfmplan@ixs\endcsname{0.609}
\expandafter\def\csname rev@rv@sdr@tfmplan@total\endcsname{0.977}
\expandafter\def\csname rev@rv@sdr@tft@all\endcsname{0.829}
\expandafter\def\csname rev@rv@sdr@tft@ixs\endcsname{0.640}
\expandafter\def\csname rev@rv@sdr@tft@total\endcsname{0.971}
\expandafter\def\csname rev@rv@sdr@tsmean@ixs\endcsname{0.737}
\expandafter\def\csname rev@rv@sdr@tsmean@total\endcsname{1.020}
\expandafter\def\csname rev@rv@sdr@tsplan@ixs\endcsname{0.872}
\expandafter\def\csname rev@rv@sdr@tsplan@total\endcsname{4.181}
\expandafter\def\csname rev@rv@sdr@world@all\endcsname{0.761}
\expandafter\def\csname rev@rv@sdr@world@ixs\endcsname{0.600}
\expandafter\def\csname rev@rv@sdr@world@total\endcsname{0.879}
\expandafter\def\csname rev@rv@sna@chronos@all\endcsname{2.840}
\expandafter\def\csname rev@rv@sna@chronos@ixs\endcsname{0.708}
\expandafter\def\csname rev@rv@sna@chronos@total\endcsname{4.410}
\expandafter\def\csname rev@rv@sna@ens@all\endcsname{0.919}
\expandafter\def\csname rev@rv@sna@ens@ixs\endcsname{0.562}
\expandafter\def\csname rev@rv@sna@ens@total\endcsname{1.181}
\expandafter\def\csname rev@rv@sna@ensfour@ixs\endcsname{0.876}
\expandafter\def\csname rev@rv@sna@ensfour@total\endcsname{4.689}
\expandafter\def\csname rev@rv@sna@enstimestral@ixs\endcsname{0.986}
\expandafter\def\csname rev@rv@sna@enstimestral@total\endcsname{5.934}
\expandafter\def\csname rev@rv@sna@lgb@all\endcsname{0.870}
\expandafter\def\csname rev@rv@sna@lgb@ixs\endcsname{0.578}
\expandafter\def\csname rev@rv@sna@lgb@total\endcsname{1.097}
\expandafter\def\csname rev@rv@sna@lift@all\endcsname{1.023}
\expandafter\def\csname rev@rv@sna@lift@ixs\endcsname{0.598}
\expandafter\def\csname rev@rv@sna@lift@total\endcsname{1.026}
\expandafter\def\csname rev@rv@sna@naive@all\endcsname{1.494}
\expandafter\def\csname rev@rv@sna@naive@ixs\endcsname{1.010}
\expandafter\def\csname rev@rv@sna@naive@total\endcsname{1.790}
\expandafter\def\csname rev@rv@sna@tfm@all\endcsname{1.204}
\expandafter\def\csname rev@rv@sna@tfm@ixs\endcsname{0.677}
\expandafter\def\csname rev@rv@sna@tfm@total\endcsname{1.581}
\expandafter\def\csname rev@rv@sna@tfmplan@all\endcsname{0.946}
\expandafter\def\csname rev@rv@sna@tfmplan@ixs\endcsname{0.605}
\expandafter\def\csname rev@rv@sna@tfmplan@total\endcsname{1.181}
\expandafter\def\csname rev@rv@sna@tft@all\endcsname{1.041}
\expandafter\def\csname rev@rv@sna@tft@ixs\endcsname{0.654}
\expandafter\def\csname rev@rv@sna@tft@total\endcsname{1.301}
\expandafter\def\csname rev@rv@sna@tsmean@ixs\endcsname{0.736}
\expandafter\def\csname rev@rv@sna@tsmean@total\endcsname{6.576}
\expandafter\def\csname rev@rv@sna@tsplan@ixs\endcsname{1.944}
\expandafter\def\csname rev@rv@sna@tsplan@total\endcsname{16.272}
\expandafter\def\csname rev@rv@sna@world@all\endcsname{1.095}
\expandafter\def\csname rev@rv@sna@world@ixs\endcsname{0.595}
\expandafter\def\csname rev@rv@sna@world@total\endcsname{1.454}
\expandafter\def\csname rev@rw@ana@alllevels@lgb\endcsname{0.12}
\expandafter\def\csname rev@rw@ana@alllevels@tfmplan\endcsname{0.33}
\expandafter\def\csname rev@rw@ana@alllevels@world\endcsname{0.55}
\expandafter\def\csname rev@rw@ana@bottom@lgb\endcsname{0.64}
\expandafter\def\csname rev@rw@ana@bottom@tfmplan\endcsname{0.27}
\expandafter\def\csname rev@rw@ana@bottom@world\endcsname{0.09}
\expandafter\def\csname rev@rw@ana@total@lgb\endcsname{0.03}
\expandafter\def\csname rev@rw@ana@total@tfmplan\endcsname{0.33}
\expandafter\def\csname rev@rw@ana@total@world\endcsname{0.64}
\expandafter\def\csname rev@rw@bjc@alllevels@lgb\endcsname{0.45}
\expandafter\def\csname rev@rw@bjc@alllevels@tfmplan\endcsname{0.23}
\expandafter\def\csname rev@rw@bjc@alllevels@world\endcsname{0.32}
\expandafter\def\csname rev@rw@bjc@bottom@lgb\endcsname{0.41}
\expandafter\def\csname rev@rw@bjc@bottom@tfmplan\endcsname{0.41}
\expandafter\def\csname rev@rw@bjc@bottom@world\endcsname{0.18}
\expandafter\def\csname rev@rw@bjc@total@lgb\endcsname{0.43}
\expandafter\def\csname rev@rw@bjc@total@tfmplan\endcsname{0.18}
\expandafter\def\csname rev@rw@bjc@total@world\endcsname{0.39}
\expandafter\def\csname rev@rw@che@alllevels@lgb\endcsname{0.48}
\expandafter\def\csname rev@rw@che@alllevels@tfmplan\endcsname{0.49}
\expandafter\def\csname rev@rw@che@alllevels@world\endcsname{0.03}
\expandafter\def\csname rev@rw@che@bottom@lgb\endcsname{0.59}
\expandafter\def\csname rev@rw@che@bottom@tfmplan\endcsname{0.41}
\expandafter\def\csname rev@rw@che@bottom@world\endcsname{0.00}
\expandafter\def\csname rev@rw@che@total@lgb\endcsname{0.33}
\expandafter\def\csname rev@rw@che@total@tfmplan\endcsname{0.35}
\expandafter\def\csname rev@rw@che@total@world\endcsname{0.32}
\expandafter\def\csname rev@rw@fav@alllevels@lgb\endcsname{0.33}
\expandafter\def\csname rev@rw@fav@alllevels@tfmplan\endcsname{0.13}
\expandafter\def\csname rev@rw@fav@alllevels@world\endcsname{0.53}
\expandafter\def\csname rev@rw@fav@bottom@lgb\endcsname{0.22}
\expandafter\def\csname rev@rw@fav@bottom@tfmplan\endcsname{0.43}
\expandafter\def\csname rev@rw@fav@bottom@world\endcsname{0.35}
\expandafter\def\csname rev@rw@fav@total@lgb\endcsname{0.33}
\expandafter\def\csname rev@rw@fav@total@tfmplan\endcsname{0.08}
\expandafter\def\csname rev@rw@fav@total@world\endcsname{0.58}
\expandafter\def\csname rev@rw@frat@alllevels@lgb\endcsname{0.55}
\expandafter\def\csname rev@rw@frat@alllevels@tfmplan\endcsname{0.45}
\expandafter\def\csname rev@rw@frat@alllevels@world\endcsname{0.00}
\expandafter\def\csname rev@rw@frat@bottom@lgb\endcsname{0.40}
\expandafter\def\csname rev@rw@frat@bottom@tfmplan\endcsname{0.45}
\expandafter\def\csname rev@rw@frat@bottom@world\endcsname{0.15}
\expandafter\def\csname rev@rw@frat@total@lgb\endcsname{0.50}
\expandafter\def\csname rev@rw@frat@total@tfmplan\endcsname{0.50}
\expandafter\def\csname rev@rw@frat@total@world\endcsname{0.00}
\expandafter\def\csname rev@rw@fre@alllevels@lgb\endcsname{0.71}
\expandafter\def\csname rev@rw@fre@alllevels@tfmplan\endcsname{0.02}
\expandafter\def\csname rev@rw@fre@alllevels@world\endcsname{0.27}
\expandafter\def\csname rev@rw@fre@bottom@lgb\endcsname{0.63}
\expandafter\def\csname rev@rw@fre@bottom@tfmplan\endcsname{0.16}
\expandafter\def\csname rev@rw@fre@bottom@world\endcsname{0.21}
\expandafter\def\csname rev@rw@fre@total@lgb\endcsname{0.69}
\expandafter\def\csname rev@rw@fre@total@tfmplan\endcsname{0.01}
\expandafter\def\csname rev@rw@fre@total@world\endcsname{0.30}
\expandafter\def\csname rev@rw@mfive@alllevels@lgb\endcsname{0.45}
\expandafter\def\csname rev@rw@mfive@alllevels@tfmplan\endcsname{0.02}
\expandafter\def\csname rev@rw@mfive@alllevels@world\endcsname{0.53}
\expandafter\def\csname rev@rw@mfive@bottom@lgb\endcsname{0.27}
\expandafter\def\csname rev@rw@mfive@bottom@tfmplan\endcsname{0.42}
\expandafter\def\csname rev@rw@mfive@bottom@world\endcsname{0.32}
\expandafter\def\csname rev@rw@mfive@total@lgb\endcsname{0.35}
\expandafter\def\csname rev@rw@mfive@total@tfmplan\endcsname{0.03}
\expandafter\def\csname rev@rw@mfive@total@world\endcsname{0.62}
\expandafter\def\csname rev@rw@sdr@alllevels@lgb\endcsname{0.50}
\expandafter\def\csname rev@rw@sdr@alllevels@tfmplan\endcsname{0.20}
\expandafter\def\csname rev@rw@sdr@alllevels@world\endcsname{0.30}
\expandafter\def\csname rev@rw@sdr@bottom@lgb\endcsname{0.41}
\expandafter\def\csname rev@rw@sdr@bottom@tfmplan\endcsname{0.36}
\expandafter\def\csname rev@rw@sdr@bottom@world\endcsname{0.23}
\expandafter\def\csname rev@rw@sdr@total@lgb\endcsname{0.52}
\expandafter\def\csname rev@rw@sdr@total@tfmplan\endcsname{0.16}
\expandafter\def\csname rev@rw@sdr@total@world\endcsname{0.32}
\expandafter\def\csname rev@rw@sna@alllevels@lgb\endcsname{0.47}
\expandafter\def\csname rev@rw@sna@alllevels@tfmplan\endcsname{0.37}
\expandafter\def\csname rev@rw@sna@alllevels@world\endcsname{0.16}
\expandafter\def\csname rev@rw@sna@bottom@lgb\endcsname{0.50}
\expandafter\def\csname rev@rw@sna@bottom@tfmplan\endcsname{0.34}
\expandafter\def\csname rev@rw@sna@bottom@world\endcsname{0.16}
\expandafter\def\csname rev@rw@sna@total@lgb\endcsname{0.38}
\expandafter\def\csname rev@rw@sna@total@tfmplan\endcsname{0.41}
\expandafter\def\csname rev@rw@sna@total@world\endcsname{0.21}
\expandafter\def\csname rev@rwin@che@lift@ixsmax\endcsname{3.57}
\expandafter\def\csname rev@rwin@che@lift@ixsmaxorigin\endcsname{1}
\expandafter\def\csname rev@rwin@che@lift@ixsmedian\endcsname{0.63}
\expandafter\def\csname rev@rwin@che@lift@n\endcsname{6}
\expandafter\def\csname rev@rwin@che@world@ixsmax\endcsname{7.12}
\expandafter\def\csname rev@rwin@che@world@ixsmaxorigin\endcsname{1}
\expandafter\def\csname rev@rwin@che@world@ixsmedian\endcsname{0.63}
\expandafter\def\csname rev@rwin@che@world@n\endcsname{6}
\expandafter\def\csname rev@rwin@sdr@world@ixsmax\endcsname{0.62}
\expandafter\def\csname rev@rwin@sdr@world@ixsmaxorigin\endcsname{2}
\expandafter\def\csname rev@rwin@sdr@world@ixsmedian\endcsname{0.57}
\expandafter\def\csname rev@rwin@sdr@world@n\endcsname{2}
\expandafter\def\csname rev@rwin@sna@lift@ixsmax\endcsname{0.73}
\expandafter\def\csname rev@rwin@sna@lift@ixsmaxorigin\endcsname{1}
\expandafter\def\csname rev@rwin@sna@lift@ixsmedian\endcsname{0.57}
\expandafter\def\csname rev@rwin@sna@lift@n\endcsname{6}
\expandafter\def\csname rev@rwin@sna@world@ixsmax\endcsname{0.75}
\expandafter\def\csname rev@rwin@sna@world@ixsmaxorigin\endcsname{1}
\expandafter\def\csname rev@rwin@sna@world@ixsmedian\endcsname{0.57}
\expandafter\def\csname rev@rwin@sna@world@n\endcsname{6}
\newcommand{\rv}[3]{\revget{rv@#1@#2@#3}}
\newcommand{\rf}[3]{\revget{rf@#1@#2@#3}}
\newcommand{\rpair}[5]{\revget{rpair@#1@#2@#3@#4@#5}}
\newcommand{\rab}[4]{\revget{rab@#1@#2@#3@#4}}
\newcommand{\rw}[3]{\revget{rw@#1@#2@#3}}
\newcommand{\rdec}[3]{\revget{rdec@#1@#2@#3}}
\newcommand{\rint}[4]{\revget{rint@#1@#2@#3@#4}}
\newcommand{\rintold}[4]{\revget{rintold@#1@#2@#3@#4}}
\newcommand{\rrec}[3]{\revget{rrec@#1@#2@#3}}
\newcommand{\rper}[5]{\revget{rper@#1@#2@#3@#4@#5}}
\newcommand{\rmech}[4]{\revget{rmech@#1@#2@#3@#4}}
\newcommand{\rsf}[3]{\revget{rsf@#1@#2@#3}}
\newcommand{\rtail}[4]{\revget{rtail@#1@#2@#3@#4}}
\newcommand{\rrank}[4]{\revget{rrank@#1@#2@#3@#4}}
\newcommand{\rpan}[5]{\revget{rpan@#1@#2@#3@#4@#5}}
\newcommand{\raft}[3]{\revget{raft@#1@#2@#3}}
\newcommand{\rcount}[1]{\revget{rcount@#1}}
\newcommand{\rwin}[3]{\revget{rwin@#1@#2@#3}}
\newcommand{\rreg}[3]{\revget{rreg@#1@#2@#3}}
\newcommand{\rgrain}[3]{\revget{rgrain@#1@#2@#3}}
\newcommand{\rcore}[3]{\revget{rcore@#1@#2@#3}}
\newcommand{\rsg}[2]{\revget{rsg@#1@#2}}
\newcommand{\rcc}[4]{\revget{rcc@#1@#2@#3@#4}}
\makeatother

